Mixture Models for Photometric Redshifts

Determining photometric redshifts to high accuracy is paramount to measure distances in wide-field cosmological experiments. With only photometric information at hand, photo-zs are prone to systematic uncertainties in the intervening extinction and the unknown underlying spectral-energy distribution of different astrophysical sources. Here, we aim to resolve these model degeneracies and obtain a clear separation between intrinsic physical properties of astrophysical sources and extrinsic systematics. We aim at estimates of the full photo-z probability distributions, and their uncertainties. We perform a probabilistic photo-z determination using Mixture Density Networks (MDN). The training data-set is composed of optical ($griz$) point-spread-function and model magnitudes and extinction measurements from the SDSS-DR15, and WISE midinfrared ($3.4 \mu$m and $4.6 \mu$m) model magnitudes. We use Infinite Gaussian Mixture models to classify the objects in our data-set as stars, galaxies or quasars, and to determine the number of MDN components to achieve optimal performance. The fraction of objects that are correctly split into the main classes is 94%. Our method improves the bias of photometric redshift estimation (i.e. the mean $\Delta z$ = (zp - zs)/(1 + zs)) by one order of magnitude compared to the SDSS photo-z, and decreases the fraction of $3 \sigma$ outliers (i.e. 3rms$(\Delta z) < \Delta z$). The relative, root-mean-square systematic uncertainty in our resulting photo-zs is down to 1.7% for low-redshift galaxies (zs $<$ 0.5). We have demonstrated the feasibility of machine-learning based methods that produce full probability distributions for photo-z estimates with a performance that is competitive with state-of-the art techniques. Our method can be applied to wide-field surveys where extinction can vary significantly across the sky and with sparse spectroscopic calibration samples.

==> OLD/aastex61cls <==
%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% AASTeX61.cls                                  %%
%% October 5, 2016                               %%
%% Copyright 2016 American Astronomical Society  %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\currversion{6.1}

%%
%%    These files are distributed
%%    WITHOUT ANY WARRANTY; without even the implied warranty of
%%    MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.
%% 
%% \CharacterTable
%%  {Upper-case    \A\B\C\D\E\F\G\H\I\J\K\L\M\N\O\P\Q\R\S\T\U\V\W\X\Y\Z
%%   Lower-case    \a\b\c\d\e\f\g\h\i\j\k\l\m\n\o\p\q\r\s\t\u\v\w\x\y\z
%%   Digits        \0\1\2\3\4\5\6\7\8\9
%%   Exclamation   \!     Double quote  \"     Hash (number) \#
%%   Dollar        \$     Percent       \%     Ampersand     \&
%%   Acute accent  \'     Left paren    \(     Right paren   \)
%%   Asterisk      \*     Plus          \+     Comma         \,
%%   Minus         \-     Point         \.     Solidus       \/
%%   Colon         \:     Semicolon     \;     Less than     \<
%%   Equals        \=     Greater than  \>     Question mark \?
%%   Commercial at \@     Left bracket  \[     Backslash     \\
%%   Right bracket \]     Circumflex    \^     Underscore    \_
%%   Grave accent  \`     Left brace    \{     Vertical bar  \|
%%   Right brace   \}     Tilde         \~}%
%%
%%%     date            = "9/19/2016",
%%%     author          = "Amy Hendrickson (mailto:amyh@texnology.com)" 
%%%                            including 
%%%                       1) code from emulateapj.cls, version 01/23/15(marked below)
%%%                            written by Alexey Vikhlinin, which relies on RevTeX4-1
%%%                            for much functionality;
%%%                       2) some code from aastex (marked below)
%%%                       3) Original work by Amy Hendrickson (marked below) for
%%%                       extensive table tools, including easy decimal entry and splitting
%%%                       tables horizontally into 2 or 3 pieces, for tabular and deluxetable
%%%                       environments; rotate tables; gridlines for use in positioning figures, 
%%%                       track changes.

%%% This work may be distributed and/or modified under the 
%%% conditions of the LaTeX Project Public License, either version 1.3c 
%%% of this license or (at your option) any later version.
%%% The latest version of this license is in
%%%  http://www.latex-project.org/lppl.txt
%%% and version 1.3 or later is part of all distributions of LaTeX 
%%% version 2005/12/01 or later.
%
%%% This work has the LPPL maintenance status `maintained'.
%
%%% The Current Maintainer of this work is Greg Schwarz <greg.schwarz@aas.org> 
%%% This work consists of the file aastex.cls

%%%     copyright       = "Copyright (C) 2016 American Astronomical Society
%%%
%%%                        This work may be distributed and/or modified under the
%%%                        conditions of the LaTeX Project Public License, either version 1.3
%%%                        of this license or (at your option) any later version.
%%%                        The latest version of this license is in
%%%                        http://www.latex-project.org/lppl.txt
%%%                        and version 1.3 or later is part of all distributions of LaTeX
%%%                        version 2003/12/01 or later.
%%%
%%%                        This work has the LPPL maintenance status "maintained".
%%%
%%%                        The Current Maintainer of this work is the American Astronomical Society.
%%%
%%%                        This work consists of all files listed in the document README.
%%%
%%%     address         = "American Astronomical Society
%%%                        USA",
%%%     telephone       = "+1 ???",
%%%     FAX             = "",
%%%     email           = "aastex-help@aas.org",
%%%     codetable       = "ISO/ASCII",
%%%     keywords        = "latex, AAS, journal",
%%%     supported       = "yes",
%%%     abstract        = "formatter for AAS journal submissions",
%%%  }

\ProvidesClass{aastex61}%%%
 [2016/04/16 Version 6.1/AAS markup document class]%
{}
\ClassInfo{aastex}{%
^^J
^^J
 Original \protect\LaTeX2.09 style
 by Chris Biemesderfer (chris@seagoat.com).
^^J
 Adapted to \protect\LaTeXe\space
 by A. Ogawa (ogawa@teleport.com)%
^^J
emulateapj.cls included, Copyright 2000-2015 Alexey Vikhlinin
^^J
Rewrite and update of emulateapj.cls,
revised and enhanced with table macros, gridlines, draft watermark,^^J
track changes, new `modern' style and much more, by Amy Hendrickson,%
^^J
 (amyh@texnology.com, http://www.texnology.com)
^^J
^^J
}%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% aastex.cls version 2.0 is a based on emulateapj.cls, version January 23, 2015,
%% and an older version of aastex.cls, with many additional functionalities.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Options. Document style options, and additional feature options.

% These are the General document style options, 6 choices

%   manuscript	: onecolumn, doublespace, 12pt fonts

%%  Preprints are like manuscript, except they are single spaced.
%   preprint	: onecolumn, single space, 12pt fonts
%   preprint2	: twocolumn, single space, 12pt fonts

%% Modern is new design developed by David Hogg and Daniel Foreman-Mackey
%   modern      : one column, single space, 10pt fonts, more stylish

%   twocolumn	: a two column article, single space, 10pt  fonts

% Default document style option
%   onecolumn	: a one column article; single space, 10pt fonts

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Additional feature options:

%   revtex4 	: will produce an error message and demand to download revtex4-1. 
%   twocolappendix: make 2 column appendix // produces error message. 
%      onecolappendix: make 1 column appendix is the default. // not needed because it is the default
%      astrosymb	: Loads Astrosymb font and define \astro commands. 
%      tighten	: Makes baselineskip slightly smaller, only works with twocolumn option.
%%    author can also use the commands \tighten, or \singlespace or \doublespace in the body of their article
%%    to get this change to the baselineskip
%      times	: uses times font as the default
%      linenumbers	: turn on lineno package.
%      trackchanges : required to see the revision mark up and print output
%      letteredappendix: (was numbered appendix) Not needed because it is the default, will label appendix sections A, B, ...
%      numberedappendix: Legacy command, will produce same results as lettered appendix, since we don't want more
%                        than one `section 1' in article: will cause problems for cross referencing.


\newif\ifmanu
\newif\iftwelvepoint
\newif\ifmodern
\newif\ifdoublespace
\newif\if@two@col
\newif\ifonecolstyle
\newif\iftwocolstyle

 \DeclareOption{manuscript}{\twelvepointtrue\@two@colfalse\doublespacetrue\manutrue}%

%% Preprints are like manuscript but are single spaced:
\newif\ifpreprint
 \DeclareOption{preprint}{\@two@colfalse\preprinttrue\twelvepointtrue}%

\newif\ifpreprinttwo
 \DeclareOption{preprint2}{\@two@coltrue\preprinttwotrue\twelvepointtrue}% 


%% New design suggested by
\DeclareOption{modern}{\@two@colfalse\twelvepointtrue\moderntrue}

%% left in from older version, in case it could be useful:

\DeclareOption{twocolumn}{\twocolstyletrue\@two@coltrue}

%% default style
\DeclareOption{onecolumn}{\onecolstyletrue}

%% obsolete option
\DeclareOption{revtex4}{\typeout{=================^^J^^J!!! The revtex4 option no longer
 allowed!^^J^^J Please download revtex4-1.cls^^J^^J
 Thank-you!^^J^^J=================}\stop}

\newif\if@two@col@app
\DeclareOption{twocolappendix}{\typeout{^^J^^J The option^^J
`twocolappendix' no
longer works! onecolappendix is preferred,^^J
and is the default.^^J^^J}\stop}%\@two@col@apptrue}
\DeclareOption{onecolappendix}{\@two@col@appfalse}%% this is default

\newif\iflongauthor
\DeclareOption{longauthor}{\global\longauthortrue}

\newlength{\bibbaselineskip}\setlength{\bibbaselineskip}{3.075mm}

 \DeclareOption{astrosymb}{
   \def\astro#1{\leavevmode\hbox{\astro@font#1}}%
   \def\load@astro@font{%
\iftwelvepoint
 \font\astro@font=Astrosym at 8pt
\else
 \font\astro@font=Astrosym at 7pt
\fi
}%
   \AtBeginDocument{\load@astro@font}
 }

%% Default definition for \astro, in case astrosymb option has not
%% been used:
\def\astro#1{\typeout{^^J^^J Please use class option `astrosymb' to
access fonts for the \string\astro\space command
^^J^^J
}\stop}

   \def\apjsecfont{\normalsize}
   \def\secnum@size{\small}
   \def\subsecnum@size{\normalsize}

    \def\AppendixApjSectionMarkInTitle#1{\relax}
\newif\ifletteredappendix
     \DeclareOption{letteredappendix}{\global\letteredappendixtrue
       \def\AppendixApjSectionMarkInTitle#1{#1.\ }
     }

%% this option is obsolete, since letteredappendix is a more logical name;
%%  but keeping it here in case someone uses it, set to be the same as
%% letteredappendix.
     \DeclareOption{numberedappendix}{\global\letteredappendixtrue
       \def\AppendixApjSectionMarkInTitle#1{#1.\ }
     }

     \newif\if@number@appendix@floats\@number@appendix@floatsfalse
     \DeclareOption{appendixfloats}{
       \@number@appendix@floatstrue
     }

%%%%%%%%%%%%%
%% AH

%% This option changes the baselineskips in the definitions of \normalsize etc
%% to make them a bit smaller.
\newif\iftighten
\DeclareOption{tighten}{\global\tightentrue}

%% AH
\newif\iftimes
\DeclareOption{times}{\global\timestrue}

\newif\ifnumlines
\DeclareOption{linenumbers}{\global\numlinestrue}

\newif\iftrack
\DeclareOption{trackchanges}{\global\tracktrue}

%% End AH Options

\ExecuteOptions{onecolumn,onecolappendix,letteredappendix}% 

\ProcessOptions	

%%%%%%%%%%%%%
%

 \iftimes
%% Might be better to use apjfonts, from Alexey Vikhlinin's website
%% http://hea-www.harvard.edu/~alexey/emulateapj/apjfonts.sty
%%\usepackage{apjfonts}
%% but times.sty is ubiquitous, and many people may not have apjfonts.sty
%% or the fonts that it calls.
%% default fonts:
\usepackage{times}
 \fi

%%%%%%%%%%%%%

 \IfFileExists{revtex4-1.cls}{
    \def\@revtex@cls{revtex4-1}
  }{
\typeout{^^J^^J Please update your system to include
revtex4-1.cls^^J^^J}\stop
  }
\def\@revtex@cls{revtex4-1}
\let\@startsection@from@latex=\@startsection


%% Passing options to revtex while loading:
  \iftwelvepoint
      \iflongauthor
         \LoadClass[nofootinbib,showkeys,twoside,floatfix,unsortedaddress,flushbottom,12pt,aps,pra]
          {\@revtex@cls}
     \else
        \LoadClass[nofootinbib,showkeys,twoside,floatfix,superscriptaddress,flushbottom,12pt,aps,pra]
       {\@revtex@cls}
     \fi
  \else %not twelvepoint
     \iflongauthor
         \LoadClass[nofootinbib,showkeys,twoside,floatfix,unsortedaddress,flushbottom,10pt,aps,pra]
         {\@revtex@cls}
     \else
        \LoadClass[nofootinbib,showkeys,twoside,floatfix,superscriptaddress,flushbottom,10pt,aps,pra]
        {\@revtex@cls}
    \fi
  \fi

%%%%%%%%%%%%%%%%%%%%

\def\blankaffiliation{~}%

%% needed?
 \def\@eapj@cap@font{\bfseries}
 \def\@eapj@figname{Figure}
 \def\@eapj@tabname{Table}

% Restore natbib package without sorting. 
\def\NAT@sort{0}
\def\NAT@cmprs{0}

% only redefine sort@cites for natbib versions < 2009
\@ifundefined{NAT@sort@cites@}{\def\NAT@sort@cites#1{\edef\NAT@cite@list{#1}}}%

\RequirePackage{latexsym}% 
\RequirePackage{graphicx}% 
\RequirePackage{amssymb}% 

\newcommand{\bibstyle@aas}{\bibpunct{(}{)}{;}{a}{}{,}}% 
\@citestyle{aas}% 

\let\@startsection=\@startsection@from@latex
\def\baselinestretch{1.0}

%% a bit more vertical space between horizontal lines, makes table more readable
\AtBeginDocument{\def\arraystretch{1.2}}

%% needed?
\def\raggedcolumn@sw#1#2{#2}  % implement flushbottom as it was in revtex4

\RequirePackage{epsf,graphicx}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Font families
%% modification of bk10.clo, and bk12.clo, standard LaTeX distribution
%%
%% Implements doublespace used in `manuscript' option
%% Implements `tighten' option: make baselineskip smaller if `tighten' is used
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% tighten only works with two column styles:
\iftwocolstyle\else\global\tightenfalse\fi

%%% preprint, preprint2, manuscript are 12pt
%% Modified bk12.clo
\iftwelvepoint

\renewcommand\normalsize{%
\ifdoublespace % manuscript
  \iftighten
   \@setfontsize\normalsize\@xiipt{20}%
  \else
   \@setfontsize\normalsize\@xiipt{24}%
  \fi
\else
  \iftighten
   \@setfontsize\normalsize\@xiipt{13}%
   \else
      \ifmodern
      \@setfontsize\normalsize\@xiipt{16}%
      \else
        \@setfontsize\normalsize\@xiipt{15}%
      \fi
   \fi
\fi %% end doublespace/no double space
   \abovedisplayskip 12\p@ \@plus3\p@ \@minus7\p@
   \abovedisplayshortskip \z@ \@plus3\p@
   \belowdisplayshortskip 6.5\p@ \@plus3.5\p@ \@minus3\p@
   \belowdisplayskip \abovedisplayskip
   \let\@listi\@listI}

\normalsize

\renewcommand\small{%
\ifdoublespace % manuscript
   \@setfontsize\small\@xipt{20}%
\else
\ifmodern
   \@setfontsize\small\@xipt{12}%
\else
   \@setfontsize\small\@xipt{13.6}%
\fi\fi
%% end doublespace/no double space
   \abovedisplayskip 11\p@ \@plus3\p@ \@minus6\p@
   \abovedisplayshortskip \z@ \@plus3\p@
   \belowdisplayshortskip 6.5\p@ \@plus3.5\p@ \@minus3\p@
   \def\@listi{\leftmargin\leftmargini
               \topsep 9\p@ \@plus3\p@ \@minus5\p@
               \parsep 4.5\p@ \@plus2\p@ \@minus\p@
               \itemsep \parsep}%
   \belowdisplayskip \abovedisplayskip
}

\renewcommand\footnotesize{%
\ifdoublespace % manuscriptstyle
   \@setfontsize\footnotesize\@xpt{18}
\else
   \ifmodern
   \@setfontsize\footnotesize\@xpt{11}%
   \else
   \@setfontsize\footnotesize\@xpt\@xiipt
\fi\fi
   \abovedisplayskip 10\p@ \@plus2\p@ \@minus5\p@
   \abovedisplayshortskip \z@ \@plus3\p@
   \belowdisplayshortskip 6\p@ \@plus3\p@ \@minus3\p@
   \def\@listi{\leftmargin\leftmargini
               \topsep 6\p@ \@plus2\p@ \@minus2\p@
               \parsep 3\p@ \@plus2\p@ \@minus\p@
               \itemsep \parsep}%
   \belowdisplayskip \abovedisplayskip
}
\ifdoublespace % manuscript style
\renewcommand\scriptsize{\@setfontsize\scriptsize\@viiipt{14}}
\renewcommand\tiny{\@setfontsize\tiny\@vipt{10}}
\renewcommand\large{\@setfontsize\large\@xivpt{18}}
\renewcommand\Large{\@setfontsize\Large\@xviipt{22}}
\renewcommand\LARGE{\@setfontsize\LARGE\@xxpt{25}}
\renewcommand\huge{\@setfontsize\huge\@xxvpt{30}}
\else
\renewcommand\scriptsize{\@setfontsize\scriptsize\@viiipt{9.5}}
\renewcommand\tiny{\@setfontsize\tiny\@vipt\@viipt}
\renewcommand\large{\@setfontsize\large\@xivpt{22}}
\renewcommand\Large{\@setfontsize\Large\@xviipt{24}}
\renewcommand\LARGE{\@setfontsize\LARGE\@xxpt{28}}
\renewcommand\huge{\@setfontsize\huge\@xxvpt{30}}
\fi
\let\Huge=\huge
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\else %% not twelvepoint, now tenpoint
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% no doublespace here, because the only doublespace is in `manuscript style' which is 12pt

\renewcommand\normalsize{%
\iftighten
   \@setfontsize\normalsize\@xpt{11.5}%
\else
   \@setfontsize\normalsize\@xpt{12.5}%
\fi
   \abovedisplayskip 10\p@ \@plus2\p@ \@minus5\p@
   \abovedisplayshortskip \z@ \@plus3\p@
   \belowdisplayshortskip 6\p@ \@plus3\p@ \@minus3\p@
   \belowdisplayskip \abovedisplayskip
   \let\@listi\@listI}

\normalsize

\renewcommand\small{%
\iftighten
   \@setfontsize\small\@ixpt{12}%
\else
   \@setfontsize\small\@ixpt{11}%
\fi
   \abovedisplayskip 8.5\p@ \@plus3\p@ \@minus4\p@
   \abovedisplayshortskip \z@ \@plus2\p@
   \belowdisplayshortskip 4\p@ \@plus2\p@ \@minus2\p@
   \def\@listi{\leftmargin\leftmargini
               \topsep 4\p@ \@plus2\p@ \@minus2\p@
               \parsep 2\p@ \@plus\p@ \@minus\p@
               \itemsep \parsep}%
   \belowdisplayskip \abovedisplayskip
}

\renewcommand\footnotesize{%
\iftighten
   \@setfontsize\footnotesize\@viiipt{9}%
\else
   \@setfontsize\footnotesize\@viiipt{9.5}% standard eightpoint size
\fi
   \abovedisplayskip 6\p@ \@plus2\p@ \@minus4\p@
   \abovedisplayshortskip \z@ \@plus\p@
   \belowdisplayshortskip 3\p@ \@plus\p@ \@minus2\p@
   \def\@listi{\leftmargin\leftmargini
               \topsep 3\p@ \@plus\p@ \@minus\p@
               \parsep 2\p@ \@plus\p@ \@minus\p@
               \itemsep \parsep}%
   \belowdisplayskip \abovedisplayskip
}

%% Standard 10pt font sizes
\renewcommand\scriptsize{\@setfontsize\scriptsize\@viipt\@viiipt}
\renewcommand\tiny{\@setfontsize\tiny\@vpt\@vipt}
\renewcommand\large{\@setfontsize\large\@xiipt{14}}
\renewcommand\Large{\@setfontsize\Large\@xivpt{18}}
\renewcommand\LARGE{\@setfontsize\LARGE\@xviipt{22}}
\renewcommand\huge{\@setfontsize\huge\@xxpt{25}}
\renewcommand\Huge{\@setfontsize\Huge\@xxvpt{30}}

\fi

%% End font sizes
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\setlength\smallskipamount{3\p@ \@plus 1\p@ \@minus 1\p@}
\setlength\medskipamount{6\p@ \@plus 2\p@ \@minus 2\p@}
\setlength\bigskipamount{12\p@ \@plus 4\p@ \@minus 4\p@}
\setlength\headheight{12\p@}
\def\@listi{\leftmargin\leftmargini
            \parsep 4\p@ \@plus2\p@ \@minus\p@
            \topsep 8\p@ \@plus2\p@ \@minus4\p@
            \itemsep4\p@ \@plus2\p@ \@minus\p@}
\let\@listI\@listi
\@listi
\def\@listii {\leftmargin\leftmarginii
              \labelwidth\leftmarginii
              \advance\labelwidth-\labelsep
              \topsep    4\p@ \@plus2\p@ \@minus\p@
              \parsep    2\p@ \@plus\p@  \@minus\p@
              \itemsep   \parsep}
\def\@listiii{\leftmargin\leftmarginiii
              \labelwidth\leftmarginiii
              \advance\labelwidth-\labelsep
              \topsep    2\p@ \@plus\p@\@minus\p@
              \parsep    \z@
              \partopsep \p@ \@plus\z@ \@minus\p@
              \itemsep   \topsep}
\def\@listiv {\leftmargin\leftmarginiv
              \labelwidth\leftmarginiv
              \advance\labelwidth-\labelsep}
\def\@listv  {\leftmargin\leftmarginv
              \labelwidth\leftmarginv
              \advance\labelwidth-\labelsep}
\def\@listvi {\leftmargin\leftmarginvi
              \labelwidth\leftmarginvi
              \advance\labelwidth-\labelsep}

%  ****************************************************
%  *             TWO AND SINGLE ONE COLUMN STYLES: AV *
%  ****************************************************
%

%%%%% include atbeginend.sty by AV:

% Copy \begin and \end to \BeginEnvironment and \EndEnvironment
\let\BeginEnvironment=\begin
\let\EndEnvironment=\end
%% \ifundefined from TeXbook
\def\IfUnDef#1{\expandafter\ifx\csname#1\endcsname\relax}
% Null command needed to eat its argument
\def\NullCom#1{}
\def\begin#1{%
% if defined \BeforeBeg for this environment, execute it
\IfUnDef{BeforeBeg#1}\else\csname BeforeBeg#1\endcsname\fi%
\IfUnDef{AfterBeg#1}% This is done to skip the command for environments
                     % which can take arguments, like multicols; YOU MUST NOT
                     % USE \AfterBegin{...}{...} for such environments! 
        \let\SaveBegEnd=\BeginEnvironment%
\else
        % Start this environment
                \BeginEnvironment{#1}%
        % and execute code after \begin{environment}
                \csname AfterBeg#1\endcsname
        \let\SaveBegEnd=\NullCom
\fi
\SaveBegEnd{#1}
}
\def\end#1{%
% execute code before \end{environment}
\IfUnDef{BeforeEnd#1}\else\csname BeforeEnd#1\endcsname\fi%
% close this environment
\EndEnvironment{#1}
% and execute code after \begin{environment}
\IfUnDef{AfterEnd#1}\else\csname AfterEnd#1\endcsname\fi%
}
\long\def\BeforeBegin#1#2{\expandafter\gdef\csname BeforeBeg#1\endcsname {#2}}
\long\def\BeforeEnd  #1#2{\expandafter\gdef\csname BeforeEnd#1\endcsname {#2}}
\long\def\AfterBegin #1#2{\expandafter\gdef\csname AfterBeg#1\endcsname {#2}}
\long\def\AfterEnd   #1#2{\expandafter\gdef\csname AfterEnd#1\endcsname{#2}}

%%%% end of atbeginend.sty

%  ****************************************
%  *            PAGE LAYOUT               *
%  ****************************************

% Page size, spacing parameters, etc. 

\textwidth=7.1in
\columnsep=0.3125in
\parindent=0.125in
\voffset=-20mm
\hoffset=-7.5mm

\topmargin=0in
\headheight=.15in
\headsep=0.5in
\oddsidemargin=0in
\evensidemargin=0in
\parskip=0cm

\tolerance=600          % 3x "normal" value; cuts down on overfull complaints

%% AV,MM, to have 64 lines per column, with textheight 25cm:
\textheight=64\baselineskip
\textheight=\baselinestretch\textheight
\ifdim\textheight>25.2cm\textheight=25.0cm\fi

%% so that the margin at the bottom of the page is about equal to margin at top. -- AH
\advance\textheight -54pt

\topskip\baselineskip
\maxdepth\baselineskip



\def\eqsecnum{
    \@newctr{equation}[section]
    \def\theequation{\hbox{\normalsize\arabic{section}-\arabic{equation}}}}

%% running heads:
\def\lefthead#1{\gdef\@versohead{#1}} \lefthead{\relax}
\def\righthead#1{\gdef\@rectohead{#1}} \righthead{\relax}
\let\shorttitle\lefthead
\let\shortauthors\righthead

\def\ps@apjheads{\let\@mkboth\markboth
     \def\@evenfoot{}
    \def\@evenhead{\lower9mm\hbox to\textwidth{
                     \rm\thepage\hfil \rm\textsc{\@rectohead} \hfil}}}
    \def\@oddfoot{}
    \def\@oddhead{\lower9mm\hbox to\textwidth{
                     \hfil\rm\textsc{\@versohead}\hfil \rm\thepage}}

\pagestyle{apjheads}

\@twosidetrue

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%    TITLE PAGE                                                  %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\long\def\frontmatter@title@above{
\ifmodern
\vglue-18pt
{\footnotesize
\raggedright
{\sc Draft version \today}\\[2pt]
{\footnotesize
Typeset using \LaTeX\ {\bf modern} style in AASTeX61}
\vskip48pt
}
\else
%%
\ifpreprint
\vspace*{-\headsep}\vspace*{\headheight}
\footnotesize
\noindent{\sc Draft version \today}\\[2pt]
{\footnotesize Typeset using \LaTeX\ {\bf preprint} style in AASTeX61}
\par\vspace*{-\baselineskip}\vspace*{0.625in}
\else
%%
\ifpreprinttwo
\vspace*{-\headsep}\vspace*{\headheight}
\footnotesize
{\footnotesize\textsc{\@journalinfo}}\par
{\footnotesize Typeset using \LaTeX\ {\bf preprint2} style in AASTeX61}
\par\vspace*{-\baselineskip}\vspace*{0.625in}
\else
%%
\iftwocolstyle
\vspace*{-\headsep}\vspace*{\headheight}
\footnotesize
{\footnotesize\textsc{\@journalinfo}}\par
{\footnotesize Typeset using \LaTeX\ {\bf twocolumn} style in AASTeX61}
\par\vspace*{-\baselineskip}\vspace*{0.625in}
\else
\ifmanu
\vspace*{-\headsep}\vspace*{\headheight}
\footnotesize
\noindent\textsc{\@journalinfo}\\[-8pt]
{\footnotesize Typeset using \LaTeX\ {\bf manuscript} style in AASTeX61}
\par\vspace*{-\baselineskip}\vspace*{0.625in}
\else
%% Default
\vspace*{-\headsep}\vspace*{\headheight}
\footnotesize
{\footnotesize\textsc{\@journalinfo}}\par
{\footnotesize Typeset using \LaTeX\ default style in AASTeX61}%% default style
\par\vspace*{-\baselineskip}\vspace*{0.625in}
\fi\fi\fi\fi\fi
}%

\def\frontmatter@title@produce{%
 \begingroup
\ifnumlines\nolinenumbers\fi
 \frontmatter@title@above
  \frontmatter@title@format
  \@title
\vskip12pt
  \@ifx{\@title@aux\@title@aux@cleared}{}{%
  \expandafter\frontmatter@footnote\expandafter{\@title@aux}%
  }%
  \par
%% \class@warn{Unused short title ignored}%
\ifmodern
\vskip-42pt
\else
\ifmanu
\vskip-60pt
\else
  \frontmatter@title@below
\fi
\fi
 \endgroup
}%

\newcount\fncount
\newcount\endfncount
\long\def\tempfootnote#1{\global\advance\fncount by 1\relax%
\expandafter\gdef\csname footnote\the\fncount\endcsname{#1}}

\long\def\abstracttempfootnote#1{\global\advance\fncount by 1\relax%
\expandafter\gdef\csname absfootnote\the\fncount\endcsname{#1}}

\def\tempfootnoteintitle#1{}

\long\def\ltx@foottext#1#2{%
 \begingroup
  \expandafter\ltx@make@current@footnote\expandafter{\@mpfn}{#1}%
\@footnotetext{#2}%
 \endgroup
}%

\def\kickoutfootnotes{\c@footnote=0\relax%
\loop\advance\endfncount by 1\relax%
\expandafter\ifx\csname footnote\the\endfncount\endcsname\relax%
\else%
\def\thempfn{\fnsymbol{footnote}}%
\advance\c@footnote by 1\relax%
\unskip\footnote{\csname footnote\the\endfncount\endcsname}%
\repeat}



%% 
\renewcommand\title[2][]{%
\def\@title{\setbox0=\vbox{\let\footnote\tempfootnote #2}%
{\let\footnote\tempfootnoteintitle\uppercase{#2}}
\kickoutfootnotes
\ifdoublespace\vskip 3\baselineskip\fi
}%
 \def\@shorttitle{#1}%
 \let\@AF@join\@title@join
}%


\def\frontmatter@title@format{\normalsize\centering}

\def\frontmatter@title@below{\vskip12pt}%

\def\frontmatter@authorformat{\small\scshape
\ifmodern
\vskip48pt
\centering
\leftskip=.05in plus 1fil
\rightskip=.05in plus 1 fil
\baselineskip=13pt
\else
\centering
\fi
}%


\def\frontmatter@affiliationfont{\normalfont\footnotesize\it
\ifmodern\baselineskip=14pt\fi
\iflongauthor\else
\rightskip-12pt plus 1fil
\leftskip6pt \parindent-4pt
\fi
}%

\def\frontmatter@finalspace{\vskip-24pt}%\vspace*{-\baselineskip}\vspace*{0.375in}}

\def\@separator{\\}%

\newcounter{front@matter@foot@note}\setcounter{front@matter@foot@note}{0}

\iflongauthor
\renewcommand\affiliation[1]{%
 \move@AU\move@AF%
\iflongauthor\let\@listand\relax\fi
 \begingroup%
  \@affiliation{%\hspace*{2mm}
\ifnum\countauthors<\AuthorCollaborationLimit
 #1\ifmodern\iflongauthor\baselineskip=12pt\else\vskip2pt\fi\else\baselineskip=12pt\fi\fi
\ifnum\countauthors=\AuthorCollaborationLimit
 #1\ifmodern\iflongauthor\baselineskip=12pt\else\vskip2pt\fi\else\baselineskip=12pt\fi\fi
\iflongauthor\vskip-12pt\ifnum\countauthors>\AuthorCollaborationLimit\iftwelvepoint\vskip-3pt\else\iftwocolstyle\else\vskip-6pt\fi\fi\fi%
\fi
}%
}%
\else
%% older version
\renewcommand\affiliation[1]{%
 \move@AU\move@AF%
 \begingroup%
  \@affiliation{%\hspace*{2mm}
 #1\ifmodern\iflongauthor\baselineskip=12pt\else\vskip2pt\fi\else\baselineskip=12pt\fi}%
}%
\fi %% end switch for longauthor


%   ABSTRACT
\def\frontmatter@abstractfont{\normalsize\parindent=9pt
}%
%\def\frontmatter@abstractwidth{6in}
\def\frontmatter@preabstractspace{12pt}
\def\frontmatter@postabstractspace{12pt}

\def\abstractname{ABSTRACT}
\long\def\frontmatter@abstractheading{%
 \begingroup
  \centering
  \abstractname
  \vskip 1mm
  \par
 \endgroup
}%

\newif\ifabstract%
\renewenvironment{frontmatter@abstract}{%
  \aftermaketitle@chk{\begin{abstract}}%
\global\abstracttrue
  \global\setbox\absbox\vbox\bgroup
   \color@begingroup
   \columnwidth\textwidth
   \hsize\columnwidth
   \@parboxrestore
   \def\@mpfn{mpfootnote}\def\thempfn{\thempfootnote)}\c@mpfootnote\z@ % should be footnote, not mpfootnote?
%   \let\@footnotetext\frontmatter@footnotetext
   \minipagefootnote@init
   \let\set@listindent\set@listindent@
   \let\@listdepth\@mplistdepth \@mplistdepth\z@
   \let@environment{description}{frontmatter@description}%
   \@minipagerestore
   \@setminipage
    \frontmatter@abstractheading
    \frontmatter@abstractfont
%    \let\footnote\mini@note
    \expandafter\everypar\expandafter{\the\everypar\addcontents@abstract\everypar{}}%
\ifnumlines\let\go\linenumbers\else\let\go\relax\fi\go
}{%
\ifnumlines\let\go\endlinenumbers\else\let\go\relax\fi\go
    \par
    \unskip
    \minipagefootnote@here
    \@minipagefalse   %% added 24 May 89
    \color@endgroup
\egroup% end setbox\absbox
}%

\let\abstract\frontmatter@abstract

\def\frontmatter@abstract@produce{%
  \par
  \preprintsty@sw{%
   \do@output@MVL{%
    \vskip\frontmatter@preabstractspace
    \vskip200\p@\@plus1fil
    \penalty-200\relax
    \vskip-200\p@\@plus-1fil
   }%
  }{%
   \addvspace{\frontmatter@preabstractspace}%
  }%
   \begingroup
    \dimen@\baselineskip
    \setbox\z@\vtop{\unvcopy\absbox}%
    \advance\dimen@-\ht\z@\advance\dimen@-\prevdepth
    \@ifdim{\dimen@>\z@}{\vskip\dimen@}{}%
   \endgroup
   \begingroup
    \prep@absbox
\unvbox\absbox
    \post@absbox
   \endgroup
  \@ifx{\@empty\mini@notes}{}{\mini@notes\par}%
  \addvspace\frontmatter@postabstractspace
\global\abstractfalse
}%

\newif\ifbib


%  ****************************************
%  *             KEYWORDS                 *
%  ****************************************


  \def\@keys@name{\textit{Keywords:}\/~\mbox{}}%

\newlength{\keys@width}
\def\frontmatter@keys@format{\ifmodern\vskip0pt\else\vspace*{0.5mm}\fi%
  \settowidth{\keys@width}{\normalsize\@keys@name}%
  \rightskip=0.5in\leftskip=\rightskip\parindent=0pt%
    \hangindent=\keys@width\hangafter=1\normalsize}%
\def\@keywords@produce#1{%
 \showKEYS@sw{%
  \begingroup%
   \frontmatter@keys@format%
   \@keys@name#1\par
  \endgroup
 }{%
  \@if@empty{#1}{}{%
   \class@warn{If you want your keywords to appear in your output, use document class option showkeys}%
  }%
 }%
}%

\let\subjectheadings=\keywords


%  ****************************************
%  *             FOOTNOTES                *
%  ****************************************

%% legacy notes and footnote code

% Footnotes on the last page: user issues \lastpagefootnotes. It catches all
% footnotes and issues them before \begin{refernces} or
% \begin{\thebibliography} or \begin{appendix}, whichever comes first,
% at the end of right column.  
%% ???
\newcounter{lastfootnote}
\let\orig@footnote=\footnote
%
\def\spit@out@footnotes@{\addtocounter{footnote}{-\c@lastfootnote}\vspace*{-\baselineskip}\vspace*{\skip\footins}\bgroup\footnotesize\lastfootnote\par\egroup\let\footnote=\orig@footnote}
%
\let\spit@out@footnotes\relax
%
\long\def\lastpagefootnotes{%
\raggedbottom% Have to use flushbottom with revtex4-1 but it eats away
             % last page footnotes
\setcounter{lastfootnote}{0}
\long\gdef\lastfootnote{\mbox{}}
\let\spit@out@footnotes\spit@out@footnotes@
\long\def\footnote##1{\refstepcounter{lastfootnote}\footnotemark\g@addto@macro\lastfootnote{\\[\footnotesep]\refstepcounter{footnote}\mbox{}\hspace*{3mm}\textsuperscript{\thefootnote}~##1}}
% We need to mess with footnotes in appendix only if it is in a
% different mode (twocol vs onecol) than the main text
\def\mess@with@appendix@footnotes{
\BeforeBegin{appendix}{\spit@out@footnotes\let\spit@out@footnotes\relax}
\BeforeEnd{appendix}{\spit@out@footnotes\let\spit@out@footnotes\relax}
\AfterEnd{appendix}{\let\footnote=\orig@footnote}
}

\if@two@col
  \if@two@col@app\else
    \mess@with@appendix@footnotes
  \fi
\fi

\BeforeBegin{references}{\spit@out@footnotes\let\spit@out@footnotes\relax}
\BeforeBegin{thebibliography}{\spit@out@footnotes\let\spit@out@footnotes\relax}
% in case \lastpagefootnotes were given inside \begin{appendix}\end{appendix},
\AfterEnd{references}{\let\footnote=\orig@footnote}
\AfterEnd{thebibliography}{\let\footnote=\orig@footnote}
}
\let\lastpagefootnote=\lastpagefootnotes

%% probably not needed:
\def\notetoeditor#1{}%   % We do not need notes to editor in the preprint
\def\placetable#1{}%   % We do not need notes to editor in the preprint
\def\placefigure#1{}%   % We do not need notes to editor in the preprint

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\ifdoublespace %used for manuscript
\footnotesep 12pt
\skip\footins 36pt
\else
\footnotesep 12pt
\skip\footins 24pt
\fi

\let\footnoterule\relax

\def\@makefntext#1{\mbox{}\hspace*{3mm}\@makefnmark~#1}


%  ****************************************
%  *             SECTIONS                 *
%  ****************************************

\setcounter{secnumdepth}{3}

\newif\if@firstsection \@firstsectiontrue

\def\section{%
\if@firstsection
      \maketitle
\global\@firstsectionfalse
     \setcounter{footnote}{\thefront@matter@foot@note}%
     \let\footnotetext=\old@foot@note@text
     \let\footnotemark=\old@foot@note@mark
   \clearpage
   \if@two@col
   \twocolumngrid
   \fi
\fi
    \@startsection{section}{1}{\z@}{9pt plus 1pt minus
    1pt}{4pt}{\apjsecfont\center}} 

\def\subsection{\@startsection{subsection}{2}{\z@}{9pt plus 1pt minus 1pt}{4pt}%
  {\normalsize\itshape \center}}

\def\subsubsection{\@startsection{subsubsection}{3}{\z@}%
  {2ex plus 1ex minus .2ex}{1ex plus .2ex}{\small\itshape \center}}

\def\paragraph{\@startsection{paragraph}{4}{\z@}%
  {1.5ex plus 1ex minus .2ex}{0pt}{\small\itshape}}

\def\subparagraph{\@startsection{subparagraph}{5}{\z@}%
  {1ex plus 1ex minus .2ex}{-0.5\parindent}{\small\itshape}}


\def\thesection{\arabic{section}}
\def\thesubsection{\thesection.\arabic{subsection}}
\def\thesubsubsection{\thesubsection.\arabic{subsubsection}}
\def\theparagraph{\thesubsubsection.\arabic{paragraph}}
\def\p@section        {}
\def\p@subsection     {}
\def\p@subsubsection  {}
\def\p@paragraph      {}
\def\p@subparagraph   {}


\def\sec@upcase#1{\uppercase{#1}}
\def\subsec@upcase#1{\relax{#1}}

%
% How the section number will appear in the section title - AV
\def\ApjSectionMarkInTitle#1{#1.\ }
\def\ApjSectionpenalty{0}


\def\@sect#1#2#3#4#5#6[#7]#8%
{\ifnum#2=1\setbox0=\hbox{\def\label##1{\gdef\templabel{##1}}#7}\fi
\@tempskipa #5\relax 
 \ifdim \@tempskipa >\z@ \begingroup
     #6\relax 
  \ifnum #2>\c@secnumdepth \def \@svsec {}\else 
    \refstepcounter{#1} \edef \@svsec {\ApjSectionMarkInTitle 
    {\csname the#1\endcsname}}\fi
  \@hangfrom {\hskip #3\relax 
    \ifnum #2=1{\secnum@size {\rm\@svsec~}}%
    \else {\subsecnum@size {\rm\@svsec~}}\fi }%
  {\interlinepenalty \@M 
   \ifnum #2=1\sec@upcase{#8}%
   \else \subsec@upcase{#8}\fi\par}\endgroup 
  \csname #1mark\endcsname {#7}\addcontentsline{toc}{#1}%
  {\ifnum #2>\c@secnumdepth \else \protect \numberline 
     {\csname the#1\endcsname }\fi #7}%
  \else 
  \ifnum #2>\c@secnumdepth \def \@svsec {}\else 
    \refstepcounter{#1} \edef \@svsec {\ApjSectionMarkInTitle 
    {\csname the#1\endcsname}}\fi
    \def \@svsechd {#6\hskip #3%
    \ifnum #2=1{\secnum@size{\rm\@svsec~}}\else{\subsecnum@size{\rm\@svsec~}}\fi%
    \ifnum #2=1\sec@upcase{#8}\else\subsec@upcase{#8}\fi%
    \ifnum #2=4\hskip 0.4ex{\rm ---}\fi%
     \csname #1mark\endcsname {#7}\addcontentsline{toc}{#1}%
      {\ifnum #2>\c@secnumdepth \else \protect \numberline {\csname
      the#1\endcsname }\fi #7}}\fi \@xsect {#5} \penalty \ApjSectionpenalty
%-refstepcounter is now within a group. So \@currentlabel, which is normally
%-set by \refstepcounter is hidden within a group. Need to set it manually. 
\protected@edef\@currentlabel{\csname p@#1\endcsname\csname
the#1\endcsname} 
\expandafter\ifx\csname templabel\endcsname\relax
\let\go\relax
\else
\def\go{\label{\templabel}}\fi\go
\let\templabel\relax
}

\def\@ssect#1#2#3#4#5{\@tempskipa #3\relax
   \ifdim \@tempskipa>\z@
     \begingroup #4\@hangfrom{\hskip #1}{\interlinepenalty \@M
       \sec@upcase{#5}\par}\endgroup
   \else \def\@svsechd{#4\hskip #1\relax \sec@upcase{#5}}\fi
    \@xsect{#3}
% MM:
\penalty \ApjSectionpenalty}


\def\acknowledgments{\vskip 5.8mm plus 1mm minus 1mm}
\let\acknowledgements=\acknowledgments                  % second spelling


%  ****************************************
%  *          APPENDIX                    *
%  ****************************************

\newcounter{remember@figure@num}
\newcounter{remember@table@num}


% this was an environment earlier, which doesn't make sense since we don't
% do \begin{appendix}...\end{appendix}. Changed to \appendix which is how it is used.

%   numberedappendix: Needed to label appendix sections A, B, .
%   appendixfloats: Needed. ??

\newif\ifappendixon
\def\appendix{
\global\appendixontrue
\onecolumngrid
%\clearpage
% \vrule used for extra space; otherwise revtex4-1 sometimes eats
% away the last line before appendix
        \noindent\mbox{}\vrule height 24pt width0pt\hfill{\apjsecfont APPENDIX}\hfill\mbox{}\par
        \nopagebreak\medskip\@nobreaktrue\def\ApjSectionpenalty{\@M}
        \@firstsectionfalse
          \setcounter{section}{0}
          \setcounter{subsection}{0}
          \setcounter{equation}{0}
%%
\ifletteredappendix
          \def\thesection{\Alph{section}}
          \def\theequation{\hbox{\Alph{section}\arabic{equation}}}
%% these are NOT supposed to reset to zero
%\setcounter{table}{0}
%\setcounter{figure}{0}
\fi
%%
\if@number@appendix@floats
% we don't want to set equations to zero in appendix, because there
% might then be two equation 1's, etc., confusing for cross referencing.
%\setcounter{equation}{0}
          \def\thesection{\Alph{section}}
          \def\theequation{\hbox{\Alph{section}\arabic{equation}}}
          \def\section{
\@startsection {section}{1}{\z@} 
            {10pt}{5pt}{\centering\scshape\apjsecfont}}
\else
% Do not use appendix numbers in the titles
          \def\ApjSectionMarkInTitle{\AppendixApjSectionMarkInTitle}
\fi
}
%

%%

%  ****************************************
%  *          BIBLIOGRAPHY                *
%  ****************************************

\renewenvironment{references}[0]{
  \onecolumngrid
  \par
  \vspace{10pt plus 3pt}
  \noindent \makebox[\textwidth][c]{\small\scshape REFERENCES}
  \par
  \vspace*{4pt plus 3pt}
  \set@column@hsize{2}\twocolumngrid
  \parindent=0cm \parskip=0cm
  \def\baselinestretch{1.0}
  \footnotesize \baselineskip=\baselinestretch\bibbaselineskip plus 1pt
  minus 1pt \interlinepenalty \@M
  \hyphenpenalty=10000
  \frenchspacing    % AV - to get right spacing after ``et al.'' 
  \def\refpar{\par\hangindent=1.2em\hangafter=1}}
{
  \onecolumngrid
}

% redefine thebibliography

% remove numbers from the reference list
\def\@biblabel#1{\relax}

\newskip\bibskip
\bibskip=0pt plus 1pt
\let\savebibitem\bibitem
\def\bibitem{\vskip\bibskip\savebibitem}
\newdimen\bibindent
\renewenvironment{thebibliography}[1]{\global\bibtrue

\onecolumngrid
\vspace{20pt}
\goodbreak
    \hbox to\textwidth{\hss\normalsize REFERENCES\hss}
\vspace{6pt}\parskip=0pt
\twocolumngrid 
\par
 \raggedright
\small
\ifmodern\else
 \vspace{10pt plus 3pt}\fi
\par
\topsep=0pt
 \list{}%
   {
     \parindent=0pt \parskip=1pt plus 1pt \parsep=0pt % AV
     \bibindent=0pt                          %
\ifmodern\vskip-12pt
\baselineskip=13pt plus 1pt
\else
\ifdoublespace
\baselineskip=20pt
\else
\baselineskip=13pt plus 1pt \fi\fi \interlinepenalty \@M  % AV
     \frenchspacing    % AV - to get right spacing after ``et al.'' 
     \hyphenpenalty=10000
     \itemindent=-1.0em                      %
     \itemsep=0pt                            %
     \listparindent=0pt                      %
     \settowidth\labelwidth{0pt} %
     \labelsep=0pt                           %
     \leftmargin=1.0em
     \advance\leftmargin\labelsep
%%%      \usecounter{enumiv}%
      \let\p@enumiv\@empty
      \renewcommand\theenumiv{\relax}}%
    \sloppy\clubpenalty10000\widowpenalty10000%
    \sfcode`\.\@m\relax
%%%\item[] This May be necessary, but causes extra vertical space in first column
%%%          of the bibliography.
}
  {\def\@noitemerr
    {\@latex@warning{Empty `thebibliography' environment}}%
\endlist
    \onecolumngrid % to balance references
\global\bibfalse
\newpage
  }

% %% AV: 

\def\reference{\@ifnextchar\bgroup {\@reference}
        {\@latexerr{Missing key on reference command}
        {Each reference command should have a key corresponding to a markcite somewhere in the text}}}
\def\@reference#1{\refpar}

%% subtitle header and journal info, legacy, probably not needed
% \def\submitted#1{\gdef\@submitted{#1}}
% \let\slugcomment\submitted   % slugcomment == submitted
% \submitted{Draft version \today}
% \journalinfo{\@submitted}

 \def\journalinfo#1{\gdef\@journalinfo{#1}}
 \journalinfo{Draft version \today}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Equations                                             %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% EQNARRAY with reduced spacing around tab characters - AV
\def\eqnarray{%
  \stepcounter{equation}%
  \def\@currentlabel{\p@equation\theequation}%
  \global\@eqnswtrue
  \setlength{\arraycolsep}{0.25\arraycolsep}
  \m@th
  \global\@eqcnt\z@
  \tabskip\@centering
  \let\\\@eqncr
  $$\everycr{}\halign to\displaywidth\bgroup
  \hskip\@centering$\displaystyle\tabskip\z@skip{##}$\@eqnsel
  &\global\@eqcnt\@ne\hskip \tw@\arraycolsep \hfil${##}$\hfil
  &\global\@eqcnt\tw@ \hskip \tw@\arraycolsep
  $\displaystyle{##}$\hfil\tabskip\@centering
  &\global\@eqcnt\thr@@ \hb@xt@\z@\bgroup\hss##\egroup
  \tabskip\z@skip
  \cr
  }

%  ****************************************
%  *         TABLES AND FIGURES           *
%  ****************************************

\def\@arstrut@hline@clnc{0.5\p@}% % Klootch: magic number

\setcounter{topnumber}{7}

\setlength{\belowcaptionskip}{4pt}% 
\setlength{\abovecaptionskip}{5pt}

\setlength{\textfloatsep}{9pt}
\setlength{\dbltextfloatsep}{0pt}

%  \addtolength{\textfloatsep}{17mm plus 10mm minus 10mm}
 % \addtolength{\dbltextfloatsep}{7mm plus 10mm minus 10mm}


\renewcommand{\topfraction}{1.0}
\renewcommand{\bottomfraction}{1.0}
\renewcommand{\textfraction}{0.0}
\renewcommand{\dbltopfraction}{0.85}
\renewcommand{\dblfloatpagefraction}{0.85}
\setcounter{topnumber}{9}
\setcounter{bottomnumber}{9}
\setcounter{totalnumber}{20}
\setcounter{dbltopnumber}{9} 

% Copied from revtex4.cls; without it, captions are centered
\def\@xfloat@prep{%
  \let\footnote\footnote@latex
  \def\@mpfn{mpfootnote}%
  \def\thempfn{\thempfootnote}%
  \c@mpfootnote\z@
  \let\@footnotetext\@mpfootnotetext
  \let\H@@footnotetext\@mpfootnotetext
  \let\@makefntext\@mpmakefntext
}%


%%%%%%%%%%%% \cutinhead

%% Number of \pt@ncol set when \tablecolumns{} used at beginning of
%% deluxetable.

\def\@ptabularcr{\\}
\newcommand\cutinhead[1]{% 
 \noalign{\vskip 1.5ex}% 
 \hline 
 \@ptabularcr 
 \noalign{\vskip -1.5ex}% 
 \multicolumn{\pt@ncol}{c}{#1}% 
 \@ptabularcr 
 \noalign{\vskip .8ex}% 
 \hline 
 \@ptabularcr 
 \noalign{\vskip -2ex}% 
}% 

\newcommand\sidehead[1]{% 
 \noalign{\vskip 1.5ex}% 
%  \hline 
%  \@ptabularcr 
%  \noalign{\vskip -1.5ex}% 
 \multicolumn{\pt@ncol}{l}{#1}% 
 \@ptabularcr 
 \noalign{\vskip .8ex}% 
%  \hline 
%  \@ptabularcr 
%  \noalign{\vskip -2ex}% 
}% 


%% these don't seem to be relevant:
\newcommand\figcaption{\@testopt{\@xfigcaption}{}}% 
%% suggested by Joern Wilms
\def\@figcaption#1{{\def\@captype{figure}\caption{\footnotesize #1}}}
\def\@xfigcaption[#1]#2{{\def\@captype{figure}\caption{\footnotesize
#2}}}

\def\thefigure{\@arabic\c@figure}

\def\fnum@figure{{\footnotesize{\@eapj@cap@font\rm
\mbox{\@eapj@figname~\thefigure}% <== was period here
}}}

\def\thetable{\@arabic\c@table}
%%% Table captions without making a floating table
\def\tabcaption{\@ifnextchar[{\@xtabcaption}{\@tabcaption}}
\def\@tabcaption#1{{\def\@captype{table}\caption{#1}}}
\def\@xtabcaption[#1]#2{{\def\@captype{table}\caption{#2}}}
\def\fnum@table{{\@eapj@cap@font \@eapj@tabname~\thetable}}

 \let\fnum@ptable=\fnum@table
 \def\fnum@ptablecont{{\centering{\scshape Table~\thetable}---{\itshape
 Continued}}}% 
 \long\def\@make@caption@text#1#2{% 
   {\small\centering#1{\scshape #2}\par\vskip1.4ex}
 }% 

\long\def\@makecaption@plano@cont#1#2{% 
  {\small \centering#1\par}\vskip1.4ex\relax
}% 


%% Commands from aastex.cls:
\newcommand\dataset{\@testopt\@dataset{[}}%
\def\@dataset[#1]#2{#2}%
\newcommand\facility{\@testopt\@facility{[}}%
\def\@facility[#1]#2{{\vskip6pt{\large\it Facility:} #2}}%

\newcommand\facilities{\@testopt\@facilities{[}}%
\def\@facilities[#1]#2{{\vskip6pt{\large\it Facilities:} #2}}%

\newcommand\software{\@testopt\@software{[}}%
\def\@software[#1]#2{{\vskip6pt{\large\it Software:} #2}}%

\newcommand\object{\@testopt\@object{[}}%
\def\@object[#1]#2{#2}%
\newcommand\objectname{\@testopt\@objectname{[]}}% 
\def\@objectname[#1]#2{#2}% 
\newlength{\plot@width}
\def\eps@scaling{1.0}% 
\newcommand\epsscale[1]{\def\eps@scaling{#1}}% 
\newcommand\plotone[1]{% 
 \centering 
 \leavevmode 
 \setlength{\plot@width}{0.85\linewidth}
 \includegraphics[width={\eps@scaling\plot@width}]{#1}% 
}% 
\newcommand\plottwo[2]{% 
 \centering 
 \leavevmode 
 \setlength{\plot@width}{0.425\linewidth}
 \includegraphics[width={\eps@scaling\plot@width}]{#1}% 
 \hfil 
 \includegraphics[width={\eps@scaling\plot@width}]{#2}% 
}% 
\newcommand\plotfiddle[7]{% 
 \centering 
 \leavevmode 
 \vbox\@to#2{\rule{\z@}{#2}}% 
 \includegraphics[% 
  scale=#4, 
  angle=#3, 
  origin=c 
 ]{#1}% 
}% 
\newcommand\figurenum[1]{% 
 \def\thefigure{#1}% 
 \let\@currentlabel\thefigure 
 \addtocounter{figure}{\m@ne}% 
}% 

\newcommand\phn{\phantom{0}}% 
\newcommand\phd{\phantom{.}}% 
\newcommand\phs{\phantom{$-$}}% 
\newcommand\phm[1]{\phantom{#1}}% 
\let\la=\lesssim            % For Springer A&A compliance... 
\let\ga=\gtrsim 
\newcommand\sq{\mbox{\rlap{$\sqcap$}$\sqcup$}}% 
\newcommand\arcdeg{\mbox{$^\circ$}}% 
\newcommand\arcmin{\mbox{$^\prime$}}% 
\newcommand\arcsec{\mbox{$^{\prime\prime}$}}% 
\newcommand\fd{\mbox{$.\!\!^{\mathrm d}$}}% 
\newcommand\fh{\mbox{$.\!\!^{\mathrm h}$}}% 
\newcommand\fm{\mbox{$.\!\!^{\mathrm m}$}}% 
\newcommand\fs{\mbox{$.\!\!^{\mathrm s}$}}% 
\newcommand\fdg{\mbox{$.\!\!^\circ$}}% 
\newcommand\farcm@mss{\mbox{$.\mkern-4mu^\prime$}}% 
\let\farcm\farcm@mss 
\newcommand\farcs@mss{\mbox{$.\!\!^{\prime\prime}$}}% 
\let\farcs\farcs@mss 
\newcommand\fp{\mbox{$.\!\!^{\scriptscriptstyle\mathrm p}$}}% 
\newcommand\micron{\mbox{$\mu$m}}% 
\def\farcm@apj{% 
 \mbox{.\kern -0.7ex\raisebox{.9ex}{\scriptsize$\prime$}}% 
}% 
\def\farcs@apj{% 
 \mbox{% 
  \kern  0.13ex.% 
  \kern -0.95ex\raisebox{.9ex}{\scriptsize$\prime\prime$}% 
  \kern -0.1ex% 
 }% 
}% 
 

\newcommand\ion[2]{#1$\;${%
\ifx\@currsize\normalsize\small \else
\ifx\@currsize\small\footnotesize \else
\ifx\@currsize\footnotesize\scriptsize \else
\ifx\@currsize\scriptsize\tiny \else
\ifx\@currsize\large\normalsize \else
\ifx\@currsize\Large\large
\fi\fi\fi\fi\fi\fi
\rmfamily\@Roman{#2}}\relax}% 

\renewcommand\case[2]{\mbox{$\frac{#1}{#2}$}}% 
\renewcommand\slantfrac{\case}% 
\newcommand\onehalf{\slantfrac{1}{2}}% 
\newcommand\onethird{\slantfrac{1}{3}}% 
\newcommand\twothirds{\slantfrac{2}{3}}% 
\newcommand\onequarter{\slantfrac{1}{4}}% 
\newcommand\threequarters{\slantfrac{3}{4}}% 
\newcommand\ubvr{\mbox{$U\!BV\!R$}}%% UBVR system 
\newcommand\ub{\mbox{$U\!-\!B$}}%   % U-B 
\newcommand\bv{\mbox{$B\!-\!V$}}%   % B-V 
\renewcommand\vr{\mbox{$V\!-\!R$}}%   % V-R ++
\newcommand\ur{\mbox{$U\!-\!R$}}%   % U-R 

%% need this change so that it works correctly in tables:
{\catcode`\$=\active
\gdef\nodata{ ~$\cdots$~ }}% 

\newcommand\diameter{\ooalign{\hfil/\hfil\crcr\mathhexbox20D}}% 
\newcommand\degr{\arcdeg}% 
\newcommand\Sun{\sun}% 
\newcommand\Sol{\sun}% 
\newcommand\sun{\odot}% 
\newcommand\Mercury{\astro{\char1}}% Mercury symbol, "1" 
\newcommand\Venus{\astro{\char2}}% Venus symbol, "2" 
\newcommand\Earth{\earth}% 
\newcommand\Terra{\earth}% 
\newcommand\earth{\oplus}% 
\newcommand\Mars{\astro{\char4}}% Mars symbol, "4" 
\newcommand\Jupiter{\astro{\char5}}% Jupiter symbol, "5" 
\newcommand\Saturn{\astro{\char6}}% Saturn symbol, "6" 
\newcommand\Uranus{\astro{\char7}}% Uranus symbol, "7" 
\newcommand\Neptune{\astro{\char8}}% Neptune symbol, "8" 
\newcommand\Pluto{\astro{\char9}}% Pluo symbol, "9" 
\newcommand\Moon{\astro{\char10}}% Moon symbol, "M" 
\newcommand\Luna{\Moon}% 
\newcommand\Aries{\astro{\char11}}% 
\newcommand\VEq{\Aries}% vernal equinox (Aries) 
\newcommand\Taurus{\astro{\char12}}% 
\newcommand\Gemini{\astro{\char13}}% 
\newcommand\Cancer{\astro{\char14}}% 
\newcommand\Leo{\astro{\char15}}% 
\newcommand\Virgo{\astro{\char16}}% 
\newcommand\Libra{\astro{\char17}}% 
\newcommand\AEq{\Libra}% autumnal equinox (Libra) 
\newcommand\Scorpius{\astro{\char18}}% 
\newcommand\Sagittarius{\astro{\char19}}% 
\newcommand\Capricornus{\astro{\char20}}% 
\newcommand\Aquarius{\astro{\char21}}% 
\newcommand\Pisces{\astro{\char22}}% 
 

\newcommand\sbond{\chem@bnd{\@sbnd}}%
\newcommand\dbond{\chem@bnd{\@dbnd}}%
\newcommand\tbond{\chem@bnd{\@tbnd}}%
\def\chem@bnd#1{%
 {%
  \kern.1em\relax
  \setbox\z@\hbox{M}%
  \dimen@ii.8em\relax
  \p@=.1em\relax
  \dimen@.5\ht\z@\dimen@i-\dimen@
  \advance\dimen@1.5\p@\advance\dimen@i-1.0\p@
  #1%
  \kern.1em\relax
  }%
 }%
\def\@sbnd{%
 \advance\dimen@-1.5\p@\advance\dimen@i1.5\p@
 \vrule\@height\dimen@\@depth\dimen@i\@width\dimen@ii\nobreak
 }%
\def\@dbnd{%
 \advance\dimen@-0.5\p@\advance\dimen@i0.5\p@
 \vrule\@height\dimen@\@depth\dimen@i\@width\dimen@ii\nobreak
 \advance\dimen@-1.5\p@\advance\dimen@i1.5\p@
 \hskip-\dimen@ii
 \vrule\@height\dimen@\@depth\dimen@i\@width\dimen@ii\nobreak
 }%
\def\@tbnd{%
 \vrule\@height\dimen@\@depth\dimen@i\@width\dimen@ii\nobreak
 \advance\dimen@-1.5\p@\advance\dimen@i1.5\p@
 \hskip-\dimen@ii
 \vrule\@height\dimen@\@depth\dimen@i\@width\dimen@ii\nobreak
 \advance\dimen@-1.5\p@\advance\dimen@i1.5\p@
 \hskip-\dimen@ii
 \vrule\@height\dimen@\@depth\dimen@i\@width\dimen@ii\nobreak
 }%

\newcommand\anchor[2]{#2}% 
\renewcommand\url{\@dblarg\@url}% 
\def\@url[#1]{\anchor{#1}}% 

\let\jnl@style=\rmfamily 
\def\ref@jnl#1{{\jnl@style#1}}% 
\newcommand\aj{\ref@jnl{AJ}}%        % Astronomical Journal 
\newcommand\araa{\ref@jnl{ARA\&A}}%  % Annual Review of Astron and Astrophys 
\renewcommand\apj{\ref@jnl{ApJ}}%    % Astrophysical Journal ++
\newcommand\apjl{\ref@jnl{ApJL}}     % Astrophysical Journal, Letters 
\newcommand\apjs{\ref@jnl{ApJS}}%    % Astrophysical Journal, Supplement 
\renewcommand\ao{\ref@jnl{ApOpt}}%   % Applied Optics ++
\newcommand\apss{\ref@jnl{Ap\&SS}}%  % Astrophysics and Space Science 
\newcommand\aap{\ref@jnl{A\&A}}%     % Astronomy and Astrophysics 
\newcommand\aapr{\ref@jnl{A\&A~Rv}}%  % Astronomy and Astrophysics Reviews 
\newcommand\aaps{\ref@jnl{A\&AS}}%    % Astronomy and Astrophysics, Supplement 
\newcommand\azh{\ref@jnl{AZh}}%       % Astronomicheskii Zhurnal 
\newcommand\baas{\ref@jnl{BAAS}}%     % Bulletin of the AAS 
\newcommand\icarus{\ref@jnl{Icarus}}% % Icarus
\newcommand\jrasc{\ref@jnl{JRASC}}%   % Journal of the RAS of Canada 
\newcommand\memras{\ref@jnl{MmRAS}}%  % Memoirs of the RAS 
\newcommand\mnras{\ref@jnl{MNRAS}}%   % Monthly Notices of the RAS 
\renewcommand\pra{\ref@jnl{PhRvA}}% % Physical Review A: General Physics ++
\renewcommand\prb{\ref@jnl{PhRvB}}% % Physical Review B: Solid State ++
\renewcommand\prc{\ref@jnl{PhRvC}}% % Physical Review C ++
\renewcommand\prd{\ref@jnl{PhRvD}}% % Physical Review D ++
\renewcommand\pre{\ref@jnl{PhRvE}}% % Physical Review E ++
\renewcommand\prl{\ref@jnl{PhRvL}}% % Physical Review Letters 
\newcommand\pasp{\ref@jnl{PASP}}%     % Publications of the ASP 
\newcommand\pasj{\ref@jnl{PASJ}}%     % Publications of the ASJ 
\newcommand\qjras{\ref@jnl{QJRAS}}%   % Quarterly Journal of the RAS 
\newcommand\skytel{\ref@jnl{S\&T}}%   % Sky and Telescope 
\newcommand\solphys{\ref@jnl{SoPh}}% % Solar Physics 
\newcommand\sovast{\ref@jnl{Soviet~Ast.}}% % Soviet Astronomy 
\newcommand\ssr{\ref@jnl{SSRv}}% % Space Science Reviews 
\newcommand\zap{\ref@jnl{ZA}}%       % Zeitschrift fuer Astrophysik 
\renewcommand\nat{\ref@jnl{Nature}}%  % Nature 
\newcommand\iaucirc{\ref@jnl{IAUC}}% % IAU Cirulars 
\newcommand\aplett{\ref@jnl{Astrophys.~Lett.}}%  % Astrophysics Letters 
\newcommand\apspr{\ref@jnl{Astrophys.~Space~Phys.~Res.}}% % Astrophysics Space Physics Research 
\newcommand\bain{\ref@jnl{BAN}}% % Bulletin Astronomical Institute of the Netherlands 
\newcommand\fcp{\ref@jnl{FCPh}}%   % Fundamental Cosmic Physics 
\newcommand\gca{\ref@jnl{GeoCoA}}% % Geochimica Cosmochimica Acta 
\newcommand\grl{\ref@jnl{Geophys.~Res.~Lett.}}%  % Geophysics Research Letters 
\renewcommand\jcp{\ref@jnl{JChPh}}%     % Journal of Chemical Physics 
\newcommand\jgr{\ref@jnl{J.~Geophys.~Res.}}%     % Journal of Geophysics Research 
\newcommand\jqsrt{\ref@jnl{JQSRT}}%   % Journal of Quantitiative Spectroscopy and Radiative Trasfer 
\newcommand\memsai{\ref@jnl{MmSAI}}% % Mem. Societa Astronomica Italiana 
\newcommand\nphysa{\ref@jnl{NuPhA}}%     % Nuclear Physics A 
\newcommand\physrep{\ref@jnl{PhR}}%       % Physics Reports 
\newcommand\physscr{\ref@jnl{PhyS}}%        % Physica Scripta 
\newcommand\planss{\ref@jnl{Planet.~Space~Sci.}}%  % Planetary Space Science 
\newcommand\procspie{\ref@jnl{Proc.~SPIE}}%      % Proceedings of the SPIE 

\newcommand\actaa{\ref@jnl{AcA}}%  % Acta Astronomica
\newcommand\caa{\ref@jnl{ChA\&A}}%  % Chinese Astronomy and Astrophysics
\newcommand\cjaa{\ref@jnl{ChJA\&A}}%  % Chinese Journal of Astronomy and Astrophysics
\newcommand\jcap{\ref@jnl{JCAP}}%  % Journal of Cosmology and Astroparticle Physics
\newcommand\na{\ref@jnl{NewA}}%  % New Astronomy
\newcommand\nar{\ref@jnl{NewAR}}%  % New Astronomy Review
\newcommand\pasa{\ref@jnl{PASA}}%  % Publications of the Astron. Soc. of Australia
\newcommand\rmxaa{\ref@jnl{RMxAA}}%  % Revista Mexicana de Astronomia y Astrofisica

%% added feb 9, 2016
\newcommand\maps{\ref@jnl{M\&PS}}% Meteoritics and Planetary Science
\newcommand\aas{\ref@jnl{AAS Meeting Abstracts}}% American Astronomical Society Meeting Abstracts
\newcommand\dps{\ref@jnl{AAS/DPS Meeting Abstracts}}% American Astronomical Society/Division for Planetary Sciences Meeting Abstracts



\let\astap=\aap 
\let\apjlett=\apjl 
\let\apjsupp=\apjs 
\let\applopt=\ao 

\newcommand\ulap[1]{\vbox\@to\z@{{\vss#1}}}% 
\newcommand\dlap[1]{\vbox\@to\z@{{#1\vss}}}% 


\newcounter{table@save}

\def\tablenum#1{%
  \setcounter{table@save}{\the\c@table}
  \gdef\use@tablenum{1}
  \setcounter{table}{#1}\def\thetable{#1}\def\@currentlabel{#1}
  %\def\label##1{\save@label{##1}}
}%
\gdef\use@tablenum{0}
\def\restore@tablenum{\if\use@tablenum0\else\setcounter{table}{\the\c@table@save}\addtocounter{table}{\m@ne}\gdef\use@tablenum{0}\fi}

\def\tabletypesize#1{\gdef\currtabletypesize{#1}
\def\@table@type@size{#1}}%

\tabletypesize{\small}
\let\tablefontsize=\tabletypesize % for compatibility with old documents

\gdef\@tablecaption{}
\def\tablecaption#1{\gdef\@tablecaption{#1}}

\def\LT@endpbox{%
  \@finalstrut\@arstrutbox
  \egroup
  \the\LT@p@ftn
  \global\LT@p@ftn{}%
  \hfil}

%% Used for longtable
\def\LT@makecaption#1#2#3{%
  \LT@mcol\LT@cols c{\hbox to\z@{\hss\parbox[t]\LTcapwidth
{%
\def \@currentlabel{\thetable}
     \sbox\@tempboxa{\small #2. #3}%
     \ifdim\wd\@tempboxa>\hsize
      \small #2. #3%
     \else
       \hbox to\hsize{\hfil\box\@tempboxa\hfil}%
     \fi
    \endgraf\vskip\baselineskip}%
  \hss}}}

\let\LT@makecaption@rtx=\LT@makecaption % to fight redefinition in Revtex-4.1

\def\xfigure{figure}
%% from book.cls/ used??
\long\def\@makecaption#1#2{%
  \vskip\abovecaptionskip
\ifx\@captype\xfigure
\gdef \@currentlabel{\thefigure}
\else
\gdef \@currentlabel{\thetable}\fi
%% \small added to keep currtabletypesize from determining size of caption
  \sbox\@tempboxa{\small
{\bf #1.} #2}%
  \ifdim \wd\@tempboxa >\hsize
\small
{\bf    #1.} #2\par 
  \else
    \global \@minipagefalse
    \hb@xt@\hsize{\hfill\box\@tempboxa\hfill}%
  \fi
  \vskip\belowcaptionskip}

\newdimen\@abovenoteskip
\newcommand\tablerefs[1]{\ifdim\@abovenoteskip=0pt\global\@abovenoteskip=10pt\fi
{\small\@tableref{\parfillskip\z@ plus1fil\relax #1\endgraf}}}%

\def\@tableref#1{%
 \par
 \vspace*{3ex}%
 {%\parbox{\pt@width} %%%%
 {\hskip1em\rm References. --- #1}\par}%
}%


\global\def\tablenotemark#1{{\normalfont\textsuperscript{#1}}}
\global\def\tablenotetext#1#2{\footnotetext[#1]{\currtabletypesize\relax#2}}

%% redefined by AH below, since it wasn't working with tabular table
\global\def\tablenotetext#1#2{\vskip-8pt\vskip1sp\flushleft{\currtabletypesize
\noindent\hskip1em $^{#1}$ #2}\vskip1sp}


\newif\if@table@not@headed

%% this version of \tablehead doesn't seem to be used, so set to \xyztablehead{}
\def\xyztablehead#1{\@table@not@headedfalse%
  \kill
  \caption{\\%
    \@tablecaption}%
    \\\hline\hline%
  #1\vrule height 12pt depth 10pt width 0pt\relax 
\hskip\tabcolsep\\[.7ex]
  \hline\\[-1.5ex]
  \endfirsthead
  \caption[]{--- \emph{Continued}}\\
  \hline
  \hline\\[-1.7ex]
  #1\hskip\tabcolsep\\[.7ex]
  \hline\\[-1.5ex]
  \endhead
  \hline
  \endfoot%
}

\newlength{\table@note@skip}
\setlength{\table@note@skip}{0.5ex}
\newlength{\deluxe@table@width}
\newlength{\@d@t@a}
\newcounter{deluxe@table@num}
\newdimen\LTcapwidth

%% \ignorespaces necessary ++== depth 6pt was depth 3pt
\def\colhead#1{\multicolumn{1}{c}{\vrule depth 6pt width
0pt\relax#1}\ignorespaces}
\def\twocolhead#1{\multicolumn{2}{c}{\hss\vrule depth 6pt width
0pt\relax#1\hss}\ignorespaces}
\def\nocolhead#1{\multicolumn{1}{h}{}\ignorespaces}
\def\dcolhead#1{\multicolumn{1}{c}{$\vrule depth 6pt
width0pt\relax#1$}\ignorespaces}

%\newcounter{LT@tables}
\def\tablewidth#1{%
  \ifdim#1=\z@
  \else
  \gdef\@d@t@@flag{1}
  \if@filesw\immediate\write\@auxout{%
   \gdef\expandafter\noexpand
   \csname deluxe@table@width@\romannumeral\c@LT@tables\endcsname
   {#1}}
  \fi
  \fi
}


\def\save@natural@width{%
      \ifnum\@d@t@@flag=0
        \setlength{\@d@t@a}{0pt}%
        \let\@d@t@b=\LT@entry%
        \def\LT@entry##1##2{\addtolength{\@d@t@a}{##2}%
        }%
        \expandafter\csname LT@\romannumeral\c@deluxe@table@num\endcsname
        \setlength{\@d@t@a}{-\@d@t@a}
        \tablewidth{\the\@d@t@a}
        \def\LT@entry{\@d@t@b}
      \fi
}

\def\lt@expand@linewidth@one{\setlength\LTleft{0pt}\setlength\LTright{0pt}}
\def\lt@expand@linewidth@two{@{\extracolsep{0pt plus 1filll}}}
\def\find@table@width{%
%%% set table width using aux file and command \tablewidth
    \setcounter{deluxe@table@num}{\c@LT@tables}
    \refstepcounter{deluxe@table@num}
    \expandafter\ifx\csname deluxe@table@width@\romannumeral\c@deluxe@table@num\endcsname\relax
      \def\@d@t@{0.999\linewidth}
    \else
      \edef\@d@t@{\expandafter\csname deluxe@table@width@\romannumeral\c@deluxe@table@num\endcsname}
    \fi
    \ifdim\@d@t@<\z@% then natural width is used
      \setlength{\deluxe@table@width}{-\@d@t@}
      \setlength{\LTcapwidth}{-\@d@t@}
      \def\lt@expand@linewidth{\relax}
      \def\lt@expand@linewidth@{}
    \else% we will enclose table in the minipage of the given width and make
         % longtable to span the full minipage width
      \ifdim\@d@t@>\z@\else\def\@d@t@{0.999\linewidth}\fi
      \setlength{\deluxe@table@width}{\@d@t@}
      \setlength{\LTcapwidth}{\@d@t@}
      \def\lt@expand@linewidth{\lt@expand@linewidth@one}
      \def\lt@expand@linewidth@{\lt@expand@linewidth@two}
    \fi
}

\newlength{\abovedeluxetableskip}
\newlength{\belowdeluxetableskip}
\setlength{\abovedeluxetableskip}{0pt}
\setlength{\belowdeluxetableskip}{0pt}
\setlength{\tabcolsep}{5pt}

\setlength\doublerulesep{1.5pt}
\newdimen\lastrowheight
\def\set@last@row@height{\setlength{\lastrowheight}{\ht\strutbox}\addtolength{\lastrowheight}{\dp\strutbox}\setlength{\lastrowheight}{-\arraystretch\lastrowheight}}

\let\tableline=\colrule % Revtex said: Command \tableline is obsolete; Use \colrule instead.. 

%% 
\newtoks\DT@p@ftn 
\global\def\xtablenotetext@DT#1#2{
  \edef\@tempa{\the\DT@p@ftn\noexpand\tablenotemark{#1}~}
  \global\DT@p@ftn\expandafter{\@tempa{\@table@type@size#2}\par}}%

%%% AH %%%%%%%%%%%%%%%%%%%%%
\let\savedollar$
\catcode`\$=\active
\let$\savedollar

%%

\def\resetdecimals{\global\let\zdoit\relax\global\let\ddoit\relax}

\def\tableheadfrac#1{}
\newcount\pt@column 
\newcount\pt@ncol 

\newcommand\tablecolumns[1]{% 
 \pt@column=#1\relax 
 \pt@ncol=#1\relax 
 \global\let\pt@addcol\@empty 
}% 

%% from older version, probably can delete:
\def\@tablecom#1{% 
 \vspace*{\table@note@skip}
\par 
{\parbox{\linewidth}{\hskip1em\rmfamily {\@eapj@cap@font Note}. --- #1}\par}% 
}% 
\def\@tableref#1{% 
 \vspace*{\table@note@skip}
\par 
{\parbox{\linewidth}{\hskip1em\rmfamily {\@eapj@cap@font References}. --- #1}\par}% 
}% 
\def\spew@tblnotes{% 
 \@ifx@empty\tblref@list{}{% 
  \@tablenotes{\tblref@list}%
  \vspace*{\table@note@skip}%
  \global\let\tblref@list\@empty 
 }% 
 \@ifx@empty\tblnote@list{}{% 
  \@tablenotes{\tblnote@list}% 
  \vspace*{\table@note@skip}%
  \global\let\tblnote@list\@empty
 }
 \the\DT@p@ftn%
}% 

%% for notes on emulateapj please see http://hea-www.harvard.edu/~alexey/emulateapj
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% End of code taken from emulateapj.cls %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% New as of august 2015:

%% These commands requested AAS
\newcommand{\noprint}[1]{}
\newcommand{\figsetstart}{{\bf Fig. Set} }
\newcommand{\figsetend}{}
\newcommand{\figsetgrpstart}{}
\newcommand{\figsetgrpend}{}
\newcommand{\figsetnum}[1]{{\bf #1.}}
\newcommand{\figsettitle}[1]{ {\bf #1}}
\newcommand{\figsetgrpnum}[1]{\noprint{#1}}
\newcommand{\figsetgrptitle}[1]{\noprint{#1}}
\newcommand{\figsetplot}[1]{\noprint{#1}}
\newcommand{\figsetgrpnote}[1]{\noprint{#1}}

%% for url's in document, will allow them to break over lines.
\usepackage{url}

%% for tables continuing over pages
\usepackage{longtable}

%% for editing changes
\usepackage{xcolor}
% hyperref link defaults to "blue" (0000ff) as this matches our publisher produced pdf style
\definecolor{xlinkcolor}{cmyk}{1,1,0,0}


%% In response to request from AAS
 \usepackage[bookmarks=false,         % show bookmarks bar?
     pdfnewwindow=true,      % links in new window
     colorlinks=true,    % false: boxed links; true: colored links
     linkcolor=xlinkcolor,     % color of internal links
     citecolor=xlinkcolor,     % color of links to bibliography
     filecolor=xlinkcolor,  % color of file links
     urlcolor=xlinkcolor,      % color of external links
final=true
 ]{hyperref}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Additions to  AASTeX by Amy Hendrickson, TeXnology Inc, August 17, 2015

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Table Tools, written by Amy Hendrickson
%% for American Astronomical Society
%% August 17, 2015
%% array package is necessary:
\usepackage{array}

%%%%%%%%
%% 1) h in table preamble will makes text in that column ignored.

%%%%%%%%
%% 2) uppercase C L or R will make those columns in math mode.

%%%%%%%%
%% 3) \begin{splittabular}{<preamble B preamble>}...\end{splittabular}
%%    `B' in the preamble will show where the table should be broken. It may
%%    be used once in a preamble to break the table into two parts, or 
%%    two times in a preamble to break the table into three parts.

%%    The resulting table will position left half of table above right half of table.

%%    Care should be taken with \multicolumn so that it won't be broken between
%%    the two parts of the table. You may need to shorten the \multicolumn argument
%%    for number of columns to be appropriate to the number of columns in
%%    the new split table.

%%     In this example, for instance, we start with:
%%        \begin{tabular}{ccccccc}
%%        \multicolumn{7}{c}{\textsc{Table 1}}
%%     and change it to:
%%        \begin{splittabular}{ccccBccc}
%%        \multicolumn{4}{c}{\textsc{Table 1}}\\
%% 
%%     If you'd like to have a table number in the second half of the table,
%%     you can ask for a second multicolumn command that will position at the
%%     top of the second half of the table:
%%
%%        \begin{splittabular}{ccccBccc}
%%        \multicolumn{4}{c}{\textsc{Table 1}}&\multicolumn{3}{c}{\textsc{Table 1, Continued}}\\
%%
%%     You can do the same for the caption, and give a Continued caption for
%%     the second half of the table. Originally:
%%        \multicolumn{7}{c}{\textsc{Log of \textit{HST} Observations for
%%         NGC~6388}}
%%     Now, changed so that we get a caption on both halves of the table:
%%        \multicolumn{4}{c}{\textsc{Log of \textit{HST} Observations for
%%         NGC~6388}}&\multicolumn{3}{c}{\textsc{Log of \textit{HST} Observations for
%%         NGC~6388, Continued}}\\
%%     
%%     Similarly, you can rearrange table notes to appear at the bottom of
%%     the appropriate half of the table. For instance, starting with this,
%%     which would make table notes both appear at the bottom of the top half
%%     of the table:
%%        \multicolumn{4}{l}{\small{$\dagger$ Average distance of data set from
%%            cluster center.}}\\
%%        \multicolumn{4}{l}{$^{\rm a}$SNAP program.}\\
%%     
%%     We may substitute the following:
%%        \multicolumn{4}{l}{$^{\rm a}$SNAP program.}&\multicolumn{3}{l}{\small{$\dagger$ Average distance of data set from
%%            cluster center.}}\\
%%     
%%     Which will produce the first endnote underneath the top half of the
%%     table, and the second underneath the bottom half.
%%     
%%     Another option would be to have both endnotes appear below the bottom
%%     half of the table. Easily done:
%%        &&&&\multicolumn{3}{l}{$^{\rm a}$SNAP program.}\\
%%        &&&&\multicolumn{3}{l}{\small{$\dagger$ Average distance of data set from
%%            cluster center.}}\\
%%     %%     %%     %%     %%     %%     %%     

%%%%%%%%
%% 4) \colnumbers will make line with column numbers automatic. It will work with splittabular
%%     and splitdeluxetable as well as tabular.
%%     To use: type in \colnumbers within the table whereever you'd like it to appear, typically
%%     underneath the column headers, before the lines of data.

%%%%%%%%
%% 5) Easy Decimal numbering
%%    How to make decimal numbers in tables line up on the period:

%%     Use D (for decimal column) in table preamble for every decimal number. The decimal
%%     numbers will use two columns, one for the left part of the decimal
%%     number and one for the right part.

%%     D may be used more than once in a table preamble.

%%     If you want to type in a column header  over the decimal
%%     numbers, please use \multicolumn2c{} to span both columns.

%%     After the column headers, to start decimal numbering, 
%%     type in \decimals in the body of the table.

%%     When entering decimal numbers
%%     remember to leave a space after the decimal number, before the following &.
%%     For instance: &22.3 &35.96 \\

%%     If you'd like an empty entry, please supply a period and a space: & . &. You
%%     will not see the period in the resulting table.

%%     example:
%    \begin{tabular}{rDD}
%     \hline
%     &&&\multicolumn2c{\bf More}\\
%     &\multicolumn2c{\bf Decimals}&\multicolumn2c{\bf Decimals}\\
%     \hline
%     \hline
%     \decimals
%     one& . &34.2 \\
%     two &567.0 &21345 \\
%     three&.0 &62.5 \\
%     four&245 &5034.349923 \\
%     five&21 & \\
%     six& &21.6 
%    \end{tabular}
%%
%    Decimal numbering works within \begin{splittabular}...\end{splittabular}
%    \begin{splitdeluxetable} and \end{splitdeluxetable} for tables broken into two
%    or three parts. \colnumbers will number the columns counting both sides 
%    of the decimal number as one column; \tablehead{\colhead{}...} will make
%    the column headers position above the two columns used for one decimal
%    number as well.
%
%    Decimal numbers will be in math mode so that plus and minus signs are printed
%    correctly, expressions like `$\pm$ 1.2' or `\pm 1.2', will both work
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\let\savedollar$
\catcode`\$=\active

\let\savetabular\tabular
\def\tabular{\catcode`\&=\active\relax\catcode`\$=\active\relax\savetabular}
\long\gdef\eatone{\setbox0=\hbox\bgroup\savedollar\let$\relax}
\gdef\endeatone{\savedollar\egroup\hskip-2\tabcolsep}


%% Hide, important because it allows us to split tables horizontally
\newcolumntype{h}{>\eatone c<\endeatone}

\newcolumntype{C}{>{\bgroup\savedollar\let$\relax}c<{\savedollar\egroup}}
\newcolumntype{L}{>{\bgroup\savedollar\let$\relax}l<{\savedollar\egroup}}
\newcolumntype{R}{>{\bgroup\savedollar\let$\relax}r<{\savedollar\egroup}}

\newcolumntype{B}{>\eatone c<\endeatone}  %% used for \splittabular to indicate break in
                                          %% two or three parts of table

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Split tables into 2 or 3 parts; stack the parts
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Process table preamble

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Count number of columns in preamble

\newcount\colcount
\newcount\firstcolcount
\newcount\secondcolcount
\newcount\thirdcolcount
\newcount\columncount

%% \makeatother is necessary to keep @ from being treated as a letter
%% when counting the number of columns in table.
\makeatother
\def\xD{D}
\def\xaster{*}
\newcount\howmanyDs
\newcount\firsthowmanyDs
\newcount\secondhowmanyDs

\newif\ifD

\def\countcols#1{\ifcat#1c
\global\advance\colcount by 1\relax\fi
%%
\def\lookforD{#1}
\ifx\lookforD\xD
\global\advance\howmanyDs by 1
\global\advance\colcount by1\relax
\fi
%%
\futurelet\next\lookatnext
}
\makeatletter

\def\xeatone#1{\countcols}
\def\xrelax{\relax}

%% second conditional deals with expressions like @{} in
%% the preamble.
\def\lookatnext{\if\next\xrelax\let\go\relax
\else
\ifx\next\bgroup\let\go\xeatone\else
\let\go\countcols\fi\fi\go}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% reset line counting at \\

%% arraycr redefined to match revtex4-1
\def\new@arraycr{\relax 
\global\columncount=0\relax
\global\colheadcount=0\relax
\iffalse {\fi \ifnum 0=`}\fi \@ifstar {\global \@tbpen \@M \@xarraycr}
{\global \@tbpen \intertabularlinepenalty \@xarraycr}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Redefining & is necessary to get around \omit in \multicolumn,
%% which prevents @{} from being used to change the meaning of multicolumn.
%% Now column number and top or bottom table is used to determine whether
%% multicolumn should be turned on or off.
\let\saveampersand&

\newif\iffirstbox
\newif\ifsecondbox
\newif\ifthirdbox

\long\gdef\CheckNumberAndSwitch{\unskip\global\advance\columncount by 1\relax%
\saveampersand}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Parse and count preamble

\def\catchfirstpreamble#1B#2Z{%firstpreamble
\def\leftpreamble{#1\relax}
\colcount=0
\global\howmanyDs=0\relax
\expandafter\countcols\leftpreamble
\global\firstcolcount\the\colcount
\global\firsthowmanyDs\the\howmanyDs
\ifnum\firstcolcount>25
\typeout{^^J
-----------------------------------------------------
^^J
Warning!
^^J^^J 
Too many columns in first part of table!
^^J^^J
Maximum number of columns in each part of the table is 25. Each `D' counts as two columns.
^^J
-----------------------------------------------------
}\fi
\global\howmanyDs=0\relax
\global\colcount=0\relax
\newcolumntype{A}{#1}}

\def\catchsecondpreamble#1B#2Z{%secondpreamble
\def\rightpreamble{#2\relax}
\colcount=0
\expandafter\countcols\rightpreamble
\global\secondcolcount\colcount
\global\secondhowmanyDs\the\howmanyDs
\ifnum\secondcolcount>25
\typeout{^^J-----------------------------------------------------
^^J
Warning!
^^J^^J 
Too many columns in second part of table!
^^J^^J
Maximum number of columns in each part of the table is 25. Each `D' counts as two columns.
^^J
-----------------------------------------------------
}\fi
\global\totalcolumns=\firstcolcount
\global\advance\totalcolumns by \secondcolcount
\global\colcount=0\relax
\newcolumntype{Z}{#2}}


\def\catchsecondofthreepreamble#1B#2B#3Z{%secondpreamble
\def\rightpreamble{#2\relax}
\colcount=0
\howmanyDs=0
\expandafter\countcols\rightpreamble
\global\secondcolcount\colcount
\global\secondhowmanyDs\the\howmanyDs
\global\totalcolumns=\firstcolcount
\global\advance\totalcolumns by \secondcolcount
\global\colcount=0\relax
\newcolumntype{Z}{#2}}


\def\catchthirdpreamble#1B#2B#3Z{%firstpreamble
\def\thirdpreamble{#3}
\colcount=0
\expandafter\countcols\thirdpreamble
\global\thirdcolcount\the\colcount
\global\advance\totalcolumns by \thirdcolcount
\global\colcount=0\relax
\newcolumntype{z}{#3}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Define splittabular/endsplittabular

\newcount\PartsOfTable
\newif\ifbreaktab

\def\checkforB #1B#2B#3B{
%% defaults, may be used in \colnumbers
\gdef\tabfullpreamble{#1#2#3\relax}
\gdef\firstpreamble{#1}
\gdef\secondpreamble{#2}
\gdef\thirdpreamble{#3}
\ifx\thirdpreamble\empty
\global\PartsOfTable=2
\else
\global\PartsOfTable=3
\fi
}

\def\lookforD#1{\def\zone{#1}\ifx\zone\xD
\global\Dtrue\else\Dfalse\fi}

\newcount\columnoneandtwo
\newif\ifdonullmulticol

\newcount\colnumsused
\newcount\loopnum

\catcode`\&=\active
\let&\CheckNumberAndSwitch
\let$\savedollar

%sss
\def\splittabular{\catcode`\&=\active
\catcode`\$=\active
\global\colnumbersonfalse
\let\colnumbers\savesplitplaincolnumbers
\let\splitdecimalcolnumbers\savesplitdecimalcolnumbers
\def\decimalcolnumbers{\splitdecimalcolnumbers}
\xsplittabular}

\def\xsplittabular#1#2\end{{
\global\firsttimetrue
\let&\CheckNumberAndSwitch
\let$\savedollar
%%%
\def\endtabular{\endarray
\global\let\zdoit\relax
\global\let\ddoit\relax
\global\Dfalse}
\setbox0=\hbox{\def\firstarg{#1}\expandafter\lookforD\firstarg}
\PartsOfTable=0
\def\tempfullpreamble{#1BB}
\setbox0=\hbox{\expandafter\checkforB\tempfullpreamble}
%% Now PartsOfTable is either =2 or 3
%%
\global\colnumsused=0
\global\breaktabtrue
\global\colcount=0
%%
\ifnum\PartsOfTable=3
\let\multicolumn\threebreakmulticolumn
\else
\let\multicolumn\breakmulticolumn
\fi
%%
\def\one{#1Z}%% full preamble
\ifnum\PartsOfTable=3
\expandafter\catchfirstpreamble\one
\expandafter\catchsecondofthreepreamble\one
\expandafter\catchthirdpreamble\one
\makefirstdummycolumns %f
\makeseconddummycolumns %F
\makethirddummycolumns %E
\else %% PartsOfTable=2
\expandafter\catchfirstpreamble\one
\expandafter\catchsecondpreamble\one
\makefirstdummycolumns %f
\makeseconddummycolumns %F
\fi
%%%
\global\columncount=0
\ifnum\PartsOfTable=3
%% For table divided into three parts !!
\firstboxtrue\secondboxfalse\thirdboxfalse
%
\setbox\firsttablebox=\hbox{%
\begin{tabular}{AFE}% 
#2\crcr
\end{tabular}}
%
\hbox to \hsize{\hss\unhbox\firsttablebox\hss}
\vskip6pt
\hrule
\vskip6pt
\global\columncount=0
\firstboxfalse\secondboxtrue\thirdboxfalse
\ifcolnumberson
\let\colnumbers\xplain
\setbox\secondtablebox=\hbox{%
\begin{tabular}{fZE}% fZE
#2\crcr\end{tabular}}
\else
\setbox\secondtablebox=\hbox{
\begin{tabular}{fZE}% fZE
#2
\end{tabular}}
\fi
\hbox to \hsize{\hss\unhbox\secondtablebox\hss}
%%
\vskip6pt
\hrule
\vskip6pt
\firstboxfalse\secondboxfalse\thirdboxtrue
\global\columncount=0
\ifcolnumberson
\let\colnumbers\xplain
\setbox\thirdtablebox=\hbox{%
\begin{tabular}{fFz}% fFz
#2\crcr\end{tabular}}
\else
\setbox\thirdtablebox=\hbox{
\begin{tabular}{fFz}% fFz
#2
\end{tabular}}
\fi
\hbox to \hsize{\hss\unhbox\thirdtablebox\hss}
\else
%%
%% For table divided into two parts:
%%
\global\columncount=0
\secondboxfalse
 \setbox\firsttablebox=\hbox{%
\begin{tabular}{AF}% should be AF
#2
\end{tabular}
}
 \hbox to \hsize{\hss\unhbox\firsttablebox\hss}
\vskip6pt
\hrule
\vskip6pt
\global\columncount=0
\secondboxtrue
\ifcolnumberson
\setbox\secondtablebox=\hbox{\let\colnumbers\xplain
\begin{tabular}{fZ}% should be fZ
#2
\end{tabular}
}
\else
\setbox\secondtablebox=\hbox{
\begin{tabular}{fZ}% should be fZ
#2
\end{tabular}
}
\fi
\hbox to \hsize{\hss\unhbox\secondtablebox\hss}
%%
%% end of conditional testing for 2 or 3 part table:
\fi
%\global\breaktabfalse
}
\firsthowmanyDs=0
\secondhowmanyDs=0
\resetdecimals
\end
}

%yyy
\def\endsplittabular{\global\firsttimefalse\global\colnumbersonfalse
\global\let\splitplaincolnumbers\savesplitplaincolnumbers
\global\breaktabfalse}

\long\gdef\breakmulticolumn#1#2#3{%
\multispan{#1}%
\let&\CheckNumberAndSwitch
\ifsecondbox%
\ifnum\columncount<\firstcolcount%
\global\donullmulticoltrue%
\else%
\global\donullmulticolfalse%
\fi%
%%%
   \else% first box
\ifnum\columncount<\firstcolcount%
\global\donullmulticolfalse%
\else%
\global\donullmulticoltrue%
\fi%
\fi%
\ifdonullmulticol%
\global\advance\colheadcount by 1\relax
\begingroup
   \def\@addamp{\if@firstamp \@firstampfalse \else
                \@preamerr 5\fi}%
   \@mkpream{h}\@addtopreamble\@empty
   \endgroup
   \def\@sharp{}%
%% comment out \@arstrut to prevent blank line where multicolumn was found
%% on other parts of the table, but not on the current part.
   \@arstrut 
\@preamble
   \null\ignorespaces
\else%
\begingroup
   \def\@addamp{\if@firstamp \@firstampfalse \else
                \@preamerr 5\fi}%
   \@mkpream{#2}\@addtopreamble\@empty
   \endgroup
   \def\@sharp{#3}%
   \@arstrut \@preamble
   \null\ignorespaces
\fi%
\global\donullmulticolfalse%
\global\advance\columncount by #1\relax%
\global\advance\columncount-1\relax%
}


\long\gdef\threebreakmulticolumn#1#2#3{%
\multispan{#1}%
\columnoneandtwo=\firstcolcount\relax%
\advance\columnoneandtwo by \secondcolcount\relax%
%%
\global\donullmulticoltrue\relax%
\iffirstbox\relax%
\ifnum\columncount<\firstcolcount%
\global\donullmulticolfalse%
\fi\relax%
\ifnum\columncount=\firstcolcount\relax%
\donullmulticoltrue\fi\relax%
\else\relax%
%%
\ifsecondbox%
\ifnum\columncount=\firstcolcount\relax%
\global\donullmulticolfalse\fi\relax%
\ifnum\columncount>\firstcolcount%
\ifnum\columncount<\columnoneandtwo\relax%
\global\donullmulticolfalse\relax%
\fi\fi\relax%
\else\relax%
%%%
\ifthirdbox%
\ifnum\columncount<\columnoneandtwo%
\global\donullmulticoltrue%
\else\relax%
\global\donullmulticolfalse%
\fi\relax%
\fi%% end if third box
\fi%% end if second box
\fi%% end if first box
%%
\ifdonullmulticol%
\begingroup\relax%
\global\advance\colheadcount by 1\relax%
   \def\@addamp{\if@firstamp \@firstampfalse \else%
                \@preamerr 5\fi}%
   \@mkpream{h}\@addtopreamble\@empty%
   \endgroup%
   \def\@sharp{}%
%% comment out \@arstrut to prevent blank line where multicolumn was found
%% on other parts of the table, but not on the current part.
   \@arstrut \@preamble%
   \null\ignorespaces
\else%
\begingroup%
   \def\@addamp{\if@firstamp \@firstampfalse \else%
                \@preamerr 5\fi}%
   \@mkpream{#2}\@addtopreamble\@empty%
   \endgroup%
   \def\@sharp{#3}%
   \@arstrut \@preamble%
   \null\ignorespaces
\fi%
\global\donullmulticolfalse%
\global\advance\columncount by #1\relax%
\global\advance\columncount-1\relax%
}

%% First dummy columns is the part of the table that will not print,
%% in this case the first part to the left.
%%\makefirstdummycolumns
%%
%% and second dummy columns
%% \makeseconddummycolumns.
\gdef\makefirstdummycolumns{
\ifcase\firstcolcount
\or% 1
\newcolumntype{f}{h} % no D possible
%%%%%%%%%%%%%%%%%%
\or% 2
  \ifcase\firsthowmanyDs
  \newcolumntype{f}{hh}%% 0
  \or
  \newcolumntype{f}{d} %% 1
  \fi
%%%%%%%%%%%%%%%%%%
\or% 3
  \ifcase\firsthowmanyDs%
  \newcolumntype{f}{hhh}% 0 
  \or%
  \newcolumntype{f}{dh}% 1
  \fi%
%%%%%%%%%%%%%%%%%%
\or% 4
  \ifcase\firsthowmanyDs
   \newcolumntype{f}{hhhh} % 0 
    \or
   \newcolumntype{f}{dhh} % 1
   \or
   \newcolumntype{f}{dd} % 2 
   \fi
%%%%%%%%%%%%%%%%%%
\or% 5
  \ifcase\firsthowmanyDs
   \newcolumntype{f}{hhhhh} % 0 
    \or
   \newcolumntype{f}{dhhh} % 1
   \or
   \newcolumntype{f}{ddh} % 2 
   \fi
%%%%%%%%%%%%%%%%%%
\or% 6
  \ifcase\firsthowmanyDs
   \newcolumntype{f}{hhhhhh} % 0 
    \or
   \newcolumntype{f}{dhhhh} % 1
   \or
   \newcolumntype{f}{ddhh} % 2 
    \or
   \newcolumntype{f}{ddd} % 3
   \fi
%%%%%%%%%%%%%%%
\or % 7
  \ifcase\firsthowmanyDs
   \newcolumntype{f}{hhhhhhh} % 0 
    \or
   \newcolumntype{f}{dhhhhh} % 1
   \or
   \newcolumntype{f}{ddhhh} % 2 
   \or
   \newcolumntype{f}{dddh} % 3
   \fi
%%%%%%%%%%%%%%%%%%
\or % 8
  \ifcase\firsthowmanyDs
   \newcolumntype{f}{hhhhhhhh} % 0 
    \or
   \newcolumntype{f}{dhhhhhh} % 1
   \or
   \newcolumntype{f}{ddhhhh} % 2 
   \or
   \newcolumntype{f}{dddhh} % 3
   \or
   \newcolumntype{f}{dddd} % 4
   \fi
%%%%%%%%%%%%%%%%%%
\or % 9
  \ifcase\firsthowmanyDs
   \newcolumntype{f}{hhhhhhhhh} % 0 
    \or
   \newcolumntype{f}{dhhhhhhh} % 1
   \or
   \newcolumntype{f}{ddhhhhh} % 2 
   \or
   \newcolumntype{f}{dddhhh} % 3
   \or
   \newcolumntype{f}{ddddh} % 4
   \fi
%%%%%%%%%%%%%%%%%%
\or %10
  \ifcase\firsthowmanyDs
   \newcolumntype{f}{hhhhhhhhhh} % 0 
    \or
   \newcolumntype{f}{dhhhhhhhh} % 1
   \or
   \newcolumntype{f}{ddhhhhhh} % 2 
   \or
   \newcolumntype{f}{dddhhhh} % 3
   \or
   \newcolumntype{f}{ddddhh} % 4
   \or
   \newcolumntype{f}{ddddd} % 5
   \fi
%%%%%%%%%%%%%%%%%%
\or % 11
  \ifcase\firsthowmanyDs
   \newcolumntype{f}{hhhhhhhhhhh} % 0 
    \or
   \newcolumntype{f}{dhhhhhhhhh} % 1
   \or
   \newcolumntype{f}{ddhhhhhhh} % 2 
   \or
   \newcolumntype{f}{dddhhhhh} % 3
   \or
   \newcolumntype{f}{ddddhhh} % 4
   \or
   \newcolumntype{f}{dddddh} % 5
   \fi
%%%%%%%%%%%%%%%%%%
\or % 12
  \ifcase\firsthowmanyDs
   \newcolumntype{f}{hhhhhhhhhhhh} % 0 
    \or
   \newcolumntype{f}{dhhhhhhhhhh} % 1
   \or
   \newcolumntype{f}{ddhhhhhhhh} % 2 
   \or
   \newcolumntype{f}{dddhhhhhh} % 3
   \or
   \newcolumntype{f}{ddddhhhh} % 4
   \or
   \newcolumntype{f}{dddddhh} % 5
   \or
   \newcolumntype{f}{dddddd} % 6
   \fi
%%%%%%%%%%%%%%%%%%
\or %13
  \ifcase\firsthowmanyDs
   \newcolumntype{f}{hhhhhhhhhhhhh} % 0 
    \or
   \newcolumntype{f}{dhhhhhhhhhhh} % 1
   \or
   \newcolumntype{f}{ddhhhhhhhhh} % 2 
   \or
   \newcolumntype{f}{dddhhhhhhh} % 3
   \or
   \newcolumntype{f}{ddddhhhhh} % 4
   \or
   \newcolumntype{f}{dddddhhh} % 5
   \or
   \newcolumntype{f}{ddddddh} % 6
   \fi
%%%%%%%%%%%%%%%%%%
\or %14
  \ifcase\firsthowmanyDs
   \newcolumntype{f}{hhhhhhhhhhhhhh} % 0 
    \or
   \newcolumntype{f}{dhhhhhhhhhhhh} % 1
   \or
   \newcolumntype{f}{ddhhhhhhhhhh} % 2 
   \or
   \newcolumntype{f}{dddhhhhhhhh} % 3
   \or
   \newcolumntype{f}{ddddhhhhhh} % 4
   \or
   \newcolumntype{f}{dddddhhhh} % 5
   \or
   \newcolumntype{f}{ddddddhh} % 6
   \or
   \newcolumntype{f}{ddddddd} % 7
   \fi
%%%%%%%%%%%%%%%%%%
\or %15
  \ifcase\firsthowmanyDs
   \newcolumntype{f}{hhhhhhhhhhhhhhh} % 0 
    \or
   \newcolumntype{f}{dhhhhhhhhhhhhh} % 1
   \or
   \newcolumntype{f}{ddhhhhhhhhhhh} % 2 
   \or
   \newcolumntype{f}{dddhhhhhhhhh} % 3
   \or
   \newcolumntype{f}{ddddhhhhhhh} % 4
   \or
   \newcolumntype{f}{dddddhhhhh} % 5
   \or
   \newcolumntype{f}{ddddddhhh} % 6
   \or
   \newcolumntype{f}{dddddddh} % 7
   \fi
%%%%%%%%%%%%%%%%%%
\or %16
  \ifcase\firsthowmanyDs
   \newcolumntype{f}{hhhhhhhhhhhhhhhh} % 0 
    \or
   \newcolumntype{f}{dhhhhhhhhhhhhhh} % 1
   \or
   \newcolumntype{f}{ddhhhhhhhhhhhh} % 2 
   \or
   \newcolumntype{f}{dddhhhhhhhhhh} % 3
   \or
   \newcolumntype{f}{ddddhhhhhhhh} % 4
   \or
   \newcolumntype{f}{dddddhhhhhh} % 5
   \or
   \newcolumntype{f}{ddddddhhhh} % 6
   \or
   \newcolumntype{f}{dddddddhh} % 7
   \or
   \newcolumntype{f}{dddddddd} % 8
\fi
%%%%%%%%%%%%%%%%%%
\or %17
  \ifcase\firsthowmanyDs
   \newcolumntype{f}{hhhhhhhhhhhhhhhhh} % 0 
    \or
   \newcolumntype{f}{dhhhhhhhhhhhhhhh} % 1
   \or
   \newcolumntype{f}{ddhhhhhhhhhhhhh} % 2 
   \or
   \newcolumntype{f}{dddhhhhhhhhhhh} % 3
   \or
   \newcolumntype{f}{ddddhhhhhhhhh} % 4
   \or
   \newcolumntype{f}{dddddhhhhhhh} % 5
   \or
   \newcolumntype{f}{ddddddhhhhh} % 6
   \or
   \newcolumntype{f}{dddddddhhh} % 7
   \or
   \newcolumntype{f}{ddddddddh} % 8
\fi
%%%%%%%%%%%%%%%%%%
\or %18
  \ifcase\firsthowmanyDs
   \newcolumntype{f}{hhhhhhhhhhhhhhhhhh} % 0 
    \or
   \newcolumntype{f}{dhhhhhhhhhhhhhhhh} % 1
   \or
   \newcolumntype{f}{ddhhhhhhhhhhhhhh} % 2 
   \or
   \newcolumntype{f}{dddhhhhhhhhhhhh} % 3
   \or
   \newcolumntype{f}{ddddhhhhhhhhhh} % 4
   \or
   \newcolumntype{f}{dddddhhhhhhhh} % 5
   \or
   \newcolumntype{f}{ddddddhhhhhh} % 6
   \or
   \newcolumntype{f}{ddddddhhhh} % 7
   \or
   \newcolumntype{f}{ddddddddhh} % 8
   \or
   \newcolumntype{f}{ddddddddd} % 9
\fi
%%%%%%%%%%%%%%%%%%
\or %19
  \ifcase\firsthowmanyDs
   \newcolumntype{f}{hhhhhhhhhhhhhhhhhhh} % 0 
    \or
   \newcolumntype{f}{dhhhhhhhhhhhhhhhhh} % 1
   \or
   \newcolumntype{f}{ddhhhhhhhhhhhhhhh} % 2 
   \or
   \newcolumntype{f}{dddhhhhhhhhhhhhh} % 3
   \or
   \newcolumntype{f}{ddddhhhhhhhhhhh} % 4
   \or
   \newcolumntype{f}{dddddhhhhhhhhh} % 5
   \or
   \newcolumntype{f}{ddddddhhhhhhh} % 6
   \or
   \newcolumntype{f}{dddddddhhhhh} % 7
   \or
   \newcolumntype{f}{ddddddddhhh} % 8
   \or
   \newcolumntype{f}{ddddddddddh} % 9
\fi
%%%%%%%%%%%%%%%%%%
\or %20
  \ifcase\firsthowmanyDs
   \newcolumntype{f}{hhhhh hhhhh hhhhh hhhhh} % 0 
    \or
   \newcolumntype{f}{dhhhhhhhhhhhhhhhhhh} % 1
   \or
   \newcolumntype{f}{ddhhhhhhhhhhhhhhhh} % 2 
   \or
   \newcolumntype{f}{dddhhhhhhhhhhhhhh} % 3
   \or
   \newcolumntype{f}{ddddhhhhhhhhhhhh} % 4
   \or
   \newcolumntype{f}{dddddhhhhhhhhhh} % 5
   \or
   \newcolumntype{f}{ddddddhhhhhhhh} % 6
   \or
   \newcolumntype{f}{dddddddhhhhhh} % 7
   \or
   \newcolumntype{f}{ddddddddhhhh} % 8
   \or
   \newcolumntype{f}{dddddddddhh} % 9
   \or
   \newcolumntype{f}{dddddddddd} % 10
   \fi
%%%%%%%%%%%%%%%%%%
\or %21
  \ifcase\firsthowmanyDs
   \newcolumntype{f}{hhhhh hhhhh hhhhh hhhhh h} % 0 
   \or
   \newcolumntype{f}{dhhhhhhhhhhhhhhhhhhh} % 1
   \or
   \newcolumntype{f}{ddhhhhhhhhhhhhhhhhh} % 2 
   \or
   \newcolumntype{f}{dddhhhhhhhhhhhhhhh} % 3
   \or
   \newcolumntype{f}{ddddhhhhhhhhhhhhh} % 4
   \or
   \newcolumntype{f}{dddddhhhhhhhhhhh} % 5
   \or
   \newcolumntype{f}{ddddddhhhhhhhhh} % 6
   \or
   \newcolumntype{f}{dddddddhhhhhhh} % 7
   \or
   \newcolumntype{f}{ddddddddhhhhh} % 8
   \or
   \newcolumntype{f}{ddd ddd ddd hhh} % 9
   \or
   \newcolumntype{f}{ddd ddd ddd d h} % 10
   \fi
%%%%%%%%%%%%%%%%%%
\or %22
\ifcase\firsthowmanyDs
   \newcolumntype{f}{hhhhh hhhhh hhhhh hhhhh hh} % 0 
   \or
   \newcolumntype{f}{dhhhhhhhhhhhhhhhhhhhh} % 1
   \or
   \newcolumntype{f}{ddhhhhhhhhhhhhhhhhhh} % 2 
   \or
   \newcolumntype{f}{dddhhhhhhhhhhhhhhhh} % 3
   \or
   \newcolumntype{f}{ddddhhhhhhhhhhhhhh} % 4
   \or
   \newcolumntype{f}{dddddhhhhhhhhhhhh} % 5
   \or
   \newcolumntype{f}{ddddddhhhhhhhhhh} % 6
   \or
   \newcolumntype{f}{dddddddhhhhhhhh} % 7
   \or
   \newcolumntype{f}{ddddddddhhhhhh} % 8
   \or
   \newcolumntype{f}{ddd ddd ddd hhhh} % 9
   \or
   \newcolumntype{f}{ddd ddd ddd dhh} % 10
   \or
   \newcolumntype{f}{ddddddddddd} % 11
   \fi
%%%%%%%%%%%%%%%%%%
\or %23
\ifcase\firsthowmanyDs
   \newcolumntype{f}{hhhhh hhhhh hhhhh hhhhh hhh} % 0 
   \or
   \newcolumntype{f}{dhhhhhhhhhhhhhhhhhhhhh} % 1
   \or
   \newcolumntype{f}{ddhhhhhhhhhhhhhhhhhhh} % 2 
   \or
   \newcolumntype{f}{dddhhhhhhhhhhhhhhhhh} % 3
   \or
   \newcolumntype{f}{ddddhhhhhhhhhhhhhhh} % 4
   \or
   \newcolumntype{f}{dddddhhhhhhhhhhhhh} % 5
   \or
   \newcolumntype{f}{ddddddhhhhhhhhhhh} % 6
   \or
   \newcolumntype{f}{dddddddhhhhhhhhh} % 7
   \or
   \newcolumntype{f}{ddddddddhhhhhhh} % 8
   \or
   \newcolumntype{f}{ddd ddd ddd hhhhh} % 9
   \or
   \newcolumntype{f}{ddddddddddhhh} % 10
   \or
   \newcolumntype{f}{ddddd ddddd dh} % 11
   \fi
%%%%%%%%%%%%%%%%%%
\or %24
\ifcase\firsthowmanyDs
   \newcolumntype{f}{hhhhh hhhhh hhhhh hhhhh hhhh} % 0 
   \or
   \newcolumntype{f}{dhhhhhhhhhhhhhhhhhhhhhh} % 1
   \or
   \newcolumntype{f}{ddhhhhhhhhhhhhhhhhhhhh} % 2 
   \or
   \newcolumntype{f}{dddhhhhhhhhhhhhhhhhhh} % 3
   \or
   \newcolumntype{f}{ddddhhhhhhhhhhhhhhhh} % 4
   \or
   \newcolumntype{f}{dddddhhhhhhhhhhhhhh} % 5
   \or
   \newcolumntype{f}{ddddddhhhhhhhhhhhh} % 6
   \or
   \newcolumntype{f}{dddddddhhhhhhhhhh} % 7
   \or
   \newcolumntype{f}{ddddddddhhhhhhhh} % 8
   \or
   \newcolumntype{f}{ddd ddd ddd hhhhhh} % 9
   \or
   \newcolumntype{f}{ddddddddddhhhh} % 10
   \or
   \newcolumntype{f}{ddddd ddddd dhh} % 11
   \or
   \newcolumntype{f}{ddddd ddddd dd} % 12
   \fi
%%%%%%%%%%%%%%%%%%
\or %25
\ifcase\firsthowmanyDs
   \newcolumntype{f}{hhhhh hhhhh hhhhh hhhhh hhhhh} % 0 
   \or
   \newcolumntype{f}{dhhhhhhhhhhhhhhhhhhhhhhh} % 1
   \or
   \newcolumntype{f}{ddhhhhhhhhhhhhhhhhhhhhh} % 2 
   \or
   \newcolumntype{f}{dddhhhhhhhhhhhhhhhhhhh} % 3
   \or
   \newcolumntype{f}{ddddhhhhhhhhhhhhhhhhh} % 4
   \or
   \newcolumntype{f}{dddddhhhhhhhhhhhhhhh} % 5
   \or
   \newcolumntype{f}{ddddddhhhhhhhhhhhhh} % 6
   \or
   \newcolumntype{f}{dddddddhhhhhhhhhhh} % 7
   \or
   \newcolumntype{f}{ddddddddhhhhhhhhh} % 8
   \or
   \newcolumntype{f}{ddd ddd ddd hhhhhhh} % 9
   \or
   \newcolumntype{f}{ddddddddddhhhhh} % 10
   \or
   \newcolumntype{f}{dddddddddddhhh} % 11
   \or
   \newcolumntype{f}{ddddddddddddh} % 12
   \fi
%%%%%%%%%%%%%%%%%%
\else
\typeout{^^J----------------------------------------------------- ^^J
Warning!^^J^^J 
Too many Columns using in Splittabular. 
^^J
25 column maximum in
each part of the table.^^J Each`T' counts as two columns.
^^J-----------------------------------------------------^^J}
\fi
}


%% Second dummy columns is the part of the table that will not print,
%% in this case the part to the right.
%%\makeseconddummycolumns

\gdef\makeseconddummycolumns{%
\ifcase\secondcolcount
%0
\or
%1
\newcolumntype{F}{h} % no D possible
%%%%%%%%%%%%%%%%%%
\or
%2
  \ifcase\secondhowmanyDs
  \newcolumntype{F}{hh}%% 0
  \or
  \newcolumntype{F}{d} %% 1
  \fi
%%%%%%%%%%%%%%%%%%
\or
%3
  \ifcase\secondhowmanyDs
  \newcolumntype{F}{hhh} % 0 
  \or
  \newcolumntype{F}{dh} % 1 
  \fi
%%%%%%%%%%%%%%%%%%
\or
  \ifcase\secondhowmanyDs
   \newcolumntype{F}{hhhh} % 0 
    \or
   \newcolumntype{F}{dhh} % 1
   \or
   \newcolumntype{F}{dd} % 2 
   \fi
%%%%%%%%%%%%%%%%%%
\or
  \ifcase\secondhowmanyDs
   \newcolumntype{F}{hhhhh} % 0 
    \or
   \newcolumntype{F}{dhhh} % 1
   \or
   \newcolumntype{F}{ddh} % 2 
   \fi
%%%%%%%%%%%%%%%%%%
\or
  \ifcase\secondhowmanyDs
   \newcolumntype{F}{hhhhhh} % 0 
    \or
   \newcolumntype{F}{dhhhh} % 1
   \or
   \newcolumntype{F}{ddhh} % 2 
   \or
   \newcolumntype{F}{ddd} % 3
   \fi
%%%%%%%%%%%%%%%
\or
  \ifcase\secondhowmanyDs
   \newcolumntype{F}{hhhhhhh} % 0 
    \or
   \newcolumntype{F}{dhhhhh} % 1
   \or
   \newcolumntype{F}{ddhhh} % 2 
   \or
   \newcolumntype{F}{dddh} % 3
   \fi
%%%%%%%%%%%%%%%%%%
\or
  \ifcase\secondhowmanyDs
   \newcolumntype{F}{hhhhhhhh} % 0 
    \or
   \newcolumntype{F}{dhhhhhh} % 1
   \or
   \newcolumntype{F}{ddhhhh} % 2 
   \or
   \newcolumntype{F}{dddhh} % 3
   \or
   \newcolumntype{F}{dddd} % 4
   \fi
%%%%%%%%%%%%%%%%%%
\or
  \ifcase\secondhowmanyDs
   \newcolumntype{F}{hhhhhhhhh} % 0 
    \or
   \newcolumntype{F}{dhhhhhhh} % 1
   \or
   \newcolumntype{F}{ddhhhhh} % 2 
   \or
   \newcolumntype{F}{dddhhh} % 3
   \or
   \newcolumntype{F}{ddddh} % 4
   \fi
%%%%%%%%%%%%%%%%%%
\or
  \ifcase\secondhowmanyDs
   \newcolumntype{F}{hhhhhhhhhh} % 0 
    \or
   \newcolumntype{F}{dhhhhhhhh} % 1
   \or
   \newcolumntype{F}{ddhhhhhh} % 2 
   \or
   \newcolumntype{F}{dddhhhh} % 3
   \or
   \newcolumntype{F}{ddddhh} % 4
   \or
   \newcolumntype{F}{ddddd} % 5
   \fi
%%%%%%%%%%%%%%%%%%
\or
  \ifcase\secondhowmanyDs
   \newcolumntype{F}{hhhhhhhhhhh} % 0 
    \or
   \newcolumntype{F}{dhhhhhhhhh} % 1
   \or
   \newcolumntype{F}{ddhhhhhhh} % 2 
   \or
   \newcolumntype{F}{dddhhhhh} % 3
   \or
   \newcolumntype{F}{ddddhhh} % 4
   \or
   \newcolumntype{F}{dddddh} % 5
   \fi
%%%%%%%%%%%%%%%%%%
\or
  \ifcase\secondhowmanyDs
   \newcolumntype{F}{hhhhhhhhhhhh} % 0 
    \or
   \newcolumntype{F}{dhhhhhhhhhh} % 1
   \or
   \newcolumntype{F}{ddhhhhhhhh} % 2 
   \or
   \newcolumntype{F}{dddhhhhhh} % 3
   \or
   \newcolumntype{F}{ddddhhhh} % 4
   \or
   \newcolumntype{F}{dddddhh} % 5
   \or
   \newcolumntype{F}{dddddd} % 6
   \fi
%%%%%%%%%%%%%%%%%%
\or
  \ifcase\secondhowmanyDs
   \newcolumntype{F}{hhhhhhhhhhhhh} % 0 
    \or
   \newcolumntype{F}{dhhhhhhhhhhh} % 1
   \or
   \newcolumntype{F}{ddhhhhhhhhh} % 2 
   \or
   \newcolumntype{F}{dddhhhhhhh} % 3
   \or
   \newcolumntype{F}{ddddhhhhh} % 4
   \or
   \newcolumntype{F}{dddddhhh} % 5
   \or
   \newcolumntype{F}{ddddddh} % 6
   \fi
%%%%%%%%%%%%%%%%%%
\or
  \ifcase\secondhowmanyDs
   \newcolumntype{F}{hhhhhhhhhhhhhh} % 0 
    \or
   \newcolumntype{F}{dhhhhhhhhhhhh} % 1
   \or
   \newcolumntype{F}{ddhhhhhhhhhh} % 2 
   \or
   \newcolumntype{F}{dddhhhhhhhh} % 3
   \or
   \newcolumntype{F}{ddddhhhhhh} % 4
   \or
   \newcolumntype{F}{dddddhhhh} % 5
   \or
   \newcolumntype{F}{ddddddhh} % 6
   \or
   \newcolumntype{F}{ddddddd} % 7
   \fi
%%%%%%%%%%%%%%%%%%
\or
  \ifcase\secondhowmanyDs
   \newcolumntype{F}{hhhhhhhhhhhhhhh} % 0 
    \or
   \newcolumntype{F}{dhhhhhhhhhhhhh} % 1
   \or
   \newcolumntype{F}{ddhhhhhhhhhhh} % 2 
   \or
   \newcolumntype{F}{dddhhhhhhhhh} % 3
   \or
   \newcolumntype{F}{ddddhhhhhhh} % 4
   \or
   \newcolumntype{F}{dddddhhhhh} % 5
   \or
   \newcolumntype{F}{ddddddhhh} % 6
   \or
   \newcolumntype{F}{dddddddh} % 7
   \fi
%%%%%%%%%%%%%%%%%%
\or
  \ifcase\secondhowmanyDs
   \newcolumntype{F}{hhhhhhhhhhhhhhhh} % 0 
    \or
   \newcolumntype{F}{dhhhhhhhhhhhhhh} % 1
   \or
   \newcolumntype{F}{ddhhhhhhhhhhhh} % 2 
   \or
   \newcolumntype{F}{dddhhhhhhhhhh} % 3
   \or
   \newcolumntype{F}{ddddhhhhhhhh} % 4
   \or
   \newcolumntype{F}{dddddhhhhhh} % 5
   \or
   \newcolumntype{F}{ddddddhhhh} % 6
   \or
   \newcolumntype{F}{dddddddhh} % 7
   \or
   \newcolumntype{F}{dddddddd} % 8
\fi
%%%%%%%%%%%%%%%%%%
\or
  \ifcase\secondhowmanyDs
   \newcolumntype{F}{hhhhhhhhhhhhhhhhh} % 0 
    \or
   \newcolumntype{F}{dhhhhhhhhhhhhhhh} % 1
   \or
   \newcolumntype{F}{ddhhhhhhhhhhhhh} % 2 
   \or
   \newcolumntype{F}{dddhhhhhhhhhhh} % 3
   \or
   \newcolumntype{F}{ddddhhhhhhhhh} % 4
   \or
   \newcolumntype{F}{dddddhhhhhhh} % 5
   \or
   \newcolumntype{F}{ddddddhhhhh} % 6
   \or
   \newcolumntype{F}{dddddddhhh} % 7
   \or
   \newcolumntype{F}{ddddddddh} % 8
\fi
%%%%%%%%%%%%%%%%%%
\or
  \ifcase\secondhowmanyDs
   \newcolumntype{F}{hhhhhhhhhhhhhhhhhh} % 0 
    \or
   \newcolumntype{F}{dhhhhhhhhhhhhhhhh} % 1
   \or
   \newcolumntype{F}{ddhhhhhhhhhhhhhh} % 2 
   \or
   \newcolumntype{F}{dddhhhhhhhhhhhh} % 3
   \or
   \newcolumntype{F}{ddddhhhhhhhhhh} % 4
   \or
   \newcolumntype{F}{dddddhhhhhhhh} % 5
   \or
   \newcolumntype{F}{ddddddhhhhhh} % 6
   \or
   \newcolumntype{F}{dddddddhhhh} % 7
   \or
   \newcolumntype{F}{ddddddddhh} % 8
   \or
   \newcolumntype{F}{ddddddddd} % 9
\fi
%%%%%%%%%%%%%%%%%%
\or
  \ifcase\secondhowmanyDs
   \newcolumntype{F}{hhhhhhhhhhhhhhhhhhh} % 0 
    \or
   \newcolumntype{F}{dhhhhhhhhhhhhhhhhh} % 1
   \or
   \newcolumntype{F}{ddhhhhhhhhhhhhhhh} % 2 
   \or
   \newcolumntype{F}{dddhhhhhhhhhhhhh} % 3
   \or
   \newcolumntype{F}{ddddhhhhhhhhhhh} % 4
   \or
   \newcolumntype{F}{dddddhhhhhhhhh} % 5
   \or
   \newcolumntype{F}{ddddddhhhhhhh} % 6
   \or
   \newcolumntype{F}{dddddddhhhhh} % 7
   \or
   \newcolumntype{F}{ddddddddhhh} % 8
   \or
   \newcolumntype{F}{dddddddddh} % 9
\fi
%%%%%%%%%%%%%%%%%%
\or
  \ifcase\secondhowmanyDs
   \newcolumntype{F}{hhhhh hhhhh hhhhh hhhhh} % 0 
    \or
   \newcolumntype{F}{dhhhhhhhhhhhhhhhhhh} % 1
   \or
   \newcolumntype{F}{ddhhhhhhhhhhhhhhhh} % 2 
   \or
   \newcolumntype{F}{dddhhhhhhhhhhhhhh} % 3
   \or
   \newcolumntype{F}{ddddhhhhhhhhhhhh} % 4
   \or
   \newcolumntype{F}{dddddhhhhhhhhhh} % 5
   \or
   \newcolumntype{F}{ddddddhhhhhhhh} % 6
   \or
   \newcolumntype{F}{dddddddhhhhhh} % 7
   \or
   \newcolumntype{F}{ddddddddhhhh} % 8
   \or
   \newcolumntype{F}{dddddddddhh} % 9
   \or
   \newcolumntype{F}{dddddddddd} % 10
   \fi
%%%%%%%%%%%%%%%%%%
\or
  \ifcase\secondhowmanyDs
   \newcolumntype{F}{hhhhh hhhhh hhhhh hhhhh h} % 0 
   \or
   \newcolumntype{F}{dhhhhhhhhhhhhhhhhhhh} % 1
   \or
   \newcolumntype{F}{ddhhhhhhhhhhhhhhhhh} % 2 
   \or
   \newcolumntype{F}{dddhhhhhhhhhhhhhhh} % 3
   \or
   \newcolumntype{F}{ddddhhhhhhhhhhhhh} % 4
   \or
   \newcolumntype{F}{dddddhhhhhhhhhhh} % 5
   \or
   \newcolumntype{F}{ddddddhhhhhhhhh} % 6
   \or
   \newcolumntype{F}{dddddddhhhhhhh} % 7
   \or
   \newcolumntype{F}{ddddddddhhhhh} % 8
   \or
   \newcolumntype{F}{ddd ddd ddd hhh} % 9
   \or
   \newcolumntype{F}{ddd ddd ddd d h} % 10
   \fi
%%%%%%%%%%%%%%%%%%
\or
\ifcase\secondhowmanyDs
   \newcolumntype{F}{hhhhh hhhhh hhhhh hhhhh hh} % 0 
   \or
   \newcolumntype{F}{dhhhhhhhhhhhhhhhhhhhh} % 1
   \or
   \newcolumntype{F}{ddhhhhhhhhhhhhhhhhhh} % 2 
   \or
   \newcolumntype{F}{dddhhhhhhhhhhhhhhhh} % 3
   \or
   \newcolumntype{F}{ddddhhhhhhhhhhhhhh} % 4
   \or
   \newcolumntype{F}{dddddhhhhhhhhhhhh} % 5
   \or
   \newcolumntype{F}{ddddddhhhhhhhhhh} % 6
   \or
   \newcolumntype{F}{dddddddhhhhhhhh} % 7
   \or
   \newcolumntype{F}{ddddddddhhhhhh} % 8
   \or
   \newcolumntype{F}{ddd ddd ddd hhhh} % 9
   \or
   \newcolumntype{F}{ddddddddddhh} % 10
   \or
   \newcolumntype{F}{ddddddddddd} % 11
   \fi
%%%%%%%%%%%%%%%%%%
\or
\ifcase\secondhowmanyDs
   \newcolumntype{F}{hhhhh hhhhh hhhhh hhhhh hhh} % 0 
   \or
   \newcolumntype{F}{dhhhhhhhhhhhhhhhhhhhhh} % 1
   \or
   \newcolumntype{F}{ddhhhhhhhhhhhhhhhhhhh} % 2 
   \or
   \newcolumntype{F}{dddhhhhhhhhhhhhhhhhh} % 3
   \or
   \newcolumntype{F}{ddddhhhhhhhhhhhhhhh} % 4
   \or
   \newcolumntype{F}{dddddhhhhhhhhhhhhh} % 5
   \or
   \newcolumntype{F}{ddddddhhhhhhhhhhh} % 6
   \or
   \newcolumntype{F}{dddddddhhhhhhhhh} % 7
   \or
   \newcolumntype{F}{ddddddddhhhhhhh} % 8
   \or
   \newcolumntype{F}{ddd ddd ddd hhhhh} % 9
   \or
   \newcolumntype{F}{ddddddddddhhh} % 10
   \or
   \newcolumntype{F}{ddddd ddddd dh} % 11
   \fi
%%%%%%%%%%%%%%%%%%
\or
\ifcase\secondhowmanyDs
   \newcolumntype{F}{hhhhh hhhhh hhhhh hhhhh hhhh} % 0 
   \or
   \newcolumntype{F}{dhhhhhhhhhhhhhhhhhhhhhh} % 1
   \or
   \newcolumntype{F}{ddhhhhhhhhhhhhhhhhhhhh} % 2 
   \or
   \newcolumntype{F}{dddhhhhhhhhhhhhhhhhhh} % 3
   \or
   \newcolumntype{F}{ddddhhhhhhhhhhhhhhhh} % 4
   \or
   \newcolumntype{F}{dddddhhhhhhhhhhhhhh} % 5
   \or
   \newcolumntype{F}{ddddddhhhhhhhhhhhh} % 6
   \or
   \newcolumntype{F}{dddddddhhhhhhhhhh} % 7
   \or
   \newcolumntype{F}{ddddddddhhhhhhhh} % 8
   \or
   \newcolumntype{F}{ddd ddd ddd hhhhhh} % 9
   \or
   \newcolumntype{F}{ddddddddddhhhh} % 10
   \or
   \newcolumntype{F}{ddddd ddddd dhh} % 11
   \or
   \newcolumntype{F}{ddddd ddddd dd} % 12
   \fi
%%%%%%%%%%%%%%%%%%
\or
\ifcase\secondhowmanyDs
   \newcolumntype{F}{hhhhh hhhhh hhhhh hhhhh hhhhh} % 0 
   \or
   \newcolumntype{F}{dhhhhhhhhhhhhhhhhhhhhhhh} % 1
   \or
   \newcolumntype{F}{ddhhhhhhhhhhhhhhhhhhhhh} % 2 
   \or
   \newcolumntype{F}{dddhhhhhhhhhhhhhhhhhhh} % 3
   \or
   \newcolumntype{F}{ddddhhhhhhhhhhhhhhhhh} % 4
   \or
   \newcolumntype{F}{dddddhhhhhhhhhhhhhhh} % 5
   \or
   \newcolumntype{F}{ddddddhhhhhhhhhhhhh} % 6
   \or
   \newcolumntype{F}{dddddddhhhhhhhhhhh} % 7
   \or
   \newcolumntype{F}{ddddddddhhhhhhhhh} % 8
   \or
   \newcolumntype{F}{ddd ddd ddd hhhhhhh} % 9
   \or
   \newcolumntype{F}{ddddddddddhhhhh} % 10
   \or
   \newcolumntype{F}{ddddd ddddd dhhh} % 11
   \or
   \newcolumntype{F}{ddddd ddddd ddh} % 12
   \fi
%%%%%%%%%%%%%%%%%%
\else
\typeout{^^J----------------------------------------------------- ^^J
Warning!^^J^^J 
Too many Columns using in Splittabular. 
^^J
25 column maximum in
each part of the table.^^J Each`D' counts as two columns.
^^J-----------------------------------------------------^^J}
\fi
}

%% we don't have to worry about D's in this section, fortunately.
\gdef\makethirddummycolumns{
\ifcase\thirdcolcount 
\or\newcolumntype{E}{h}
\or\newcolumntype{E}{hh}
\or\newcolumntype{E}{hhh}
\or\newcolumntype{E}{hhhh}
\or\newcolumntype{E}{hhhhh}
\or\newcolumntype{E}{hhhhhh}
\or\newcolumntype{E}{hhhhhhh}
\or\newcolumntype{E}{hhhhhhhh}
\or\newcolumntype{E}{hhhhhhhhh}
\or\newcolumntype{E}{hhhhhhhhhh}
\or\newcolumntype{E}{hhhhhhhhhhh}
\or\newcolumntype{E}{hhhhhhhhhhhh}
\or\newcolumntype{E}{hhhhhhhhhhhhh}
\or\newcolumntype{E}{hhhhhhhhhhhhhh}
\or\newcolumntype{E}{hhhhhhhhhhhhhhh}
\or\newcolumntype{E}{hhhhhhhhhhhhhhhh}
\or\newcolumntype{E}{hhhhhhhhhhhhhhhhh}
\or\newcolumntype{E}{hhhhhhhhhhhhhhhhhh}
\or\newcolumntype{E}{hhhhhhhhhhhhhhhhhhh}
\or\newcolumntype{E}{hhhhhhhhhhhhhhhhhhhh}
\or\newcolumntype{E}{hhhhhhhhhhhhhhhhhhhhh}
\or\newcolumntype{E}{hhhhhhhhhhhhhhhhhhhhhh}
\or\newcolumntype{E}{hhhhhhhhhhhhhhhhhhhhhhh}
\or\newcolumntype{E}{hhhhhhhhhhhhhhhhhhhhhhhh}
\or\newcolumntype{E}{hhhhhhhhhhhhhhhhhhhhhhhhh} %% up to 25 columns
\else \typeout{^^J-----------------------------------------------------^^J
Warning!
^^J^^J Too many Columns in Splittabular. 
^^J
25 column maximum in
each part of the table.^^J
Each `D' counts as two columns.
^^J-----------------------------------------------------^^J}\fi
}

%%%%%%%%%%%%%%%%%
%% Colnums

%% defaults

\gdef\settabnumdefaults{%
\loopnum=0\relax\loop%
\ifnum\loopnum<31\relax%
\expandafter\gdef\csname tab\the\loopnum\endcsname{%
\multicolumn1{c}{\global\advance\colnumsused by 1\relax%
(\the\colnumsused)}}%
\global\advance\loopnum by1\repeat}

%%%%%%%%%%%%%%%%%%%%%%%%%
%% this version of countcols  is for \colnumbers
\newcount\totalcolumncount
\def\xH{h}

\makeatother
\def\tabcountcols#1{\ifcat#1c
\global\advance\colcount by 1\relax\fi%
%%
\def\lookforD{#1}%
\ifx\lookforD\xD%
\expandafter\gdef\csname tab\the\colcount\endcsname{%
\multicolumn2{c}{\global\advance\colnumsused by 1\relax%
(\the\colnumsused)}}%
\fi%
\ifx\lookforD\xH%
\expandafter\gdef\csname tab\the\colcount\endcsname{%
\multicolumn1{h}{}}%
\fi%
%%
\futurelet\next\tablookatnext}

\def\tabxeatone#1{\tabcountcols}

%% second conditional deals with expressions like @{} in
%% the preamble.
\def\tablookatnext{\if\next\xrelax\let\xgo\relax\else%
\ifx\next\bgroup\let\xgo\tabxeatone\else\let\xgo\tabcountcols\fi\fi\xgo}
\makeatletter
%%%%%%%%%%%%%%%

\newcount\totalcolumns
\newbox\firsttablebox
\newbox\secondtablebox
\newbox\thirdtablebox
\newif\ifdbreaktab

%% A loop would be more elegant, of course, but using & in a loop
%% within a table column produces errors.
%% was\tabnumberline, now \colnumbers

%% Is this test necessary?
%\newif\ifcolumnums

\newif\ifcolnumberson
\def\deluxecolnumbers{\global\colnumbersontrue}

\def\colnumbers{\omit\\\omit\xcolnumbers}
\def\xcolnumbers{\global\let\colnumbers\xcolnumbers%
\global\colnumbersontrue\let&\CheckNumberAndSwitch%
\global\colcount=0\relax%
\global\totalcolumncount=0\relax%
%% above here
\settabnumdefaults%
%% Now, change the columns that have `D' to be \multicolumn2c, by redefining
%% the \csname tab<number>\endcsname
%%
\expandafter\tabcountcols\tabfullpreamble%
\global\totalcolumncount=\the\colcount\relax%
\global\colcount=0\relax%
\ifbreaktab\else\ifdbreaktab\else\global\colnumsused=0\relax\fi\fi%
%%
%
\ifdeluxe\ifbreaktab\\\else\\[-6pt]\fi%\hline% not above
\else%
\\[-14pt]\fi%
\ifcase\totalcolumncount%
\or%
\csname tab1\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname%
\or
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname&%
\csname tab15\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname&%
\csname tab15\endcsname&\csname tab16\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname&%
\csname tab15\endcsname&\csname tab16\endcsname&%
\csname tab17\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname&%
\csname tab15\endcsname&\csname tab16\endcsname&%
\csname tab17\endcsname&\csname tab18\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname&%
\csname tab15\endcsname&\csname tab16\endcsname&%
\csname tab17\endcsname&\csname tab18\endcsname&%
\csname tab19\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname&%
\csname tab15\endcsname&\csname tab16\endcsname&%
\csname tab17\endcsname&\csname tab18\endcsname&%
\csname tab19\endcsname&\csname tab20\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname&%
\csname tab15\endcsname&\csname tab16\endcsname&%
\csname tab17\endcsname&\csname tab18\endcsname&%
\csname tab19\endcsname&\csname tab20\endcsname&%
\csname tab21\endcsname%
\or%22
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname&%
\csname tab15\endcsname&\csname tab16\endcsname&%
\csname tab17\endcsname&\csname tab18\endcsname&%
\csname tab19\endcsname&\csname tab20\endcsname&%
\csname tab21\endcsname&\csname tab22\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname&%
\csname tab15\endcsname&\csname tab16\endcsname&%
\csname tab17\endcsname&\csname tab18\endcsname&%
\csname tab19\endcsname&\csname tab20\endcsname&%
\csname tab21\endcsname&\csname tab22\endcsname&%
\csname tab23\endcsname%
\or% 24
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname&%
\csname tab15\endcsname&\csname tab16\endcsname&%
\csname tab17\endcsname&\csname tab18\endcsname&%
\csname tab19\endcsname&\csname tab20\endcsname&%
\csname tab21\endcsname&\csname tab22\endcsname&%
\csname tab23\endcsname&\csname tab24\endcsname%
\or% 25
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname&%
\csname tab15\endcsname&\csname tab16\endcsname&%
\csname tab17\endcsname&\csname tab18\endcsname&%
\csname tab19\endcsname&\csname tab20\endcsname&%
\csname tab21\endcsname&\csname tab22\endcsname&%
\csname tab23\endcsname&\csname tab24\endcsname&%
\csname tab25\endcsname%
\or% 
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname&%
\csname tab15\endcsname&\csname tab16\endcsname&%
\csname tab17\endcsname&\csname tab18\endcsname&%
\csname tab19\endcsname&\csname tab20\endcsname&%
\csname tab21\endcsname&\csname tab22\endcsname&%
\csname tab23\endcsname&\csname tab24\endcsname&%
\csname tab25\endcsname&\csname tab26\endcsname%
\or% 27
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname&%
\csname tab15\endcsname&\csname tab16\endcsname&%
\csname tab17\endcsname&\csname tab18\endcsname&%
\csname tab19\endcsname&\csname tab20\endcsname&%
\csname tab21\endcsname&\csname tab22\endcsname&%
\csname tab23\endcsname&\csname tab24\endcsname&%
\csname tab25\endcsname&\csname tab26\endcsname&%
\csname tab27\endcsname%
\or% 28
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname&%
\csname tab15\endcsname&\csname tab16\endcsname&%
\csname tab17\endcsname&\csname tab18\endcsname&%
\csname tab19\endcsname&\csname tab20\endcsname&%
\csname tab21\endcsname&\csname tab22\endcsname&%
\csname tab23\endcsname&\csname tab24\endcsname&%
\csname tab25\endcsname&\csname tab26\endcsname&%
\csname tab27\endcsname&\csname tab28\endcsname%
\or% 29
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname&%
\csname tab15\endcsname&\csname tab16\endcsname&%
\csname tab17\endcsname&\csname tab18\endcsname&%
\csname tab19\endcsname&\csname tab20\endcsname&%
\csname tab21\endcsname&\csname tab22\endcsname&%
\csname tab23\endcsname&\csname tab24\endcsname&%
\csname tab25\endcsname&\csname tab26\endcsname&%
\csname tab27\endcsname&\csname tab28\endcsname&%
\csname tab29\endcsname%
\or% 30
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname&%
\csname tab15\endcsname&\csname tab16\endcsname&%
\csname tab17\endcsname&\csname tab18\endcsname&%
\csname tab19\endcsname&\csname tab20\endcsname&%
\csname tab21\endcsname&\csname tab22\endcsname&%
\csname tab23\endcsname&\csname tab24\endcsname&%
\csname tab25\endcsname&\csname tab26\endcsname&%
\csname tab27\endcsname&\csname tab28\endcsname&%
\csname tab29\endcsname&\csname tab30\endcsname%
\else%
\typeout{^^J^^J
Sorry, more than 30 columns cannot be numbered with^^J
\string\colnumbers. Please number the columns manually.^^J
Thank you!^^J}\fi%
%\ifbreaktab
\\\hline% below, hline is wanted
%\else
\noalign{\vskip-13pt}
%\vrule height 28pt width0pt %the \vrule is in the line below colnumbers; 
                          % it causes all the vrules on that line to grow to 28pt.
                          % The -14pt will cause the lower line to overlap the upper line.
                          % Complication, needed to add this vrule to Z and z in order to
                          % have it also work for split tabular.
%\fi
}


\let\savecolnumbers\colnumbers

\gdef\plaincolnumbers{%
\omit\\\omit%
\global\colnumbersontrue\let&\CheckNumberAndSwitch%
\global\colcount=0\relax%
\global\totalcolumncount=0\relax%
%% above here
\settabnumdefaults%
%% Now, change the columns that have `D' to be \multicolumn2c, by redefining
%% the \csname tab<number>\endcsname
%%
\expandafter\tabcountcols\tabfullpreamble%
\global\totalcolumncount=\the\colcount\relax%
\global\colcount=0\relax%
\ifbreaktab\else\ifdbreaktab\else\global\colnumsused=0\relax\fi\fi%
%%
\\\ifcase\totalcolumncount%
\or%
\csname tab1\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname%
\or
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname&%
\csname tab15\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname&%
\csname tab15\endcsname&\csname tab16\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname&%
\csname tab15\endcsname&\csname tab16\endcsname&%
\csname tab17\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname&%
\csname tab15\endcsname&\csname tab16\endcsname&%
\csname tab17\endcsname&\csname tab18\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname&%
\csname tab15\endcsname&\csname tab16\endcsname&%
\csname tab17\endcsname&\csname tab18\endcsname&%
\csname tab19\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname&%
\csname tab15\endcsname&\csname tab16\endcsname&%
\csname tab17\endcsname&\csname tab18\endcsname&%
\csname tab19\endcsname&\csname tab20\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname&%
\csname tab15\endcsname&\csname tab16\endcsname&%
\csname tab17\endcsname&\csname tab18\endcsname&%
\csname tab19\endcsname&\csname tab20\endcsname&%
\csname tab21\endcsname%
\or%22
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname&%
\csname tab15\endcsname&\csname tab16\endcsname&%
\csname tab17\endcsname&\csname tab18\endcsname&%
\csname tab19\endcsname&\csname tab20\endcsname&%
\csname tab21\endcsname&\csname tab22\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname&%
\csname tab15\endcsname&\csname tab16\endcsname&%
\csname tab17\endcsname&\csname tab18\endcsname&%
\csname tab19\endcsname&\csname tab20\endcsname&%
\csname tab21\endcsname&\csname tab22\endcsname&%
\csname tab23\endcsname%
\or% 24
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname&%
\csname tab15\endcsname&\csname tab16\endcsname&%
\csname tab17\endcsname&\csname tab18\endcsname&%
\csname tab19\endcsname&\csname tab20\endcsname&%
\csname tab21\endcsname&\csname tab22\endcsname&%
\csname tab23\endcsname&\csname tab24\endcsname%
\or% 25
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname&%
\csname tab15\endcsname&\csname tab16\endcsname&%
\csname tab17\endcsname&\csname tab18\endcsname&%
\csname tab19\endcsname&\csname tab20\endcsname&%
\csname tab21\endcsname&\csname tab22\endcsname&%
\csname tab23\endcsname&\csname tab24\endcsname&%
\csname tab25\endcsname%
\or% 
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname&%
\csname tab15\endcsname&\csname tab16\endcsname&%
\csname tab17\endcsname&\csname tab18\endcsname&%
\csname tab19\endcsname&\csname tab20\endcsname&%
\csname tab21\endcsname&\csname tab22\endcsname&%
\csname tab23\endcsname&\csname tab24\endcsname&%
\csname tab25\endcsname&\csname tab26\endcsname%
\or% 27
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname&%
\csname tab15\endcsname&\csname tab16\endcsname&%
\csname tab17\endcsname&\csname tab18\endcsname&%
\csname tab19\endcsname&\csname tab20\endcsname&%
\csname tab21\endcsname&\csname tab22\endcsname&%
\csname tab23\endcsname&\csname tab24\endcsname&%
\csname tab25\endcsname&\csname tab26\endcsname&%
\csname tab27\endcsname%
\or% 28
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname&%
\csname tab15\endcsname&\csname tab16\endcsname&%
\csname tab17\endcsname&\csname tab18\endcsname&%
\csname tab19\endcsname&\csname tab20\endcsname&%
\csname tab21\endcsname&\csname tab22\endcsname&%
\csname tab23\endcsname&\csname tab24\endcsname&%
\csname tab25\endcsname&\csname tab26\endcsname&%
\csname tab27\endcsname&\csname tab28\endcsname%
\or% 29
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname&%
\csname tab15\endcsname&\csname tab16\endcsname&%
\csname tab17\endcsname&\csname tab18\endcsname&%
\csname tab19\endcsname&\csname tab20\endcsname&%
\csname tab21\endcsname&\csname tab22\endcsname&%
\csname tab23\endcsname&\csname tab24\endcsname&%
\csname tab25\endcsname&\csname tab26\endcsname&%
\csname tab27\endcsname&\csname tab28\endcsname&%
\csname tab29\endcsname%
\or% 30
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname&%
\csname tab15\endcsname&\csname tab16\endcsname&%
\csname tab17\endcsname&\csname tab18\endcsname&%
\csname tab19\endcsname&\csname tab20\endcsname&%
\csname tab21\endcsname&\csname tab22\endcsname&%
\csname tab23\endcsname&\csname tab24\endcsname&%
\csname tab25\endcsname&\csname tab26\endcsname&%
\csname tab27\endcsname&\csname tab28\endcsname&%
\csname tab29\endcsname&\csname tab30\endcsname%
\else%
\typeout{^^J^^J
Sorry, more than 30 columns cannot be numbered with^^J
\string\colnumbers. Please number the columns manually.^^J
Thank you!^^J}\fi%
\\\hline% below, hline is wanted
%\\\noalign{\vskip-30pt}
%\vrule height 28pt width0pt %the \vrule is in the line below colnumbers; 
                          % it causes all the vrules on that line to grow to 28pt.
                          % The -14pt will cause the lower line to overlap the upper line.
                          % Complication, needed to add this vrule to Z and z in order to
                          % have it also work for split tabular.
}

\let\saveplaincolnumbers\plaincolnumbers


\def\splitplaincolnumbers{%
\omit\\\omit%
\xplain}

\let\savesplitplaincolnumbers\splitplaincolnumbers

\newif\iffirsttime
\firsttimetrue
\gdef\xplain{%
\global\let\plaincolnumbers\xplain%
\global\colnumbersontrue\let&\CheckNumberAndSwitch%
\global\colcount=0\relax%
\global\totalcolumncount=0\relax%
%% above here
\settabnumdefaults%
%% Now, change the columns that have `D' to be \multicolumn2c, by redefining
%% the \csname tab<number>\endcsname
%%
\expandafter\tabcountcols\tabfullpreamble%
\global\totalcolumncount=\the\colcount\relax%
\global\colcount=0\relax%
\ifbreaktab\else\ifdbreaktab\else\global\colnumsused=0\relax\fi\fi%
%%
\iffirsttime
\\%\hline% above not wanted
\else
\\[-12pt]%\hline% above not wanted
\fi
\ifcase\totalcolumncount%
\or%
\csname tab1\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname%
\or
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname&%
\csname tab15\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname&%
\csname tab15\endcsname&\csname tab16\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname&%
\csname tab15\endcsname&\csname tab16\endcsname&%
\csname tab17\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname&%
\csname tab15\endcsname&\csname tab16\endcsname&%
\csname tab17\endcsname&\csname tab18\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname&%
\csname tab15\endcsname&\csname tab16\endcsname&%
\csname tab17\endcsname&\csname tab18\endcsname&%
\csname tab19\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname&%
\csname tab15\endcsname&\csname tab16\endcsname&%
\csname tab17\endcsname&\csname tab18\endcsname&%
\csname tab19\endcsname&\csname tab20\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname&%
\csname tab15\endcsname&\csname tab16\endcsname&%
\csname tab17\endcsname&\csname tab18\endcsname&%
\csname tab19\endcsname&\csname tab20\endcsname&%
\csname tab21\endcsname%
\or%22
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname&%
\csname tab15\endcsname&\csname tab16\endcsname&%
\csname tab17\endcsname&\csname tab18\endcsname&%
\csname tab19\endcsname&\csname tab20\endcsname&%
\csname tab21\endcsname&\csname tab22\endcsname%
\or%
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname&%
\csname tab15\endcsname&\csname tab16\endcsname&%
\csname tab17\endcsname&\csname tab18\endcsname&%
\csname tab19\endcsname&\csname tab20\endcsname&%
\csname tab21\endcsname&\csname tab22\endcsname&%
\csname tab23\endcsname%
\or% 24
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname&%
\csname tab15\endcsname&\csname tab16\endcsname&%
\csname tab17\endcsname&\csname tab18\endcsname&%
\csname tab19\endcsname&\csname tab20\endcsname&%
\csname tab21\endcsname&\csname tab22\endcsname&%
\csname tab23\endcsname&\csname tab24\endcsname%
\or% 25
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname&%
\csname tab15\endcsname&\csname tab16\endcsname&%
\csname tab17\endcsname&\csname tab18\endcsname&%
\csname tab19\endcsname&\csname tab20\endcsname&%
\csname tab21\endcsname&\csname tab22\endcsname&%
\csname tab23\endcsname&\csname tab24\endcsname&%
\csname tab25\endcsname%
\or% 
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname&%
\csname tab15\endcsname&\csname tab16\endcsname&%
\csname tab17\endcsname&\csname tab18\endcsname&%
\csname tab19\endcsname&\csname tab20\endcsname&%
\csname tab21\endcsname&\csname tab22\endcsname&%
\csname tab23\endcsname&\csname tab24\endcsname&%
\csname tab25\endcsname&\csname tab26\endcsname%
\or% 27
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname&%
\csname tab15\endcsname&\csname tab16\endcsname&%
\csname tab17\endcsname&\csname tab18\endcsname&%
\csname tab19\endcsname&\csname tab20\endcsname&%
\csname tab21\endcsname&\csname tab22\endcsname&%
\csname tab23\endcsname&\csname tab24\endcsname&%
\csname tab25\endcsname&\csname tab26\endcsname&%
\csname tab27\endcsname%
\or% 28
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname&%
\csname tab15\endcsname&\csname tab16\endcsname&%
\csname tab17\endcsname&\csname tab18\endcsname&%
\csname tab19\endcsname&\csname tab20\endcsname&%
\csname tab21\endcsname&\csname tab22\endcsname&%
\csname tab23\endcsname&\csname tab24\endcsname&%
\csname tab25\endcsname&\csname tab26\endcsname&%
\csname tab27\endcsname&\csname tab28\endcsname%
\or% 29
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname&%
\csname tab15\endcsname&\csname tab16\endcsname&%
\csname tab17\endcsname&\csname tab18\endcsname&%
\csname tab19\endcsname&\csname tab20\endcsname&%
\csname tab21\endcsname&\csname tab22\endcsname&%
\csname tab23\endcsname&\csname tab24\endcsname&%
\csname tab25\endcsname&\csname tab26\endcsname&%
\csname tab27\endcsname&\csname tab28\endcsname&%
\csname tab29\endcsname%
\or% 30
\csname tab1\endcsname&\csname tab2\endcsname&%
\csname tab3\endcsname&\csname tab4\endcsname&%
\csname tab5\endcsname&\csname tab6\endcsname&%
\csname tab7\endcsname&\csname tab8\endcsname&%
\csname tab9\endcsname&\csname tab10\endcsname&%
\csname tab11\endcsname&\csname tab12\endcsname&%
\csname tab13\endcsname&\csname tab14\endcsname&%
\csname tab15\endcsname&\csname tab16\endcsname&%
\csname tab17\endcsname&\csname tab18\endcsname&%
\csname tab19\endcsname&\csname tab20\endcsname&%
\csname tab21\endcsname&\csname tab22\endcsname&%
\csname tab23\endcsname&\csname tab24\endcsname&%
\csname tab25\endcsname&\csname tab26\endcsname&%
\csname tab27\endcsname&\csname tab28\endcsname&%
\csname tab29\endcsname&\csname tab30\endcsname%
\else%
\typeout{^^J^^J
Sorry, more than 30 columns cannot be numbered with^^J
\string\colnumbers. Please number the columns manually.^^J
Thank you!^^J}\fi%
\\\hline% below, hline is wanted
\iffirsttime
\\\noalign{\vskip-30pt}
\vrule height 28pt width0pt %the \vrule is in the line below colnumbers; 
                          % it causes all the vrules on that line to grow to 28pt.
                          % The -14pt will cause the lower line to overlap the upper line.
                          % Complication, needed to add this vrule to Z and z in order to
                          % have it also work for split tabular.
\fi\global\firsttimefalse
}

\def\decimalcolnumbers{\crcr\saveplaincolnumbers\\%
\noalign{\global\savetabskip\tabskip
\tabskip=0pt
\global\let\extracolsep\relax
\global\let\ddoit\saveddoit
\global\let\zdoit\savezdoit
\vskip-32pt
}{\vrule height28pt depth0pt width0pt}\relax}

\def\splitdecimalcolnumbers{\\[-15pt]%
\savesplitplaincolnumbers
\global\colnumbersonfalse
\\\noalign{\vskip-32pt %!!!
\global\savetabskip\tabskip
\tabskip=0pt
\global\let\extracolsep\relax
\global\let\ddoit\saveddoit
\global\let\zdoit\savezdoit
}\vrule height 28pt width0pt %!!!
\global\let\splitdecimalcolnumbers\secondsplitdecimalcolnumbers}

\def\secondsplitdecimalcolnumbers{\omit\\%[-15pt]
\plaincolnumbers
\global\colnumbersonfalse
\\\noalign{\vskip-26pt %!!! was -28pt
\global\savetabskip\tabskip
\tabskip=0pt
\global\let\extracolsep\relax
\global\let\ddoit\saveddoit
\global\let\zdoit\savezdoit
}\\\relax}

\let\savesplitdecimalcolnumbers\splitdecimalcolnumbers

%%AAA
\newif\ifdeluxestar
\expandafter\def\csname
deluxetable*\endcsname{\deluxestartrue\bgroup\floattrue
\hsize=\textwidth	
\deluxetable}

\expandafter\def\csname enddeluxetable*\endcsname{\enddeluxetable
\egroup
\global\colnumbersonfalse
\global\deluxedecimalsfalse
\global\deluxestarfalse
}

\def\deluxedecimalcolnumbers{\deluxedecimalstrue\colnumbersontrue}
\def\deluxetablecaption#1{\gdef\@tablecaption{#1}}

\newif\ifstartlongtable
\def\startlongtable{\global\startlongtabletrue}

\newif\iffloat
\def\floattable{\global\deluxestartrue\global\floattrue}

%% for equivalent but in \begin...\end form.
\def\floatrotatetable{\global\deluxestartrue\global\floattrue}
\let\endfloatrotatetable\relax

\def\deluxetable{
\global\deluxetrue
\catcode`\&=\active
\catcode`\$=\active
\let\tablecaption\deluxetablecaption
\deluxetablecaption{}
%% july 2016
% \iffloat
% \let\go\ydeluxetable
% \else\let\go\longdeluxetable\fi\go%}
%% aug 2016
\ifstartlongtable
   \ifdeluxestar
\vskip12pt
   \if@two@col\onecolumngrid
   \vskip12pt
   \fi\fi
\let\go\longdeluxetable
\else
\let\go\ydeluxetable
\fi\go
}

\def\ydeluxetable#1{%
\@ifnextchar[{\xdeluxetable{#1}}{\zdeluxetable{#1}}}

% x and z are the same, except that xdeluxetable allows optional square bracket arg, like [h].
\def\xdeluxetable#1[#2]{\global\breaktabtrue
\let\colnumbers\deluxecolnumbers
\global\deluxedecimalsfalse
\let\decimals\deluxedecimals
\let\decimalcolnumbers\deluxedecimalcolnumbers
\let\tablehead\ztablehead
\gdef\tabfullpreamble{#1}%<<== needed
\def\endtabular{\endarray
\global\let\zdoit\relax
\global\let\tdoit\relax
\global\Dfalse}
\global\colnumsused=0
\global\breaktabtrue
\global\colcount=0
%%
%%%%%%%%%%%%
  \lineskiplimit=\z@ % restore default setting
\ifdeluxestar
\gdef\two{#2}\gdef\checkh{h}
\ifx\two\checkh\onecolumngrid\fi
\begin{table*}[#2]\hsize=\textwidth\else
  \begin{table}[#2]\fi
\noindent\setbox\splitbox=\vtop\bgroup%
\currtabletypesize
    \vspace*{\abovedeluxetableskip}
%%
\def\startdata##1\enddata{%
\currtabletypesize
\setbox0=\hbox{
\begin{tabular}{#1}
\pt@head
##1\end{tabular}}
\expandafter\ifx\csname @tablecaption\endcsname\empty\else

\noindent\hbox
to\hsize{\hss\vtop{\hsize=\wd0
\caption{\@tablecaption}}\hss}\vskip3pt\fi
\global\setbox3\hbox{%
\begin{tabular}{#1}%
\hline\hline\noalign{\vskip-9pt}%
\pt@head%
##1\omit\\\omit\\\hline\end{tabular}}

%\noindent\hskip-1.25em %% kludge! but seems necessary
\hbox to\hsize{\hss\copy3\hss}
\global\setbox4\vtop\bgroup\ifdeluxestar\hsize=\textwidth\else\hsize=\wd0\fi\leftskip6pt\parindent-6pt
}}

\def\zdeluxetable#1{\global\breaktabtrue
\let\colnumbers\deluxecolnumbers
\global\deluxedecimalsfalse
\let\decimals\deluxedecimals
\let\decimalcolnumbers\deluxedecimalcolnumbers
\let\tablehead\ztablehead
\gdef\tabfullpreamble{#1}%<<== needed
\def\endtabular{\endarray
\global\let\zdoit\relax
\global\let\tdoit\relax
\global\Dfalse}
\global\breaktabtrue
\global\colnumsused=0
\global\colcount=0
%%
%%%%%%%%%%%%
  \lineskiplimit=\z@ % restore default setting
\ifdeluxestar
\begin{table*}\hsize=\textwidth\else
  \begin{table}\fi
\noindent\setbox\splitbox=\vtop\bgroup%
\currtabletypesize
    \vspace*{\abovedeluxetableskip}
%%
\def\startdata##1\enddata{%
\currtabletypesize
\setbox0=\hbox{\colnumbersonfalse
\begin{tabular}{#1}
\pt@head
##1\end{tabular}}%
\expandafter\ifx\csname @tablecaption\endcsname\empty\else

\noindent\hbox
to\hsize{\hss\vtop{\hsize=\wd0
\caption{\@tablecaption}}\hss}\vskip3pt\fi
\global\setbox3\hbox{%
\begin{tabular}{#1}%
\hline\hline\noalign{\vskip-9pt}%
\pt@head%

##1\omit\\\omit\\\hline\end{tabular}}%%<<== original
\vskip-\parskip
\noindent\hbox to\hsize{\hss\copy3\hss}
\global\setbox4\vtop\bgroup\hsize=\wd0\relax
\leftskip6pt\parindent-6pt
}}

%% go to \end{deluxetable}, after longdeluxetable

\newbox\longtablebox
\def\longdeluxetable#1{
\global\rotateonfalse
\let\colnumbers\deluxecolnumbers
\global\deluxedecimalsfalse
\let\decimals\deluxedecimals
\let\decimalcolnumbers\deluxedecimalcolnumbers
\let\tablehead\ztablehead
\gdef\tabfullpreamble{#1}%<<== needed
\def\endtabular{\endarray
\global\let\zdoit\relax
\global\let\tdoit\relax
\global\Dfalse}
\global\colnumsused=0
\global\colcount=0
%%
%%%%%%%%%%%%
  \lineskiplimit=\z@ % restore default setting
\let\enddeluxetable\endlongdeluxetable
    \vspace*{\abovedeluxetableskip}
%%
\def\startdata##1\enddata{%
\global\setbox\longtablebox=\hbox{\currtabletypesize
\tabcolsep=3pt
\begin{tabular}{#1}
\pt@head
##1\end{tabular}}
%%%
\bgroup\centering
\def\table@hook{\currtabletypesize}
      \LTcapwidth=\wd\longtablebox
\begin{longtable}{#1}
\caption{\hsize=\wd\longtablebox 
\advance\baselineskip2pt
\@tablecaption}\\
\hline\hline\noalign{\vskip-9pt}% prob ok
\pt@head%
\endfirsthead

\noalign{\centerline{\small 
{\bf Table \thetable}\ \it(continued)}\vskip6pt}
\hline\hline
\noalign{\vskip-12pt}
\pt@head%
\endhead

\hline
\multicolumn{\totalcolumns}{c}{\vrule height 24pt width0pt\small\it
Table \thetable\
continued  \if@two@col\else on next page\fi}\\ 
\endfoot

\hline%\nobreak
\endlastfoot

##1
\end{longtable}
\vglue-24pt
\egroup
\global\setbox4=\vtop\bgroup
\ifdim\wd\longtablebox>\textwidth
\hsize=\textwidth
\else
\hsize=\wd\longtablebox\fi
\leftskip=6pt
\parindent=-6pt
\currtabletypesize
\global\startlongtablefalse
}% end data, endlongtable
}


\def\endlongdeluxetable{\vrule depth 6pt width 0pt
\vskip1sp
\egroup
\ifdim\dp4>6pt
\vbox{%\vglue-3.5\baselineskip %% why this dimension??
\hbox to \columnwidth{\hfill
\vtop{\hsize\wd\longtablebox
\leftskip=6pt\parindent-6pt
\copy4}\hfill}
}\fi
\ifdeluxestar
 \if@two@col
\vglue\ht4
 \twocolumngrid
 \hsize=\columnwidth
\fi\fi%
\global\colnumbersonfalse
\global\deluxedecimalsfalse
\global\rotateonfalse
%\global\floatfalse
\if@two@col\vskip12pt\twocolumngrid\fi
\relax}

%% bbb
%% \end{deluxetable}:
\def\enddeluxetable{%
\egroup%end box 4
\ifdim\dp4>6pt
\hbox to\hsize{\hss\copy4\hss}
\fi
\egroup% end splitbox
\centering
\ifrotateon\global\rotateonfalse
\rotatebox{90}{\hbox to\textheight{\hfill\vbox{
\unvbox\splitbox
\vspace*{\belowdeluxetableskip}}\hfill}}
\else
\centering\unvbox\splitbox
\vspace*{\belowdeluxetableskip}
\vspace*{24pt}
\fi
\ifdeluxestar\end{table*}\global\deluxestarfalse
\if@two@col
\twocolumngrid\hsize=\columnwidth\fi%% check this!!
\else\end{table}\fi
\gdef\colnumbers{\saveplaincolnumbers}
\global\breaktabfalse
\global\deluxefalse
\global\colnumbersonfalse
\global\deluxedecimalsfalse
\global\rotateonfalse
\startlongtablefalse
%\global\floatfalse
}%% check this!!



\newbox\splitbox
\newif\ifdeluxe
\def\splitdeluxetable{\global\deluxetrue\catcode`\&=\active
\catcode`\$=\active
\xsplitdeluxetable}

\def\xsplitdeluxetable#1{\global\breaktabtrue
\let\colnumbers\deluxecolnumbers
\let\decimals\deluxedecimals
\global\deluxedecimalsfalse
\let\decimalcolnumbers\deluxedecimalcolnumbers
\let\tablehead\xtablehead
\gdef\tabfullpreamble{#1}
\def\endtabular{\endarray
\global\let\zdoit\relax
\global\let\tdoit\relax
\global\Dfalse}
%%% modification of emulateapj \deluxetable %%%%
\setbox0=\hbox{\def\firstarg{#1}\expandafter\lookforD\firstarg}
\gdef\temppreamble{#1\relax}
\PartsOfTable=0
\def\tempfullpreamble{#1BB}
\setbox0=\hbox{\expandafter\checkforB\tempfullpreamble}
%% Now PartsOfTable is either =2 or 3
%%
\gdef\one{#1Z}
\global\colnumsused=0
\global\breaktabtrue
\global\colcount=0
%%
\ifnum\PartsOfTable=3
\let\multicolumn\threebreakmulticolumn
\else
\let\multicolumn\breakmulticolumn
\fi
%%%%%%%%%%%%
  \lineskiplimit=\z@ % restore default setting
  \gdef\tblnote@list{}
  \gdef\tblref@list{}
\ifsplitstar
  \begin{table*}\else
  \begin{table}\fi
\noindent\setbox\splitbox=\vtop\bgroup%
\currtabletypesize
    \vspace*{\abovedeluxetableskip}
\let\startdata\xstartdata}
%% \end{splitdeluxetable}:

\newdimen\movetabledown

\def\endsplitdeluxetable{\vskip1sp\egroup%% end box with tablenotes
\hbox to \hsize{\hss\copy4\hss}
\egroup
\vskip1pt
\ifrotateon\global\rotateonfalse
\vskip\movetabledown\rotatebox{90}{\vbox{\noindent\unvbox\splitbox %
\vspace*{\belowdeluxetableskip}
}}\global\movetabledown=0pt\else
\noindent\unvbox\splitbox
\vspace*{\belowdeluxetableskip}
\fi
\ifsplitstar
\end{table*}
\else
\end{table}\fi
\gdef\colnumbers{\saveplaincolnumbers}
\tabletypesize{\small}
\global\breaktabfalse
\global\deluxefalse
\global\splitstarfalse
\global\colnumbersonfalse
\global\deluxedecimalsfalse
}

\newif\ifsplitstar
\expandafter\def\csname splitdeluxetable*\endcsname{\global\splitstartrue\splitdeluxetable}
\expandafter\def\csname endsplitdeluxetable*\endcsname{\endsplitdeluxetable\global\splitstarfalse 
\global\colnumbersonfalse
\global\deluxedecimalsfalse
}

\newdimen\maxtablewidth

\gdef\NoTableCaption{\global\@table@not@headedtrue}

%% For splitdeluxetable

%%% ====================================================== %%%
\gdef\dbreaktabular{\catcode`\&=\active
\let&\CheckNumberAndSwitch\xdbreaktabular}

\long\gdef\xdbreaktabular#1{%% #1=contents of table
{\global\maxtablewidth=0pt
\let&\CheckNumberAndSwitch
\let$\savedollar
\global\colnumsused=0
%%
\global\dbreaktabtrue
\global\colcount=0
%%
\ifnum\PartsOfTable=3
\let\multicolumn\threebreakmulticolumn
\else
\let\multicolumn\breakmulticolumn
\fi
%%
\ifnum\PartsOfTable=3
\expandafter\catchfirstpreamble\one
\expandafter\catchsecondofthreepreamble\one
\expandafter\catchthirdpreamble\one
\makefirstdummycolumns
\makeseconddummycolumns
\makethirddummycolumns
\else %% PartsOfTable=2
\ifnum\PartsOfTable=2
\expandafter\catchfirstpreamble\one
\expandafter\catchsecondpreamble\one
\makefirstdummycolumns
\makeseconddummycolumns
\fi\fi
%%%
\global\columncount=0
\ifnum\PartsOfTable=3
%% For table divided into three parts
\firstboxtrue\secondboxfalse\thirdboxfalse
\setbox\firsttablebox=\hbox{%
\begin{tabular}{AFE}
\ifx\csname pt@head\endcsname\relax\else
\pt@head\fi#1\crcr\end{tabular}}
\global\maxtablewidth=\wd\firsttablebox

\noindent\hbox to \hsize{\hss\unhbox\firsttablebox\hss}
\vskip6pt
\hrule
\vskip6pt
\global\columncount=0
\firstboxfalse\secondboxtrue\thirdboxfalse
\ifcolnumberson%
\setbox\secondtablebox=\hbox{%
\let\savecolnumbers\xcolnumbers%
\notfirsttrue%
\begin{tabular}{fZE} %fZE !!!
\ifx\csname pt@head\endcsname\relax\else%
\pt@head\fi#1\crcr\end{tabular}}
\else
%%
\setbox\secondtablebox=\hbox{%
\begin{tabular}{fZE}%
\ifx\csname pt@head\endcsname\relax\else%
\pt@head\fi\\[-14pt]%
#1\crcr%
\end{tabular}}
\fi
\ifdim\wd\secondtablebox>\maxtablewidth
\global\maxtablewidth\wd\secondtablebox\fi

\noindent\hbox to \hsize{\hss\unhbox\secondtablebox\hss}
%%
\vskip6pt
\hrule
\vskip6pt
\firstboxfalse\secondboxfalse\thirdboxtrue
\global\columncount=0
\ifcolnumberson
\notfirsttrue
\setbox\thirdtablebox=\hbox{
\let\savecolnumbers\xcolnumbers
\notfirsttrue
\begin{tabular}{fFz}
\ifx\csname pt@head\endcsname\relax\else
\pt@head\fi#1\crcr\end{tabular}}
\else
\setbox\thirdtablebox=\hbox{
\begin{tabular}{fFz}
\ifx\csname pt@head\endcsname\relax\else
\pt@head\fi\\[-14pt]
#1
\end{tabular}}
\fi
\ifdim\wd\thirdtablebox>\maxtablewidth
\global\maxtablewidth\wd\thirdtablebox\fi

\noindent\hbox to \hsize{\hss\unhbox\thirdtablebox\hss}
\vskip6pt
\hrule
\else
%% Original for table divided into two parts
\global\columncount=0
\secondboxfalse
\setbox\firsttablebox=\hbox{%
\begin{tabular}{AF}
\ifx\csname pt@head\endcsname\relax\else
\pt@head\fi%
#1\end{tabular}}
\global\maxtablewidth=\wd\firsttablebox
\hbox to \hsize{\hss\unhbox\firsttablebox\hss}
\vskip6pt
\hrule
\vskip6pt
\global\columncount=0
\secondboxtrue
\ifcolnumberson
\setbox\secondtablebox=\hbox{%
\let\savecolnumbers\xcolnumbers
\notfirsttrue
\begin{tabular}{fZ}%%
\ifx\csname pt@head\endcsname\relax\else%
\pt@head\fi#1\crcr%%= tablecontents
\end{tabular}}%
\else
\setbox\secondtablebox=\hbox{%
\begin{tabular}{fZ}%% was 12
\ifx\csname pt@head\endcsname\relax\else%
\pt@head\fi\\[-14pt]%
#1%%= tablecontents
\end{tabular}}\fi
\ifdim\wd\secondtablebox>\maxtablewidth
\global\maxtablewidth\wd\secondtablebox\fi

\noindent\hbox to \hsize{\hss\unhbox\secondtablebox\hss}
\vskip6pt
\hrule
\secondboxtrue
%%
%% end of conditional testing for 2 or 3 part table:
\fi
%%
\global\dbreaktabfalse}}
%%% ====================================================== %%%

\newif\ifnotfirst
%% @@@@
%% xstartdata, modified from \startdata in emulateapj, for splitdeluxetable
\gdef\xstartdata#1\enddata{\def\tablecontents{%
\ifcolnumberson%
\\ \savecolnumbers\\[2pt]\fi%
\ifdeluxedecimals\savedecimals\fi%
#1}%
\currtabletypesize%
\setbox2=\vtop{\dbreaktabular{\tablecontents}}%
%
\expandafter\ifx\csname @tablecaption\endcsname\empty\else

\noindent\hbox
to\hsize{\hss\vtop{\hsize=\maxtablewidth\caption{\@tablecaption}}\hss}\vskip3pt\fi
\dbreaktabular{\tablecontents\noalign{\global\let\zdoit\relax
\global\let\ddoit\relax}}
\parindent=0pt
\global\setbox4=\vtop\bgroup% egroup in enddeluxetable
\currtabletypesize
\ifsplitstar
\hsize=\textwidth\else\hsize=245.3pt\fi
\parindent=-6pt \leftskip=6pt 
}

\def\tablecomments#1{{\small\vskip3pt\indent\vrule height 11pt depth 2pt
width 0pt\currtabletypesize{\sc Note}---{#1}\vskip1sp}}

\def\tablenotetext#1#2{{\currtabletypesize\vskip1pt\indent\vrule
height 11pt depth
2pt width0pt\relax$^{\hbox to 5pt{$#1$}}$#2\vskip1sp}}

\def\tablerefs#1{{\small\vskip3pt\indent\vrule height 11pt depth 2pt
width 0pt\currtabletypesize{\bf References}---{#1}\vskip1sp}}

\let\tablereferences\tablerefs

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% 5. Simple entry decimal numbers

%% extra unused args are to get rid of unnecessary commands revtex puts in
\gdef\lookfordecimal#1#2#3#4.#5 {\gdef\xone{{\let$\relax\savedollar#4\savedollar}}
\gdef\xtwo{#5}\ifx\xtwo\empty\else\gdef\xtwo{{\let$\relax\savedollar#5\savedollar}}\fi}

%% D 
\def\newdoit{\setbox0=\hbox\bgroup\zdoit}
\def\endnewdoit{\egroup\unhbox0}

\long\gdef\zdoit#1 {\let$\relax
\def\bothcols{#1 }%
\setbox0=\hbox{\let$\relax\expandafter\lookfordecimal\bothcols{}{}{}{}.{} }%
\xdoit}

\global\let\savezdoit\zdoit
\let\zdoit\relax

\gdef\xdoit{\relax\hskip\tabcolsep\relax\xone&\tabskip=0pt%
\ifx\xtwo\empty\let\go\relax\else.\def\go{\xtwo}\fi\go}

%% d
\def\xnewdoit{\setbox0=\hbox\bgroup\ddoit}
\def\xendnewdoit{\egroup}

\long\gdef\ddoit#1#2#3{\xxdoit}
\let\saveddoit\ddoit
\let\ddoit\relax

%% to delete all D material: 

\gdef\xxdoit{&}

\newcolumntype{D}{>\newdoit r<{\endnewdoit} @{}l}%% 
\newcolumntype{d}{>\xnewdoit h<{\xendnewdoit} @{}h} %% 

\newdimen\savetabskip
\gdef\decimals{\noalign{\global\savetabskip\tabskip
\tabskip=0pt
\global\let\extracolsep\relax
\global\let\ddoit\saveddoit
\global\let\zdoit\savezdoit
}}

\let\savedecimals\decimals

%% to allow \decimals to be used before \startdata:
\newif\ifdeluxedecimals
\def\deluxedecimals{\global\deluxedecimalstrue}

%%%%%%%%%
%% This needed to be redefined so that \colhead in \tablehead would span both parts
%% of decimal numbers.

%% in case there isn't a table head
\let\pt@head\relax

%% for splitdeluxetable
\def\xtablehead{\catcode`\&=\active%
\catcode`\$=\active%
\xxtablehead}

\def\xxtablehead#1{%
\let&\CheckNumberAndSwitch%
\gdef\pt@head{%
\hline\hline%
\multicolumn1c{\tempcounter=0
\expandafter\getDs\tabfullpreamble\relax
\global\colcount=0
\global\colheadcount=0}%
\\[-10pt]% this is right 
#1\ifcolnumberson%
\ifnotfirst\\[-22pt]\fi
\else\\\hline\\[-8pt]\fi% space below hline for 2nd and 3rd part of split table
}%
%
}

\def\ztablehead{\catcode`\&=\active%
\catcode`\$=\active%
\zztablehead}

%%
\def\zztablehead#1{\let&\CheckNumberAndSwitch%
\gdef\pt@head{%
%% this is needed:
\multicolumn1c{\expandafter\getDs\tabfullpreamble\relax
\global\tempcounter=0
\global\colcount=0
\global\colheadcount=0}\\%
#1
\ifcolnumberson\\[6pt]
\savecolnumbers\vrule height 11pt depth 4pt width 0pt\relax%
\\[6pt]
\ifdeluxedecimals\\[-14pt] % 
\savedecimals\fi
\else \vrule depth 6pt
width0pt\\\ifdeluxedecimals\savedecimals\fi\hline\fi%
}}


\newcount\tempcounter

\gdef\getDs#1{\let&\CheckNumberAndSwitch
\def\lookforD{#1}%
\ifx\lookforD\xD%
\expandafter\gdef\csname col\the\tempcounter\endcsname{2}\else
\expandafter\gdef\csname col\the\tempcounter\endcsname{1}\fi 
\global\advance\tempcounter by 1
\futurelet\next\checkingpreamble}

\gdef\checkingpreamble{\ifx\next\relax
\let\go\relax\else\let\go\getDs\fi\go}

%%% Something like this could be used to automate the width of colheads in the tablehead,
%% making those that match the D in preamble are multicolumn2c instead of
%% multicolumn 1c.
\newcount\colheadcount
\newcommand\xcolhead[1]{\multicolumn{\expandafter\ifx\csname
col\the\colheadcount\endcsname\relax 1\else\expandafter%
\csname col\the\colheadcount\endcsname\fi}{c}{\vrule depth 4pt width %% 
0pt#1\relax\global\advance\colheadcount
by 1\relax}\ignorespaces}%
%

%%
\extrarowheight=2pt
%% from revtex4-1, additions on top
%% fix for \usepackage{amsmath} and 
%% any matrix environment
\def\matrixpreamble{*\c@MaxMatrixCols c}
%% this causes problem, must be fixed!
%\let\save@array@array@new\@array@array@new
\def\@array@array@new[#1]#2{%
\ifbreaktab
\else
%%% added so that we can use \colnumbers in any tabular environment
%%% and avoid error messages for breaktabular
\def\catchpreamble{#2\relax}
\gdef\tabfullpreamble{#2\relax}
{\colcount=0
%% important fix, makes it possible to use amsmath and matrices.
\def\two{#2}
\ifx\matrixpreamble\two
\else
\expandafter\countcols\catchpreamble
\global\totalcolumns=\colcount\fi}
\fi
%%% end of additions
  \@tempdima\ht\strutbox
  \advance\@tempdima by\extrarowheight
  \setbox\@arstrutbox\hbox{%
   \vrule \@height\arraystretch\@tempdima
          \@depth \arraystretch\dp\strutbox
          \@width \z@
  }%
  \begingroup
   \@mkpream{#2}%
   \xdef\@preamble{\@preamble}%
  \endgroup
  \prepdef\@preamble{%
   \tabskip\tabmid@skip
    \@arstrut
  }%
  \appdef\@preamble{%
   \tabskip\tabright@skip
   \cr
   \array@row@pre
  }%
  \@arrayleft
  \@nameuse{@array@align@#1}%
  \m@th
  \let\\\new@arraycr %<<== defined above, original plus reset counters
  \let\tabularnewline\\%
  \let\par\@empty
  \let\@sharp##%
  \set@typeset@protect
  \lineskip\z@\baselineskip\z@
  \tabskip\tableft@skip
  \everycr{}%
  \expandafter\halign\expandafter\@halignto\expandafter\bgroup\@preamble
}%

%% \rotate 
\newif\ifrotateon
\def\rotate{\global\floattrue\iffloat\global\let\go\relax\global\rotateontrue\else
\global\rotateonfalse 
\let\go\relax
%\def\go{\vskip48pt\huge
%{\tt \string\floattable\space must precede table using
%\string\rotate !!}}
\fi\go}

\def\colnumbers{\plaincolnumbers}

%% add 6pt of space between table and following text:
\let\saveendtable\endtable
\def\endtable{\vskip6pt\saveendtable}
\expandafter \let \csname endtable*\endcsname = \endtable
%%

\newbox\rotatetablebox
\def\rotatetable{%
\global\startlongtabletrue\setbox\rotatetablebox=\vbox\bgroup
}
\def\endrotatetable{\egroup
\vglue\movetabledown
\hbox to
\textwidth{\hss\rotatebox{90}{\hbox{\box\rotatetablebox}}\hss}
\global\movetabledown=0pt\relax
\global\startlongtablefalse
}


\expandafter\def\csname rotatetable*\endcsname{%
\global\startlongtabletrue\setbox\rotatetablebox=\vbox to
\textwidth\bgroup\vfill}


\expandafter\def\csname endrotatetable*\endcsname{\vfill\egroup
\vbox to \textheight{\vfill
\vglue\movetabledown
\hbox to
\textwidth{\hss\rotatebox{90}{\box\rotatetablebox}\hss}\global\movetabledown=0pt\relax 
\vfill}
\clearpage
\if@two@col
\twocolumngrid
\global\startlongtablefalse
}


\def\longrotatetable{%
   \if@two@col\onecolumngrid\clearpage
   \fi
\clearpage
   \clearpage
  \begingroup
\expandafter\def\csname deluxetable*\endcsname{\deluxetable}
\expandafter\def\csname enddeluxetable*\endcsname{\enddeluxetable}
\global\floatfalse
\global\startlongtabletrue
\def\LS@rot{%
  \setbox\@outputbox\vbox{\hbox{\rotatebox{90}{\box\@outputbox}}}}

\let\LS@makecol=\@makecol
\let\LS@makefcolumn=\@makefcolumn

  \vsize=\textwidth
  \hsize=\textheight
  \linewidth=\hsize
  \columnwidth=\hsize
  \@colroom=\vsize
  \textheight=\vsize
  \@colht=\vsize
  \def\@makecol{\LS@makecol\LS@rot}%
  \def\@makefcolumn##1{\LS@makefcolumn{##1}\LS@rot}}
\def\endlongrotatetable{%
\onecolumngrid %% ??
\clearpage
  \ifGin@pdftex
    \pdfpageattr{/Rotate 90}
  \fi
  \clearpage
  \endgroup
   \if@two@col\twocolumngrid\fi
\clearpage
  \global\@colht=\textheight
  \global\vsize=\textheight
  \global\@colroom=\textheight}


\newif\ifGin@pdftex
\Gin@pdftexfalse
\DeclareOption{pdftex}{%
  \PassOptionsToPackage\CurrentOption{graphicx}
  \Gin@pdftextrue
}

\DeclareOption*{\PassOptionsToPackage\CurrentOption{graphicx}}
\ProcessOptions

%% set &, $ catcode back to normal:

\catcode`&=4
\catcode`$=3



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% end table tools
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Gridlines for positioning multiple illustrations in 
%% one figure environment.

\def\gridline#1{\vskip6pt\hbox to\hsize{#1}\vskip6pt}

\def\boxedfig#1#2#3{\hfill\fbox{\vbox{\parskip=0pt\relax
\hsize=#2
\includegraphics[width=#2]{#1}\vskip2pt\vtop{\hsize=#2
\centerline{#3}}}}\hfill}

\def\fig#1#2#3{\hfill\vbox{\parskip=0pt\hsize=#2
\includegraphics[width=#2]{#1}\vskip2pt\vtop{\centering
\footnotesize
\hsize=#2
#3\vskip1pt
}}\hfill}

\def\leftfig#1#2#3{\vbox{\parskip=0pt\relax\hsize=#2
\includegraphics[width=#2]{#1}\vskip2pt\vtop{\hsize=#2
\centering
#3\vskip1sp\vskip1sp}}\hfill}

\def\rightfig#1#2#3{\hfill\vbox{\parskip=0pt\relax\hsize=#2
\includegraphics[width=#2]{#1}\vskip2pt\vtop{\hsize=#2
\centering#3\vskip1sp}}}

\def\rotatefig#1#2#3#4{\hfill\vbox{\centering\parskip=0pt\hsize=#3
\includegraphics[width=#3,angle=#1]{#2}\vskip2pt\vtop{\centering
\footnotesize
\hsize=#3
#4\vskip1pt
}}\hfill}

%%%%%%%%%% End Grid line Macros %%%%%%%%%%

%%%%%%%%%% Color Editing Macros %%%%%%%%%%
%% \turnoffedit or \turnoffedits
%% will prevent all \edit<number>{text}, all
%% \collaborationcomment<number>{text}, and all
%% \authorcomment<number>{text} from producing any text.

\newif\ifturnoffedit
\def\turnoffedit{\global\turnoffedittrue}
\def\turnoffedits{\global\turnoffedittrue}

\newif\ifturnoffone
\newif\ifturnofftwo
\newif\ifturnoffthree

%% \turnoffeditone to only turn off only \edit1, \collaborationcomment1 and \authorcomment1 :
\def\turnoffeditone{\turnoffonetrue}

%% \turnoffedittwo to only turn off only \edit2, \collaborationcomment2 and \authorcomment2 :
\def\turnoffedittwo{\turnofftwotrue}

%% \turnoffeditthree to only turn off only \edit3, \collaborationcomment3 and \authorcomment3 :
\def\turnoffeditthree{\turnoffthreetrue}

%% Other choices can be made, but this should be
%% standardized, so didn't make an user interface
%% to change the colors easily.

\expandafter\def\csname editcolor1\endcsname{magenta}
\expandafter\def\csname editcolor2\endcsname{blue}
\expandafter\def\csname editcolor3\endcsname{violet}

\newcount\colorcount
\def\edit#1#2{{\colorcount=#1\relax%
\ifturnoffedit\let\go\ignorespaces\else%
\let\go\relax%
\color{\csname editcolor\the\colorcount\endcsname}%
\ifnum\colorcount=1{\ifturnoffone\else\bf#2\ \fi}\else%
\ifnum\colorcount=2{\ifturnofftwo\else\it#2\ \fi}\else%
\ifnum\colorcount=3{\ifturnoffthree\else#2\ \fi}\fi\fi\fi\fi%
}\go}

\def\collaborationcomment#1#2{{\colorcount=#1
\ifturnoffedit\let\go\ignorespaces\else%
\let\go\relax%
\color{\csname editcolor\the\colorcount\endcsname}
\ifnum\colorcount=1{\ifturnoffone\else\bf (Collaboration~note: #2)\ \fi}\else
\ifnum\colorcount=2{\ifturnofftwo\else\it (Collaboration~note: #2)\ \fi}\else
\ifnum\colorcount=3{\ifturnoffthree\else (Collaboration~note: #2)\ \fi}\fi\fi\fi\fi%
\go}}

\def\authorcomment#1#2{{\colorcount=#1
\ifturnoffedit\let\go\ignorespaces\else%
\let\go\relax%
\color{\csname editcolor\the\colorcount\endcsname}
\ifnum\colorcount=1{\ifturnoffone\else\bf (Author~note: #2)\ \fi}\else
\ifnum\colorcount=2{\ifturnofftwo\else\it (Author~note: #2)\ \fi}\else
\ifnum\colorcount=3{\ifturnoffthree\else (Author~note: #2)\ \fi}\fi\fi\fi\fi%
\go}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Draft watermark

\definecolor{ltgray}{gray}{.9}% .89
\font\bighelv=phvr at 2in %
\def\setwatermarkfontsize#1{\font\bighelv=phvr at #1}

\def\watermark#1{\def\thewatermark{\hbox to\textwidth{\vtop to
1.1\textheight{\vss
\hskip24pt\rotatebox{60}{\hbox{\bighelv \color{ltgray} 
\uppercase{#1}}}\vss}}\hss}}
\let\thewatermark\empty

%% Used in titlepage definition, as \pagestyle{titlepage}
\def\ps@titlepage{%
  \let\@mkboth\@gobbletwo
\def\@oddhead{\ifx\thewatermark\empty\hfill\else
\hbox to \textwidth{\rlap{\thewatermark}\hfill}\fi}
\let\@oddfoot\@empty
\let\@evenhead\@empty\let\@evenfoot\@empty}

% end of watermark definitions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand*\submitjournal[1]
{\def\@submitted{Submitted to #1}}%

%% this one is used
\def\titleblock@produce{%
 \begingroup
 \ltx@footnote@pop
 \def\@mpfn{mpfootnote}% 
 \def\thempfn{\thempfootnote}%
 \c@mpfootnote\z@
 \let\@makefnmark\frontmatter@makefnmark
  \frontmatter@setup
  \thispagestyle{titlepage}\label{FirstPage}%
\ifmodern\leftskip=0pt\rightskip\leftskip\fi
  \frontmatter@title@produce
  \groupauthors@sw{%
   \frontmatter@author@produce@group
  }{%
   \frontmatter@author@produce@script
  }%
  \frontmatter@RRAPformat{%
\vskip12pt
   \expandafter\produce@RRAP\expandafter{\@date}%
   \expandafter\produce@RRAP\expandafter{\@received}%
   \expandafter\produce@RRAP\expandafter{\@revised}%
   \expandafter\produce@RRAP\expandafter{\@accepted}%
   \expandafter\produce@RRAP\expandafter{\@published}%
  }%
\expandafter\ifx\csname @submitted\endcsname\relax\else
\vskip6pt
\expandafter\produce@RRAP\expandafter{\centerline{\@submitted\hbox
to 20pt{\hfill}}\vskip12pt}%
\fi
  \frontmatter@abstract@produce
  \@ifx@empty\@pacs{}{%
   \@pacs@produce\@pacs
  }%
  \@ifx@empty\@keywords{}{%
   \@keywords@produce\@keywords
  }%
  \par
  \frontmatter@finalspace
 \endgroup
}%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Highlight Figure
\definecolor{ltblue}{cmyk}{.5,.1,.1,0}

\long\def\highlightfigure#1{\centerline{
\fboxrule=4pt
\fboxsep=12pt
\fcolorbox{ltblue}{white}{\hbox to
.93\textwidth{\hss$\vcenter{\advance\hsize -24pt #1}$\hss}}}\gdef\highlightfigure{\typeout{^^J^^JERROR!^^J^^J
Only One Highlighted Figure per Article!^^J^^J}\stop}}


%%%%%%%%%%%%%
%% Line numbering

\ifnumlines
\usepackage{lineno}

\linenumbers*[1]
\if@two@col
\advance\linenumbersep -4pt
\else
\advance\linenumbersep 12pt
\fi\fi


\gdef\specialbibitem#1[#2]#3#4{
{\tt\string\bibitem}[#2]{\tt\string{\string}}
#4}

\let\savecite\cite
\let\savecitep\citep
\let\savecitet\citet
\def\specialcite#1{\hbox{\savecite{#1}}}
\def\specialcitep#1{\hbox{\savecitep{#1}}}
\def\specialcitet#1{\hbox{\savecitet{#1}}}
\let\saveref\ref
\def\specialref#1{\hbox{\saveref{#1}}}

%%%%%%%%%%%%%%%%%%%%%%%%%
%% Track Changes
%% Amy Hendrickson, Nov 2015
%% Change Jan 2016, to allow list of changes
%% to give line and page numbers for more than one entry on the same line.
%% Change Feb 2016, to allow optional argument for time/date, and/or editor initials, etc.


\providecolor{trackchange}{rgb}{1,0,0}
\providecolor{explain}{rgb}{.5,0,.5}

\newif\ifsilent

\newcount\refchangenumber
\def\added{\@ifnextchar[{\xadded}{\yadded}}

\long\def\xadded[#1]#2{%
\iftrack {\global\advance\refchangenumber by 1\relax%
\vtop to 0pt{\vss
\hypertarget{link\the\refchangenumber}{}
\vskip14pt}%
\ifnumlines%
\ifabstract\else%
\xdef\doit{\noexpand\linelabel{\the\refchangenumber}}\doit\fi\else%
\xdef\doit{\noexpand\label{\the\refchangenumber}{}{}{}}\doit\fi}%
{\color{trackchange}(Added: [#1] #2)}%%
\ifabstract\label{\the\refchangenumber}%
\expandafter\gdef\csname
changenum\the\refchangenumber\endcsname{Added: [#1]
\textcolor{trackchange}{#2}\global\silenttrue}%
\else\expandafter\gdef\csname
changenum\the\refchangenumber\endcsname{Added: [#1]
\textcolor{trackchange}{\let\bibitem\specialbibitem #2}\global\silentfalse}\fi%
\else#2\fi}



\long\def\yadded#1{%
\iftrack{\global\advance\refchangenumber by 1\relax%
\vtop to 0pt{\vss
\hypertarget{link\the\refchangenumber}{}
\vskip14pt}%
\ifnumlines\ifabstract\else%
\xdef\doit{\noexpand\linelabel{\the\refchangenumber}}\doit\fi\else%
\xdef\doit{\noexpand\label{\the\refchangenumber}{}{}{}}\doit%
\fi}%
{\color{trackchange}(Added: #1)}%%
\ifabstract%
\label{\the\refchangenumber}%
\expandafter\gdef\csname
changenum\the\refchangenumber\endcsname{Added:
\textcolor{trackchange}{#1},
\global\silenttrue}\else
\expandafter\gdef\csname
changenum\the\refchangenumber\endcsname{Added:
\textcolor{trackchange}{\let\bibitem\specialbibitem #1},%
\global\silentfalse}\fi%
\else#1\fi}



\def\deleted{\@ifnextchar[{\xdeleted}{\ydeleted}}

\long\def\xdeleted[#1]#2{\iftrack{\global\advance\refchangenumber by
1\relax%
\vtop to 0pt{\vss
\hypertarget{link\the\refchangenumber}{}
\vskip14pt}%
\ifnumlines\ifabstract\else%
\xdef\doit{\noexpand\linelabel{\the\refchangenumber}}\doit\fi%
\else%
\xdef\doit{\noexpand\label{\the\refchangenumber}}\doit\fi%
}%
{\color{trackchange}%
\ifbib\let\sout\relax\fi%
\let\citep\specialcitep%
\let\citet\specialcitet%
\let\ref\specialref\let\cite\specialcite (Deleted: [#1] \sout{#2})
}%
\ifabstract\label{\the\refchangenumber}%
\expandafter\gdef\csname
changenum\the\refchangenumber\endcsname{Deleted: [#1]
{\color{trackchange}%
\let\citet\specialcitet%
\let\citep\specialcitep%
\let\cite\specialcite\sout{#2}}\global\silenttrue}%
\else
\expandafter\gdef\csname
changenum\the\refchangenumber\endcsname{Deleted: [#1] 
{\color{trackchange}%
\let\bibitem\specialbibitem%
\let\ref\specialref%
\let\cite\specialcite%
\let\citep\specialcitep%
\let\citet\specialcitet%
\sout{#2}
}\global\silentfalse}\fi%
\fi}

\long\def\ydeleted#1{\iftrack{\global\advance\refchangenumber by 1\relax%
\vtop to 0pt{\vss
\hypertarget{link\the\refchangenumber}{}
\vskip14pt}%
\ifnumlines\ifabstract\else%
\xdef\doit{\noexpand\linelabel{\the\refchangenumber}}\doit\fi%
\else%
\xdef\doit{\noexpand\label{\the\refchangenumber}{}{}{}}\doit%
\fi}%
%%
{\color{trackchange}%
\ifbib\let\sout\relax\fi%
\let\citep\specialcitep%
\let\citet\specialcitet%
\let\ref\specialref\let\cite\specialcite(Deleted: \sout{#1}
)}%
\ifabstract\label{\the\refchangenumber}%
\expandafter\gdef\csname changenum\the\refchangenumber\endcsname{Deleted:
{\color{trackchange}\let\ref\specialref%
\let\citep\specialcitep%
\let\citet\specialcitet%
\let\cite\specialcite\sout{#1}}\global\silenttrue}%
\else
\expandafter\gdef\csname changenum\the\refchangenumber\endcsname{Deleted:
{\color{trackchange}%
\let\citep\specialcitep%
\let\citet\specialcitet%
\let\bibitem\specialbibitem%
\let\ref\specialref%
\let\cite\specialcite\sout{#1}}\global\silentfalse}\fi%
\fi}


\def\replaced{\@ifnextchar[{\xreplaced}{\yreplaced}}

\long\def\xreplaced[#1]#2#3{%
\iftrack\global\advance\refchangenumber by 1\relax%
\vtop to 0pt{\vss
\hypertarget{link\the\refchangenumber}{}
\vskip14pt}%
\ifnumlines\ifabstract\else\xdef\doit{\noexpand\linelabel{\the\refchangenumber}}\doit\fi\else%
\xdef\doit{\noexpand\label{\the\refchangenumber}}\doit\fi%
{\ifbib\let\sout\relax\fi
\let\citep\specialcitep%
\let\citet\specialcitet%
\let\cite\specialcite\color{trackchange}(Replaced: [#1] \sout{#2}}%
{\color{black}replaced with:} {\let\ref\specialref%
\let\citep\specialcitep%
\let\citet\specialcitet%
\let\cite\specialcite\color{trackchange} #3)}%
\ifabstract\label{\the\refchangenumber}%
\expandafter\gdef\csname
changenum\the\refchangenumber\endcsname{Replaced: [#1]
{\let\citep\specialcitep%
\let\citet\specialcitet%
\let\cite\specialcite\color{trackchange}\sout{#2}} {\color{black} replaced with:}
{\color{trackchange}#3}, \global\silenttrue}%
\else
\expandafter\gdef\csname
changenum\the\refchangenumber\endcsname{Replaced: [#1]
{\ifbib\let\sout\relax\fi\let\bibitem\specialbibitem
\let\citep\specialcitep%
\let\citet\specialcitet%
\let\cite\specialcite\color{trackchange}\sout{#2}
} {\color{black} replaced with:}
{\let\bibitem\specialbibitem\color{trackchange}#3}, \global\silentfalse}\fi%
\else#3\fi}

\long\def\yreplaced#1#2{%
\iftrack\global\advance\refchangenumber by 1\relax%
\vtop to 0pt{\vss
\hypertarget{link\the\refchangenumber}{}
\vskip14pt}%
\ifnumlines\ifabstract\else\xdef\doit{\noexpand\linelabel{\the\refchangenumber}}\doit\fi\else%
\xdef\doit{\noexpand\label{\the\refchangenumber}}\doit\fi%
{\ifbib\let\sout\relax\fi\let\ref\specialref%
\let\citep\specialcitep%
\let\citet\specialcitet%
\let\cite\specialcite\color{trackchange}(Replaced: %\sout
{#1}
}%
{\color{black}replaced with:}
{\color{trackchange} #2)}%
\ifabstract\label{\the\refchangenumber}%
\expandafter\gdef\csname changenum\the\refchangenumber\endcsname{Replaced:
{\let\cite\specialcite%
\let\citep\specialcitep%
\let\citet\specialcitet%
\color{trackchange}\sout{#1}} {\color{black} replaced with:}
{\color{trackchange}#2},\global\silenttrue}%
\else
\expandafter\gdef\csname
changenum\the\refchangenumber\endcsname{Replaced:
{\ifbib\let\sout\relax\fi\let\bibitem\specialbibitem
\let\citep\specialcitep%
\let\citet\specialcitet%
\let\cite\specialcite\color{trackchange}\sout{#1}
} {\color{black} replaced with:}
{\let\bibitem\specialbibitem\color{trackchange}#2}, \global\silentfalse}\fi%
\else#2\fi}

\def\explain{\@ifnextchar[{\xexplain}{\yexplain}}

\def\xexplain[#1]#2{\iftrack\ {\it\color{explain} [Explanation of change:
#2 (#1)]\ }\fi}

\def\yexplain#1{\iftrack\ {\it\color{explain} [Explanation of change:
#1]\ }\fi}

\newcount\listchangenum

\def\listofchanges{
\clearpage
\iftrack
\ifnum\refchangenumber>0
\ifnumlines\nolinenumbers\fi
\vskip36pt
\hrule
\noindent{\vrule height 14pt width0pt depth 6pt\large\bf List of Changes}
\hrule
\vskip18pt
\nobreak
{\parskip=4pt \parindent=0pt
\loop
\global\silentfalse
\vskip-1pt\relax
\global\advance\listchangenum by 1\relax
\expandafter\ifx\csname changenum\the\listchangenum\endcsname\relax
\else
\csname changenum\the\listchangenum\endcsname\ 
on page
%% can't get hyperlink to work correctly for page numbers, works but error messages.
\hyperlink{link\the\listchangenum}{\bf\pageref{\the\listchangenum}}%
\ifnumlines%
\ifsilent\global\silentfalse \else%
\setbox0=\hbox{\lineref{\the\listchangenum}}%
\ifdim\wd0<20pt%
, line\
\hyperlink{link\the\listchangenum}{\lineref{\the\listchangenum}}%
\fi
\fi\fi.\relax
\repeat}
\fi\fi
\thispagestyle{empty}
}

\PassOptionsToPackage{normalem}{ulem}
\usepackage{ulem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% From earlier version of AASTeX, for usefulness and 
%% backward compatibility, with some requested additions

\let\jnl@style=\rmfamily
\def\ref@jnl#1{{\jnl@style#1}}%

%%%
\renewcommand\memsai{\ref@jnl{Mem.~Soc.~Astron.~Italiana}}%
          % Mem. Societa Astronomica Italiana
%% longer version:
\newcommand\memsocai{Mem. Societ\`a Astronomica Italiana}
\newcommand\aspconf{Ast. Soc. of the Pac. Conference Series}

\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao

%%% More useful commands from Earlier version of Aastex:
\let\la=\lesssim            % For Springer A&A compliance...
\let\ga=\gtrsim

\let\farcm\farcm@mss
\let\farcs\farcs@mss

\def\farcm@apj{%
 \mbox{.\kern -0.7ex\raisebox{.9ex}{\scriptsize$\prime$}}%
}%

\def\farcs@apj{%
 \mbox{%
  \kern  0.13ex.%
  \kern -0.95ex\raisebox{.9ex}{\scriptsize$\prime\prime$}%
  \kern -0.1ex%
 }%
}%

\def\chem@bnd#1{%
 {%
  \kern.1em\relax
  \setbox\z@\hbox{M}%
  \dimen@ii.8em\relax
  \p@=.1em\relax
  \dimen@.5\ht\z@\dimen@i-\dimen@
  \advance\dimen@1.5\p@\advance\dimen@i-1.0\p@
  #1%
  \kern.1em\relax
  }%
 }%
\def\@sbnd{%
 \advance\dimen@-1.5\p@\advance\dimen@i1.5\p@
 \vrule\@height\dimen@\@depth\dimen@i\@width\dimen@ii\nobreak
 }%
\def\@dbnd{%
 \advance\dimen@-0.5\p@\advance\dimen@i0.5\p@
 \vrule\@height\dimen@\@depth\dimen@i\@width\dimen@ii\nobreak
 \advance\dimen@-1.5\p@\advance\dimen@i1.5\p@
 \hskip-\dimen@ii
 \vrule\@height\dimen@\@depth\dimen@i\@width\dimen@ii\nobreak
 }%
\def\@tbnd{%
 \vrule\@height\dimen@\@depth\dimen@i\@width\dimen@ii\nobreak
 \advance\dimen@-1.5\p@\advance\dimen@i1.5\p@
 \hskip-\dimen@ii
 \vrule\@height\dimen@\@depth\dimen@i\@width\dimen@ii\nobreak
 \advance\dimen@-1.5\p@\advance\dimen@i1.5\p@
 \hskip-\dimen@ii
 \vrule\@height\dimen@\@depth\dimen@i\@width\dimen@ii\nobreak
 }%

\renewcommand\LaTeX{%
 \leavevmode
 L%
 \raise.42ex\hbox{%
  \count@=\the\fam
  $\fam\count@\scriptstyle\kern-.3em A$%
 }%
 \kern-.15em\TeX
}%

%% added Feb 2, 2016, redefining definition of \caption made with hyperref
%% package. Making \caption[] be the default, to prevent sending caption 
%% text to listoftables or listoffigures, which we are not going to use
%% anyway. This change enables track changes commands to work in captions.

\def\caption{\numlinesfalse
\ifx\@captype\@undefined 
\@latex@error {\noexpand \caption outside float}\@ehd 
\expandafter \@gobble \else 
\H@refstepcounter \@captype \let \Hy@tempa \@caption \@ifundefined
{float@caption}{}
{\expandafter \ifx \csname @float@c@\@captype\endcsname
\float@caption\let\Hy@tempa\Hy@float@caption\fi} 
\expandafter\@firstofone\fi 
{\@dblarg {\Hy@tempa \@captype}}[]}


\def\@caption#1[#2]#3{{\small\rm\expandafter \ifx \csname if@capstart\expandafter \endcsname 
\csname iftrue\endcsname \global \let \@currentHref \hc@currentHref \else \hyper@makecurrent {\@captype }\fi 
\@ifundefined {NR@gettitle}{\def \@currentlabelname{\thesection\relax #2}}
{\NR@gettitle {#2}}\par 
%\addcontentsline {\csname ext@#1\endcsname }{#1}{\protect \numberline {\csname the#1\endcsname }{\ignorespaces #2}}
\begingroup \@parboxrestore \if@minipage \@setminipage \fi \normalsize 
\expandafter\ifx \csname if@capstart\expandafter \endcsname 
\csname iftrue\endcsname \global \@capstartfalse 
\@makecaption {\bf\csname fnum@#1\endcsname }{\ignorespaces #3}
\else \@makecaption {\bf\csname fnum@#1\endcsname }{\ignorespaces \ifHy@nesting 
\expandafter \hyper@@anchor \expandafter {\@currentHref }{#3}\else 
\Hy@raisedlink {\expandafter \hyper@@anchor \expandafter
{\@currentHref }{\relax }}{#3}\fi }\fi \par \endgroup}}


\newcommand\tablebreak{\\[-11pt]\noalign{\break}\\ }

%% As suggested by Greg Schwarz, Gus Meunch, Feb 11

\def\dataset{\@ifnextchar[{\ydataset}{\xdataset}}
\def\ydataset[#1]#2{\href{#2}{[#1]}}
\def\xdataset#1{\href{#1}{[DATASET]}}

%% this seems in the middle of nowhere...
\advance\columnsep6pt

%%%%%%%%%%
%% macros to give hyperref link to authors when orcid numbers
%% are supplied with \author[0000-2345-3333-0023]{author name}
 \def\lookforbracket{\ifx\next[\let\go\xauthor
 \else\let\go\yauthor\fi\go}
 
\def\author{\futurelet\next\lookforbracket}

\def\new@author@def#1#2{%
 \move@AU\move@AF\move@AUAF
 \let\@AF@join\@author@join
 \def\@author{{\href{http://orcid.org/#1}{#2}}{}}%
}%

\def\orciderrormessage{
\typeout{^^J^^J [\firstarg]\space Invalid ORCID Identifier!^^J^^J The ID
should consist of
four sets of four digits,^^J separated with -, ie,
0000-0012-3245-1234 or ^^J
0000-0012-3245-123X
^^J^^J
Please fix, or don't use square bracket argument with
\string\author[]\string{\string}
^^J^^J}
}

%% Tests to see if author gave reasonable Orcid number;
%% if not, stops processing and gives error message.
\newif\ifbadOrcid
\def\lookatOrcid #1-#2-#3-#4-{
\def\one{#1}\def\two{#2}\def\three{#3}\def\four{#4}
\ifx\one\empty 
\global\badOrcidtrue
\else
\ifx\two\empty
\global\badOrcidtrue
\else
\ifx\three\empty
\global\badOrcidtrue
\else
\ifx\four\empty
\global\badOrcidtrue
\fi\fi\fi\fi
}

\def\lookforDigits #1#2#3#4{
\def\xone{#1}\def\xtwo{#2}\def\xthree{#3}\def\xfour{#4}
%%
\ifx\xone\empty 
\global\badOrcidtrue
\else
  \ifcat \xone 1\else
  \global\badOrcidtrue\fi
\fi
%%%
\ifx\xtwo\empty 
\global\badOrcidtrue
\else
 \ifcat \xtwo 1\else
  \global\badOrcidtrue\fi
\fi
%%%
\ifx\xthree\empty 
\global\badOrcidtrue
\else
 \ifcat \xthree 1\else
  \global\badOrcidtrue\fi
\fi
%%%
\ifx\xfour\empty 
\global\badOrcidtrue
\else
 \ifcat \xfour 1\else
  \global\badOrcidtrue\fi
\fi
}

\def\FinallookforDigits #1#2#3#4{
\def\xone{#1}\def\xtwo{#2}\def\xthree{#3}\def\xfour{#4}
%%
\ifx\xone\empty 
\global\badOrcidtrue
\else
  \ifcat \xone 1\else
  \global\badOrcidtrue\fi
\fi
%%%
\ifx\xtwo\empty 
\global\badOrcidtrue
\else
 \ifcat \xtwo 1\else
  \global\badOrcidtrue\fi
\fi
%%%
\ifx\xthree\empty 
\global\badOrcidtrue
\else
 \ifcat \xthree 1\else
  \global\badOrcidtrue\fi
\fi
%%%
\ifx\xfour\empty 
\global\badOrcidtrue
\else
   \ifcat \xfour 1\else
      \if\xfour X
      \else
      \global\badOrcidtrue\fi
   \fi
\fi
}





%% Last digit might be X
\def\xauthor[#1]#2{\def\testone{#1-}\def\firstarg{#1}
\setbox0=\hbox{\expandafter\lookatOrcid\testone {}-{}-{}-{}-
\expandafter\lookforDigits\one {}{}{}{}
\expandafter\lookforDigits\two {}{}{}{}
\expandafter\lookforDigits\three {}{}{}{}
\expandafter\FinallookforDigits\four {}{}{}{}}
%%
\ifbadOrcid\let\go\orciderrormessage
\else\let\go\relax\fi\go
\ifbadOrcid\let\go\stop\else\let\go\relax\fi\go
\new@author@def{#1}{#2}}

\def\yauthor{\@author@def{}}

\def\altaffilmark#1{\typeout{^^J^^J\string\altaffilmark\space is no longer
needed. It will not do anything.^^J Please use
\string\altaffiliation\string{\string} instead.^^J^^J}\stop}

\def\altaffiltext#1{\typeout{^^J^^J\string\altaffiltext\space is no longer
needed. It will not do anything.^^J Please use
\string\altaffiliation\string{\string} instead.^^J^^J}\stop}





%% We do not need \and in list of authors. It is taken care of
%% automatically. Below is the definition from revtex4-1:
% 
%\renewcommand\frontmatter@and{\class@err{\protect\and\space is not
% supported}}

\newcount\AuthorCollaborationLimit
\let\AuthorCallLimit\AuthorCollaborationLimit
%% no limit for default
\AuthorCollaborationLimit=100
\newcount\largestAffilNum

\def\lookfornumbers#1#2#3#4#5#6#7#8#9{\def\one{#1}
\def\two{#2}
\def\three{#3}
\def\four{#4}
\def\five{#5}
\def\six{#6}
\def\seven{#7}
\def\eight{#8}
\def\nine{#9}
\ifnum\one>\largestAffilNum
\global\largestAffilNum=\one\fi
%%%
\ifx\two\empty\else
\ifnum\two>\largestAffilNum
\global\largestAffilNum=\two\fi\fi
%%%
\ifx\three\empty\else
\ifnum\three>\largestAffilNum
\global\largestAffilNum=\three\fi\fi
%%%
\ifx\four\empty\else
\ifnum\four>\largestAffilNum
\global\largestAffilNum=\four\fi\fi
%%%
\ifx\five\empty\else
\ifnum\five>\largestAffilNum
\global\largestAffilNum=\five\fi\fi
%%%
\ifx\six\empty\else
\ifnum\six>\largestAffilNum
\global\largestAffilNum=\six\fi\fi
%%%
\ifx\seven\empty\else
\ifnum\seven>\largestAffilNum
\global\largestAffilNum=\seven\fi\fi
%%%
\ifx\eight\empty\else
\ifnum\eight>\largestAffilNum
\global\largestAffilNum=\eight\fi\fi
%%%
\ifx\nine\empty\else
\ifnum\nine>\largestAffilNum
\global\largestAffilNum=\nine\fi\fi
}
\newcount\countauthors


\gdef\newcomma@space{\hskip-3pt\textsuperscript{,}}%

\def\doEtAl{\rm et al.\gdef\doEtAl{\relax}}

\def\doauthor#1#2#3{%
\iflongauthor\vskip6pt\fi
\global\advance\countauthors by 1
\ifnum\countauthors>\AuthorCollaborationLimit
\doEtAl
\else
\ifnum\AuthorCollaborationLimit=1
\let\@listand\relax
\fi
  \ignorespaces\leavevmode\hbox{#1\unskip\@listcomma}% nice, keeps name from breaking across lines
\fi
  \begingroup
\ifnum\countauthors>\AuthorCollaborationLimit\else
  #3% all affil numbers
\ifx\@affilID@temp\empty
\else%
\setbox0=\hbox{\expandafter\lookfornumbers\@affilID@temp{}{}{}{}{}{}{}{}{}}%
\fi\fi
%% #2= \altaffiliation{} or \email{} or possibly anything other than author, affiliation, or collaboration 
%%\endgroup{}{} %%this works.
  \@if@empty{#2}{\endgroup{}{}}
{\ifnum\countauthors>\AuthorCollaborationLimit\else
\endgroup{\comma@space}{}\frontmatter@footnote{#2}\fi}%
\ifnum\countauthors>\AuthorCollaborationLimit\else  \space \@listand\fi
}%

\def\xxxdoauthor#1#2#3{%
\iflongauthor\vskip12pt\fi
\global\advance\countauthors by 1
\ifnum\countauthors>\AuthorCollaborationLimit
\iflongauthor\vskip6pt\fi
\doEtAl
\else
\ifnum\AuthorCollaborationLimit=\countauthors
\iflongauthor\vskip6pt\fi
\let\@listand\relax
\fi
  \ignorespaces\leavevmode\hbox{#1\unskip\@listcomma}% nice, keeps name from breaking across lines
\fi
  \begingroup
\ifnum\countauthors>\AuthorCollaborationLimit\else
%% author names:
  #3% 
%all affil numbers:
\ifx\@affilID@temp\empty
\else%
\setbox0=\hbox{\expandafter\lookfornumbers\@affilID@temp{}{}{}{}{}{}{}{}{}}%
\fi\fi
%% #2= \altaffiliation{} or \email{} or possibly anything other than author, affiliation, or collaboration 
%%\endgroup{}{}
  \@if@empty{#2}{\endgroup{}{}}
{\ifnum\countauthors>\AuthorCollaborationLimit\else
\endgroup{\comma@space}{}\frontmatter@footnote{#2}\fi}%
\ifnum\countauthors>\AuthorCollaborationLimit\else  \space \@listand\fi
}%


%%%
%% set \affil to match \affiliation found in revtex, since authors are accustomed to using \affil{}
\let\affil\affiliation

\newif\iffirstaffil
\firstaffiltrue

\def\@affil@script#1#2#3#4{%
%\ifmodern
\iffirstaffil\vskip24pt 
\global\firstaffilfalse\fi%\fi
 \@ifnum{#1=\z@}{}{%
  \par
  \begingroup
   \frontmatter@affiliationfont
   \@ifnum{\c@affil<\affil@cutoff}{}{%
\def\one{#1}
\ifnum\one<\largestAffilNum
%% this makes the numbers
   \def\@thefnmark{#1}\@makefnmark\fi
\ifnum\one=\largestAffilNum
   \def\@thefnmark{#1}\@makefnmark\fi
   }%
% this makes the text
\ifnum\one<\largestAffilNum
   \ignorespaces#3%
\fi
\ifnum\one=\largestAffilNum
   \ignorespaces#3%
\fi
   \@if@empty{#4}{}{\frontmatter@footnote{#4}}%
   \par
  \endgroup
 }%
}%

\def\frontmatter@maketitle{%
\@author@finish
\if@firstsection
  \title@column\titleblock@produce
\onecolumngrid
\else
%
\global\firstaffiltrue
 \title@column\secondtitleblock@produce
\fi
  \suppressfloats[t]%
%% Prevent these from being turned off so that
%% we can use \maketitle again for \AllAuthors.
%%
%  \let\and\relax
  \let\affiliation\@gobble
  \let\author\@gobble
%  \let\@AAC@list\@empty
%  \let\@AFF@list\@empty
%  \let\@AFG@list\@empty
%  \let\@AF@join\@AF@join@error
%  \let\email\@gobble
%  \let\@address\@empty
% \let\maketitle\relax
%  \let\thanks\@gobble
\if@firstsection
  \let\abstract\@undefined\let\endabstract\@undefined
  \titlepage@sw{%
   \vfil
   \clearpage
  }{}%
\fi
}%

\let\maketitle\frontmatter@maketitle

\def\secondtitleblock@produce{%
 \begingroup
  \ltx@footnote@pop
  \def\@mpfn{footnote}%
  \def\thempfn{\thefootnote}%
  \c@footnote\z@
  \let\@makefnmark\frontmatter@makefnmark
%  \frontmatter@setup
  \thispagestyle{titlepage}%\label{FirstPage}%
%  \frontmatter@title@produce
  \groupauthors@sw{%
   \frontmatter@author@produce@group
  }{%
   \frontmatter@author@produce@script
  }%
  \endgroup
}%


\def\allauthors{%% this conditional keeps \allauthors from turning on
%%                 unless \AuthorCollaborationLimit is used:
\ifnum\AuthorCollaborationLimit>0
\ifnumlines\nolinenumbers\fi
\onecolumngrid
\clearpage
\AuthorCollaborationLimit=100
\largestAffilNum=100
{\vskip6pt\vskip1sp\centerline{\large\bf All Authors and
Affiliations\vrule depth 18pt width0pt}\nobreak
\maketitle
\fi
}}

\let\AllAuthors\allauthors

%% no club or widow lines
\widowpenalty=10000
\clubpenalty\widowpenalty
\setlength{\footnotesep}{8pt}

\ifmodern
\setlength{\voffset}{0in}
\setlength{\hoffset}{0in}
\setlength{\textwidth}{6in}
\setlength{\textheight}{9.2in}
\setlength{\headheight}{0ex}
\setlength{\headsep}{36pt} % this is 2 lines in ``manuscript''
\setlength{\footnotesep}{0in}
\setlength{\topmargin}{-\headsep}
\setlength{\oddsidemargin}{0.25in}
\setlength{\evensidemargin}{0.25in}
\setlength{\parindent}{0.54\baselineskip}
\sloppy\sloppypar
\fi


\def\figurename{Figure}
\def\tablename{Table}
\def\fnum@figure{{\bf\figurename~\thefigure}}
\def\fnum@table{{\bf\tablename~\thetable}}

\def\tempfootmark#1{}

\newcount\c@affilcount

 \renewcommand*\altaffiliation[2][]{%
 \@AF@join{#1#2\ifmodern\baselineskip=14pt\fi
}%
 }%

\def\correspondingauthor#1{{
\renewcommand\thefootnote{\hskip-12pt}
\footnote{Corresponding author: #1\ifmodern\vrule depth 5pt
width 0pt\relax\fi}}}

\let\saveemail\email
\def\email#1{{\let\ltx@footmark\tempfootmark
\saveemail{}}
{\renewcommand\thefootnote{\hskip-12.1pt}
\footnote{\href{mailto: #1}{#1}\ifmodern\vrule depth 7pt width
0pt\relax\else\ifmanu\vskip-4pt\else\vrule depth 7pt width 0pt\fi\fi}}}


\def\nocollaboration{%
\iflongauthor
\collaboration{\vbox to 0pt{\vss ---\vskip9pt}}
\else
\collaboration{\vbox to 0pt{\vss ---\vskip4pt}}
\fi
}

%% gets rid of () around collaboration
\def\@collaboration@present#1#2#3#4{%
\par
 \begingroup
  \frontmatter@collaboration@above
  \@affilID@def{}%
  \@tempcnta\z@
  \@author@present{}{\ignorespaces#3\unskip}{#4}%
  \par
 \endgroup
\iflongauthor\vskip-6pt\else
\vskip6pt\fi
 \set@listcomma@list#1%
}%


%% get rid of \jobname Notes being sent to .aux file:
%\let\bibdata@app\relax
%\def\pre@bibdata{}

\def\frontmatter@author@produce@script{%
  \begingroup
    \let\@author@present\@author@present@script
    \frontmatterverbose@sw{\typeout{\string\frontmatter@author@produce@script:}\say\@AAC@list\say\@AFF@list\say\@AFG@list}{}%
    \let\AU@temp\@empty
    \@tempcnta\z@
    \let\AF@opr \@gobble
    \def\AU@opr{\@author@count\@tempcnta}%
    \def\CO@opr{\@collaboration@count\AU@temp\@tempcnta}%
    \@AAC@list
    \expandafter\CO@opr\@author@cleared
    \begingroup
     \frontmatter@authorformat
     \let\AF@opr \@affilID@def
     \let\AU@opr \@author@present
     \def\CO@opr{\@collaboration@present\AU@temp}%
     \set@listcomma@list\AU@temp
     \@AAC@list
%% \, added to definition taken from revtex4-1 to prevent error message.
\,     \unskip\unskip
     \par
    \endgroup
    \begingroup
     \frontmatter@above@affiliation@script
     \let\AFF@opr \@affil@script
     \@AFF@list
     \frontmatter@footnote@produce
     \par
    \endgroup
  \endgroup
}%

\let\auto@bib\relax

\newif\iffirstaffil
\firstaffiltrue

%% These commands were in aastex earlier; I redefined.
\def\tighten{\global\tightentrue\normalsize}
\let\tightenlines=\tighten
\def\singlespace{\par\global\doublespacefalse\global\tightenfalse\normalsize}
\def\doublespace{\par\global\doublespacetrue\global\tightenfalse\normalsize}

\bibliographystyle{aasjournal}

\endinput

%% Change Log
September 21, 2016
Finishing Version 6.1 update

=====================
August 27, 2016                               
Many changes

=====================
August 17
Many changes:

%% note:
%% this keeps tables from being set to \small, code used in Revtex4-1
\let\table@hook\relax

=====================
Feb 29, changes to table macros to center caption even if table is wider than
width of text; give error message if user asks to rotate table but
forgets to use \floattable before table; make rotating table be full
text width even if called for in double columns.

March 1, reworking figure and table numbering for appendices. 
Deleted recent definition of \appendix, returned to earlier version
with additions.

================













==> OLD/apjfontssty <==
% Wed Dec  4 20:36:44 1996
% Alexey Vikhlinin <alexey@head-cfa.harvard.edu>
% Maxim Markevitch <maxim@head-cfa.harvard.edu>
% This is a style file to use Times fonts for text and math, using CM versions
% for greek letters and math symbols. Works for both LaTeX2e and older LaTeX
% 2.09. 
% 
% Report any bugs or problems to alexey@head-cfa.harvard.edu
%
%  Nov 4 2003:  \AA was broken because of redefinition of \r
%


\@ifundefined{documentclass}{
%% This part is used with Latex 2.09. No boldface. The part for Latex2e is
%% below.

% latex style with times roman text and times italic math (MM)

% plain text:

\def\@mrm{unmr}% times - roman, version Nimbus
\def\@mit{ptmri}% times - italic
\def\@msl{ptmro}% times - oblique
\def\@mbf{ptmb}% times - bold
\def\@mcsc{ptmrc}% times - roman - small caps
\def\@mtt{pcrr}% courier
\def\@mss{phvr}% helvetica


% math text font:

\font\twfvmi = ptmri at 25pt
\font\twtymi = ptmri at 20pt
\font\svtnmi = ptmri at 17pt
\font\frtnmi = ptmri at 14pt
\font\twlmi  = ptmri at 12pt
\font\elvmi  = ptmri at 11pt
\font\tenmi  = ptmri at 10pt
\font\ninmi  = ptmri at 9pt
\font\egtmi  = ptmri at 8pt
\font\sevmi  = ptmri at 7pt
\font\sixmi  = ptmri at 6pt
\font\fivmi  = ptmri at 5pt 

% math symbol font (Symbol from ctan/fonts/psfonts/adobe/times) 
% reencoded by texmital.enc):

%\font\twfvcmmi = zpsycmrv at 25pt
%\font\twtycmmi = zpsycmrv at 20pt
%\font\svtncmmi = zpsycmrv at 17pt
%\font\frtncmmi = zpsycmrv at 14pt
%\font\twlcmmi  = zpsycmrv at 12pt
%\font\elvcmmi  = zpsycmrv at 11pt
%\font\tencmmi  = zpsycmrv at 10pt
%\font\nincmmi  = zpsycmrv at 9pt 
%\font\egtcmmi  = zpsycmrv at 8pt 
%\font\sevcmmi  = zpsycmrv at 7pt 
%\font\sixcmmi  = zpsycmrv at 6pt 
%\font\fivcmmi  = zpsycmrv at 5pt 
% cmmi greek is better:
\font\twfvcmmi = cmmi10 at 25pt
\font\twtycmmi = cmmi10 at 20pt
\font\svtncmmi = cmmi10 at 17pt
\font\frtncmmi = cmmi10 at 14pt
\font\twlcmmi  = cmmi10 at 12pt
\font\elvcmmi  = cmmi10 at 11pt
\font\tencmmi  = cmmi10 at 10pt
\font\nincmmi  = cmmi9
\font\egtcmmi  = cmmi8
\font\sevcmmi  = cmmi7
\font\sixcmmi  = cmmi6
\font\fivcmmi  = cmmi5


%%% these are pieces from dvips/contrib/timesmat.sty:

% Put cmmi back into TeX, as a new maths alphabet, so that we
% can get back the Greek & other characters missing in Times.

% (MM: I found experimantally that textfont9 is the first unused font)
\def\@tempa{9}

% Tell TeX where cmmi is.
% Assumes \@ptsize is defined by article, report, book
\ifcase \@ptsize
  \textfont\@tempa\tencmmi
  \scriptfont\@tempa\sevcmmi
  \scriptscriptfont\@tempa\fivcmmi
\or
  \textfont\@tempa\elvcmmi
  \scriptfont\@tempa\sevcmmi
  \scriptscriptfont\@tempa\fivcmmi
\or
  \textfont\@tempa\twlcmmi
  \scriptfont\@tempa\egtcmmi
  \scriptscriptfont\@tempa\sixcmmi
\fi

% cmmi and Times-italic have different positions for some punctuation marks
%% (MM: this may be replaced by re-encoding times-italic by texmital.enc)
% \mathcode`\ ="8000 % \space
% \mathcode`\!="5021
% \mathcode`\'="8000 % ^\prime
% \mathcode`\(="4028
% \mathcode`\)="5029
% \mathcode`\*="22.4 % \ast
% \mathcode`\+="202B
\mathcode`\,="602C
% \mathcode`\-="2200
\mathcode`\.="002E
\mathcode`\/="002F
% \mathcode`\:="303A
% \mathcode`\;="603B
\mathcode`\<="303C
% \mathcode`\=="303D
\mathcode`\>="303E
% \mathcode`\?="503F
% \mathcode`\[="405B
% \mathcode`\\="026E % \backslash
% \mathcode`\]="505D
% \mathcode`\_="8000 % \_
% \mathcode`\{="4266
% \mathcode`\|="026A
% \mathcode`\}="5267
\mathchardef\ldotp="602E % ldot as a punctuation mark

% Put back the missing lowercase Greek characters.
\mathchardef\alpha="0\@tempa 0B
\mathchardef\beta="0\@tempa 0C
\mathchardef\gamma="0\@tempa 0D
\mathchardef\delta="0\@tempa 0E
\mathchardef\epsilon="0\@tempa 0F
\mathchardef\zeta="0\@tempa 10
\mathchardef\eta="0\@tempa 11
\mathchardef\theta="0\@tempa 12
\mathchardef\iota="0\@tempa 13
\mathchardef\kappa="0\@tempa 14
\mathchardef\lambda="0\@tempa 15
\mathchardef\mu="0\@tempa 16
\mathchardef\nu="0\@tempa 17
\mathchardef\xi="0\@tempa 18
\mathchardef\pi="0\@tempa 19
\mathchardef\rho="0\@tempa 1A
\mathchardef\sigma="0\@tempa 1B
\mathchardef\tau="0\@tempa 1C
\mathchardef\upsilon="0\@tempa 1D
\mathchardef\phi="0\@tempa 1E
\mathchardef\chi="0\@tempa 1F
\mathchardef\psi="0\@tempa 20
\mathchardef\omega="0\@tempa 21
\mathchardef\varepsilon="0\@tempa 22
\mathchardef\vartheta="0\@tempa 23
\mathchardef\varpi="0\@tempa 24
\mathchardef\varrho="0\@tempa 25
\mathchardef\varsigma="0\@tempa 26
\mathchardef\varphi="0\@tempa 27

% Put back other missing characters.
\mathchardef\imath="0110
\mathchardef\jmath="0\@tempa 7C
\mathchardef\ell="0\@tempa 60
\mathchardef\wp="0\@tempa 7D
\mathchardef\partial="0\@tempa 40
\mathchardef\flat="0\@tempa 5B
\mathchardef\natural="0\@tempa 5C
\mathchardef\sharp="0\@tempa 5D
\mathchardef\smile="3\@tempa 5E
\mathchardef\frown="3\@tempa 5F
\mathchardef\leftharpoonup="3\@tempa 28
\mathchardef\leftharpoondown="3\@tempa 29
\mathchardef\rightharpoonup="3\@tempa 2A
\mathchardef\rightharpoondown="3\@tempa 2B
\mathchardef\lhook="3\@tempa 2C \def\hookrightarrow{\lhook\joinrel\rightarrow}
\mathchardef\rhook="3\@tempa 2D \def\hookleftarrow{\leftarrow\joinrel\rhook}
\mathchardef\star="2\@tempa 3F
\mathchardef\vecMC="0\@tempa 7E
\def\vec{\mathaccent\the\vecMC }


\input psfonts.sty
\input psgreek.sty
}
%
% This is LaTeX2e style by Alexey Vikhlinin to mix Times for text and math
% and CM for greek and symbols.
%
%
%
%
%
{
\def\fileversion{5.2}
\def\filedate{1995/08/16}
\def\docdate {1995/03/12}
\NeedsTeXFormat{LaTeX2e}
\ProvidesPackage{apjfonts}[\filedate{} Times + math package]

\let\rold\r
\def\AA{\rold A}
\RequirePackage[T1]{fontenc} \let\r\relax

\DeclareOption{onecolumn}{
\relax   % this style is often used as \usepackage{emulateapj,timesfonts}
}
\ExecuteOptions{}
\ProcessOptions

\renewcommand{\sfdefault}{phv}
\renewcommand{\rmdefault}{ptm}
\renewcommand{\ttdefault}{pcr}

\DeclareSymbolFont{cmoperators}   {OT1}{cmr}{m}{n}
\DeclareSymbolFont{cmitoperators} {OT1}{cmr}{m}{it}
\DeclareSymbolFont{operators}     {OT1}{ptm}{m}{n}
%\DeclareSymbolFont{ptmoperators}  {OT1}{ptmcm}{m}{n}
\DeclareSymbolFont{letters}       {OML}{ptmcm}{m}{it}
%\DeclareSymbolFont{rusletters}    {OML}{petersburg}{m}{it}
\DeclareSymbolFont{ptmletters}    {OML}{ptmcm}{m}{it}
\DeclareSymbolFont{cmletters}     {OML}{cmm}{m}{it}
\DeclareSymbolFont{symbols}       {OMS}{cmsy}{m}{n}
\DeclareSymbolFont{ptmsymbols}    {U}{psy}{m}{n}
\DeclareSymbolFont{largesymbols}  {OMX}{cmex}{m}{n}
\DeclareSymbolFont{bold}          {OT1}{ptm}{bx}{n}
\DeclareSymbolFont{italic}        {OT1}{ptm}{m}{it}

\SetSymbolFont{cmoperators}   {bold}{OT1}{cmr}{b}{n}
\SetSymbolFont{cmitoperators} {bold}{OT1}{cmr}{bx}{it}
\SetSymbolFont{operators}     {bold}{OT1}{ptm}{bx}{n}
%\SetSymbolFont{ptmoperators}  {bold}{OT1}{ptmCM}{b}{n}
\SetSymbolFont{letters}       {bold}{OML}{ptmCM}{b}{it}
%\SetSymbolFont{rusletters}    {bold}{OML}{petersburg}{bx}{it}
\SetSymbolFont{ptmletters}    {bold}{OML}{ptmCM}{b}{it}
\SetSymbolFont{cmletters}     {bold}{OML}{cmm}{b}{it}
\SetSymbolFont{symbols}       {bold}{OMS}{cmsy}{b}{n}
\SetSymbolFont{largesymbols}  {bold}{OMX}{cmex}{m}{n}
\SetSymbolFont{bold}          {bold}{OT1}{ptm}{bx}{n}
\SetSymbolFont{italic}        {bold}{OT1}{ptm}{b}{it}


\DeclareMathAlphabet{\mathbf}{OT1}{ptm}{bx}{n}
\DeclareMathAlphabet{\mathit}{OT1}{ptm}{m}{it}
\DeclareMathAlphabet{\mathbit}{OT1}{ptm}{bx}{it}

\DeclareMathSymbol{\omicron}{0}{operators}{`\o}

\thinmuskip=2mu 
\medmuskip=2.5mu plus 1mu minus 1mu
\thickmuskip=4mu plus 1.5mu minus 1mu

% \everydisplay {\thinmuskip=2mu \medmuskip=2.5mu plus 1mu minus 1mu%
%       \thickmuskip=4mu plus 1.5mu minus 1mu}
% \thinmuskip=2mu 
% \medmuskip=2mu  minus 1mu
% \thickmuskip=2mu  minus 1mu

% % \def\boldmath{%
% %    \@warning{there is no bold Symbol font}%
% %    \global\let\boldmath=\relax
% % }


%\DeclareMathSymbol{/}   {\mathord}{cmletters}{'075}
%\DeclareMathSymbol{=}   {\mathrel}{cmoperators}{'075}
%\DeclareMathSymbol{+}   {\mathbin}{cmoperators}{'053}
%\DeclareMathSymbol{(}   {\mathopen}{cmoperators}{'050}
%\DeclareMathSymbol{)}   {\mathclose}{cmoperators}{'051}

%\DeclareMathSymbol{>}   {\mathrel}{ptmsymbols}{62}
%\DeclareMathSymbol{<}   {\mathrel}{ptmsymbols}{60}
\DeclareMathSymbol{-}   {\mathbin}{ptmsymbols}{45}
\DeclareMathSymbol{+}   {\mathbin}{ptmsymbols}{43}
%\DeclareMathSymbol{/}   {\mathord}{ptmsymbols}{164}

\DeclareMathSymbol{\alpha}   {\mathord}{cmletters}{'013}
\DeclareMathSymbol{\beta}    {\mathord}{cmletters}{'014}
\DeclareMathSymbol{\gamma}   {\mathord}{cmletters}{'015}
\DeclareMathSymbol{\delta}   {\mathord}{cmletters}{'016}
\DeclareMathSymbol{\epsilon} {\mathord}{cmletters}{'017}
\DeclareMathSymbol{\zeta}    {\mathord}{cmletters}{'020}
\DeclareMathSymbol{\eta}     {\mathord}{cmletters}{'021}
\DeclareMathSymbol{\theta}   {\mathord}{cmletters}{'022}
\DeclareMathSymbol{\iota}    {\mathord}{cmletters}{'023}
\DeclareMathSymbol{\kappa}   {\mathord}{cmletters}{'024}
\DeclareMathSymbol{\lambda}  {\mathord}{cmletters}{'025}
\DeclareMathSymbol{\mu}      {\mathord}{cmletters}{'026}
\DeclareMathSymbol{\nu}      {\mathord}{cmletters}{'027}
\DeclareMathSymbol{\xi}      {\mathord}{cmletters}{'030}
%%% \DeclareMathSymbol{o}        {\mathord}{cmletters}{'157}
\DeclareMathSymbol{\pi}      {\mathord}{cmletters}{'031}
\DeclareMathSymbol{\rho}     {\mathord}{cmletters}{'032}
\DeclareMathSymbol{\sigma}   {\mathord}{cmletters}{'033}
\DeclareMathSymbol{\tau}     {\mathord}{cmletters}{'034}
\DeclareMathSymbol{\upsilon} {\mathord}{cmletters}{'035}
\DeclareMathSymbol{\phi}     {\mathord}{cmletters}{'036}
\DeclareMathSymbol{\chi}     {\mathord}{cmletters}{'037}
\DeclareMathSymbol{\psi}     {\mathord}{cmletters}{'040}
\DeclareMathSymbol{\omega}   {\mathord}{cmletters}{'041}



\DeclareMathSymbol{\varepsilon}   {\mathord}{cmletters}{'042}
\DeclareMathSymbol{\vartheta}     {\mathord}{cmletters}{'043}
\DeclareMathSymbol{\varomega}     {\mathord}{cmletters}{'044}
\DeclareMathSymbol{\varrho}       {\mathord}{cmletters}{'045}
\DeclareMathSymbol{\varsigma}     {\mathord}{cmletters}{'046}
\DeclareMathSymbol{\varphi}       {\mathord}{cmletters}{'047}

\DeclareMathSymbol{\partial}   {\mathord}{cmletters}{'100}
% Partial - from russian fonts
% \DeclareMathSymbol{\partial}   {\mathord}{rusletters}{"C4} % correct for WIN
                                                        % enc + reencoding

\DeclareMathSymbol{\ell}       {\mathord}{cmletters}{'140}
\DeclareMathSymbol{\ell}       {\mathord}{cmletters}{'140}
\def\hbar{{\raise-0.15truept\hbox{$\mkern-0.5mu\barbar$}\mkern-8.5muh}}


\DeclareMathSymbol\Gamma    {\mathord}{cmoperators}{"00}
\DeclareMathSymbol\Delta    {\mathord}{cmoperators}{"01}
\DeclareMathSymbol\Theta    {\mathord}{cmoperators}{"02}
\DeclareMathSymbol\Lambda   {\mathord}{cmoperators}{"03}
\DeclareMathSymbol\Xi       {\mathord}{cmoperators}{"04}
\DeclareMathSymbol\Pi       {\mathord}{cmoperators}{"05}
\DeclareMathSymbol\Sigma    {\mathord}{cmoperators}{"06}
\DeclareMathSymbol\Upsilon  {\mathord}{cmoperators}{"07}
\DeclareMathSymbol\Phi      {\mathord}{cmoperators}{"08}
\DeclareMathSymbol\Psi      {\mathord}{cmoperators}{"09}
\DeclareMathSymbol\Omega    {\mathord}{cmoperators}{"0A}




\DeclareMathSymbol\varGamma    {\mathord}{cmletters}{"00}
\DeclareMathSymbol\varDelta    {\mathord}{cmletters}{"01}
\DeclareMathSymbol\varTheta    {\mathord}{cmletters}{"02}
\DeclareMathSymbol\varLambda   {\mathord}{cmletters}{"03}
\DeclareMathSymbol\varXi       {\mathord}{cmletters}{"04}
\DeclareMathSymbol\varPi       {\mathord}{cmletters}{"05}
\DeclareMathSymbol\varSigma    {\mathord}{cmletters}{"06}
\DeclareMathSymbol\varUpsilon  {\mathord}{cmletters}{"07}
\DeclareMathSymbol\varPhi      {\mathord}{cmletters}{"08}
\DeclareMathSymbol\varPsi      {\mathord}{cmletters}{"09}
\DeclareMathSymbol\varOmega    {\mathord}{cmletters}{"0A}

\DeclareMathAccent{\acute}  {\mathalpha}{cmoperators}{'023}
\DeclareMathAccent{\bar}    {\mathalpha}{cmoperators}{'026}
\DeclareMathAccent{\breve}  {\mathalpha}{cmoperators}{'025}
\DeclareMathAccent{\check}  {\mathalpha}{cmoperators}{'024}
\DeclareMathAccent{\ddot}   {\mathalpha}{cmitoperators}{'177}
\DeclareMathAccent{\dot}    {\mathalpha}{cmitoperators}{'137}
\DeclareMathAccent{\grave}  {\mathalpha}{cmoperators}{'022}
\DeclareMathAccent{\hat}    {\mathalpha}{cmoperators}{'136}
\DeclareMathAccent{\tild}   {\mathalpha}{cmoperators}{'176}
\DeclareMathAccent{\vec}    {\mathord}  {cmletters}  {"7E}

\DeclareMathSymbol{\barbar}    {\mathalpha}{cmoperators}{'026}
}

\endinput


==> OLD/natbibsty <==
%%
%% This is file `natbib.sty',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% natbib.dtx  (with options: `package,all')
%% =============================================
%% IMPORTANT NOTICE:
%% 
%% This program can be redistributed and/or modified under the terms
%% of the LaTeX Project Public License Distributed from CTAN
%% archives in directory macros/latex/base/lppl.txt; either
%% version 1 of the License, or any later version.
%% 
%% This is a generated file.
%% It may not be distributed without the original source file natbib.dtx.
%% 
%% Full documentation can be obtained by LaTeXing that original file.
%% Only a few abbreviated comments remain here to describe the usage.
%% =============================================
%% Copyright 1993-2006 Patrick W Daly
%% Max-Planck-Institut f\"ur Sonnensystemforschung
%% Max-Planck-Str. 2
%% D-37191 Katlenburg-Lindau
%% Germany
%% E-mail: daly@linmpi.mpg.de
\NeedsTeXFormat{LaTeX2e}[1995/06/01]
\ProvidesPackage{natbib}
        [2006/03/22 7.3 (PWD)]
 % This package reimplements the LaTeX \cite command to be used for various
 % citation styles, both author-year and numerical. It accepts BibTeX
 % output intended for many other packages, and therefore acts as a
 % general, all-purpose citation-style interface.
 %
 % With standard numerical .bst files, only numerical citations are
 % possible. With an author-year .bst file, both numerical and
 % author-year citations are possible.
 %
 % If author-year citations are selected, \bibitem must have one of the
 %   following forms:
 %   \bibitem[Jones et al.(1990)]{key}...
 %   \bibitem[Jones et al.(1990)Jones, Baker, and Williams]{key}...
 %   \bibitem[Jones et al., 1990]{key}...
 %   \bibitem[\protect\citeauthoryear{Jones, Baker, and Williams}{Jones
 %       et al.}{1990}]{key}...
 %   \bibitem[\protect\citeauthoryear{Jones et al.}{1990}]{key}...
 %   \bibitem[\protect\astroncite{Jones et al.}{1990}]{key}...
 %   \bibitem[\protect\citename{Jones et al., }1990]{key}...
 %   \harvarditem[Jones et al.]{Jones, Baker, and Williams}{1990}{key}...
 %
 % This is either to be made up manually, or to be generated by an
 % appropriate .bst file with BibTeX.
 %                            Author-year mode     ||   Numerical mode
 % Then, \citet{key}  ==>>  Jones et al. (1990)    ||   Jones et al. [21]
 %       \citep{key}  ==>> (Jones et al., 1990)    ||   [21]
 % Multiple citations as normal:
 % \citep{key1,key2}  ==>> (Jones et al., 1990; Smith, 1989) || [21,24]
 %                           or  (Jones et al., 1990, 1991)  || [21,24]
 %                           or  (Jones et al., 1990a,b)     || [21,24]
 % \cite{key} is the equivalent of \citet{key} in author-year mode
 %                         and  of \citep{key} in numerical mode
 % Full author lists may be forced with \citet* or \citep*, e.g.
 %       \citep*{key}      ==>> (Jones, Baker, and Williams, 1990)
 % Optional notes as:
 %   \citep[chap. 2]{key}    ==>> (Jones et al., 1990, chap. 2)
 %   \citep[e.g.,][]{key}    ==>> (e.g., Jones et al., 1990)
 %   \citep[see][pg. 34]{key}==>> (see Jones et al., 1990, pg. 34)
 %  (Note: in standard LaTeX, only one note is allowed, after the ref.
 %   Here, one note is like the standard, two make pre- and post-notes.)
 %   \citealt{key}          ==>> Jones et al. 1990
 %   \citealt*{key}         ==>> Jones, Baker, and Williams 1990
 %   \citealp{key}          ==>> Jones et al., 1990
 %   \citealp*{key}         ==>> Jones, Baker, and Williams, 1990
 % Additional citation possibilities (both author-year and numerical modes)
 %   \citeauthor{key}       ==>> Jones et al.
 %   \citeauthor*{key}      ==>> Jones, Baker, and Williams
 %   \citeyear{key}         ==>> 1990
 %   \citeyearpar{key}      ==>> (1990)
 %   \citetext{priv. comm.} ==>> (priv. comm.)
 % Note: full author lists depends on whether the bib style supports them;
 %       if not, the abbreviated list is printed even when full requested.
 %
 % For names like della Robbia at the start of a sentence, use
 %   \Citet{dRob98}         ==>> Della Robbia (1998)
 %   \Citep{dRob98}         ==>> (Della Robbia, 1998)
 %   \Citeauthor{dRob98}    ==>> Della Robbia
 %
 %
 % Citation aliasing is achieved with
 %   \defcitealias{key}{text}
 %   \citetalias{key}  ==>> text
 %   \citepalias{key}  ==>> (text)
 %
 % Defining the citation style of a given bib style:
 % Use \bibpunct (in the preamble only) with 6 mandatory arguments:
 %    1. opening bracket for citation
 %    2. closing bracket
 %    3. citation separator (for multiple citations in one \cite)
 %    4. the letter n for numerical styles, s for superscripts
 %        else anything for author-year
 %    5. punctuation between authors and date
 %    6. punctuation between years (or numbers) when common authors missing
 % One optional argument is the character coming before post-notes. It
 %   appears in square braces before all other arguments. May be left off.
 % Example (and default) \bibpunct[, ]{(}{)}{;}{a}{,}{,}
 %
 % To make this automatic for a given bib style, named newbib, say, make
 % a local configuration file, natbib.cfg, with the definition
 %   \newcommand{\bibstyle@newbib}{\bibpunct...}
 % Then the \bibliographystyle{newbib} will cause \bibstyle@newbib to
 % be called on THE NEXT LATEX RUN (via the aux file).
 %
 % Such preprogrammed definitions may be invoked in the text (preamble only)
 %  by calling \citestyle{newbib}. This is only useful if the style specified
 %  differs from that in \bibliographystyle.
 %
 % With \citeindextrue and \citeindexfalse, one can control whether the
 % \cite commands make an automatic entry of the citation in the .idx
 % indexing file. For this, \makeindex must also be given in the preamble.
 %
 % Package Options: (for selecting punctuation)
 %   round  -  round parentheses are used (default)
 %   square -  square brackets are used   [option]
 %   curly  -  curly braces are used      {option}
 %   angle  -  angle brackets are used    <option>
 %   colon  -  multiple citations separated by colon (default)
 %   comma  -  separated by comma
 %   authoryear - selects author-year citations (default)
 %   numbers-  selects numerical citations
 %   super  -  numerical citations as superscripts
 %   sort   -  sorts multiple citations according to order in ref. list
 %   sort&compress   -  like sort, but also compresses numerical citations
 %   compress - compresses without sorting
 %   longnamesfirst  -  makes first citation full author list
 %   sectionbib - puts bibliography in a \section* instead of \chapter*
 % Punctuation so selected dominates over any predefined ones.
 % Package options are called as, e.g.
 %        \usepackage[square,comma]{natbib}
 % LaTeX the source file natbib.dtx to obtain more details
 % or the file natnotes.tex for a brief reference sheet.
 %-----------------------------------------------------------
\@ifclassloaded{agu2001}{\PackageError{natbib}
  {The agu2001 class already includes natbib coding,\MessageBreak
   so you should not add it explicitly}
  {Type <Return> for now, but then later remove\MessageBreak
   the command \protect\usepackage{natbib} from the document}
  \endinput}{}
\@ifclassloaded{aguplus}{\PackageError{natbib}
  {The aguplus class already includes natbib coding,\MessageBreak
   so you should not add it explicitly}
  {Type <Return> for now, but then later remove\MessageBreak
   the command \protect\usepackage{natbib} from the document}
  \endinput}{}
\@ifclassloaded{nlinproc}{\PackageError{natbib}
  {The nlinproc class already includes natbib coding,\MessageBreak
   so you should not add it explicitly}
  {Type <Return> for now, but then later remove\MessageBreak
   the command \protect\usepackage{natbib} from the document}
  \endinput}{}
\@ifclassloaded{egs}{\PackageError{natbib}
  {The egs class already includes natbib coding,\MessageBreak
   so you should not add it explicitly}
  {Type <Return> for now, but then later remove\MessageBreak
   the command \protect\usepackage{natbib} from the document}
  \endinput}{}
\@ifclassloaded{egu}{\PackageError{natbib}
  {The egu class already includes natbib coding,\MessageBreak
   so you should not add it explicitly}
  {Type <Return> for now, but then later remove\MessageBreak
   the command \protect\usepackage{natbib} from the document}
  \endinput}{}
 % Define citation punctuation for some author-year styles
 % One may add and delete at this point
 % Or put additions into local configuration file natbib.cfg
\newcommand\bibstyle@chicago{\bibpunct{(}{)}{;}{a}{,}{,}}
\newcommand\bibstyle@named{\bibpunct{[}{]}{;}{a}{,}{,}}
\newcommand\bibstyle@agu{\bibpunct{[}{]}{;}{a}{,}{,~}}%Amer. Geophys. Union
\newcommand\bibstyle@egs{\bibpunct{(}{)}{;}{a}{,}{,}}%Eur. Geophys. Soc.
\newcommand\bibstyle@agsm{\bibpunct{(}{)}{,}{a}{}{,}\gdef\harvardand{\&}}
\newcommand\bibstyle@kluwer{\bibpunct{(}{)}{,}{a}{}{,}\gdef\harvardand{\&}}
\newcommand\bibstyle@dcu{\bibpunct{(}{)}{;}{a}{;}{,}\gdef\harvardand{and}}
\newcommand\bibstyle@aa{\bibpunct{(}{)}{;}{a}{}{,}} %Astronomy & Astrophysics
\newcommand\bibstyle@pass{\bibpunct{(}{)}{;}{a}{,}{,}}%Planet. & Space Sci
\newcommand\bibstyle@anngeo{\bibpunct{(}{)}{;}{a}{,}{,}}%Annales Geophysicae
\newcommand\bibstyle@nlinproc{\bibpunct{(}{)}{;}{a}{,}{,}}%Nonlin.Proc.Geophys.
 % Define citation punctuation for some numerical styles
\newcommand\bibstyle@cospar{\bibpunct{/}{/}{,}{n}{}{}%
     \gdef\NAT@biblabelnum##1{##1.}}
\newcommand\bibstyle@esa{\bibpunct{(Ref.~}{)}{,}{n}{}{}%
     \gdef\NAT@biblabelnum##1{##1.\hspace{1em}}}
\newcommand\bibstyle@nature{\bibpunct{}{}{,}{s}{}{\textsuperscript{,}}%
     \gdef\NAT@biblabelnum##1{##1.}}
 % The standard LaTeX styles
\newcommand\bibstyle@plain{\bibpunct{[}{]}{,}{n}{}{,}}
\let\bibstyle@alpha=\bibstyle@plain
\let\bibstyle@abbrv=\bibstyle@plain
\let\bibstyle@unsrt=\bibstyle@plain
 % The author-year modifications of the standard styles
\newcommand\bibstyle@plainnat{\bibpunct{[}{]}{,}{a}{,}{,}}
\let\bibstyle@abbrvnat=\bibstyle@plainnat
\let\bibstyle@unsrtnat=\bibstyle@plainnat
\newif\ifNAT@numbers \NAT@numbersfalse
\newif\ifNAT@super \NAT@superfalse
\DeclareOption{numbers}{\NAT@numberstrue
   \ExecuteOptions{square,comma,nobibstyle}}
\DeclareOption{super}{\NAT@supertrue\NAT@numberstrue
   \renewcommand\NAT@open{}\renewcommand\NAT@close{}
   \ExecuteOptions{nobibstyle}}
\DeclareOption{authoryear}{\NAT@numbersfalse
   \ExecuteOptions{round,colon,bibstyle}}
\DeclareOption{round}{%
      \renewcommand\NAT@open{(} \renewcommand\NAT@close{)}
   \ExecuteOptions{nobibstyle}}
\DeclareOption{square}{%
      \renewcommand\NAT@open{[} \renewcommand\NAT@close{]}
   \ExecuteOptions{nobibstyle}}
\DeclareOption{angle}{%
      \renewcommand\NAT@open{$<$} \renewcommand\NAT@close{$>$}
   \ExecuteOptions{nobibstyle}}
\DeclareOption{curly}{%
      \renewcommand\NAT@open{\{} \renewcommand\NAT@close{\}}
   \ExecuteOptions{nobibstyle}}
\DeclareOption{comma}{\renewcommand\NAT@sep{,}
   \ExecuteOptions{nobibstyle}}
\DeclareOption{colon}{\renewcommand\NAT@sep{;}
   \ExecuteOptions{nobibstyle}}
\DeclareOption{nobibstyle}{\let\bibstyle=\@gobble}
\DeclareOption{bibstyle}{\let\bibstyle=\@citestyle}
\newif\ifNAT@openbib \NAT@openbibfalse
\DeclareOption{openbib}{\NAT@openbibtrue}
\DeclareOption{sectionbib}{\def\NAT@sectionbib{on}}
\def\NAT@sort{0}
\def\NAT@cmprs{0}
\DeclareOption{sort}{\def\NAT@sort{1}}
\DeclareOption{compress}{\def\NAT@cmprs{1}}
\DeclareOption{sort&compress}{\def\NAT@sort{1}\def\NAT@cmprs{1}}
\@ifpackageloaded{cite}{\PackageWarningNoLine{natbib}
  {The `cite' package should not be used\MessageBreak
   with natbib. Use option `sort' instead}\ExecuteOptions{sort}}{}
\@ifpackageloaded{citeref}{\PackageError{natbib}
  {The `citeref' package must be loaded after natbib}%
  {Move \protect\usepackage{citeref} to after \string\usepackage{natbib}}}{}
\newif\ifNAT@longnames\NAT@longnamesfalse
\DeclareOption{longnamesfirst}{\NAT@longnamestrue}
\DeclareOption{nonamebreak}{\def\NAT@nmfmt#1{\mbox{\NAT@up#1}}}
\def\NAT@nmfmt#1{{\NAT@up#1}}
\renewcommand\bibstyle[1]{\@ifundefined{bibstyle@#1}{\relax}
     {\csname bibstyle@#1\endcsname}}
\AtBeginDocument{\global\let\bibstyle=\@gobble}
\let\@citestyle\bibstyle
\newcommand\citestyle[1]{\@citestyle{#1}\let\bibstyle\@gobble}
\@onlypreamble{\citestyle}\@onlypreamble{\@citestyle}
\newcommand\bibpunct[7][, ]%
  {\gdef\NAT@open{#2}\gdef\NAT@close{#3}\gdef
   \NAT@sep{#4}\global\NAT@numbersfalse\ifx #5n\global\NAT@numberstrue
   \else
   \ifx #5s\global\NAT@numberstrue\global\NAT@supertrue
   \fi\fi
   \gdef\NAT@aysep{#6}\gdef\NAT@yrsep{#7}%
   \gdef\NAT@cmt{#1}%
   \global\let\bibstyle\@gobble
  }
\@onlypreamble{\bibpunct}
\newcommand\NAT@open{(} \newcommand\NAT@close{)}
\newcommand\NAT@sep{;}
\ProcessOptions
\newcommand\NAT@aysep{,} \newcommand\NAT@yrsep{,}
\newcommand\NAT@cmt{, }
\newcommand\NAT@cite%
    [3]{\ifNAT@swa\NAT@@open\if*#2*\else#2\ \fi
        #1\if*#3*\else\NAT@cmt#3\fi\NAT@@close\else#1\fi\endgroup}
\newcommand\NAT@citenum%
    [3]{\ifNAT@swa\NAT@@open\if*#2*\else#2\ \fi
        #1\if*#3*\else\NAT@cmt#3\fi\NAT@@close\else#1\fi\endgroup}
\newcommand\NAT@citesuper[3]{\ifNAT@swa
\unskip\kern\p@\textsuperscript{\NAT@@open#1\NAT@@close}%
   \if*#3*\else\ (#3)\fi\else #1\fi\endgroup}
\providecommand
  \textsuperscript[1]{\mbox{$^{\mbox{\scriptsize#1}}$}}
\providecommand\@firstofone[1]{#1}
\newcommand\NAT@citexnum{}
\def\NAT@citexnum[#1][#2]#3{%
 \NAT@sort@cites{#3}%
 \let\@citea\@empty
  \@cite{\def\NAT@num{-1}\let\NAT@last@yr\relax\let\NAT@nm\@empty
    \@for\@citeb:=\NAT@cite@list\do
    {\edef\@citeb{\expandafter\@firstofone\@citeb}%
     \if@filesw\immediate\write\@auxout{\string\citation{\@citeb}}%
       \@ifundefined{@cprwrite}{}{\expandafter\@cprwrite\@citeb=}\fi
     \@ifundefined{b@\@citeb\@extra@b@citeb}{%
       {\reset@font\bfseries?}
        \NAT@citeundefined\PackageWarning{natbib}%
       {Citation `\@citeb' on page \thepage \space undefined}}%
     {\let\NAT@last@num\NAT@num\let\NAT@last@nm\NAT@nm
      \NAT@parse{\@citeb}%
      \ifNAT@longnames\@ifundefined{bv@\@citeb\@extra@b@citeb}{%
        \let\NAT@name=\NAT@all@names
        \global\@namedef{bv@\@citeb\@extra@b@citeb}{}}{}%
      \fi
      \ifNAT@full\let\NAT@nm\NAT@all@names\else
        \let\NAT@nm\NAT@name\fi
      \ifNAT@swa
       \ifnum\NAT@ctype>1\relax\@citea
        \hyper@natlinkstart{\@citeb\@extra@b@citeb}%
            \ifnum\NAT@ctype=2\relax\NAT@test{\NAT@ctype}%
            \else\NAT@alias
            \fi\hyper@natlinkend\else
       \ifnum\NAT@cmprs>0
         \begingroup\catcode`\_=8
            \ifcat _\ifnum\z@<0\NAT@num _\else A\fi
              \global\let\NAT@nm=\NAT@num \else \gdef\NAT@nm{-2}\fi
            \ifcat _\ifnum\z@<0\NAT@last@num _\else A\fi
              \global\@tempcnta=\NAT@last@num \global\advance\@tempcnta by\@ne
              \else \global\@tempcnta\m@ne\fi
         \endgroup
         \ifnum\NAT@nm=\@tempcnta
           \ifx\NAT@last@yr\relax
             \edef\NAT@last@yr{\@citea \mbox{%
              \noexpand\hyper@natlinkstart{\@citeb\@extra@b@citeb}{%
               \noexpand\citenumfont{\NAT@num}}\hyper@natlinkend}}%
           \else
             \edef\NAT@last@yr{--\penalty\@m\mbox{%
              \noexpand\hyper@natlinkstart{\@citeb\@extra@b@citeb}{%
             \noexpand\citenumfont{\NAT@num}}\hyper@natlinkend}}%
           \fi
         \else
           \NAT@last@yr \@citea \mbox{\hyper@natlinkstart{\@citeb\@extra@b@citeb}%
              {\citenumfont{\NAT@num}}\hyper@natlinkend}%
           \let\NAT@last@yr\relax
         \fi
       \else
         \@citea \mbox{\hyper@natlinkstart{\@citeb\@extra@b@citeb}%
           {\citenumfont{\NAT@num}}\hyper@natlinkend}%
       \fi
       \fi
       \def\@citea{\NAT@sep\penalty\@m\NAT@space}%
      \else
        \ifcase\NAT@ctype\relax
          \ifx\NAT@last@nm\NAT@nm \NAT@yrsep\penalty\@m\NAT@space\else
          \@citea \NAT@test{1}\ \NAT@@open
          \if*#1*\else#1\ \fi\fi \NAT@mbox{%
          \hyper@natlinkstart{\@citeb\@extra@b@citeb}%
          {\citenumfont{\NAT@num}}\hyper@natlinkend}%
          \def\@citea{\NAT@@close\NAT@sep\penalty\@m\ }%
        \or\@citea
          \hyper@natlinkstart{\@citeb\@extra@b@citeb}%
           \NAT@test{\NAT@ctype}\hyper@natlinkend
          \def\@citea{\NAT@sep\penalty\@m\ }%
        \or\@citea
          \hyper@natlinkstart{\@citeb\@extra@b@citeb}%
           \NAT@test{\NAT@ctype}\hyper@natlinkend
          \def\@citea{\NAT@sep\penalty\@m\ }%
        \or\@citea
          \hyper@natlinkstart{\@citeb\@extra@b@citeb}%
           \NAT@alias\hyper@natlinkend
          \def\@citea{\NAT@sep\penalty\@m\ }%
        \fi
      \fi
      }}%
      \ifnum\NAT@cmprs>0\relax\NAT@last@yr\fi
      \ifNAT@swa\else\ifnum\NAT@ctype=0\if*#2*\else
      \NAT@cmt#2\fi \NAT@@close\fi\fi}{#1}{#2}}
\newcommand\NAT@test[1]{\ifnum#1=1 \ifx\NAT@nm\NAT@noname
  {\reset@font\bfseries(author?)}\PackageWarning{natbib}
  {Author undefined for citation`\@citeb'
   \MessageBreak
   on page \thepage}\else \NAT@nm \fi
  \else \if\relax\NAT@date\relax
  {\reset@font\bfseries(year?)}\PackageWarning{natbib}
  {Year undefined for citation`\@citeb'
   \MessageBreak
   on page \thepage}\else \NAT@date \fi \fi}
\let\citenumfont=\relax
\newcommand\NAT@citex{}
\def\NAT@citex%
  [#1][#2]#3{%
  \NAT@sort@cites{#3}%
  \let\@citea\@empty
  \@cite{\let\NAT@nm\@empty\let\NAT@year\@empty
    \@for\@citeb:=\NAT@cite@list\do
    {\edef\@citeb{\expandafter\@firstofone\@citeb}%
     \if@filesw\immediate\write\@auxout{\string\citation{\@citeb}}%
       \@ifundefined{@cprwrite}{}{\expandafter\@cprwrite\@citeb=}\fi
     \@ifundefined{b@\@citeb\@extra@b@citeb}{\@citea%
       {\reset@font\bfseries ?}\NAT@citeundefined
                 \PackageWarning{natbib}%
       {Citation `\@citeb' on page \thepage \space undefined}\def\NAT@date{}}%
     {\let\NAT@last@nm=\NAT@nm\let\NAT@last@yr=\NAT@year
     \NAT@parse{\@citeb}%
      \ifNAT@longnames\@ifundefined{bv@\@citeb\@extra@b@citeb}{%
        \let\NAT@name=\NAT@all@names
        \global\@namedef{bv@\@citeb\@extra@b@citeb}{}}{}%
      \fi
     \ifNAT@full\let\NAT@nm\NAT@all@names\else
       \let\NAT@nm\NAT@name\fi
     \ifNAT@swa\ifcase\NAT@ctype
       \if\relax\NAT@date\relax
         \@citea\hyper@natlinkstart{\@citeb\@extra@b@citeb}%
         \NAT@nmfmt{\NAT@nm}\NAT@date\hyper@natlinkend
       \else
         \ifx\NAT@last@nm\NAT@nm\NAT@yrsep
            \ifx\NAT@last@yr\NAT@year
              \def\NAT@temp{{?}}%
              \ifx\NAT@temp\NAT@exlab\PackageWarningNoLine{natbib}%
               {Multiple citation on page \thepage: same authors and
               year\MessageBreak without distinguishing extra
               letter,\MessageBreak appears as question mark}\fi
              \hyper@natlinkstart{\@citeb\@extra@b@citeb}\NAT@exlab
              \hyper@natlinkend
            \else\unskip\
              \hyper@natlinkstart{\@citeb\@extra@b@citeb}\NAT@date
              \hyper@natlinkend
            \fi
         \else\@citea\hyper@natlinkstart{\@citeb\@extra@b@citeb}%
           \NAT@nmfmt{\NAT@nm}%
           \hyper@natlinkbreak{\NAT@aysep\ }{\@citeb\@extra@b@citeb}%
           \NAT@date\hyper@natlinkend
         \fi
       \fi
     \or\@citea\hyper@natlinkstart{\@citeb\@extra@b@citeb}%
         \NAT@nmfmt{\NAT@nm}\hyper@natlinkend
     \or\@citea\hyper@natlinkstart{\@citeb\@extra@b@citeb}%
         \NAT@date\hyper@natlinkend
     \or\@citea\hyper@natlinkstart{\@citeb\@extra@b@citeb}%
         \NAT@alias\hyper@natlinkend
     \fi \def\@citea{\NAT@sep\ }%
     \else\ifcase\NAT@ctype
        \if\relax\NAT@date\relax
          \@citea\hyper@natlinkstart{\@citeb\@extra@b@citeb}%
          \NAT@nmfmt{\NAT@nm}\hyper@natlinkend
        \else
         \ifx\NAT@last@nm\NAT@nm\NAT@yrsep
            \ifx\NAT@last@yr\NAT@year
              \def\NAT@temp{{?}}%
              \ifx\NAT@temp\NAT@exlab\PackageWarningNoLine{natbib}%
               {Multiple citation on page \thepage: same authors and
               year\MessageBreak without distinguishing extra
               letter,\MessageBreak appears as question mark}\fi
              \hyper@natlinkstart{\@citeb\@extra@b@citeb}\NAT@exlab
              \hyper@natlinkend
            \else\unskip\
              \hyper@natlinkstart{\@citeb\@extra@b@citeb}\NAT@date
              \hyper@natlinkend
            \fi
         \else\@citea\hyper@natlinkstart{\@citeb\@extra@b@citeb}%
           \NAT@nmfmt{\NAT@nm}%
           \hyper@natlinkbreak{\ \NAT@@open\if*#1*\else#1\ \fi}%
              {\@citeb\@extra@b@citeb}%
           \NAT@date\hyper@natlinkend\fi
        \fi
       \or\@citea\hyper@natlinkstart{\@citeb\@extra@b@citeb}%
         \NAT@nmfmt{\NAT@nm}\hyper@natlinkend
       \or\@citea\hyper@natlinkstart{\@citeb\@extra@b@citeb}%
         \NAT@date\hyper@natlinkend
       \or\@citea\hyper@natlinkstart{\@citeb\@extra@b@citeb}%
         \NAT@alias\hyper@natlinkend
       \fi \if\relax\NAT@date\relax\def\@citea{\NAT@sep\ }%
           \else\def\@citea{\NAT@@close\NAT@sep\ }\fi
     \fi
     }}\ifNAT@swa\else\if*#2*\else\NAT@cmt#2\fi
     \if\relax\NAT@date\relax\else\NAT@@close\fi\fi}{#1}{#2}}
\newif\ifNAT@par \NAT@partrue
\newcommand\NAT@@open{\ifNAT@par\NAT@open\fi}
\newcommand\NAT@@close{\ifNAT@par\NAT@close\fi}
\newcommand\NAT@alias{\@ifundefined{al@\@citeb\@extra@b@citeb}{%
  {\reset@font\bfseries(alias?)}\PackageWarning{natbib}
  {Alias undefined for citation `\@citeb'
  \MessageBreak on page \thepage}}{\@nameuse{al@\@citeb\@extra@b@citeb}}}
\let\NAT@up\relax
\newcommand\NAT@Up[1]{{\let\protect\@unexpandable@protect\let~\relax
  \expandafter\NAT@deftemp#1}\expandafter\NAT@UP\NAT@temp}
\newcommand\NAT@deftemp[1]{\xdef\NAT@temp{#1}}
\newcommand\NAT@UP[1]{\let\@tempa\NAT@UP\ifcat a#1\MakeUppercase{#1}%
  \let\@tempa\relax\else#1\fi\@tempa}
\newcommand\shortcites[1]{%
  \@bsphack\@for\@citeb:=#1\do
  {\edef\@citeb{\expandafter\@firstofone\@citeb}%
   \global\@namedef{bv@\@citeb\@extra@b@citeb}{}}\@esphack}
\newcommand\NAT@biblabel[1]{\hfill}
\newcommand\NAT@biblabelnum[1]{\bibnumfmt{#1}}
\newcommand\bibnumfmt[1]{[#1]}
\def\@tempa#1{[#1]}
\ifx\@tempa\@biblabel\let\@biblabel\@empty\fi
\newcommand\NAT@bibsetnum[1]{\settowidth\labelwidth{\@biblabel{#1}}%
   \setlength{\leftmargin}{\labelwidth}\addtolength{\leftmargin}{\labelsep}%
   \setlength{\itemsep}{\bibsep}\setlength{\parsep}{\z@}%
   \ifNAT@openbib
     \addtolength{\leftmargin}{\bibindent}%
     \setlength{\itemindent}{-\bibindent}%
     \setlength{\listparindent}{\itemindent}%
     \setlength{\parsep}{0pt}%
   \fi
}
\newlength{\bibhang}
\setlength{\bibhang}{1em}
\newlength{\bibsep}
{\@listi \global\bibsep\itemsep \global\advance\bibsep by\parsep}

\newcommand\NAT@bibsetup%
   [1]{\setlength{\leftmargin}{\bibhang}\setlength{\itemindent}{-\leftmargin}%
       \setlength{\itemsep}{\bibsep}\setlength{\parsep}{\z@}}
\newcommand\NAT@set@cites{\ifNAT@numbers
  \ifNAT@super \let\@cite\NAT@citesuper
     \def\NAT@mbox##1{\unskip\nobreak\hspace{1\p@}\textsuperscript{##1}}%
     \let\citeyearpar=\citeyear
     \let\NAT@space\relax\else
     \let\NAT@mbox=\mbox
     \let\@cite\NAT@citenum \def\NAT@space{ }\fi
  \let\@citex\NAT@citexnum
  \ifx\@biblabel\@empty\let\@biblabel\NAT@biblabelnum\fi
  \let\@bibsetup\NAT@bibsetnum
  \def\natexlab##1{}%
 \else
  \let\@cite\NAT@cite
  \let\@citex\NAT@citex
  \let\@biblabel\NAT@biblabel
  \let\@bibsetup\NAT@bibsetup
  \def\natexlab##1{##1}%
 \fi}
\AtBeginDocument{\NAT@set@cites}
\AtBeginDocument{\ifx\SK@def\@undefined\else
\ifx\SK@cite\@empty\else
  \SK@def\@citex[#1][#2]#3{\SK@\SK@@ref{#3}\SK@@citex[#1][#2]{#3}}\fi
\ifx\SK@citeauthor\@undefined\def\HAR@checkdef{}\else
  \let\citeauthor\SK@citeauthor
  \let\citefullauthor\SK@citefullauthor
  \let\citeyear\SK@citeyear\fi
\fi}
\newif\ifNAT@full\NAT@fullfalse
\newif\ifNAT@swa
\DeclareRobustCommand\citet
   {\begingroup\NAT@swafalse\def\NAT@ctype{0}\NAT@partrue
     \@ifstar{\NAT@fulltrue\NAT@citetp}{\NAT@fullfalse\NAT@citetp}}
\newcommand\NAT@citetp{\@ifnextchar[{\NAT@@citetp}{\NAT@@citetp[]}}
\newcommand\NAT@@citetp{}
\def\NAT@@citetp[#1]{\@ifnextchar[{\@citex[#1]}{\@citex[][#1]}}
\DeclareRobustCommand\citep
   {\begingroup\NAT@swatrue\def\NAT@ctype{0}\NAT@partrue
         \@ifstar{\NAT@fulltrue\NAT@citetp}{\NAT@fullfalse\NAT@citetp}}
\DeclareRobustCommand\cite
    {\begingroup\def\NAT@ctype{0}\NAT@partrue\NAT@swatrue
      \@ifstar{\NAT@fulltrue\NAT@cites}{\NAT@fullfalse\NAT@cites}}
\newcommand\NAT@cites{\@ifnextchar [{\NAT@@citetp}{%
     \ifNAT@numbers\else
     \NAT@swafalse
     \fi
    \NAT@@citetp[]}}
\DeclareRobustCommand\citealt
   {\begingroup\NAT@swafalse\def\NAT@ctype{0}\NAT@parfalse
         \@ifstar{\NAT@fulltrue\NAT@citetp}{\NAT@fullfalse\NAT@citetp}}
\DeclareRobustCommand\citealp
   {\begingroup\NAT@swatrue\def\NAT@ctype{0}\NAT@parfalse
         \@ifstar{\NAT@fulltrue\NAT@citetp}{\NAT@fullfalse\NAT@citetp}}
\DeclareRobustCommand\citeauthor
   {\begingroup\NAT@swafalse\def\NAT@ctype{1}\NAT@parfalse
    \@ifstar{\NAT@fulltrue\NAT@citetp}{\NAT@fullfalse\NAT@citetp}}
\DeclareRobustCommand\Citet
   {\begingroup\NAT@swafalse\def\NAT@ctype{0}\NAT@partrue
     \let\NAT@up\NAT@Up
     \@ifstar{\NAT@fulltrue\NAT@citetp}{\NAT@fullfalse\NAT@citetp}}
\DeclareRobustCommand\Citep
   {\begingroup\NAT@swatrue\def\NAT@ctype{0}\NAT@partrue
     \let\NAT@up\NAT@Up
         \@ifstar{\NAT@fulltrue\NAT@citetp}{\NAT@fullfalse\NAT@citetp}}
\DeclareRobustCommand\Citealt
   {\begingroup\NAT@swafalse\def\NAT@ctype{0}\NAT@parfalse
     \let\NAT@up\NAT@Up
         \@ifstar{\NAT@fulltrue\NAT@citetp}{\NAT@fullfalse\NAT@citetp}}
\DeclareRobustCommand\Citealp
   {\begingroup\NAT@swatrue\def\NAT@ctype{0}\NAT@parfalse
     \let\NAT@up\NAT@Up
         \@ifstar{\NAT@fulltrue\NAT@citetp}{\NAT@fullfalse\NAT@citetp}}
\DeclareRobustCommand\Citeauthor
   {\begingroup\NAT@swafalse\def\NAT@ctype{1}\NAT@parfalse
     \let\NAT@up\NAT@Up
    \@ifstar{\NAT@fulltrue\NAT@citetp}{\NAT@fullfalse\NAT@citetp}}
\DeclareRobustCommand\citeyear
   {\begingroup\NAT@swafalse\def\NAT@ctype{2}\NAT@parfalse\NAT@citetp}
\DeclareRobustCommand\citeyearpar
   {\begingroup\NAT@swatrue\def\NAT@ctype{2}\NAT@partrue\NAT@citetp}
\newcommand\citetext[1]{\NAT@open#1\NAT@close}
\DeclareRobustCommand\citefullauthor
   {\citeauthor*}
\newcommand\defcitealias[2]{%
   \@ifundefined{al@#1\@extra@b@citeb}{}
   {\PackageWarning{natbib}{Overwriting existing alias for citation #1}}
   \@namedef{al@#1\@extra@b@citeb}{#2}}
\DeclareRobustCommand\citetalias{\begingroup
   \NAT@swafalse\def\NAT@ctype{3}\NAT@parfalse\NAT@citetp}
\DeclareRobustCommand\citepalias{\begingroup
   \NAT@swatrue\def\NAT@ctype{3}\NAT@partrue\NAT@citetp}
\renewcommand\nocite[1]{\@bsphack
  \@for\@citeb:=#1\do{%
    \edef\@citeb{\expandafter\@firstofone\@citeb}%
    \if@filesw\immediate\write\@auxout{\string\citation{\@citeb}}\fi
    \if*\@citeb\else
    \@ifundefined{b@\@citeb\@extra@b@citeb}{%
       \NAT@citeundefined \PackageWarning{natbib}%
       {Citation `\@citeb' undefined}}{}\fi}%
  \@esphack}
\newcommand\NAT@parse[1]{{%
     \let\protect=\@unexpandable@protect\let~\relax
     \let\active@prefix=\@gobble
     \xdef\NAT@temp{\csname b@#1\@extra@b@citeb\endcsname}}%
     \expandafter\NAT@split\NAT@temp
     \expandafter\NAT@parse@date\NAT@date??????@@%
     \ifciteindex\NAT@index\fi
}
\newcommand\NAT@split[4]{%
  \gdef\NAT@num{#1}\gdef\NAT@name{#3}\gdef\NAT@date{#2}%
  \gdef\NAT@all@names{#4}%
  \ifx\NAT@noname\NAT@all@names \gdef\NAT@all@names{#3}\fi}
\newcommand\NAT@parse@date{}
\def\NAT@parse@date#1#2#3#4#5#6@@{%
  \ifnum\the\catcode`#1=11\def\NAT@year{}\def\NAT@exlab{#1}\else
  \ifnum\the\catcode`#2=11\def\NAT@year{#1}\def\NAT@exlab{#2}\else
  \ifnum\the\catcode`#3=11\def\NAT@year{#1#2}\def\NAT@exlab{#3}\else
  \ifnum\the\catcode`#4=11\def\NAT@year{#1#2#3}\def\NAT@exlab{#4}\else
    \def\NAT@year{#1#2#3#4}\def\NAT@exlab{{#5}}\fi\fi\fi\fi}
\newcommand\NAT@index{}
\let\NAT@makeindex=\makeindex
\renewcommand\makeindex{\NAT@makeindex
  \renewcommand\NAT@index{\@bsphack\begingroup
     \def~{\string~}\@wrindex{\NAT@idxtxt}}}
\newcommand\NAT@idxtxt{\NAT@name\ \NAT@open\NAT@date\NAT@close}
\@ifundefined{@indexfile}{}{\let\NAT@makeindex\relax\makeindex}
\newif\ifciteindex \citeindexfalse
\newcommand\citeindextype{default}
\newcommand\NAT@index@alt{{\let\protect=\noexpand\let~\relax
  \xdef\NAT@temp{\NAT@idxtxt}}\expandafter\NAT@exp\NAT@temp\@nil}
\newcommand\NAT@exp{}
\def\NAT@exp#1\@nil{\mbox{}\index[\citeindextype]{#1}}

\AtBeginDocument{%
\@ifpackageloaded{index}{\let\NAT@index=\NAT@index@alt}{}}
\newcommand\NAT@ifcmd{\futurelet\NAT@temp\NAT@ifxcmd}
\newcommand\NAT@ifxcmd{\ifx\NAT@temp\relax\else\expandafter\NAT@bare\fi}
\def\NAT@bare#1(#2)#3(@)#4\@nil#5{%
  \if @#2
  \expandafter\NAT@apalk#1, , \@nil{#5}\else
  \stepcounter{NAT@ctr}%
  \NAT@wrout{\arabic {NAT@ctr}}{#2}{#1}{#3}{#5}
\fi
}
\newcommand\NAT@wrout[5]{%
\if@filesw
      {\let\protect\noexpand\let~\relax
       \immediate
       \write\@auxout{\string\bibcite{#5}{{#1}{#2}{{#3}}{{#4}}}}}\fi
\ignorespaces}
\def\NAT@noname{{}}
\renewcommand\bibitem{%
  \@ifnextchar[{\@lbibitem}{%
    \global\NAT@stdbsttrue
    \stepcounter{NAT@ctr}\@lbibitem[\arabic{NAT@ctr}]}}
\def\@lbibitem[#1]#2{%
  \if\relax\@extra@b@citeb\relax\else
    \@ifundefined{br@#2\@extra@b@citeb}{}{%
     \@namedef{br@#2}{\@nameuse{br@#2\@extra@b@citeb}}}\fi
   \@ifundefined{b@#2\@extra@b@citeb}{\def\NAT@num{}}{\NAT@parse{#2}}%
   \item[\hfil\hyper@natanchorstart{#2\@extra@b@citeb}\@biblabel{\NAT@num}%
    \hyper@natanchorend]%
    \NAT@ifcmd#1(@)(@)\@nil{#2}}
\ifx\SK@lbibitem\@undefined\else
   \let\SK@lbibitem\@lbibitem
   \def\@lbibitem[#1]#2{%
     \SK@lbibitem[#1]{#2}\SK@\SK@@label{#2}\ignorespaces}\fi
\newif\ifNAT@stdbst \NAT@stdbstfalse

\AtEndDocument
  {\ifNAT@stdbst\if@filesw\immediate\write\@auxout{\string
   \global\string\NAT@numberstrue}\fi\fi
  }
\providecommand\bibcite{}
\renewcommand\bibcite[2]{\@ifundefined{b@#1\@extra@binfo}\relax
     {\NAT@citemultiple
      \PackageWarningNoLine{natbib}{Citation `#1' multiply defined}}%
  \global\@namedef{b@#1\@extra@binfo}{#2}}
\AtEndDocument{\NAT@swatrue\let\bibcite\NAT@testdef}
\newcommand\NAT@testdef[2]{%
  \def\NAT@temp{#2}\expandafter \ifx \csname b@#1\@extra@binfo\endcsname
    \NAT@temp \else \ifNAT@swa \NAT@swafalse
       \PackageWarningNoLine{natbib}{Citation(s) may have
          changed.\MessageBreak
          Rerun to get citations correct}\fi\fi}
\newcommand\NAT@apalk{}
\def\NAT@apalk#1, #2, #3\@nil#4{\if\relax#2\relax
  \global\NAT@stdbsttrue
  \NAT@wrout{#1}{}{}{}{#4}\else
  \stepcounter{NAT@ctr}%
  \NAT@wrout{\arabic {NAT@ctr}}{#2}{#1}{}{#4}\fi}
\newcommand\citeauthoryear{}
\def\citeauthoryear#1#2#3(@)(@)\@nil#4{\stepcounter{NAT@ctr}\if\relax#3\relax
   \NAT@wrout{\arabic {NAT@ctr}}{#2}{#1}{}{#4}\else
   \NAT@wrout{\arabic {NAT@ctr}}{#3}{#2}{#1}{#4}\fi}
\newcommand\citestarts{\NAT@open}
\newcommand\citeends{\NAT@close}
\newcommand\betweenauthors{and}
\newcommand\astroncite{}
\def\astroncite#1#2(@)(@)\@nil#3{\stepcounter{NAT@ctr}\NAT@wrout{\arabic
{NAT@ctr}}{#2}{#1}{}{#3}}
\newcommand\citename{}
\def\citename#1#2(@)(@)\@nil#3{\expandafter\NAT@apalk#1#2, \@nil{#3}}
\newcommand\harvarditem[4][]%
    {\if\relax#1\relax\bibitem[#2(#3)]{#4}\else
        \bibitem[#1(#3)#2]{#4}\fi }
\newcommand\harvardleft{\NAT@open}
\newcommand\harvardright{\NAT@close}
\newcommand\harvardyearleft{\NAT@open}
\newcommand\harvardyearright{\NAT@close}
\AtBeginDocument{\providecommand{\harvardand}{and}}
\newcommand\harvardurl[1]{\textbf{URL:} \textit{#1}}
\providecommand\bibsection{}
\@ifundefined{chapter}%
  {\renewcommand\bibsection{\section*{\refname
    \@mkboth{\MakeUppercase{\refname}}{\MakeUppercase{\refname}}}}}
  {\@ifundefined{NAT@sectionbib}%
    {\renewcommand\bibsection{\chapter*{\bibname
     \@mkboth{\MakeUppercase{\bibname}}{\MakeUppercase{\bibname}}}}}
    {\renewcommand\bibsection{\section*{\bibname
     \ifx\@mkboth\@gobbletwo\else\markright{\MakeUppercase{\bibname}}\fi}}}}
\@ifclassloaded{amsart}%
  {\renewcommand\bibsection{\section*{\refname}}}{}
\@ifclassloaded{amsbook}%
  {\renewcommand\bibsection{\chapter*{\bibname}}}{}
\@ifundefined{bib@heading}{}{\let\bibsection\bib@heading}
\newcounter{NAT@ctr}
\renewenvironment{thebibliography}[1]{%
 \bibsection\parindent \z@\bibpreamble\bibfont\list
   {\@biblabel{\arabic{NAT@ctr}}}{\@bibsetup{#1}%
    \setcounter{NAT@ctr}{0}}%
    \ifNAT@openbib
      \renewcommand\newblock{\par}
    \else
      \renewcommand\newblock{\hskip .11em \@plus.33em \@minus.07em}%
    \fi
    \sloppy\clubpenalty4000\widowpenalty4000
    \sfcode`\.=1000\relax
    \let\citeN\cite \let\shortcite\cite
    \let\citeasnoun\cite
 }{\def\@noitemerr{%
  \PackageWarning{natbib}
     {Empty `thebibliography' environment}}%
  \endlist\vskip-\lastskip}
\let\bibfont\relax
\let\bibpreamble\relax
\providecommand\reset@font{\relax}
\providecommand\bibname{Bibliography}
\providecommand\refname{References}
\newcommand\NAT@citeundefined{\gdef \NAT@undefined {%
    \PackageWarningNoLine{natbib}{There were undefined citations}}}
\let \NAT@undefined \relax
\newcommand\NAT@citemultiple{\gdef \NAT@multiple {%
    \PackageWarningNoLine{natbib}{There were multiply defined citations}}}
\let \NAT@multiple \relax
\AtEndDocument{\NAT@undefined\NAT@multiple}
\providecommand\@mkboth[2]{}
\providecommand\MakeUppercase{\uppercase}
\providecommand{\@extra@b@citeb}{}
\gdef\@extra@binfo{}
\providecommand\hyper@natanchorstart[1]{}
\providecommand\hyper@natanchorend{}
\providecommand\hyper@natlinkstart[1]{}
\providecommand\hyper@natlinkend{}
\providecommand\hyper@natlinkbreak[2]{#1}
\@ifundefined{bbl@redefine}{}{%
 \bbl@redefine\nocite#1{%
  \@safe@activestrue\org@nocite{#1}\@safe@activesfalse}%
\bbl@redefine\@lbibitem[#1]#2{%
  \@safe@activestrue\org@@lbibitem[#1]{#2}\@safe@activesfalse}%
}
\AtBeginDocument{\@ifundefined{bbl@redefine}{}{%
\bbl@redefine\@citex[#1][#2]#3{%
  \@safe@activestrue\org@@citex[#1][#2]{#3}\@safe@activesfalse}%
\bbl@redefine\NAT@testdef#1#2{%
  \@safe@activestrue\org@NAT@testdef{#1}{#2}\@safe@activesfalse}%
\@ifundefined{org@@lbibitem}{%
\bbl@redefine\@lbibitem[#1]#2{%
  \@safe@activestrue\org@@lbibitem[#1]{#2}\@safe@activesfalse}}{}%
}}
\ifnum\NAT@sort>0
\newcommand\NAT@sort@cites[1]{%
\@tempcntb\m@ne
\let\@celt\delimiter
\def\NAT@num@list{}%
\def\NAT@cite@list{}%
\def\NAT@nonsort@list{}%
\@for \@citeb:=#1\do{\NAT@make@cite@list}%
\edef\NAT@cite@list{\NAT@cite@list\NAT@nonsort@list}%
\edef\NAT@cite@list{\expandafter\NAT@xcom\NAT@cite@list @@}}
\begingroup \catcode`\_=8
\gdef\NAT@make@cite@list{%
     \edef\@citeb{\expandafter\@firstofone\@citeb}%
    \@ifundefined{b@\@citeb\@extra@b@citeb}{\def\NAT@num{A}}%
    {\NAT@parse{\@citeb}}%
      \ifcat _\ifnum\z@<0\NAT@num _\else A\fi
       \@tempcnta\NAT@num \relax
       \ifnum \@tempcnta>\@tempcntb
          \edef\NAT@num@list{\NAT@num@list \@celt{\NAT@num}}%
          \edef\NAT@cite@list{\NAT@cite@list\@citeb,}%
          \@tempcntb\@tempcnta
       \else
          \let\NAT@@cite@list=\NAT@cite@list \def\NAT@cite@list{}%
          \edef\NAT@num@list{\expandafter\NAT@num@celt \NAT@num@list \@gobble @}%
          {\let\@celt=\NAT@celt\NAT@num@list}%
       \fi
    \else
       \edef\NAT@nonsort@list{\NAT@nonsort@list\@citeb,}%
 \fi}
\endgroup
\def\NAT@celt#1{\ifnum #1<\@tempcnta
  \xdef\NAT@cite@list{\NAT@cite@list\expandafter\NAT@nextc\NAT@@cite@list @@}%
  \xdef\NAT@@cite@list{\expandafter\NAT@restc\NAT@@cite@list}%
 \else
  \xdef\NAT@cite@list{\NAT@cite@list\@citeb,\NAT@@cite@list}\let\@celt\@gobble%
 \fi}
\def\NAT@num@celt#1#2{\ifx \@celt #1%
     \ifnum #2<\@tempcnta
        \@celt{#2}%
        \expandafter\expandafter\expandafter\NAT@num@celt
     \else
        \@celt{\number\@tempcnta}\@celt{#2}%
  \fi\fi}
\def\NAT@nextc#1,#2@@{#1,}
\def\NAT@restc#1,#2{#2}
\def\NAT@xcom#1,@@{#1}
\else
 \newcommand\NAT@sort@cites[1]{\edef\NAT@cite@list{#1}}\fi
\InputIfFileExists{natbib.cfg}
       {\typeout{Local config file natbib.cfg used}}{}
%% 
%% <<<<< End of generated file <<<<<<
%%
%% End of file `natbib.sty'.

==> OLD/supernovabib <==
.@ARTICLE{2016ATel.9782....1T,
   author = {{Tartaglia}, L. and {Sand}, D. and {Valenti}, S.},
    title = "{The discovery of DLT15am/AT 2016ija}",
  journal = {The Astronomer's Telegram},
 keywords = {Supernovae, Transient},
     year = 2016,
    month = nov,
   volume = 9782,
   adsurl = {http://adsabs.harvard.edu/abs/2016ATel.9782....1T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015A&A...579A..40S,
   author = {{Smartt}, S.~J. and {Valenti}, S. and {Fraser}, M. and {Inserra}, C. and
	{Young}, D.~R. and {Sullivan}, M. and {Pastorello}, A. and {Benetti}, S. and 
	{Gal-Yam}, A. and {Knapic}, C. and {Molinaro}, M. and {Smareglia}, R. and 
	{Smith}, K.~W. and {Taubenberger}, S. and {Yaron}, O. and {Anderson}, J.~P. and 
	{Ashall}, C. and {Balland}, C. and {Baltay}, C. and {Barbarino}, C. and 
	{Bauer}, F.~E. and {Baumont}, S. and {Bersier}, D. and {Blagorodnova}, N. and 
	{Bongard}, S. and {Botticella}, M.~T. and {Bufano}, F. and {Bulla}, M. and 
	{Cappellaro}, E. and {Campbell}, H. and {Cellier-Holzem}, F. and 
	{Chen}, T.-W. and {Childress}, M.~J. and {Clocchiatti}, A. and 
	{Contreras}, C. and {Dall'Ora}, M. and {Danziger}, J. and {de Jaeger}, T. and 
	{De Cia}, A. and {Della Valle}, M. and {Dennefeld}, M. and {Elias-Rosa}, N. and 
	{Elman}, N. and {Feindt}, U. and {Fleury}, M. and {Gall}, E. and 
	{Gonzalez-Gaitan}, S. and {Galbany}, L. and {Morales Garoffolo}, A. and 
	{Greggio}, L. and {Guillou}, L.~L. and {Hachinger}, S. and {Hadjiyska}, E. and 
	{Hage}, P.~E. and {Hillebrandt}, W. and {Hodgkin}, S. and {Hsiao}, E.~Y. and 
	{James}, P.~A. and {Jerkstrand}, A. and {Kangas}, T. and {Kankare}, E. and 
	{Kotak}, R. and {Kromer}, M. and {Kuncarayakti}, H. and {Leloudas}, G. and 
	{Lundqvist}, P. and {Lyman}, J.~D. and {Hook}, I.~M. and {Maguire}, K. and 
	{Manulis}, I. and {Margheim}, S.~J. and {Mattila}, S. and {Maund}, J.~R. and 
	{Mazzali}, P.~A. and {McCrum}, M. and {McKinnon}, R. and {Moreno-Raya}, M.~E. and
	{Nicholl}, M. and {Nugent}, P. and {Pain}, R. and {Pignata}, G. and 
	{Phillips}, M.~M. and {Polshaw}, J. and {Pumo}, M.~L. and {Rabinowitz}, D. and 
	{Reilly}, E. and {Romero-Ca{\~n}izales}, C. and {Scalzo}, R. and 
	{Schmidt}, B. and {Schulze}, S. and {Sim}, S. and {Sollerman}, J. and 
	{Taddia}, F. and {Tartaglia}, L. and {Terreran}, G. and {Tomasella}, L. and 
	{Turatto}, M. and {Walker}, E. and {Walton}, N.~A. and {Wyrzykowski}, L. and 
	{Yuan}, F. and {Zampieri}, L.},
    title = "{PESSTO: survey description and products from the first data release by the Public ESO Spectroscopic Survey of Transient Objects}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1411.0299},
 primaryClass = "astro-ph.SR",
 keywords = {instrumentation: spectrographs, methods: data analysis, techniques: spectroscopic, surveys, supernovae: general},
     year = 2015,
    month = jul,
   volume = 579,
      eid = {A40},
    pages = {A40},
      doi = {10.1051/0004-6361/201425237},
   adsurl = {http://adsabs.harvard.edu/abs/2015A%26A...579A..40S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2016arXiv161205560C,
   author = {{Chambers}, K.~C. and {Magnier}, E.~A. and {Metcalfe}, N. and 
	{Flewelling}, H.~A. and {Huber}, M.~E. and {Waters}, C.~Z. and 
	{Denneau}, L. and {Draper}, P.~W. and {Farrow}, D. and {Finkbeiner}, D.~P. and 
	{Holmberg}, C. and {Koppenhoefer}, J. and {Price}, P.~A. and 
	{Saglia}, R.~P. and {Schlafly}, E.~F. and {Smartt}, S.~J. and 
	{Sweeney}, W. and {Wainscoat}, R.~J. and {Burgett}, W.~S. and 
	{Grav}, T. and {Heasley}, J.~N. and {Hodapp}, K.~W. and {Jedicke}, R. and 
	{Kaiser}, N. and {Kudritzki}, R.-P. and {Luppino}, G.~A. and 
	{Lupton}, R.~H. and {Monet}, D.~G. and {Morgan}, J.~S. and {Onaka}, P.~M. and 
	{Stubbs}, C.~W. and {Tonry}, J.~L. and {Banados}, E. and {Bell}, E.~F. and 
	{Bender}, R. and {Bernard}, E.~J. and {Botticella}, M.~T. and 
	{Casertano}, S. and {Chastel}, S. and {Chen}, W.-P. and {Chen}, X. and 
	{Cole}, S. and {Deacon}, N. and {Frenk}, C. and {Fitzsimmons}, A. and 
	{Gezari}, S. and {Goessl}, C. and {Goggia}, T. and {Goldman}, B. and 
	{Grebel}, E.~K. and {Hambly}, N.~C. and {Hasinger}, G. and {Heavens}, A.~F. and 
	{Heckman}, T.~M. and {Henderson}, R. and {Henning}, T. and {Holman}, M. and 
	{Hopp}, U. and {Ip}, W.-H. and {Isani}, S. and {Keyes}, C.~D. and 
	{Koekemoer}, A. and {Kotak}, R. and {Long}, K.~S. and {Lucey}, J.~R and 
	{Liu}, M. and {Martin}, N.~F. and {McLean}, B. and {Morganson}, E. and 
	{Murphy}, D.~N.~A. and {Nieto-Santisteban}, M.~A. and {Norberg}, P. and 
	{Peacock}, J.~A. and {Pier}, E.~A. and {Postman}, M. and {Primak}, N. and 
	{Rae}, C. and {Rest}, A. and {Riess}, A. and {Riffeser}, A. and 
	{Rix}, H.~W. and {Roser}, S. and {Schilbach}, E. and {Schultz}, A.~S.~B. and 
	{Scolnic}, D. and {Szalay}, A. and {Seitz}, S. and {Shiao}, B. and 
	{Small}, E. and {Smith}, K.~W. and {Soderblom}, D. and {Taylor}, A.~N. and 
	{Thakar}, A.~R. and {Thiel}, J. and {Thilker}, D. and {Urata}, Y. and 
	{Valenti}, J. and {Walter}, F. and {Watters}, S.~P. and {Werner}, S. and 
	{White}, R. and {Wood-Vasey}, W.~M. and {Wyse}, R.},
    title = "{The Pan-STARRS1 Surveys}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1612.05560},
 primaryClass = "astro-ph.IM",
 keywords = {Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
     year = 2016,
    month = dec,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv161205560C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2011PASP..123...58T,
   author = {{Tonry}, J.~L.},
    title = "{An Early Warning System for Asteroid Impact}",
  journal = {\pasp},
archivePrefix = "arXiv",
   eprint = {1011.1028},
 primaryClass = "astro-ph.IM",
     year = 2011,
    month = jan,
   volume = 123,
    pages = {58},
      doi = {10.1086/657997},
   adsurl = {http://adsabs.harvard.edu/abs/2011PASP..123...58T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2013AJ....146...86T,
   author = {{Tully}, R.~B. and {Courtois}, H.~M. and {Dolphin}, A.~E. and 
	{Fisher}, J.~R. and {H{\'e}raudeau}, P. and {Jacobs}, B.~A. and 
	{Karachentsev}, I.~D. and {Makarov}, D. and {Makarova}, L. and 
	{Mitronova}, S. and {Rizzi}, L. and {Shaya}, E.~J. and {Sorce}, J.~G. and 
	{Wu}, P.-F.},
    title = "{Cosmicflows-2: The Data}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1307.7213},
 keywords = {catalogs, galaxies: distances and redshifts},
     year = 2013,
    month = oct,
   volume = 146,
      eid = {86},
    pages = {86},
      doi = {10.1088/0004-6256/146/4/86},
   adsurl = {http://adsabs.harvard.edu/abs/2013AJ....146...86T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009PASP..121.1395L,
   author = {{Law}, N.~M. and {Kulkarni}, S.~R. and {Dekany}, R.~G. and {Ofek}, E.~O. and 
	{Quimby}, R.~M. and {Nugent}, P.~E. and {Surace}, J. and {Grillmair}, C.~C. and 
	{Bloom}, J.~S. and {Kasliwal}, M.~M. and {Bildsten}, L. and 
	{Brown}, T. and {Cenko}, S.~B. and {Ciardi}, D. and {Croner}, E. and 
	{Djorgovski}, S.~G. and {van Eyken}, J. and {Filippenko}, A.~V. and 
	{Fox}, D.~B. and {Gal-Yam}, A. and {Hale}, D. and {Hamam}, N. and 
	{Helou}, G. and {Henning}, J. and {Howell}, D.~A. and {Jacobsen}, J. and 
	{Laher}, R. and {Mattingly}, S. and {McKenna}, D. and {Pickles}, A. and 
	{Poznanski}, D. and {Rahmer}, G. and {Rau}, A. and {Rosing}, W. and 
	{Shara}, M. and {Smith}, R. and {Starr}, D. and {Sullivan}, M. and 
	{Velur}, V. and {Walters}, R. and {Zolkower}, J.},
    title = "{The Palomar Transient Factory: System Overview, Performance, and First Results}",
  journal = {\pasp},
archivePrefix = "arXiv",
   eprint = {0906.5350},
 primaryClass = "astro-ph.IM",
     year = 2009,
    month = dec,
   volume = 121,
    pages = {1395},
      doi = {10.1086/648598},
   adsurl = {http://adsabs.harvard.edu/abs/2009PASP..121.1395L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2018ApJ...853...62T,
   author = {{Tartaglia}, L. and {Sand}, D.~J. and {Valenti}, S. and {Wyatt}, S. and 
	{Anderson}, J.~P. and {Arcavi}, I. and {Ashall}, C. and {Botticella}, M.~T. and 
	{Cartier}, R. and {Chen}, T.-W. and {Cikota}, A. and {Coulter}, D. and 
	{Della Valle}, M. and {Foley}, R.~J. and {Gal-Yam}, A. and {Galbany}, L. and 
	{Gall}, C. and {Haislip}, J.~B. and {Harmanen}, J. and {Hosseinzadeh}, G. and 
	{Howell}, D.~A. and {Hsiao}, E.~Y. and {Inserra}, C. and {Jha}, S.~W. and 
	{Kankare}, E. and {Kilpatrick}, C.~D. and {Kouprianov}, V.~V. and 
	{Kuncarayakti}, H. and {Maccarone}, T.~J. and {Maguire}, K. and 
	{Mattila}, S. and {Mazzali}, P.~A. and {McCully}, C. and {Melandri}, A. and 
	{Morrell}, N. and {Phillips}, M.~M. and {Pignata}, G. and {Piro}, A.~L. and 
	{Prentice}, S. and {Reichart}, D.~E. and {Rojas-Bravo}, C. and 
	{Smartt}, S.~J. and {Smith}, K.~W. and {Sollerman}, J. and {Stritzinger}, M.~D. and 
	{Sullivan}, M. and {Taddia}, F. and {Young}, D.~R.},
    title = "{The Early Detection and Follow-up of the Highly Obscured Type II Supernova 2016ija/DLT16am}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1711.03940},
 primaryClass = "astro-ph.HE",
 keywords = {galaxies: individual: NGC 1532, supernovae: general, supernovae: individual: SN 2016ija, DLT16am},
     year = 2018,
    month = jan,
   volume = 853,
      eid = {62},
    pages = {62},
      doi = {10.3847/1538-4357/aaa014},
   adsurl = {http://adsabs.harvard.edu/abs/2018ApJ...853...62T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{1998ApJ...500..525S,
   author = {{Schlegel}, D.~J. and {Finkbeiner}, D.~P. and {Davis}, M.},
    title = "{Maps of Dust Infrared Emission for Use in Estimation of Reddening and Cosmic Microwave Background Radiation Foregrounds}",
  journal = {\apj},
   eprint = {astro-ph/9710327},
 keywords = {COSMOLOGY: DIFFUSE RADIATION, COSMOLOGY: COSMIC MICROWAVE BACKGROUND, ISM: DUST, EXTINCTION, INTERPLANETARY MEDIUM, INFRARED: ISM: CONTINUUM, Cosmology: Cosmic Microwave Background, Cosmology: Diffuse Radiation, ISM: Dust, Extinction, Infrared: ISM: Continuum, Interplanetary Medium},
     year = 1998,
    month = jun,
   volume = 500,
    pages = {525-553},
      doi = {10.1086/305772},
   adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...500..525S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1973A&A....24..337S,
   author = {{Shakura}, N.~I. and {Sunyaev}, R.~A.},
    title = "{Black holes in binary systems. Observational appearance.}",
  journal = {\aap},
     year = 1973,
   volume = 24,
    pages = {337-355},
   adsurl = {http://adsabs.harvard.edu/abs/1973A%26A....24..337S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1989ApJ...345..245C,
   author = {{Cardelli}, J.~A. and {Clayton}, G.~C. and {Mathis}, J.~S.},
    title = "{The relationship between infrared, optical, and ultraviolet extinction}",
  journal = {\apj},
 keywords = {Infrared Spectra, Interstellar Extinction, Ultraviolet Spectra, Visible Spectrum, Computational Astrophysics, Interstellar Matter, Iue},
     year = 1989,
    month = oct,
   volume = 345,
    pages = {245-256},
      doi = {10.1086/167900},
   adsurl = {http://adsabs.harvard.edu/abs/1989ApJ...345..245C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1998ApJ...498..541K,
   author = {{Kennicutt}, Jr., R.~C.},
    title = "{The Global Schmidt Law in Star-forming Galaxies}",
  journal = {\apj},
   eprint = {astro-ph/9712213},
 keywords = {GALAXIES: EVOLUTION, GALAXIES: ISM, GALAXIES: SPIRAL, GALAXIES: STELLAR CONTENT, GALAXIES: STARBURST, STARS: FORMATION, Galaxies: Evolution, Galaxies: ISM, Galaxies: Spiral, Galaxies: Starburst, Galaxies: Stellar Content, Stars: Formation},
     year = 1998,
    month = may,
   volume = 498,
    pages = {541-552},
      doi = {10.1086/305588},
   adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...498..541K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1977ApJ...217..425M,
   author = {{Mathis}, J.~S. and {Rumpl}, W. and {Nordsieck}, K.~H.},
    title = "{The size distribution of interstellar grains}",
  journal = {\apj},
 keywords = {Cosmic Dust, Interstellar Extinction, Interstellar Matter, Particle Size Distribution, Enstatite, Graphite, Magnetite, Olivine, Polarization Characteristics, Ultraviolet Astronomy},
     year = 1977,
    month = oct,
   volume = 217,
    pages = {425-433},
      doi = {10.1086/155591},
   adsurl = {http://adsabs.harvard.edu/abs/1977ApJ...217..425M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1995ApJS..101..181W,
   author = {{Woosley}, S.~E. and {Weaver}, T.~A.},
    title = "{The Evolution and Explosion of Massive Stars. II. Explosive Hydrodynamics and Nucleosynthesis}",
  journal = {\apjs},
 keywords = {HYDRODYNAMICS, NUCLEAR REACTIONS, NUCLEOSYNTHESIS, ABUNDANCES, STARS: EVOLUTION, STARS: INTERIORS, STARS: SUPERNOVAE: GENERAL},
     year = 1995,
    month = nov,
   volume = 101,
    pages = {181},
      doi = {10.1086/192237},
   adsurl = {http://adsabs.harvard.edu/abs/1995ApJS..101..181W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1908AnP...330..377M,
   author = {{Mie}, G.},
    title = "{Beitr{\"a}ge zur Optik tr{\"u}ber Medien, speziell kolloidaler Metall{\"o}sungen}",
  journal = {Annalen der Physik},
     year = 1908,
   volume = 330,
    pages = {377-445},
      doi = {10.1002/andp.19083300302},
   adsurl = {http://adsabs.harvard.edu/abs/1908AnP...330..377M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1986PASP...98..609H,
   author = {{Horne}, K.},
    title = "{An optimal extraction algorithm for CCD spectroscopy}",
  journal = {\pasp},
 keywords = {Astronomical Spectroscopy, Charge Coupled Devices, Data Reduction, Spectrum Analysis, Image Processing, Iteration, Optimization, Spatial Resolution, Stellar Spectra, Variance (Statistics)},
     year = 1986,
    month = jun,
   volume = 98,
    pages = {609-617},
      doi = {10.1086/131801},
   adsurl = {http://adsabs.harvard.edu/abs/1986PASP...98..609H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2003ARA&A..41..241D,
   author = {{Draine}, B.~T.},
    title = "{Interstellar Dust Grains}",
  journal = {\araa},
   eprint = {astro-ph/0304489},
     year = 2003,
   volume = 41,
    pages = {241-289},
      doi = {10.1146/annurev.astro.41.011802.094840},
   adsurl = {http://adsabs.harvard.edu/abs/2003ARA%26A..41..241D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2003ApJ...591..288H,
   author = {{Heger}, A. and {Fryer}, C.~L. and {Woosley}, S.~E. and {Langer}, N. and 
	{Hartmann}, D.~H.},
    title = "{How Massive Single Stars End Their Life}",
  journal = {\apj},
   eprint = {astro-ph/0212469},
 keywords = {Black Hole Physics, Gamma Rays: Bursts, Stars: Early-Type, Stars: Neutron, Stars: Supernovae: General},
     year = 2003,
    month = jul,
   volume = 591,
    pages = {288-300},
      doi = {10.1086/375341},
   adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...591..288H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2001AJ....122..549V,
   author = {{Vanden Berk}, D.~E. and {Richards}, G.~T. and {Bauer}, A. and 
	{Strauss}, M.~A. and {Schneider}, D.~P. and {Heckman}, T.~M. and 
	{York}, D.~G. and {Hall}, P.~B. and {Fan}, X. and {Knapp}, G.~R. and 
	{Anderson}, S.~F. and {Annis}, J. and {Bahcall}, N.~A. and {Bernardi}, M. and 
	{Briggs}, J.~W. and {Brinkmann}, J. and {Brunner}, R. and {Burles}, S. and 
	{Carey}, L. and {Castander}, F.~J. and {Connolly}, A.~J. and 
	{Crocker}, J.~H. and {Csabai}, I. and {Doi}, M. and {Finkbeiner}, D. and 
	{Friedman}, S. and {Frieman}, J.~A. and {Fukugita}, M. and {Gunn}, J.~E. and 
	{Hennessy}, G.~S. and {Ivezi{\'c}}, {\v Z}. and {Kent}, S. and 
	{Kunszt}, P.~Z. and {Lamb}, D.~Q. and {Leger}, R.~F. and {Long}, D.~C. and 
	{Loveday}, J. and {Lupton}, R.~H. and {Meiksin}, A. and {Merelli}, A. and 
	{Munn}, J.~A. and {Newberg}, H.~J. and {Newcomb}, M. and {Nichol}, R.~C. and 
	{Owen}, R. and {Pier}, J.~R. and {Pope}, A. and {Rockosi}, C.~M. and 
	{Schlegel}, D.~J. and {Siegmund}, W.~A. and {Smee}, S. and {Snir}, Y. and 
	{Stoughton}, C. and {Stubbs}, C. and {SubbaRao}, M. and {Szalay}, A.~S. and 
	{Szokoly}, G.~P. and {Tremonti}, C. and {Uomoto}, A. and {Waddell}, P. and 
	{Yanny}, B. and {Zheng}, W.},
    title = "{Composite Quasar Spectra from the Sloan Digital Sky Survey}",
  journal = {\aj},
   eprint = {astro-ph/0105231},
 keywords = {Galaxies: Quasars: Emission Lines, Galaxies: Quasars: General},
     year = 2001,
    month = aug,
   volume = 122,
    pages = {549-564},
      doi = {10.1086/321167},
   adsurl = {http://adsabs.harvard.edu/abs/2001AJ....122..549V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2003Natur.423..847H,
   author = {{Hjorth}, J. and {Sollerman}, J. and {M{\o}ller}, P. and {Fynbo}, J.~P.~U. and 
	{Woosley}, S.~E. and {Kouveliotou}, C. and {Tanvir}, N.~R. and 
	{Greiner}, J. and {Andersen}, M.~I. and {Castro-Tirado}, A.~J. and 
	{Castro Cer{\'o}n}, J.~M. and {Fruchter}, A.~S. and {Gorosabel}, J. and 
	{Jakobsson}, P. and {Kaper}, L. and {Klose}, S. and {Masetti}, N. and 
	{Pedersen}, H. and {Pedersen}, K. and {Pian}, E. and {Palazzi}, E. and 
	{Rhoads}, J.~E. and {Rol}, E. and {van den Heuvel}, E.~P.~J. and 
	{Vreeswijk}, P.~M. and {Watson}, D. and {Wijers}, R.~A.~M.~J.
	},
    title = "{A very energetic supernova associated with the {$\gamma$}-ray burst of 29 March 2003}",
  journal = {\nat},
   eprint = {astro-ph/0306347},
     year = 2003,
    month = jun,
   volume = 423,
    pages = {847-850},
      doi = {10.1038/nature01750},
   adsurl = {http://adsabs.harvard.edu/abs/2003Natur.423..847H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2003PASP..115..928K,
   author = {{Kennicutt}, Jr., R.~C. and {Armus}, L. and {Bendo}, G. and 
	{Calzetti}, D. and {Dale}, D.~A. and {Draine}, B.~T. and {Engelbracht}, C.~W. and 
	{Gordon}, K.~D. and {Grauer}, A.~D. and {Helou}, G. and {Hollenbach}, D.~J. and 
	{Jarrett}, T.~H. and {Kewley}, L.~J. and {Leitherer}, C. and 
	{Li}, A. and {Malhotra}, S. and {Regan}, M.~W. and {Rieke}, G.~H. and 
	{Rieke}, M.~J. and {Roussel}, H. and {Smith}, J.-D.~T. and {Thornley}, M.~D. and 
	{Walter}, F.},
    title = "{SINGS: The SIRTF Nearby Galaxies Survey}",
  journal = {\pasp},
   eprint = {astro-ph/0305437},
 keywords = {ISM: Dust, Extinction, Galaxies: Evolution, Galaxies: ISM, infrared: galaxies, Stars: Formation, Surveys},
     year = 2003,
    month = aug,
   volume = 115,
    pages = {928-952},
      doi = {10.1086/376941},
   adsurl = {http://adsabs.harvard.edu/abs/2003PASP..115..928K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2006AJ....132..117F,
   author = {{Fan}, X. and {Strauss}, M.~A. and {Becker}, R.~H. and {White}, R.~L. and 
	{Gunn}, J.~E. and {Knapp}, G.~R. and {Richards}, G.~T. and {Schneider}, D.~P. and 
	{Brinkmann}, J. and {Fukugita}, M.},
    title = "{Constraining the Evolution of the Ionizing Background and the Epoch of Reionization with z\~{}6 Quasars. II. A Sample of 19 Quasars}",
  journal = {\aj},
   eprint = {astro-ph/0512082},
 keywords = {Cosmology: Observations, Galaxies: Intergalactic Medium, Galaxies: Quasars: Absorption Lines, Galaxies: Quasars: General},
     year = 2006,
    month = jul,
   volume = 132,
    pages = {117-136},
      doi = {10.1086/504836},
   adsurl = {http://adsabs.harvard.edu/abs/2006AJ....132..117F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{1992apa..book.....F,
   author = {{Frank}, J. and {King}, A. and {Raine}, D.},
    title = "{Accretion power in astrophysics.}",
booktitle = {Camb.~Astrophys.~Ser., Vol.~21,},
     year = 1992,
   adsurl = {http://adsabs.harvard.edu/abs/1992apa..book.....F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2001AJ....122.2833F,
   author = {{Fan}, X. and {Narayanan}, V.~K. and {Lupton}, R.~H. and {Strauss}, M.~A. and 
	{Knapp}, G.~R. and {Becker}, R.~H. and {White}, R.~L. and {Pentericci}, L. and 
	{Leggett}, S.~K. and {Haiman}, Z. and {Gunn}, J.~E. and {Ivezi{\'c}}, {\v Z}. and 
	{Schneider}, D.~P. and {Anderson}, S.~F. and {Brinkmann}, J. and 
	{Bahcall}, N.~A. and {Connolly}, A.~J. and {Csabai}, I. and 
	{Doi}, M. and {Fukugita}, M. and {Geballe}, T. and {Grebel}, E.~K. and 
	{Harbeck}, D. and {Hennessy}, G. and {Lamb}, D.~Q. and {Miknaitis}, G. and 
	{Munn}, J.~A. and {Nichol}, R. and {Okamura}, S. and {Pier}, J.~R. and 
	{Prada}, F. and {Richards}, G.~T. and {Szalay}, A. and {York}, D.~G.
	},
    title = "{A Survey of z$\gt$5.8 Quasars in the Sloan Digital Sky Survey. I. Discovery of Three New Quasars and the Spatial Density of Luminous Quasars at z\~{}6}",
  journal = {\aj},
   eprint = {astro-ph/0108063},
 keywords = {Galaxies: Intergalactic Medium, Galaxies: Quasars: Absorption Lines, Galaxies: Quasars: Emission Lines, Galaxies: Quasars: General},
     year = 2001,
    month = dec,
   volume = 122,
    pages = {2833-2849},
      doi = {10.1086/324111},
   adsurl = {http://adsabs.harvard.edu/abs/2001AJ....122.2833F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2003AJ....125.1649F,
   author = {{Fan}, X. and {Strauss}, M.~A. and {Schneider}, D.~P. and {Becker}, R.~H. and 
	{White}, R.~L. and {Haiman}, Z. and {Gregg}, M. and {Pentericci}, L. and 
	{Grebel}, E.~K. and {Narayanan}, V.~K. and {Loh}, Y.-S. and 
	{Richards}, G.~T. and {Gunn}, J.~E. and {Lupton}, R.~H. and 
	{Knapp}, G.~R. and {Ivezi{\'c}}, {\v Z}. and {Brandt}, W.~N. and 
	{Collinge}, M. and {Hao}, L. and {Harbeck}, D. and {Prada}, F. and 
	{Schaye}, J. and {Strateva}, I. and {Zakamska}, N. and {Anderson}, S. and 
	{Brinkmann}, J. and {Bahcall}, N.~A. and {Lamb}, D.~Q. and {Okamura}, S. and 
	{Szalay}, A. and {York}, D.~G.},
    title = "{A Survey of z$\gt$5.7 Quasars in the Sloan Digital Sky Survey. II. Discovery of Three Additional Quasars at z$\gt$6}",
  journal = {\aj},
   eprint = {astro-ph/0301135},
 keywords = {Cosmology: Gravitational Lensing, Galaxies: Quasars: Absorption Lines, Galaxies: Quasars: Emission Lines, Galaxies: Quasars: General},
     year = 2003,
    month = apr,
   volume = 125,
    pages = {1649-1659},
      doi = {10.1086/368246},
   adsurl = {http://adsabs.harvard.edu/abs/2003AJ....125.1649F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2003PASP..115..389V,
   author = {{Vacca}, W.~D. and {Cushing}, M.~C. and {Rayner}, J.~T.},
    title = "{A Method of Correcting Near-Infrared Spectra for Telluric Absorption}",
  journal = {\pasp},
   eprint = {astro-ph/0211255},
 keywords = {Atmospheric Effects, Methods: Data Analysis, Techniques: Spectroscopic},
     year = 2003,
    month = mar,
   volume = 115,
    pages = {389-409},
      doi = {10.1086/346193},
   adsurl = {http://adsabs.harvard.edu/abs/2003PASP..115..389V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010ARA&A..48..339B,
   author = {{Bastian}, N. and {Covey}, K.~R. and {Meyer}, M.~R.},
    title = "{A Universal Stellar Initial Mass Function? A Critical Look at Variations}",
  journal = {\araa},
archivePrefix = "arXiv",
   eprint = {1001.2965},
     year = 2010,
    month = sep,
   volume = 48,
    pages = {339-389},
      doi = {10.1146/annurev-astro-082708-101642},
   adsurl = {http://adsabs.harvard.edu/abs/2010ARA%26A..48..339B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2003ApJ...594..279G,
   author = {{Gordon}, K.~D. and {Clayton}, G.~C. and {Misselt}, K.~A. and 
	{Landolt}, A.~U. and {Wolff}, M.~J.},
    title = "{A Quantitative Comparison of the Small Magellanic Cloud, Large Magellanic Cloud, and Milky Way Ultraviolet to Near-Infrared Extinction Curves}",
  journal = {\apj},
   eprint = {astro-ph/0305257},
 keywords = {ISM: Dust, Extinction, Galaxies: ISM, Galaxies: Magellanic Clouds, Ultraviolet: ISM},
     year = 2003,
    month = sep,
   volume = 594,
    pages = {279-293},
      doi = {10.1086/376774},
   adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...594..279G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2008MNRAS.388.1595D,
   author = {{da Cunha}, E. and {Charlot}, S. and {Elbaz}, D.},
    title = "{A simple model to interpret the ultraviolet, optical and infrared emission from galaxies}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0806.1020},
 keywords = {dust, extinction , galaxies: ISM , galaxies: stellar content , infrared: galaxies},
     year = 2008,
    month = aug,
   volume = 388,
    pages = {1595-1617},
      doi = {10.1111/j.1365-2966.2008.13535.x},
   adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.388.1595D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2002ApJ...565..773T,
   author = {{Telfer}, R.~C. and {Zheng}, W. and {Kriss}, G.~A. and {Davidsen}, A.~F.
	},
    title = "{The Rest-Frame Extreme-Ultraviolet Spectral Properties of Quasi-stellar Objects}",
  journal = {\apj},
   eprint = {astro-ph/0109531},
 keywords = {Galaxies: Quasars: Emission Lines, Galaxies: Quasars: General, Ultraviolet: Galaxies},
     year = 2002,
    month = feb,
   volume = 565,
    pages = {773-785},
      doi = {10.1086/324689},
   adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...565..773T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1996ApJ...469..740J,
   author = {{Jones}, A.~P. and {Tielens}, A.~G.~G.~M. and {Hollenbach}, D.~J.
	},
    title = "{Grain Shattering in Shocks: The Interstellar Grain Size Distribution}",
  journal = {\apj},
 keywords = {ISM: DUST, EXTINCTION, SHOCK WAVES, STARS: SUPERNOVAE: GENERAL, METHODS: NUMERICAL},
     year = 1996,
    month = oct,
   volume = 469,
    pages = {740},
      doi = {10.1086/177823},
   adsurl = {http://adsabs.harvard.edu/abs/1996ApJ...469..740J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1998ApJ...501..643D,
   author = {{Dwek}, E.},
    title = "{The Evolution of the Elemental Abundances in the Gas and Dust Phases of the Galaxy}",
  journal = {\apj},
   eprint = {astro-ph/9707024},
 keywords = {ISM: DUST, EXTINCTION, GALAXY: ABUNDANCES, GALAXY: EVOLUTION, GALAXY: STELLAR CONTENT, ISM: ABUNDANCES, ISM: GENERAL},
     year = 1998,
    month = jul,
   volume = 501,
    pages = {643},
      doi = {10.1086/305829},
   adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...501..643D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012ApJ...754L..29W,
   author = {{Whitaker}, K.~E. and {van Dokkum}, P.~G. and {Brammer}, G. and 
	{Franx}, M.},
    title = "{The Star Formation Mass Sequence Out to z = 2.5}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1205.0547},
 keywords = {galaxies: evolution, galaxies: formation, galaxies: high-redshift},
     year = 2012,
    month = aug,
   volume = 754,
      eid = {L29},
    pages = {L29},
      doi = {10.1088/2041-8205/754/2/L29},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...754L..29W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011A&A...536A.105V,
   author = {{Vernet}, J. and {Dekker}, H. and {D'Odorico}, S. and {Kaper}, L. and 
	{Kjaergaard}, P. and {Hammer}, F. and {Randich}, S. and {Zerbi}, F. and 
	{Groot}, P.~J. and {Hjorth}, J. and {Guinouard}, I. and {Navarro}, R. and 
	{Adolfse}, T. and {Albers}, P.~W. and {Amans}, J.-P. and {Andersen}, J.~J. and 
	{Andersen}, M.~I. and {Binetruy}, P. and {Bristow}, P. and {Castillo}, R. and 
	{Chemla}, F. and {Christensen}, L. and {Conconi}, P. and {Conzelmann}, R. and 
	{Dam}, J. and {de Caprio}, V. and {de Ugarte Postigo}, A. and 
	{Delabre}, B. and {di Marcantonio}, P. and {Downing}, M. and 
	{Elswijk}, E. and {Finger}, G. and {Fischer}, G. and {Flores}, H. and 
	{Fran{\c c}ois}, P. and {Goldoni}, P. and {Guglielmi}, L. and 
	{Haigron}, R. and {Hanenburg}, H. and {Hendriks}, I. and {Horrobin}, M. and 
	{Horville}, D. and {Jessen}, N.~C. and {Kerber}, F. and {Kern}, L. and 
	{Kiekebusch}, M. and {Kleszcz}, P. and {Klougart}, J. and {Kragt}, J. and 
	{Larsen}, H.~H. and {Lizon}, J.-L. and {Lucuix}, C. and {Mainieri}, V. and 
	{Manuputy}, R. and {Martayan}, C. and {Mason}, E. and {Mazzoleni}, R. and 
	{Michaelsen}, N. and {Modigliani}, A. and {Moehler}, S. and 
	{M{\o}ller}, P. and {Norup S{\o}rensen}, A. and {N{\o}rregaard}, P. and 
	{P{\'e}roux}, C. and {Patat}, F. and {Pena}, E. and {Pragt}, J. and 
	{Reinero}, C. and {Rigal}, F. and {Riva}, M. and {Roelfsema}, R. and 
	{Royer}, F. and {Sacco}, G. and {Santin}, P. and {Schoenmaker}, T. and 
	{Spano}, P. and {Sweers}, E. and {Ter Horst}, R. and {Tintori}, M. and 
	{Tromp}, N. and {van Dael}, P. and {van der Vliet}, H. and {Venema}, L. and 
	{Vidali}, M. and {Vinther}, J. and {Vola}, P. and {Winters}, R. and 
	{Wistisen}, D. and {Wulterkens}, G. and {Zacchei}, A.},
    title = "{X-shooter, the new wide band intermediate resolution spectrograph at the ESO Very Large Telescope}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1110.1944},
 primaryClass = "astro-ph.IM",
 keywords = {instrumentation: spectrographs},
     year = 2011,
    month = dec,
   volume = 536,
      eid = {A105},
    pages = {A105},
      doi = {10.1051/0004-6361/201117752},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...536A.105V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011MNRAS.414.2446M,
   author = {{McMillan}, P.~J.},
    title = "{Mass models of the Milky Way}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1102.4340},
 keywords = {methods: statistical, Galaxy: fundamental parameters, Galaxy: kinematics and dynamics},
     year = 2011,
    month = jul,
   volume = 414,
    pages = {2446-2457},
      doi = {10.1111/j.1365-2966.2011.18564.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.414.2446M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1978Natur.272..706S,
   author = {{Shields}, G.~A.},
    title = "{Thermal continuum from acretion disks in quasars}",
  journal = {\nat},
 keywords = {Continuous Spectra, Quasars, Stellar Mass Accretion, Thermal Emission, Seyfert Galaxies},
     year = 1978,
    month = apr,
   volume = 272,
    pages = {706-708},
      doi = {10.1038/272706a0},
   adsurl = {http://adsabs.harvard.edu/abs/1978Natur.272..706S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2001MNRAS.325..726T,
   author = {{Todini}, P. and {Ferrara}, A.},
    title = "{Dust formation in primordial Type II supernovae}",
  journal = {\mnras},
   eprint = {astro-ph/0009176},
 keywords = {STARS: FORMATION, SUPERNOVAE: GENERAL, SUPERNOVAE: INDIVIDUAL: SN1987A, DUST, EXTINCTION, SUPERNOVA REMNANTS},
     year = 2001,
    month = aug,
   volume = 325,
    pages = {726-736},
      doi = {10.1046/j.1365-8711.2001.04486.x},
   adsurl = {http://adsabs.harvard.edu/abs/2001MNRAS.325..726T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1974ApJ...191..675G,
   author = {{Gehrz}, R.~D. and {Hackwell}, J.~A. and {Jones}, T.~W.},
    title = "{Infrared observations of Be stars from 2.3 to 19.5 microns.}",
  journal = {\apj},
     year = 1974,
    month = aug,
   volume = 191,
    pages = {675-684},
      doi = {10.1086/153008},
   adsurl = {http://adsabs.harvard.edu/abs/1974ApJ...191..675G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1997MNRAS.288..145P,
   author = {{Padoan}, P. and {Nordlund}, A. and {Jones}, B.~J.~T.},
    title = "{The universality of the stellar initial mass function}",
  journal = {\mnras},
   eprint = {astro-ph/9703110},
 keywords = {STARS: FORMATION, STARS: LUMINOSITY FUNCTION, MASS FUNCTION, ISM: KINEMATICS AND DYNAMICS},
     year = 1997,
    month = jun,
   volume = 288,
    pages = {145-152},
      doi = {10.1093/mnras/288.1.145},
   adsurl = {http://adsabs.harvard.edu/abs/1997MNRAS.288..145P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012Natur.484..485C,
   author = {{Cappellari}, M. and {McDermid}, R.~M. and {Alatalo}, K. and 
	{Blitz}, L. and {Bois}, M. and {Bournaud}, F. and {Bureau}, M. and 
	{Crocker}, A.~F. and {Davies}, R.~L. and {Davis}, T.~A. and 
	{de Zeeuw}, P.~T. and {Duc}, P.-A. and {Emsellem}, E. and {Khochfar}, S. and 
	{Krajnovi{\'c}}, D. and {Kuntschner}, H. and {Lablanche}, P.-Y. and 
	{Morganti}, R. and {Naab}, T. and {Oosterloo}, T. and {Sarzi}, M. and 
	{Scott}, N. and {Serra}, P. and {Weijmans}, A.-M. and {Young}, L.~M.
	},
    title = "{Systematic variation of the stellar initial mass function in early-type galaxies}",
  journal = {\nat},
archivePrefix = "arXiv",
   eprint = {1202.3308},
 primaryClass = "astro-ph.CO",
     year = 2012,
    month = apr,
   volume = 484,
    pages = {485-488},
      doi = {10.1038/nature10972},
   adsurl = {http://adsabs.harvard.edu/abs/2012Natur.484..485C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1966AdPhy..15..111F,
   author = {{Feder}, J. and {Russell}, K.~C. and {Lothe}, J. and {Pound}, G.~M.
	},
    title = "{Homogeneous nucleation and growth of droplets in vapours}",
  journal = {Advances in Physics},
     year = 1966,
    month = jan,
   volume = 15,
    pages = {111-178},
      doi = {10.1080/00018736600101264},
   adsurl = {http://adsabs.harvard.edu/abs/1966AdPhy..15..111F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1998MNRAS.301..569L,
   author = {{Larson}, R.~B.},
    title = "{Early star formation and the evolution of the stellar initial mass function in galaxies}",
  journal = {\mnras},
   eprint = {astro-ph/9808145},
 keywords = {STARS: FORMATION, STARS: LUMINOSITY FUNCTION, MASS FUNCTION, GALAXIES: EVOLUTION, GALAXIES: FORMATION, GALAXIES: STELLAR CONTENT, DARK MATTER},
     year = 1998,
    month = dec,
   volume = 301,
    pages = {569-581},
      doi = {10.1046/j.1365-8711.1998.02045.x},
   adsurl = {http://adsabs.harvard.edu/abs/1998MNRAS.301..569L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009ApJ...700.1299J,
   author = {{Jenkins}, E.~B.},
    title = "{A Unified Representation of Gas-Phase Element Depletions in the Interstellar Medium}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0905.3173},
 primaryClass = "astro-ph.GA",
 keywords = {ISM: abundances, ISM: atoms, ultraviolet: ISM},
     year = 2009,
    month = aug,
   volume = 700,
    pages = {1299-1348},
      doi = {10.1088/0004-637X/700/2/1299},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...700.1299J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1998ApJ...503..674K,
   author = {{Kim}, S. and {Staveley-Smith}, L. and {Dopita}, M.~A. and {Freeman}, K.~C. and 
	{Sault}, R.~J. and {Kesteven}, M.~J. and {McConnell}, D.},
    title = "{An H I Aperture Synthesis Mosaic of the Large Magellanic Cloud}",
  journal = {\apj},
 keywords = {GALAXIES: ISM, GALAXIES: STRUCTURE, GALAXIES: MAGELLANIC CLOUDS, RADIO LINES: GALAXIES, SURVEYS, Galaxies: ISM, Galaxies: Structure, Galaxies: Magellanic Clouds, Radio Lines: Galaxies, Surveys},
     year = 1998,
    month = aug,
   volume = 503,
    pages = {674-688},
      doi = {10.1086/306030},
   adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...503..674K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2007ApJ...663..320F,
   author = {{Fitzpatrick}, E.~L. and {Massa}, D.},
    title = "{An Analysis of the Shapes of Interstellar Extinction Curves. V. The IR-through-UV Curve Morphology}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0705.0154},
 keywords = {ISM: Dust, Extinction, Methods: Data Analysis},
     year = 2007,
    month = jul,
   volume = 663,
    pages = {320-341},
      doi = {10.1086/518158},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...663..320F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2003ApJ...598..785N,
   author = {{Nozawa}, T. and {Kozasa}, T. and {Umeda}, H. and {Maeda}, K. and 
	{Nomoto}, K.},
    title = "{Dust in the Early Universe: Dust Formation in the Ejecta of Population III Supernovae}",
  journal = {\apj},
   eprint = {astro-ph/0307108},
 keywords = {ISM: Dust, Extinction, Cosmology: Early Universe, Stars: Supernovae: General},
     year = 2003,
    month = dec,
   volume = 598,
    pages = {785-803},
      doi = {10.1086/379011},
   adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...598..785N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1999ApJS..120..299T,
   author = {{Truelove}, J.~K. and {McKee}, C.~F.},
    title = "{Evolution of Nonradiative Supernova Remnants}",
  journal = {\apjs},
 keywords = {HYDRODYNAMICS, SHOCK WAVES, ISM: SUPERNOVA REMNANTS, STARS: SUPERNOVAE: GENERAL, Hydrodynamics, Shock Waves, ISM: Supernova Remnants, Stars: Supernovae: General},
     year = 1999,
    month = feb,
   volume = 120,
    pages = {299-326},
      doi = {10.1086/313176},
   adsurl = {http://adsabs.harvard.edu/abs/1999ApJS..120..299T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2007Sci...317..924P,
   author = {{Patat}, F. and {Chandra}, P. and {Chevalier}, R. and {Justham}, S. and 
	{Podsiadlowski}, P. and {Wolf}, C. and {Gal-Yam}, A. and {Pasquini}, L. and 
	{Crawford}, I.~A. and {Mazzali}, P.~A. and {Pauldrach}, A.~W.~A. and 
	{Nomoto}, K. and {Benetti}, S. and {Cappellaro}, E. and {Elias-Rosa}, N. and 
	{Hillebrandt}, W. and {Leonard}, D.~C. and {Pastorello}, A. and 
	{Renzini}, A. and {Sabbadin}, F. and {Simon}, J.~D. and {Turatto}, M.
	},
    title = "{Detection of Circumstellar Material in a Normal Type Ia Supernova}",
  journal = {Science},
archivePrefix = "arXiv",
   eprint = {0707.2793},
     year = 2007,
    month = aug,
   volume = 317,
    pages = {924},
      doi = {10.1126/science.1143005},
   adsurl = {http://adsabs.harvard.edu/abs/2007Sci...317..924P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2003A&A...406L..55B,
   author = {{Bertoldi}, F. and {Carilli}, C.~L. and {Cox}, P. and {Fan}, X. and 
	{Strauss}, M.~A. and {Beelen}, A. and {Omont}, A. and {Zylka}, R.
	},
    title = "{Dust emission from the most distant quasars}",
  journal = {\aap},
   eprint = {astro-ph/0305116},
 keywords = {galaxies: formation, galaxies: starburst, galaxies: high-redshift, quasars: general, cosmology: observations, submillimeter},
     year = 2003,
    month = jul,
   volume = 406,
    pages = {L55-L58},
      doi = {10.1051/0004-6361:20030710},
   adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...406L..55B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012ApJ...745...69K,
   author = {{Krumholz}, M.~R. and {Dekel}, A. and {McKee}, C.~F.},
    title = "{A Universal, Local Star Formation Law in Galactic Clouds, nearby Galaxies, High-redshift Disks, and Starbursts}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1109.4150},
 keywords = {galaxies: high-redshift, galaxies: ISM, galaxies: starburst, ISM: clouds, stars: formation},
     year = 2012,
    month = jan,
   volume = 745,
      eid = {69},
    pages = {69},
      doi = {10.1088/0004-637X/745/1/69},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...745...69K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2004AJ....127.1531H,
   author = {{Harris}, J. and {Zaritsky}, D.},
    title = "{The Star Formation History of the Small Magellanic Cloud}",
  journal = {\aj},
   eprint = {astro-ph/0312100},
 keywords = {Galaxies: Evolution, Galaxies: Individual: Name: Small Magellanic Cloud, Galaxies: Stellar Content, Galaxies: Magellanic Clouds},
     year = 2004,
    month = mar,
   volume = 127,
    pages = {1531-1544},
      doi = {10.1086/381953},
   adsurl = {http://adsabs.harvard.edu/abs/2004AJ....127.1531H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012MNRAS.421...98D,
   author = {{Dav{\'e}}, R. and {Finlator}, K. and {Oppenheimer}, B.~D.},
    title = "{An analytic model for the evolution of the stellar, gas and metal content of galaxies}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1108.0426},
 keywords = {galaxies: evolution, galaxies: formation, galaxies: fundamental parameters, galaxies: haloes, galaxies: high-redshift, intergalactic medium},
     year = 2012,
    month = mar,
   volume = 421,
    pages = {98-107},
      doi = {10.1111/j.1365-2966.2011.20148.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.421...98D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2008MNRAS.385..147D,
   author = {{Dav{\'e}}, R.},
    title = "{The galaxy stellar mass-star formation rate relation: evidence for an evolving stellar initial mass function?}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0710.0381},
 keywords = {stars: luminosity function, mass function , galaxies: evolution , galaxies: formation , galaxies: high-redshift , cosmology: theory},
     year = 2008,
    month = mar,
   volume = 385,
    pages = {147-160},
      doi = {10.1111/j.1365-2966.2008.12866.x},
   adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.385..147D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013Natur.496..329R,
   author = {{Riechers}, D.~A. and {Bradford}, C.~M. and {Clements}, D.~L. and 
	{Dowell}, C.~D. and {P{\'e}rez-Fournon}, I. and {Ivison}, R.~J. and 
	{Bridge}, C. and {Conley}, A. and {Fu}, H. and {Vieira}, J.~D. and 
	{Wardlow}, J. and {Calanog}, J. and {Cooray}, A. and {Hurley}, P. and 
	{Neri}, R. and {Kamenetzky}, J. and {Aguirre}, J.~E. and {Altieri}, B. and 
	{Arumugam}, V. and {Benford}, D.~J. and {B{\'e}thermin}, M. and 
	{Bock}, J. and {Burgarella}, D. and {Cabrera-Lavers}, A. and 
	{Chapman}, S.~C. and {Cox}, P. and {Dunlop}, J.~S. and {Earle}, L. and 
	{Farrah}, D. and {Ferrero}, P. and {Franceschini}, A. and {Gavazzi}, R. and 
	{Glenn}, J. and {Solares}, E.~A.~G. and {Gurwell}, M.~A. and 
	{Halpern}, M. and {Hatziminaoglou}, E. and {Hyde}, A. and {Ibar}, E. and 
	{Kov{\'a}cs}, A. and {Krips}, M. and {Lupu}, R.~E. and {Maloney}, P.~R. and 
	{Martinez-Navajas}, P. and {Matsuhara}, H. and {Murphy}, E.~J. and 
	{Naylor}, B.~J. and {Nguyen}, H.~T. and {Oliver}, S.~J. and 
	{Omont}, A. and {Page}, M.~J. and {Petitpas}, G. and {Rangwala}, N. and 
	{Roseboom}, I.~G. and {Scott}, D. and {Smith}, A.~J. and {Staguhn}, J.~G. and 
	{Streblyanska}, A. and {Thomson}, A.~P. and {Valtchanov}, I. and 
	{Viero}, M. and {Wang}, L. and {Zemcov}, M. and {Zmuidzinas}, J.
	},
    title = "{A dust-obscured massive maximum-starburst galaxy at a redshift of 6.34}",
  journal = {\nat},
archivePrefix = "arXiv",
   eprint = {1304.4256},
 primaryClass = "astro-ph.CO",
     year = 2013,
    month = apr,
   volume = 496,
    pages = {329-333},
      doi = {10.1038/nature12050},
   adsurl = {http://adsabs.harvard.edu/abs/2013Natur.496..329R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009AJ....138.1243H,
   author = {{Harris}, J. and {Zaritsky}, D.},
    title = "{The Star Formation History of the Large Magellanic Cloud}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {0908.1422},
 keywords = {galaxies: evolution, galaxies: individual: Large Magellanic Cloud, galaxies: stellar content, Magellanic Clouds},
     year = 2009,
    month = nov,
   volume = 138,
    pages = {1243-1260},
      doi = {10.1088/0004-6256/138/5/1243},
   adsurl = {http://adsabs.harvard.edu/abs/2009AJ....138.1243H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2000AJ....120.1167F,
   author = {{Fan}, X. and {White}, R.~L. and {Davis}, M. and {Becker}, R.~H. and 
	{Strauss}, M.~A. and {Haiman}, Z. and {Schneider}, D.~P. and 
	{Gregg}, M.~D. and {Gunn}, J.~E. and {Knapp}, G.~R. and {Lupton}, R.~H. and 
	{Anderson}, Jr., J.~E. and {Anderson}, S.~F. and {Annis}, J. and 
	{Bahcall}, N.~A. and {Boroski}, W.~N. and {Brunner}, R.~J. and 
	{Chen}, B. and {Connolly}, A.~J. and {Csabai}, I. and {Doi}, M. and 
	{Fukugita}, M. and {Hennessy}, G.~S. and {Hindsley}, R.~B. and 
	{Ichikawa}, T. and {Ivezi{\'c}}, {\v Z}. and {Loveday}, J. and 
	{Meiksin}, A. and {McKay}, T.~A. and {Munn}, J.~A. and {Newberg}, H.~J. and 
	{Nichol}, R. and {Okamura}, S. and {Pier}, J.~R. and {Sekiguchi}, M. and 
	{Shimasaku}, K. and {Stoughton}, C. and {Szalay}, A.~S. and 
	{Szokoly}, G.~P. and {Thakar}, A.~R. and {Vogeley}, M.~S. and 
	{York}, D.~G.},
    title = "{The Discovery of a Luminous Z=5.80 Quasar from the Sloan Digital Sky Survey}",
  journal = {\aj},
   eprint = {astro-ph/0005414},
 keywords = {Galaxies: Intergalactic Medium, Galaxies: Quasars: Absorption Lines, Galaxies: Quasars: Emission Lines, Galaxies: Quasars: Individual: Alphanumeric: SDSSp J104433.04-012502.2},
     year = 2000,
    month = sep,
   volume = 120,
    pages = {1167-1174},
      doi = {10.1086/301534},
   adsurl = {http://adsabs.harvard.edu/abs/2000AJ....120.1167F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2007MNRAS.378..973B,
   author = {{Bianchi}, S. and {Schneider}, R.},
    title = "{Dust formation and survival in supernova ejecta}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0704.0586},
 keywords = {shock waves, supernovae: individual: Cassiopeia A, dust, extinction, supernova remnants},
     year = 2007,
    month = jul,
   volume = 378,
    pages = {973-982},
      doi = {10.1111/j.1365-2966.2007.11829.x},
   adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.378..973B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1999ApJ...523..617F,
   author = {{Falco}, E.~E. and {Impey}, C.~D. and {Kochanek}, C.~S. and 
	{Leh{\'a}r}, J. and {McLeod}, B.~A. and {Rix}, H.-W. and {Keeton}, C.~R. and 
	{Mu{\~n}oz}, J.~A. and {Peng}, C.~Y.},
    title = "{Dust and Extinction Curves in Galaxies with z$\gt$0: The Interstellar Medium of Gravitational Lens Galaxies}",
  journal = {\apj},
   eprint = {astro-ph/9901037},
 keywords = {ISM: DUST, EXTINCTION, GALAXIES: ISM, GALAXIES: PHOTOMETRY, COSMOLOGY: GRAVITATIONAL LENSING, ISM: Dust, Extinction, Galaxies: ISM, Galaxies: Photometry, Cosmology: Gravitational Lensing},
     year = 1999,
    month = oct,
   volume = 523,
    pages = {617-632},
      doi = {10.1086/307758},
   adsurl = {http://adsabs.harvard.edu/abs/1999ApJ...523..617F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1977ARA&A..15..175C,
   author = {{Chevalier}, R.~A.},
    title = "{The interaction of supernovae with the interstellar medium}",
  journal = {\araa},
 keywords = {Interstellar Matter, Supernova Remnants, Supernovae, Conductive Heat Transfer, Cosmic Rays, Energy Transfer, Gamma Rays, Gas Ionization, Kinetic Energy, Relativistic Particles, Shock Wave Interaction, Stellar Mass Ejection, Taylor Instability, X Ray Astronomy},
     year = 1977,
   volume = 15,
    pages = {175-196},
      doi = {10.1146/annurev.aa.15.090177.001135},
   adsurl = {http://adsabs.harvard.edu/abs/1977ARA%26A..15..175C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2001ApJ...560L...5D,
   author = {{Djorgovski}, S.~G. and {Castro}, S. and {Stern}, D. and {Mahabal}, A.~A.
	},
    title = "{On the Threshold of the Reionization Epoch}",
  journal = {\apjl},
   eprint = {astro-ph/0108069},
 keywords = {Cosmology: Observations, Galaxies: Formation, Galaxies: Quasars: Individual: Alphanumeric: SDSS 1044-0125},
     year = 2001,
    month = oct,
   volume = 560,
    pages = {L5-L8},
      doi = {10.1086/324175},
   adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...560L...5D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2004Natur.431..533M,
   author = {{Maiolino}, R. and {Schneider}, R. and {Oliva}, E. and {Bianchi}, S. and 
	{Ferrara}, A. and {Mannucci}, F. and {Pedani}, M. and {Roca Sogorb}, M.
	},
    title = "{A supernova origin for dust in a high-redshift quasar}",
  journal = {\nat},
   eprint = {astro-ph/0409577},
     year = 2004,
    month = sep,
   volume = 431,
    pages = {533-535},
      doi = {10.1038/nature02930},
   adsurl = {http://adsabs.harvard.edu/abs/2004Natur.431..533M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012ApJ...760....6M,
   author = {{Magdis}, G.~E. and {Daddi}, E. and {B{\'e}thermin}, M. and 
	{Sargent}, M. and {Elbaz}, D. and {Pannella}, M. and {Dickinson}, M. and 
	{Dannerbauer}, H. and {da Cunha}, E. and {Walter}, F. and {Rigopoulou}, D. and 
	{Charmandaris}, V. and {Hwang}, H.~S. and {Kartaltepe}, J.},
    title = "{The Evolving Interstellar Medium of Star-forming Galaxies since z = 2 as Probed by Their Infrared Spectral Energy Distributions}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1210.1035},
 keywords = {galaxies: evolution},
     year = 2012,
    month = nov,
   volume = 760,
      eid = {6},
    pages = {6},
      doi = {10.1088/0004-637X/760/1/6},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...760....6M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011Sci...333.1258M,
   author = {{Matsuura}, M. and {Dwek}, E. and {Meixner}, M. and {Otsuka}, M. and 
	{Babler}, B. and {Barlow}, M.~J. and {Roman-Duval}, J. and {Engelbracht}, C. and 
	{Sandstrom}, K. and {Laki{\'c}evi{\'c}}, M. and {van Loon}, J.~T. and 
	{Sonneborn}, G. and {Clayton}, G.~C. and {Long}, K.~S. and {Lundqvist}, P. and 
	{Nozawa}, T. and {Gordon}, K.~D. and {Hony}, S. and {Panuzzo}, P. and 
	{Okumura}, K. and {Misselt}, K.~A. and {Montiel}, E. and {Sauvage}, M.
	},
    title = "{Herschel Detects a Massive Dust Reservoir in Supernova 1987A}",
  journal = {Science},
archivePrefix = "arXiv",
   eprint = {1107.1477},
 primaryClass = "astro-ph.SR",
     year = 2011,
    month = sep,
   volume = 333,
    pages = {1258},
      doi = {10.1126/science.1205983},
   adsurl = {http://adsabs.harvard.edu/abs/2011Sci...333.1258M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2007Natur.447..829P,
   author = {{Pastorello}, A. and {Smartt}, S.~J. and {Mattila}, S. and {Eldridge}, J.~J. and 
	{Young}, D. and {Itagaki}, K. and {Yamaoka}, H. and {Navasardyan}, H. and 
	{Valenti}, S. and {Patat}, F. and {Agnoletto}, I. and {Augusteijn}, T. and 
	{Benetti}, S. and {Cappellaro}, E. and {Boles}, T. and {Bonnet-Bidaud}, J.-M. and 
	{Botticella}, M.~T. and {Bufano}, F. and {Cao}, C. and {Deng}, J. and 
	{Dennefeld}, M. and {Elias-Rosa}, N. and {Harutyunyan}, A. and 
	{Keenan}, F.~P. and {Iijima}, T. and {Lorenzi}, V. and {Mazzali}, P.~A. and 
	{Meng}, X. and {Nakano}, S. and {Nielsen}, T.~B. and {Smoker}, J.~V. and 
	{Stanishev}, V. and {Turatto}, M. and {Xu}, D. and {Zampieri}, L.
	},
    title = "{A giant outburst two years before the core-collapse of a massive star}",
  journal = {\nat},
   eprint = {astro-ph/0703663},
     year = 2007,
    month = jun,
   volume = 447,
    pages = {829-832},
      doi = {10.1038/nature05825},
   adsurl = {http://adsabs.harvard.edu/abs/2007Natur.447..829P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2003AJ....126.2594R,
   author = {{Reichard}, T.~A. and {Richards}, G.~T. and {Hall}, P.~B. and 
	{Schneider}, D.~P. and {Vanden Berk}, D.~E. and {Fan}, X. and 
	{York}, D.~G. and {Knapp}, G.~R. and {Brinkmann}, J.},
    title = "{Continuum and Emission-Line Properties of Broad Absorption Line Quasars}",
  journal = {\aj},
   eprint = {astro-ph/0308508},
 keywords = {Galaxies: Quasars: Absorption Lines, Galaxies: Quasars: Emission Lines, Galaxies: Quasars: General},
     year = 2003,
    month = dec,
   volume = 126,
    pages = {2594-2607},
      doi = {10.1086/379293},
   adsurl = {http://adsabs.harvard.edu/abs/2003AJ....126.2594R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2008A&A...479..453Z,
   author = {{Zhukovska}, S. and {Gail}, H.-P. and {Trieloff}, M.},
    title = "{Evolution of interstellar dust and stardust in the solar neighbourhood}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0706.1155},
 keywords = {ISM: abundances, ISM: dust, extinction, galaxies: ISM, Galaxy: evolution},
     year = 2008,
    month = feb,
   volume = 479,
    pages = {453-480},
      doi = {10.1051/0004-6361:20077789},
   adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...479..453Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010A&A...518L..25R,
   author = {{Rodighiero}, G. and {Cimatti}, A. and {Gruppioni}, C. and {Popesso}, P. and 
	{Andreani}, P. and {Altieri}, B. and {Aussel}, H. and {Berta}, S. and 
	{Bongiovanni}, A. and {Brisbin}, D. and {Cava}, A. and {Cepa}, J. and 
	{Daddi}, E. and {Dominguez-Sanchez}, H. and {Elbaz}, D. and 
	{Fontana}, A. and {F{\"o}rster Schreiber}, N. and {Franceschini}, A. and 
	{Genzel}, R. and {Grazian}, A. and {Lutz}, D. and {Magdis}, G. and 
	{Magliocchetti}, M. and {Magnelli}, B. and {Maiolino}, R. and 
	{Mancini}, C. and {Nordon}, R. and {Perez Garcia}, A.~M. and 
	{Poglitsch}, A. and {Santini}, P. and {Sanchez-Portal}, M. and 
	{Pozzi}, F. and {Riguccini}, L. and {Saintonge}, A. and {Shao}, L. and 
	{Sturm}, E. and {Tacconi}, L. and {Valtchanov}, I. and {Wetzstein}, M. and 
	{Wieprecht}, E.},
    title = "{The first Herschel view of the mass-SFR link in high-z galaxies}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1005.1089},
 keywords = {galaxies: evolution, galaxies: active, galaxies: starburst, cosmology: observations, infrared: galaxies},
     year = 2010,
    month = jul,
   volume = 518,
      eid = {L25},
    pages = {L25},
      doi = {10.1051/0004-6361/201014624},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...518L..25R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013ARA&A..51..393C,
   author = {{Conroy}, C.},
    title = "{Modeling the Panchromatic Spectral Energy Distributions of Galaxies}",
  journal = {\araa},
archivePrefix = "arXiv",
   eprint = {1301.7095},
     year = 2013,
    month = aug,
   volume = 51,
    pages = {393-455},
      doi = {10.1146/annurev-astro-082812-141017},
   adsurl = {http://adsabs.harvard.edu/abs/2013ARA%26A..51..393C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012ApJ...756..164F,
   author = {{Finkelstein}, S.~L. and {Papovich}, C. and {Salmon}, B. and 
	{Finlator}, K. and {Dickinson}, M. and {Ferguson}, H.~C. and 
	{Giavalisco}, M. and {Koekemoer}, A.~M. and {Reddy}, N.~A. and 
	{Bassett}, R. and {Conselice}, C.~J. and {Dunlop}, J.~S. and 
	{Faber}, S.~M. and {Grogin}, N.~A. and {Hathi}, N.~P. and {Kocevski}, D.~D. and 
	{Lai}, K. and {Lee}, K.-S. and {McLure}, R.~J. and {Mobasher}, B. and 
	{Newman}, J.~A.},
    title = "{Candels: The Evolution of Galaxy Rest-frame Ultraviolet Colors from z = 8 to 4}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1110.3785},
 keywords = {early universe, galaxies: evolution, galaxies: formation, galaxies: high-redshift, ultraviolet: galaxies},
     year = 2012,
    month = sep,
   volume = 756,
      eid = {164},
    pages = {164},
      doi = {10.1088/0004-637X/756/2/164},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...756..164F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010A&A...514A..67M,
   author = {{Micha{\l}owski}, M. and {Hjorth}, J. and {Watson}, D.},
    title = "{Cosmic evolution of submillimeter galaxies and their contribution to stellar mass assembly}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0905.4499},
 keywords = {galaxies: active, galaxies: evolution, galaxies: high-redshift, galaxies: ISM, galaxies: starburst, submillimeter: galaxies},
     year = 2010,
    month = may,
   volume = 514,
      eid = {A67},
    pages = {A67},
      doi = {10.1051/0004-6361/200913634},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...514A..67M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2001MNRAS.326.1027S,
   author = {{Smith}, L.~J. and {Gallagher}, J.~S.},
    title = "{M82-F: a doomed super star cluster?}",
  journal = {\mnras},
   eprint = {astro-ph/0104429},
 keywords = {GALAXIES: EVOLUTION, GALAXIES: INDIVIDUAL: M82, GALAXIES: STARBURST, GALAXIES: STAR CLUSTERS, GALAXIES: STELLAR CONTENT},
     year = 2001,
    month = sep,
   volume = 326,
    pages = {1027-1040},
      doi = {10.1046/j.1365-8711.2001.04627.x},
   adsurl = {http://adsabs.harvard.edu/abs/2001MNRAS.326.1027S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2003MNRAS.343..427M,
   author = {{Morgan}, H.~L. and {Edmunds}, M.~G.},
    title = "{Dust formation in early galaxies}",
  journal = {\mnras},
   eprint = {astro-ph/0302566},
 keywords = {ISM: abundances, dust, extinction, galaxies: high-redshift},
     year = 2003,
    month = aug,
   volume = 343,
    pages = {427-442},
      doi = {10.1046/j.1365-8711.2003.06681.x},
   adsurl = {http://adsabs.harvard.edu/abs/2003MNRAS.343..427M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012ApJ...754...25R,
   author = {{Reddy}, N.~A. and {Pettini}, M. and {Steidel}, C.~C. and {Shapley}, A.~E. and 
	{Erb}, D.~K. and {Law}, D.~R.},
    title = "{The Characteristic Star Formation Histories of Galaxies at Redshifts z \~{} 2-7}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1205.0555},
 keywords = {dust, extinction, galaxies: evolution, galaxies: formation, galaxies: high-redshift, galaxies: star formation},
     year = 2012,
    month = jul,
   volume = 754,
      eid = {25},
    pages = {25},
      doi = {10.1088/0004-637X/754/1/25},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...754...25R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010MNRAS.405.1025M,
   author = {{M{\'e}nard}, B. and {Scranton}, R. and {Fukugita}, M. and {Richards}, G.
	},
    title = "{Measuring the galaxy-mass and galaxy-dust correlations through magnification and reddening}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0902.4240},
 keywords = {gravitational lensing: weak, dust, extinction, dark matter},
     year = 2010,
    month = jun,
   volume = 405,
    pages = {1025-1039},
      doi = {10.1111/j.1365-2966.2010.16486.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.405.1025M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2007ApJ...666..955N,
   author = {{Nozawa}, T. and {Kozasa}, T. and {Habe}, A. and {Dwek}, E. and 
	{Umeda}, H. and {Tominaga}, N. and {Maeda}, K. and {Nomoto}, K.
	},
    title = "{Evolution of Dust in Primordial Supernova Remnants: Can Dust Grains Formed in the Ejecta Survive and Be Injected into the Early Interstellar Medium?}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0706.0383},
 keywords = {ISM: Dust, Extinction, Cosmology: Early Universe, Shock Waves, ISM: Supernova Remnants, Stars: Supernovae: General},
     year = 2007,
    month = sep,
   volume = 666,
    pages = {955-966},
      doi = {10.1086/520621},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...666..955N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2003Natur.424..285D,
   author = {{Dunne}, L. and {Eales}, S. and {Ivison}, R. and {Morgan}, H. and 
	{Edmunds}, M.},
    title = "{Type II supernovae as a significant source of interstellar dust}",
  journal = {\nat},
   eprint = {astro-ph/0307320},
     year = 2003,
    month = jul,
   volume = 424,
    pages = {285-287},
      doi = {10.1038/nature01792},
   adsurl = {http://adsabs.harvard.edu/abs/2003Natur.424..285D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1993ApJS...88..477W,
   author = {{Wooden}, D.~H. and {Rank}, D.~M. and {Bregman}, J.~D. and {Witteborn}, F.~C. and 
	{Tielens}, A.~G.~G.~M. and {Cohen}, M. and {Pinto}, P.~A. and 
	{Axelrod}, T.~S.},
    title = "{Airborne spectrophotometry of SN 1987A from 1.7 to 12.6 microns - Time history of the dust continuum and line emission}",
  journal = {\apjs},
 keywords = {Airborne Equipment, Infrared Stars, Line Spectra, Spectral Energy Distribution, Stellar Spectrophotometry, Supernova 1987a, Argon, Calibrating, Carbon Monoxide, Chlorine, Cobalt, Helium, Hydrogen, Iron, Nickel, Sodium, Wavelengths},
     year = 1993,
    month = oct,
   volume = 88,
    pages = {477-507},
      doi = {10.1086/191830},
   adsurl = {http://adsabs.harvard.edu/abs/1993ApJS...88..477W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2007ApJ...662..927D,
   author = {{Dwek}, E. and {Galliano}, F. and {Jones}, A.~P.},
    title = "{The Evolution of Dust in the Early Universe with Applications to the Galaxy SDSS J1148+5251}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0705.3799},
 keywords = {ISM: Dust, Extinction, Galaxies: Evolution, Galaxies: Formation, Galaxies: High-Redshift, galaxies: individual (SDSS J114816.64+525150.3), Galaxies: Starburst, Infrared: Galaxies, Infrared: General},
     year = 2007,
    month = jun,
   volume = 662,
    pages = {927-939},
      doi = {10.1086/518430},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...662..927D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012A&A...539A..31C,
   author = {{Cucciati}, O. and {Tresse}, L. and {Ilbert}, O. and {Le F{\`e}vre}, O. and 
	{Garilli}, B. and {Le Brun}, V. and {Cassata}, P. and {Franzetti}, P. and 
	{Maccagni}, D. and {Scodeggio}, M. and {Zucca}, E. and {Zamorani}, G. and 
	{Bardelli}, S. and {Bolzonella}, M. and {Bielby}, R.~M. and 
	{McCracken}, H.~J. and {Zanichelli}, A. and {Vergani}, D.},
    title = "{The star formation rate density and dust attenuation evolution over 12 Gyr with the VVDS surveys}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1109.1005},
 keywords = {cosmology: observations, galaxies: evolution, galaxies: high-redshift, galaxies: luminosity function, mass function, galaxies: star formation},
     year = 2012,
    month = mar,
   volume = 539,
      eid = {A31},
    pages = {A31},
      doi = {10.1051/0004-6361/201118010},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...539A..31C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009ApJ...705.1364T,
   author = {{Thompson}, T.~A. and {Prieto}, J.~L. and {Stanek}, K.~Z. and 
	{Kistler}, M.~D. and {Beacom}, J.~F. and {Kochanek}, C.~S.},
    title = "{A New Class of Luminous Transients and a First Census of their Massive Stellar Progenitors}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0809.0510},
 keywords = {stars: evolution, supernovae: general, supernovae: individual: SN 2008S 1999bw, surveys},
     year = 2009,
    month = nov,
   volume = 705,
    pages = {1364-1384},
      doi = {10.1088/0004-637X/705/2/1364},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...705.1364T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012A&A...539A.155M,
   author = {{Magnelli}, B. and {Lutz}, D. and {Santini}, P. and {Saintonge}, A. and 
	{Berta}, S. and {Albrecht}, M. and {Altieri}, B. and {Andreani}, P. and 
	{Aussel}, H. and {Bertoldi}, F. and {B{\'e}thermin}, M. and 
	{Bongiovanni}, A. and {Capak}, P. and {Chapman}, S. and {Cepa}, J. and 
	{Cimatti}, A. and {Cooray}, A. and {Daddi}, E. and {Danielson}, A.~L.~R. and 
	{Dannerbauer}, H. and {Dunlop}, J.~S. and {Elbaz}, D. and {Farrah}, D. and 
	{F{\"o}rster Schreiber}, N.~M. and {Genzel}, R. and {Hwang}, H.~S. and 
	{Ibar}, E. and {Ivison}, R.~J. and {Le Floc'h}, E. and {Magdis}, G. and 
	{Maiolino}, R. and {Nordon}, R. and {Oliver}, S.~J. and {P{\'e}rez Garc{\'{\i}}a}, A. and 
	{Poglitsch}, A. and {Popesso}, P. and {Pozzi}, F. and {Riguccini}, L. and 
	{Rodighiero}, G. and {Rosario}, D. and {Roseboom}, I. and {Salvato}, M. and 
	{Sanchez-Portal}, M. and {Scott}, D. and {Smail}, I. and {Sturm}, E. and 
	{Swinbank}, A.~M. and {Tacconi}, L.~J. and {Valtchanov}, I. and 
	{Wang}, L. and {Wuyts}, S.},
    title = "{A Herschel view of the far-infrared properties of submillimetre galaxies}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1202.0761},
 keywords = {galaxies: evolution, infrared: galaxies, galaxies: starburst, submillimeter: galaxies},
     year = 2012,
    month = mar,
   volume = 539,
      eid = {A155},
    pages = {A155},
      doi = {10.1051/0004-6361/201118312},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...539A.155M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2009ASPC..414..453D,
   author = {{Draine}, B.~T.},
    title = "{Interstellar Dust Models and Evolutionary Implications}",
booktitle = {Cosmic Dust - Near and Far},
     year = 2009,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 414,
archivePrefix = "arXiv",
   eprint = {0903.1658},
 primaryClass = "astro-ph.GA",
   editor = {{Henning}, T. and {Gr{\"u}n}, E. and {Steinacker}, J.},
    month = dec,
    pages = {453},
   adsurl = {http://adsabs.harvard.edu/abs/2009ASPC..414..453D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010ApJ...714..699W,
   author = {{Wang}, R. and {Carilli}, C.~L. and {Neri}, R. and {Riechers}, D.~A. and 
	{Wagg}, J. and {Walter}, F. and {Bertoldi}, F. and {Menten}, K.~M. and 
	{Omont}, A. and {Cox}, P. and {Fan}, X.},
    title = "{Molecular Gas in z \~{} 6 Quasar Host Galaxies}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1002.1561},
 keywords = {galaxies: active, galaxies: high-redshift, galaxies: starburst, molecular data, radio lines: galaxies},
     year = 2010,
    month = may,
   volume = 714,
    pages = {699-712},
      doi = {10.1088/0004-637X/714/1/699},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...714..699W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2006Sci...313..196S,
   author = {{Sugerman}, B.~E.~K. and {Ercolano}, B. and {Barlow}, M.~J. and 
	{Tielens}, A.~G.~G.~M. and {Clayton}, G.~C. and {Zijlstra}, A.~A. and 
	{Meixner}, M. and {Speck}, A. and {Gledhill}, T.~M. and {Panagia}, N. and 
	{Cohen}, M. and {Gordon}, K.~D. and {Meyer}, M. and {Fabbri}, J. and 
	{Bowey}, J.~E. and {Welch}, D.~L. and {Regan}, M.~W. and {Kennicutt}, R.~C.
	},
    title = "{Massive-Star Supernovae as Major Dust Factories}",
  journal = {Science},
   eprint = {astro-ph/0606132},
     year = 2006,
    month = jul,
   volume = 313,
    pages = {196-200},
      doi = {10.1126/science.1128131},
   adsurl = {http://adsabs.harvard.edu/abs/2006Sci...313..196S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009MNRAS.396..918M,
   author = {{Matsuura}, M. and {Barlow}, M.~J. and {Zijlstra}, A.~A. and 
	{Whitelock}, P.~A. and {Cioni}, M.-R.~L. and {Groenewegen}, M.~A.~T. and 
	{Volk}, K. and {Kemper}, F. and {Kodama}, T. and {Lagadec}, E. and 
	{Meixner}, M. and {Sloan}, G.~C. and {Srinivasan}, S.},
    title = "{The global gas and dust budget of the Large Magellanic Cloud: AGB stars and supernovae, and the impact on the ISM evolution}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0903.1123},
 keywords = {stars: AGB and post-AGB , stars: mass-loss , supernovae: general , dust, extinction , galaxies: evolution , galaxies: individual: the Magellanic Clouds},
     year = 2009,
    month = jun,
   volume = 396,
    pages = {918-934},
      doi = {10.1111/j.1365-2966.2009.14743.x},
   adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.396..918M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1983ApJ...274..175D,
   author = {{Dwek}, E.},
    title = "{The infrared echo of a type II supernova with a circumstellar dust shell - Applications to SN 1979c and SN 1980k}",
  journal = {\apj},
 keywords = {Infrared Astronomy, Stellar Envelopes, Supernovae, Thermal Emission, Cosmic Dust, Light Curve, Stellar Models, Stellar Spectrophotometry},
     year = 1983,
    month = nov,
   volume = 274,
    pages = {175-183},
      doi = {10.1086/161435},
   adsurl = {http://adsabs.harvard.edu/abs/1983ApJ...274..175D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011AJ....142..197C,
   author = {{Chomiuk}, L. and {Povich}, M.~S.},
    title = "{Toward a Unification of Star Formation Rate Determinations in the Milky Way and Other Galaxies}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1110.4105},
 keywords = {galaxies: star formation, Galaxy: fundamental parameters, H II regions, ISM: supernova remnants},
     year = 2011,
    month = dec,
   volume = 142,
      eid = {197},
    pages = {197},
      doi = {10.1088/0004-6256/142/6/197},
   adsurl = {http://adsabs.harvard.edu/abs/2011AJ....142..197C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011MNRAS.417.1510D,
   author = {{Dunne}, L. and {Gomez}, H.~L. and {da Cunha}, E. and {Charlot}, S. and 
	{Dye}, S. and {Eales}, S. and {Maddox}, S.~J. and {Rowlands}, K. and 
	{Smith}, D.~J.~B. and {Auld}, R. and {Baes}, M. and {Bonfield}, D.~G. and 
	{Bourne}, N. and {Buttiglione}, S. and {Cava}, A. and {Clements}, D.~L. and 
	{Coppin}, K.~E.~K. and {Cooray}, A. and {Dariush}, A. and {de Zotti}, G. and 
	{Driver}, S. and {Fritz}, J. and {Geach}, J. and {Hopwood}, R. and 
	{Ibar}, E. and {Ivison}, R.~J. and {Jarvis}, M.~J. and {Kelvin}, L. and 
	{Pascale}, E. and {Pohlen}, M. and {Popescu}, C. and {Rigby}, E.~E. and 
	{Robotham}, A. and {Rodighiero}, G. and {Sansom}, A.~E. and 
	{Serjeant}, S. and {Temi}, P. and {Thompson}, M. and {Tuffs}, R. and 
	{van der Werf}, P. and {Vlahakis}, C.},
    title = "{Herschel-ATLAS: rapid evolution of dust in galaxies over the last 5 billion years}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1012.5186},
 keywords = {ISM: evolution, galaxies: evolution, galaxies: ISM, submillimetre: galaxies},
     year = 2011,
    month = oct,
   volume = 417,
    pages = {1510-1533},
      doi = {10.1111/j.1365-2966.2011.19363.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.417.1510D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2007ApJ...658.1027L,
   author = {{Leroy}, A. and {Bolatto}, A. and {Stanimirovic}, S. and {Mizuno}, N. and 
	{Israel}, F. and {Bot}, C.},
    title = "{The Spitzer Survey of the Small Magellanic Cloud: Far-Infrared Emission and Cold Gas in the Small Magellanic Cloud}",
  journal = {\apj},
   eprint = {astro-ph/0611687},
 keywords = {ISM: Dust, Extinction, Galaxies: ISM, Infrared: ISM, ISM: Molecules, Galaxies: Magellanic Clouds},
     year = 2007,
    month = apr,
   volume = 658,
    pages = {1027-1046},
      doi = {10.1086/511150},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...658.1027L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2007AJ....134.1150J,
   author = {{Jiang}, L. and {Fan}, X. and {Vestergaard}, M. and {Kurk}, J.~D. and 
	{Walter}, F. and {Kelly}, B.~C. and {Strauss}, M.~A.},
    title = "{Gemini Near-Infrared Spectroscopy of Luminous z \~{} 6 Quasars: Chemical Abundances, Black Hole Masses, and Mg II Absorption}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {0707.1663},
 keywords = {galaxies: active, galaxies: high-redshift, quasars: absorption lines, quasars: emission lines, quasars: general},
     year = 2007,
    month = sep,
   volume = 134,
    pages = {1150},
      doi = {10.1086/520811},
   adsurl = {http://adsabs.harvard.edu/abs/2007AJ....134.1150J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015Natur.522..455C,
   author = {{Capak}, P.~L. and {Carilli}, C. and {Jones}, G. and {Casey}, C.~M. and 
	{Riechers}, D. and {Sheth}, K. and {Carollo}, C.~M. and {Ilbert}, O. and 
	{Karim}, A. and {Lefevre}, O. and {Lilly}, S. and {Scoville}, N. and 
	{Smolcic}, V. and {Yan}, L.},
    title = "{Galaxies at redshifts 5 to 6 with systematically low dust content and high [C II] emission}",
  journal = {\nat},
archivePrefix = "arXiv",
   eprint = {1503.07596},
     year = 2015,
    month = jun,
   volume = 522,
    pages = {455-458},
      doi = {10.1038/nature14500},
   adsurl = {http://adsabs.harvard.edu/abs/2015Natur.522..455C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011ApJ...741...12B,
   author = {{Bolatto}, A.~D. and {Leroy}, A.~K. and {Jameson}, K. and {Ostriker}, E. and 
	{Gordon}, K. and {Lawton}, B. and {Stanimirovi{\'c}}, S. and 
	{Israel}, F.~P. and {Madden}, S.~C. and {Hony}, S. and {Sandstrom}, K.~M. and 
	{Bot}, C. and {Rubio}, M. and {Winkler}, P.~F. and {Roman-Duval}, J. and 
	{van Loon}, J.~T. and {Oliveira}, J.~M. and {Indebetouw}, R.
	},
    title = "{The State of the Gas and the Relation between Gas and Star Formation at Low Metallicity: The Small Magellanic Cloud}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1107.1717},
 keywords = {galaxies: dwarf, galaxies: evolution, ISM: clouds, Magellanic Clouds},
     year = 2011,
    month = nov,
   volume = 741,
      eid = {12},
    pages = {12},
      doi = {10.1088/0004-637X/741/1/12},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...741...12B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1989ApJ...344..325K,
   author = {{Kozasa}, T. and {Hasegawa}, H. and {Nomoto}, K.},
    title = "{Formation of dust grains in the ejecta of SN 1987A}",
  journal = {\apj},
 keywords = {Cosmic Dust, Star Formation, Stellar Mass Ejection, Supernova 1987a, Carbon, Computation, Condensation, Ejecta, Grains, Metal Oxides, Nucleation},
     year = 1989,
    month = sep,
   volume = 344,
    pages = {325-331},
      doi = {10.1086/167801},
   adsurl = {http://adsabs.harvard.edu/abs/1989ApJ...344..325K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015ARA&A..53..541B,
   author = {{Boogert}, A.~C.~A. and {Gerakines}, P.~A. and {Whittet}, D.~C.~B.
	},
    title = "{Observations of the icy universe.}",
  journal = {\araa},
archivePrefix = "arXiv",
   eprint = {1501.05317},
     year = 2015,
    month = aug,
   volume = 53,
    pages = {541-581},
      doi = {10.1146/annurev-astro-082214-122348},
   adsurl = {http://adsabs.harvard.edu/abs/2015ARA%26A..53..541B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2002ApJ...581.1047D,
   author = {{de Avillez}, M.~A. and {Mac Low}, M.-M.},
    title = "{Mixing Timescales in a Supernova-driven Interstellar Medium}",
  journal = {\apj},
   eprint = {astro-ph/0208441},
 keywords = {Galaxy: Evolution, Galaxy: General, Galaxy: Structure, Hydrodynamics, ISM: Structure},
     year = 2002,
    month = dec,
   volume = 581,
    pages = {1047-1060},
      doi = {10.1086/344256},
   adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...581.1047D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1978MNRAS.183..367B,
   author = {{Barlow}, M.~J.},
    title = "{The destruction and growth of dust grains in interstellar space. I - Destruction by sputtering.}",
  journal = {\mnras},
 keywords = {Cosmic Dust, Ice, Silicate And Graphite Dust, Interstellar Radiation, Interstellar Space, Particle Interactions, Sputtering,Interstellar Matter},
     year = 1978,
    month = may,
   volume = 183,
    pages = {367-395},
      doi = {10.1093/mnras/183.3.367},
   adsurl = {http://adsabs.harvard.edu/abs/1978MNRAS.183..367B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012A&ARv..20...56C,
   author = {{Caselli}, P. and {Ceccarelli}, C.},
    title = "{Our astrochemical heritage}",
  journal = {\aapr},
archivePrefix = "arXiv",
   eprint = {1210.6368},
 keywords = {Astrochemistry, ISM: clouds, Stars: formation, Protoplanetary disks, Comets: general, Meteorites, meteors, meteoroids},
     year = 2012,
    month = oct,
   volume = 20,
      eid = {56},
    pages = {56},
      doi = {10.1007/s00159-012-0056-x},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26ARv..20...56C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010ApJ...712..942M,
   author = {{Micha{\l}owski}, M.~J. and {Watson}, D. and {Hjorth}, J.},
    title = "{Rapid Dust Production in Submillimeter Galaxies at z $\gt$ 4?}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1002.2636},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: active, galaxies: evolution, galaxies: high-redshift, galaxies: ISM, galaxies: starburst, submillimeter: galaxies},
     year = 2010,
    month = apr,
   volume = 712,
    pages = {942-950},
      doi = {10.1088/0004-637X/712/2/942},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...712..942M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015Natur.519..327W,
   author = {{Watson}, D. and {Christensen}, L. and {Knudsen}, K.~K. and 
	{Richard}, J. and {Gallazzi}, A. and {Micha{\l}owski}, M.~J.
	},
    title = "{A dusty, normal galaxy in the epoch of reionization}",
  journal = {\nat},
archivePrefix = "arXiv",
   eprint = {1503.00002},
     year = 2015,
    month = mar,
   volume = 519,
    pages = {327-330},
      doi = {10.1038/nature14164},
   adsurl = {http://adsabs.harvard.edu/abs/2015Natur.519..327W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011ApJ...743..159H,
   author = {{Hayward}, C.~C. and {Kere{\v s}}, D. and {Jonsson}, P. and 
	{Narayanan}, D. and {Cox}, T.~J. and {Hernquist}, L.},
    title = "{What Does a Submillimeter Galaxy Selection Actually Select? The Dependence of Submillimeter Flux Density on Star Formation Rate and Dust Mass}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1101.0002},
 primaryClass = "astro-ph.CO",
 keywords = {dust, extinction, galaxies: high-redshift, galaxies: interactions, galaxies: starburst, infrared: galaxies, radiative transfer, submillimeter: galaxies},
     year = 2011,
    month = dec,
   volume = 743,
      eid = {159},
    pages = {159},
      doi = {10.1088/0004-637X/743/2/159},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...743..159H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012A&A...541A..85M,
   author = {{Micha{\l}owski}, M.~J. and {Dunlop}, J.~S. and {Cirasuolo}, M. and 
	{Hjorth}, J. and {Hayward}, C.~C. and {Watson}, D.},
    title = "{The stellar masses and specific star-formation rates of submillimetre galaxies}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1108.6058},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: active, galaxies: evolution, galaxies: high-redshift, galaxies: ISM, galaxies: starburst, submillimeter: galaxies},
     year = 2012,
    month = may,
   volume = 541,
      eid = {A85},
    pages = {A85},
      doi = {10.1051/0004-6361/201016308},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...541A..85M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012A&A...540A..52C,
   author = {{Cortese}, L. and {Ciesla}, L. and {Boselli}, A. and {Bianchi}, S. and 
	{Gomez}, H. and {Smith}, M.~W.~L. and {Bendo}, G.~J. and {Eales}, S. and 
	{Pohlen}, M. and {Baes}, M. and {Corbelli}, E. and {Davies}, J.~I. and 
	{Hughes}, T.~M. and {Hunt}, L.~K. and {Madden}, S.~C. and {Pierini}, D. and 
	{di Serego Alighieri}, S. and {Zibetti}, S. and {Boquien}, M. and 
	{Clements}, D.~L. and {Cooray}, A. and {Galametz}, M. and {Magrini}, L. and 
	{Pappalardo}, C. and {Spinoglio}, L. and {Vlahakis}, C.},
    title = "{The dust scaling relations of the Herschel Reference Survey}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1201.2762},
 keywords = {dust, extinction, galaxies: evolution, submillimeter: galaxies, galaxies: clusters: individual: Virgo},
     year = 2012,
    month = apr,
   volume = 540,
      eid = {A52},
    pages = {A52},
      doi = {10.1051/0004-6361/201118499},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...540A..52C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2008ApJ...687..848W,
   author = {{Wang}, R. and {Carilli}, C.~L. and {Wagg}, J. and {Bertoldi}, F. and 
	{Walter}, F. and {Menten}, K.~M. and {Omont}, A. and {Cox}, P. and 
	{Strauss}, M.~A. and {Fan}, X. and {Jiang}, L. and {Schneider}, D.~P.
	},
    title = "{Thermal Emission from Warm Dust in the Most Distant Quasars}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0806.3022},
 keywords = {galaxies: evolution, galaxies: high-redshift, galaxies: starburst, quasars: general, submillimeter},
     year = 2008,
    month = nov,
   volume = 687,
      eid = {848-858},
    pages = {848-858},
      doi = {10.1086/591076},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...687..848W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2008ApJ...680..568S,
   author = {{Smith}, N. and {Foley}, R.~J. and {Filippenko}, A.~V.},
    title = "{Dust Formation and He II {$\lambda$}4686 Emission in the Dense Shell of the Peculiar Type Ib Supernova 2006jc}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0704.2249},
 keywords = {dust, extinction, stars: mass loss, stars: winds, outflows, stars: Wolf-Rayet, supernovae: individual: SN 2006jc},
     year = 2008,
    month = jun,
   volume = 680,
      eid = {568-579},
    pages = {568-579},
      doi = {10.1086/587860},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...680..568S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{1989LNP...350..164L,
   author = {{Lucy}, L.~B. and {Danziger}, I.~J. and {Gouiffes}, C. and {Bouchet}, P.
	},
    title = "{Dust Condensation in the Ejecta of SN 1987 A}",
booktitle = {IAU Colloq. 120: Structure and Dynamics of the Interstellar Medium},
     year = 1989,
   series = {Lecture Notes in Physics, Berlin Springer Verlag},
   volume = 350,
   editor = {{Tenorio-Tagle}, G. and {Moles}, M. and {Melnick}, J.},
    pages = {164},
      doi = {10.1007/BFb0114861},
   adsurl = {http://adsabs.harvard.edu/abs/1989LNP...350..164L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010A&A...518L.138B,
   author = {{Barlow}, M.~J. and {Krause}, O. and {Swinyard}, B.~M. and {Sibthorpe}, B. and 
	{Besel}, M.-A. and {Wesson}, R. and {Ivison}, R.~J. and {Dunne}, L. and 
	{Gear}, W.~K. and {Gomez}, H.~L. and {Hargrave}, P.~C. and {Henning}, T. and 
	{Leeks}, S.~J. and {Lim}, T.~L. and {Olofsson}, G. and {Polehampton}, E.~T.
	},
    title = "{A Herschel PACS and SPIRE study of the dust content of the Cassiopeia A supernova remnant}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1005.2688},
 keywords = {ISM: supernova remnants, dust, extinction, Infrared: ISM},
     year = 2010,
    month = jul,
   volume = 518,
      eid = {L138},
    pages = {L138},
      doi = {10.1051/0004-6361/201014585},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...518L.138B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2005ApJ...619...41S,
   author = {{Shang}, Z. and {Brotherton}, M.~S. and {Green}, R.~F. and {Kriss}, G.~A. and 
	{Scott}, J. and {Quijano}, J.~K. and {Blaes}, O. and {Hubeny}, I. and 
	{Hutchings}, J. and {Kaiser}, M.~E. and {Koratkar}, A. and {Oegerle}, W. and 
	{Zheng}, W.},
    title = "{Quasars and the Big Blue Bump}",
  journal = {\apj},
   eprint = {astro-ph/0409697},
 keywords = {Galaxies: Active, Galaxies: Nuclei, Galaxies: Quasars: General, Ultraviolet: General},
     year = 2005,
    month = jan,
   volume = 619,
    pages = {41-59},
      doi = {10.1086/426134},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...619...41S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011ApJ...742...24L,
   author = {{Lapi}, A. and {Gonz{\'a}lez-Nuevo}, J. and {Fan}, L. and {Bressan}, A. and 
	{De Zotti}, G. and {Danese}, L. and {Negrello}, M. and {Dunne}, L. and 
	{Eales}, S. and {Maddox}, S. and {Auld}, R. and {Baes}, M. and 
	{Bonfield}, D.~G. and {Buttiglione}, S. and {Cava}, A. and {Clements}, D.~L. and 
	{Cooray}, A. and {Dariush}, A. and {Dye}, S. and {Fritz}, J. and 
	{Herranz}, D. and {Hopwood}, R. and {Ibar}, E. and {Ivison}, R. and 
	{Jarvis}, M.~J. and {Kaviraj}, S. and {L{\'o}pez-Caniego}, M. and 
	{Massardi}, M. and {Micha{\l}owski}, M.~J. and {Pascale}, E. and 
	{Pohlen}, M. and {Rigby}, E. and {Rodighiero}, G. and {Serjeant}, S. and 
	{Smith}, D.~J.~B. and {Temi}, P. and {Wardlow}, J. and {van der Werf}, P.
	},
    title = "{Herschel-ATLAS Galaxy Counts and High-redshift Luminosity Functions: The Formation of Massive Early-type Galaxies}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1108.3911},
 keywords = {galaxies: evolution, galaxies: formation, galaxies: high-redshift, submillimeter: galaxies},
     year = 2011,
    month = nov,
   volume = 742,
      eid = {24},
    pages = {24},
      doi = {10.1088/0004-637X/742/1/24},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...742...24L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009ApJ...704..306K,
   author = {{Kotak}, R. and {Meikle}, W.~P.~S. and {Farrah}, D. and {Gerardy}, C.~L. and 
	{Foley}, R.~J. and {Van Dyk}, S.~D. and {Fransson}, C. and {Lundqvist}, P. and 
	{Sollerman}, J. and {Fesen}, R. and {Filippenko}, A.~V. and 
	{Mattila}, S. and {Silverman}, J.~M. and {Andersen}, A.~C. and 
	{H{\"o}flich}, P.~A. and {Pozzo}, M. and {Wheeler}, J.~C.},
    title = "{Dust and The Type II-Plateau Supernova 2004et}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0904.3737},
 primaryClass = "astro-ph.SR",
 keywords = {circumstellar matter, dust, extinction, supernovae: general, supernovae: individual: SN 2004et},
     year = 2009,
    month = oct,
   volume = 704,
    pages = {306-323},
      doi = {10.1088/0004-637X/704/1/306},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...704..306K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2006SPIE.6269E..33D,
   author = {{D'Odorico}, S. and {Dekker}, H. and {Mazzoleni}, R. and {Vernet}, J. and 
	{Guinouard}, I. and {Groot}, P. and {Hammer}, F. and {Rasmussen}, P.~K. and 
	{Kaper}, L. and {Navarro}, R. and {Pallavicini}, R. and {Peroux}, C. and 
	{Zerbi}, F.~M.},
    title = "{X-shooter UV- to K-band intermediate-resolution high-efficiency spectrograph for the VLT: status report at the final design review}",
booktitle = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
     year = 2006,
   series = {\procspie},
   volume = 6269,
    month = jun,
      eid = {626933},
    pages = {626933},
      doi = {10.1117/12.672969},
   adsurl = {http://adsabs.harvard.edu/abs/2006SPIE.6269E..33D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012ApJ...748..123S,
   author = {{Smith}, M.~W.~L. and {Gomez}, H.~L. and {Eales}, S.~A. and 
	{Ciesla}, L. and {Boselli}, A. and {Cortese}, L. and {Bendo}, G.~J. and 
	{Baes}, M. and {Bianchi}, S. and {Clemens}, M. and {Clements}, D.~L. and 
	{Cooray}, A.~R. and {Davies}, J.~I. and {De Looze}, I. and {di Serego Alighieri}, S. and 
	{Fritz}, J. and {Gavazzi}, G. and {Gear}, W.~K. and {Madden}, S. and 
	{Mentuch}, E. and {Panuzzo}, P. and {Pohlen}, M. and {Spinoglio}, L. and 
	{Verstappen}, J. and {Vlahakis}, C. and {Wilson}, C.~D. and 
	{Xilouris}, E.~M.},
    title = "{The Herschel Reference Survey: Dust in Early-type Galaxies and across the Hubble Sequence}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1112.1408},
 keywords = {galaxies: elliptical and lenticular, cD, galaxies: evolution, galaxies: ISM, submillimeter: galaxies},
     year = 2012,
    month = apr,
   volume = 748,
      eid = {123},
    pages = {123},
      doi = {10.1088/0004-637X/748/2/123},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...748..123S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014ApJ...782L...2I,
   author = {{Indebetouw}, R. and {Matsuura}, M. and {Dwek}, E. and {Zanardo}, G. and 
	{Barlow}, M.~J. and {Baes}, M. and {Bouchet}, P. and {Burrows}, D.~N. and 
	{Chevalier}, R. and {Clayton}, G.~C. and {Fransson}, C. and 
	{Gaensler}, B. and {Kirshner}, R. and {Laki{\'c}evi{\'c}}, M. and 
	{Long}, K.~S. and {Lundqvist}, P. and {Mart{\'{\i}}-Vidal}, I. and 
	{Marcaide}, J. and {McCray}, R. and {Meixner}, M. and {Ng}, C.-Y. and 
	{Park}, S. and {Sonneborn}, G. and {Staveley-Smith}, L. and 
	{Vlahakis}, C. and {van Loon}, J.},
    title = "{Dust Production and Particle Acceleration in Supernova 1987A Revealed with ALMA}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1312.4086},
 primaryClass = "astro-ph.SR",
 keywords = {galaxies: ISM, ISM: supernova remnants, Magellanic Clouds, supernovae: individual: 1987A},
     year = 2014,
    month = feb,
   volume = 782,
      eid = {L2},
    pages = {L2},
      doi = {10.1088/2041-8205/782/1/L2},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...782L...2I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011MNRAS.416.1916V,
   author = {{Valiante}, R. and {Schneider}, R. and {Salvadori}, S. and {Bianchi}, S.
	},
    title = "{The origin of the dust in high-redshift quasars: the case of SDSS J1148+5251}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1106.1418},
 keywords = {stars: AGB and post-AGB, supernovae: general, dust, extinction, galaxies: evolution, galaxies: high-redshift, quasars: general},
     year = 2011,
    month = sep,
   volume = 416,
    pages = {1916-1935},
      doi = {10.1111/j.1365-2966.2011.19168.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.416.1916V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2005MNRAS.363L..31N,
   author = {{Nagashima}, M. and {Lacey}, C.~G. and {Okamoto}, T. and {Baugh}, C.~M. and 
	{Frenk}, C.~S. and {Cole}, S.},
    title = "{The metal enrichment of elliptical galaxies in hierarchical galaxy formation models}",
  journal = {\mnras},
   eprint = {astro-ph/0504618},
 keywords = {stars: luminosity function, mass function, galaxies: clusters: general, galaxies: formation, large-scale structure of Universe},
     year = 2005,
    month = oct,
   volume = 363,
    pages = {L31-L35},
      doi = {10.1111/j.1745-3933.2005.00078.x},
   adsurl = {http://adsabs.harvard.edu/abs/2005MNRAS.363L..31N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011A&ARv..19...43G,
   author = {{Gall}, C. and {Hjorth}, J. and {Andersen}, A.~C.},
    title = "{Production of dust by massive stars at high redshift}",
  journal = {\aapr},
archivePrefix = "arXiv",
   eprint = {1108.0403},
 primaryClass = "astro-ph.CO",
 keywords = {Galaxies: high-redshift, ISM: evolution, Quasars: general, Stars: AGB and post-AGB, Stars: massive, Supernovae: general},
     year = 2011,
    month = sep,
   volume = 19,
      eid = {43},
    pages = {43},
      doi = {10.1007/s00159-011-0043-7},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26ARv..19...43G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011ApJ...738...89S,
   author = {{Skibba}, R.~A. and {Engelbracht}, C.~W. and {Dale}, D. and 
	{Hinz}, J. and {Zibetti}, S. and {Crocker}, A. and {Groves}, B. and 
	{Hunt}, L. and {Johnson}, B.~D. and {Meidt}, S. and {Murphy}, E. and 
	{Appleton}, P. and {Armus}, L. and {Bolatto}, A. and {Brandl}, B. and 
	{Calzetti}, D. and {Croxall}, K. and {Galametz}, M. and {Gordon}, K.~D. and 
	{Kennicutt}, R.~C. and {Koda}, J. and {Krause}, O. and {Montiel}, E. and 
	{Rix}, H.-W. and {Roussel}, H. and {Sandstrom}, K. and {Sauvage}, M. and 
	{Schinnerer}, E. and {Smith}, J.~D. and {Walter}, F. and {Wilson}, C.~D. and 
	{Wolfire}, M.},
    title = "{The Emission by Dust and Stars of Nearby Galaxies in the Herschel KINGFISH Survey}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1106.4022},
 keywords = {dust, extinction, galaxies: evolution, galaxies: general, galaxies: ISM, galaxies: photometry, infrared: galaxies},
     year = 2011,
    month = sep,
   volume = 738,
      eid = {89},
    pages = {89},
      doi = {10.1088/0004-637X/738/1/89},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...738...89S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011A&A...530A..44J,
   author = {{Jones}, A.~P. and {Nuth}, J.~A.},
    title = "{Dust destruction in the ISM: a re-evaluation of dust lifetimes}",
  journal = {\aap},
 keywords = {ISM: abundances, dust, extinction},
     year = 2011,
    month = jun,
   volume = 530,
      eid = {A44},
    pages = {A44},
      doi = {10.1051/0004-6361/201014440},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...530A..44J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2003ApJ...587L..67F,
   author = {{Freudling}, W. and {Corbin}, M.~R. and {Korista}, K.~T.},
    title = "{Iron Emission in z\~{}6 QSOS}",
  journal = {\apjl},
   eprint = {astro-ph/0303424},
 keywords = {Cosmology: Observations, Galaxies: Quasars: Emission Lines, Galaxies: Quasars: Individual: Alphanumeric: SDSS J083643.85+005453.3, Galaxies: Quasars: Individual: Alphanumeric: SDSS J103027.10+052455.0, Galaxies: Quasars: Individual: Alphanumeric: SDSS J104433.04-012502.2},
     year = 2003,
    month = apr,
   volume = 587,
    pages = {L67-L70},
      doi = {10.1086/375338},
   adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...587L..67F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010ApJ...713....1C,
   author = {{Cherchneff}, I. and {Dwek}, E.},
    title = "{The Chemistry of Population III Supernova Ejecta. II. The Nucleation of Molecular Clusters as a Diagnostic for Dust in the Early Universe}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1002.3060},
 primaryClass = "astro-ph.SR",
 keywords = {astrochemistry, dust, extinction, early universe, molecular processes, supernovae: general},
     year = 2010,
    month = apr,
   volume = 713,
    pages = {1-24},
      doi = {10.1088/0004-637X/713/1/1},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...713....1C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2002ApJ...572..350F,
   author = {{Fransson}, C. and {Chevalier}, R.~A. and {Filippenko}, A.~V. and 
	{Leibundgut}, B. and {Barth}, A.~J. and {Fesen}, R.~A. and {Kirshner}, R.~P. and 
	{Leonard}, D.~C. and {Li}, W. and {Lundqvist}, P. and {Sollerman}, J. and 
	{Van Dyk}, S.~D.},
    title = "{Optical and Ultraviolet Spectroscopy of SN 1995N: Evidence for Strong Circumstellar Interaction}",
  journal = {\apj},
   eprint = {astro-ph/0108149},
 keywords = {Stars: Circumstellar Matter, Stars: Mass Loss, Stars: Supernovae: Individual: Alphanumeric: SN 1995N},
     year = 2002,
    month = jun,
   volume = 572,
    pages = {350-370},
      doi = {10.1086/340295},
   adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...572..350F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2006AJ....132.2127J,
   author = {{Jiang}, L. and {Fan}, X. and {Hines}, D.~C. and {Shi}, Y. and 
	{Vestergaard}, M. and {Bertoldi}, F. and {Brandt}, W.~N. and 
	{Carilli}, C.~L. and {Cox}, P. and {Le Floc'h}, E. and {Pentericci}, L. and 
	{Richards}, G.~T. and {Rieke}, G.~H. and {Schneider}, D.~P. and 
	{Strauss}, M.~A. and {Walter}, F. and {Brinkmann}, J.},
    title = "{Probing the Evolution of Infrared Properties of z \~{} 6 Quasars: Spitzer Observations}",
  journal = {\aj},
   eprint = {astro-ph/0608006},
 keywords = {Galaxies: Active, Infrared: Galaxies, Galaxies: Quasars: General, quasars: individual (SDSS J000552.34-000655.8)},
     year = 2006,
    month = nov,
   volume = 132,
    pages = {2127-2134},
      doi = {10.1086/508209},
   adsurl = {http://adsabs.harvard.edu/abs/2006AJ....132.2127J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014ApJ...782...68T,
   author = {{Toft}, S. and {Smol{\v c}i{\'c}}, V. and {Magnelli}, B. and 
	{Karim}, A. and {Zirm}, A. and {Michalowski}, M. and {Capak}, P. and 
	{Sheth}, K. and {Schawinski}, K. and {Krogager}, J.-K. and {Wuyts}, S. and 
	{Sanders}, D. and {Man}, A.~W.~S. and {Lutz}, D. and {Staguhn}, J. and 
	{Berta}, S. and {Mccracken}, H. and {Krpan}, J. and {Riechers}, D.
	},
    title = "{Submillimeter Galaxies as Progenitors of Compact Quiescent Galaxies}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1401.1510},
 keywords = {cosmology: observations, galaxies: evolution, galaxies: high-redshift, galaxies: starburst, Galaxy: formation, submillimeter: galaxies},
     year = 2014,
    month = feb,
   volume = 782,
      eid = {68},
    pages = {68},
      doi = {10.1088/0004-637X/782/2/68},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...782...68T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012Natur.484..220N,
   author = {{Norris}, B.~R.~M. and {Tuthill}, P.~G. and {Ireland}, M.~J. and 
	{Lacour}, S. and {Zijlstra}, A.~A. and {Lykou}, F. and {Evans}, T.~M. and 
	{Stewart}, P. and {Bedding}, T.~R.},
    title = "{A close halo of large transparent grains around extreme red giant stars}",
  journal = {\nat},
archivePrefix = "arXiv",
   eprint = {1204.2640},
 primaryClass = "astro-ph.SR",
     year = 2012,
    month = apr,
   volume = 484,
    pages = {220-222},
      doi = {10.1038/nature10935},
   adsurl = {http://adsabs.harvard.edu/abs/2012Natur.484..220N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010AJ....139.2330W,
   author = {{Wachter}, S. and {Mauerhan}, J.~C. and {Van Dyk}, S.~D. and 
	{Hoard}, D.~W. and {Kafka}, S. and {Morris}, P.~W.},
    title = "{A Hidden Population of Massive Stars with Circumstellar Shells Discovered with the Spitzer Space Telescope}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1004.0399},
 keywords = {circumstellar matter, ISM: bubbles, stars: early-type, stars: emission-line, Be, stars: mass-loss, stars: Wolf-Rayet},
     year = 2010,
    month = jun,
   volume = 139,
    pages = {2330-2346},
      doi = {10.1088/0004-6256/139/6/2330},
   adsurl = {http://adsabs.harvard.edu/abs/2010AJ....139.2330W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009A&A...502..845O,
   author = {{Ormel}, C.~W. and {Paszun}, D. and {Dominik}, C. and {Tielens}, A.~G.~G.~M.
	},
    title = "{Dust coagulation and fragmentation in molecular clouds. I. How collisions between dust aggregates alter the dust size distribution}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0906.1770},
 primaryClass = "astro-ph.SR",
 keywords = {ISM: dust, extinction, ISM: clouds, turbulence, methods: numerical},
     year = 2009,
    month = aug,
   volume = 502,
    pages = {845-869},
      doi = {10.1051/0004-6361/200811158},
   adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...502..845O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1970Natur.226...62H,
   author = {{Hoyle}, F. and {Wickramasinghe}, N.~C.},
    title = "{Dust in Supernova Explosions}",
  journal = {\nat},
     year = 1970,
    month = apr,
   volume = 226,
    pages = {62-63},
      doi = {10.1038/226062a0},
   adsurl = {http://adsabs.harvard.edu/abs/1970Natur.226...62H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2004MNRAS.352..457P,
   author = {{Pozzo}, M. and {Meikle}, W.~P.~S. and {Fassia}, A. and {Geballe}, T. and 
	{Lundqvist}, P. and {Chugai}, N.~N. and {Sollerman}, J.},
    title = "{On the source of the late-time infrared luminosity of SN 1998S and other Type II supernovae}",
  journal = {\mnras},
   eprint = {astro-ph/0404533},
 keywords = {circumstellar matter, supernovae: general, supernovae: individual: SN 1998S, stars: winds, outflows, dust, extinction, infrared: stars},
     year = 2004,
    month = aug,
   volume = 352,
    pages = {457-477},
      doi = {10.1111/j.1365-2966.2004.07951.x},
   adsurl = {http://adsabs.harvard.edu/abs/2004MNRAS.352..457P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1998ApJ...499..267T,
   author = {{Tielens}, A.~G.~G.~M.},
    title = "{Interstellar Depletions and the Life Cycle of Interstellar Dust}",
  journal = {\apj},
 keywords = {ISM: DUST, EXTINCTION, ISM: ABUNDANCES, ISM: CLOUDS, ISM: Dust, Extinction, ISM: Abundances, ISM: Clouds},
     year = 1998,
    month = may,
   volume = 499,
    pages = {267-272},
      doi = {10.1086/305640},
   adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...499..267T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010MNRAS.403.1894D,
   author = {{da Cunha}, E. and {Eminian}, C. and {Charlot}, S. and {Blaizot}, J.
	},
    title = "{New insight into the relation between star formation activity and dust content in galaxies}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1001.2309},
 keywords = {dust, extinction, galaxies: evolution, galaxies: ISM, galaxies: statistics, galaxies: stellar content},
     year = 2010,
    month = apr,
   volume = 403,
    pages = {1894-1908},
      doi = {10.1111/j.1365-2966.2010.16344.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.403.1894D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012ApJ...760...96G,
   author = {{Gomez}, H.~L. and {Krause}, O. and {Barlow}, M.~J. and {Swinyard}, B.~M. and 
	{Owen}, P.~J. and {Clark}, C.~J.~R. and {Matsuura}, M. and {Gomez}, E.~L. and 
	{Rho}, J. and {Besel}, M.-A. and {Bouwman}, J. and {Gear}, W.~K. and 
	{Henning}, T. and {Ivison}, R.~J. and {Polehampton}, E.~T. and 
	{Sibthorpe}, B.},
    title = "{A Cool Dust Factory in the Crab Nebula: A Herschel Study of the Filaments}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1209.5677},
 keywords = {dust, extinction, ISM: individual objects: Crab Nebula, ISM: supernova remnants, submillimeter: ISM},
     year = 2012,
    month = nov,
   volume = 760,
      eid = {96},
    pages = {96},
      doi = {10.1088/0004-637X/760/1/96},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...760...96G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2003MNRAS.344L..74P,
   author = {{Priddey}, R.~S. and {Isaak}, K.~G. and {McMahon}, R.~G. and 
	{Robson}, E.~I. and {Pearson}, C.~P.},
    title = "{Quasars as probes of the submillimetre cosmos at z $\gt$ 5 - I. Preliminary SCUBA photometry}",
  journal = {\mnras},
   eprint = {astro-ph/0308132},
 keywords = {dust, extinction, galaxies: high-redshift, quasars: general, cosmology: observations, submillimetre},
     year = 2003,
    month = oct,
   volume = 344,
    pages = {L74-L78},
      doi = {10.1046/j.1365-8711.2003.07076.x},
   adsurl = {http://adsabs.harvard.edu/abs/2003MNRAS.344L..74P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012ApJ...755....5G,
   author = {{Goulding}, A.~D. and {Alexander}, D.~M. and {Bauer}, F.~E. and 
	{Forman}, W.~R. and {Hickox}, R.~C. and {Jones}, C. and {Mullaney}, J.~R. and 
	{Trichas}, M.},
    title = "{Deep Silicate Absorption Features in Compton-thick Active Galactic Nuclei Predominantly Arise due to Dust in the Host Galaxy}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1205.1800},
 keywords = {galaxies: active, galaxies: Seyfert, infrared: galaxies, X-rays: galaxies},
     year = 2012,
    month = aug,
   volume = 755,
      eid = {5},
    pages = {5},
      doi = {10.1088/0004-637X/755/1/5},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...755....5G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2008A&A...479..669C,
   author = {{Calura}, F. and {Pipino}, A. and {Matteucci}, F.},
    title = "{The cycle of interstellar dust in galaxies of different morphological types}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0706.2197},
 keywords = {ISM: dust, extinction, ISM: abundances, galaxies: abundances, galaxies: evolution},
     year = 2008,
    month = mar,
   volume = 479,
    pages = {669-685},
      doi = {10.1051/0004-6361:20078090},
   adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...479..669C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010A&A...523A..85G,
   author = {{Gallerani}, S. and {Maiolino}, R. and {Juarez}, Y. and {Nagao}, T. and 
	{Marconi}, A. and {Bianchi}, S. and {Schneider}, R. and {Mannucci}, F. and 
	{Oliva}, T. and {Willott}, C.~J. and {Jiang}, L. and {Fan}, X.
	},
    title = "{The extinction law at high redshift and its implications}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1006.4463},
 keywords = {dust, extinction, galaxies: ISM, intergalactic medium},
     year = 2010,
    month = nov,
   volume = 523,
      eid = {A85},
    pages = {A85},
      doi = {10.1051/0004-6361/201014721},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...523A..85G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2007MNRAS.375..753E,
   author = {{Ercolano}, B. and {Barlow}, M.~J. and {Sugerman}, B.~E.~K.},
    title = "{Dust yields in clumpy supernova shells: SN 1987A revisited}",
  journal = {\mnras},
   eprint = {astro-ph/0611719},
 keywords = {supernovae: individual: SN 1987A},
     year = 2007,
    month = mar,
   volume = 375,
    pages = {753-763},
      doi = {10.1111/j.1365-2966.2006.11336.x},
   adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.375..753E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009AJ....137.4810S,
   author = {{Srinivasan}, S. and {Meixner}, M. and {Leitherer}, C. and {Vijh}, U. and 
	{Volk}, K. and {Blum}, R.~D. and {Babler}, B.~L. and {Block}, M. and 
	{Bracker}, S. and {Cohen}, M. and {Engelbracht}, C.~W. and {For}, B.-Q. and 
	{Gordon}, K.~D. and {Harris}, J. and {Hora}, J.~L. and {Indebetouw}, R. and 
	{Markwick-Kemper}, F. and {Meade}, M. and {Misselt}, K.~A. and 
	{Sewilo}, M. and {Whitney}, B.},
    title = "{The Mass Loss Return from Evolved Stars to the Large Magellanic Cloud: Empirical Relations for Excess Emission at 8 and 24 {$\mu$}m}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {0903.1661},
 primaryClass = "astro-ph.CO",
 keywords = {infrared: stars, Magellanic Clouds, stars: AGB and post-AGB, stars: carbon, stars: mass loss},
     year = 2009,
    month = jun,
   volume = 137,
    pages = {4810-4823},
      doi = {10.1088/0004-6256/137/6/4810},
   adsurl = {http://adsabs.harvard.edu/abs/2009AJ....137.4810S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2004MNRAS.351L..29R,
   author = {{Robson}, I. and {Priddey}, R.~S. and {Isaak}, K.~G. and {McMahon}, R.~G.
	},
    title = "{Submillimetre observations of z $\gt$ 6 quasars}",
  journal = {\mnras},
   eprint = {astro-ph/0405177},
 keywords = {dust, extinction, galaxies: high-redshift, quasars: general, submillimetre},
     year = 2004,
    month = jun,
   volume = 351,
    pages = {L29-L33},
      doi = {10.1111/j.1365-2966.2004.07923.x},
   adsurl = {http://adsabs.harvard.edu/abs/2004MNRAS.351L..29R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013MNRAS.432..653D,
   author = {{Dobbs}, C.~L. and {Pringle}, J.~E.},
    title = "{The exciting lives of giant molecular clouds}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1303.4995},
 keywords = {stars: formation, ISM: clouds, ISM: evolution, galaxies: ISM},
     year = 2013,
    month = jun,
   volume = 432,
    pages = {653-667},
      doi = {10.1093/mnras/stt508},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.432..653D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011ApJ...732...63S,
   author = {{Smith}, N. and {Li}, W. and {Miller}, A.~A. and {Silverman}, J.~M. and 
	{Filippenko}, A.~V. and {Cuillandre}, J.-C. and {Cooper}, M.~C. and 
	{Matheson}, T. and {Van Dyk}, S.~D.},
    title = "{A Massive Progenitor of the Luminous Type IIn Supernova 2010jl}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1011.4150},
 primaryClass = "astro-ph.SR",
 keywords = {circumstellar matter, stars: evolution, stars: mass-loss, stars: winds, outflows, supernovae: general},
     year = 2011,
    month = may,
   volume = 732,
      eid = {63},
    pages = {63},
      doi = {10.1088/0004-637X/732/2/63},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...732...63S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012MNRAS.422.2246M,
   author = {{Marks}, M. and {Kroupa}, P. and {Dabringhausen}, J. and {Pawlowski}, M.~S.
	},
    title = "{Evidence for top-heavy stellar initial mass functions with increasing density and decreasing metallicity}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1202.4755},
 keywords = {stars: early-type, stars: formation, stars: late-type, stars: luminosity function, mass function, globular clusters: general},
     year = 2012,
    month = may,
   volume = 422,
    pages = {2246-2254},
      doi = {10.1111/j.1365-2966.2012.20767.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.422.2246M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2006SPIE.6269E..2KG,
   author = {{Goldoni}, P. and {Royer}, F. and {Fran{\c c}ois}, P. and {Horrobin}, M. and 
	{Blanc}, G. and {Vernet}, J. and {Modigliani}, A. and {Larsen}, J.
	},
    title = "{Data reduction software of the X-shooter spectrograph}",
booktitle = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
     year = 2006,
   series = {\procspie},
   volume = 6269,
    month = jun,
      eid = {62692K},
    pages = {62692K},
      doi = {10.1117/12.669986},
   adsurl = {http://adsabs.harvard.edu/abs/2006SPIE.6269E..2KG},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012A&A...548A..22M,
   author = {{Magnelli}, B. and {Saintonge}, A. and {Lutz}, D. and {Tacconi}, L.~J. and 
	{Berta}, S. and {Bournaud}, F. and {Charmandaris}, V. and {Dannerbauer}, H. and 
	{Elbaz}, D. and {F{\"o}rster-Schreiber}, N.~M. and {Graci{\'a}-Carpio}, J. and 
	{Ivison}, R. and {Maiolino}, R. and {Nordon}, R. and {Popesso}, P. and 
	{Rodighiero}, G. and {Santini}, P. and {Wuyts}, S.},
    title = "{Dust temperature and CO {\rarr} H$_{2}$ conversion factor variations in the SFR-M$_{???}$ plane}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1210.2760},
 keywords = {galaxies: evolution, infrared: galaxies, galaxies: starburst},
     year = 2012,
    month = dec,
   volume = 548,
      eid = {A22},
    pages = {A22},
      doi = {10.1051/0004-6361/201220074},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...548A..22M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010A&A...522A..15M,
   author = {{Micha{\l}owski}, M.~J. and {Murphy}, E.~J. and {Hjorth}, J. and 
	{Watson}, D. and {Gall}, C. and {Dunlop}, J.~S.},
    title = "{Dust grain growth in the interstellar medium of 5 $\lt$ z $\lt$ 6.5 quasars}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1006.5466},
 keywords = {dust, extinction, galaxies: high-redshift, galaxies: ISM, submillimeter: galaxies, quasars: general},
     year = 2010,
    month = nov,
   volume = 522,
      eid = {A15},
    pages = {A15},
      doi = {10.1051/0004-6361/201014902},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...522A..15M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2007ApJ...661L...9S,
   author = {{Stratta}, G. and {Maiolino}, R. and {Fiore}, F. and {D'Elia}, V.
	},
    title = "{Dust Properties at z = 6.3 in the Host Galaxy of GRB 050904}",
  journal = {\apjl},
   eprint = {astro-ph/0703349},
 keywords = {ISM: Dust, Extinction, Galaxies: High-Redshift, Galaxies: ISM, Gamma Rays: Bursts},
     year = 2007,
    month = may,
   volume = 661,
    pages = {L9-L12},
      doi = {10.1086/518502},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...661L...9S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2003MNRAS.339.1183P,
   author = {{Priddey}, R.~S. and {Isaak}, K.~G. and {McMahon}, R.~G. and 
	{Omont}, A.},
    title = "{The SCUBA Bright Quasar Survey (SBQS) - II. Unveiling the quasar epoch at submillimetre wavelengths}",
  journal = {\mnras},
   eprint = {astro-ph/0211646},
 keywords = {dust, extinction, quasars: general, galaxies: starburst, cosmology: observations, submillimetre},
     year = 2003,
    month = mar,
   volume = 339,
    pages = {1183-1188},
      doi = {10.1046/j.1365-8711.2003.06279.x},
   adsurl = {http://adsabs.harvard.edu/abs/2003MNRAS.339.1183P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012MNRAS.424..951H,
   author = {{Hayward}, C.~C. and {Jonsson}, P. and {Kere{\v s}}, D. and 
	{Magnelli}, B. and {Hernquist}, L. and {Cox}, T.~J.},
    title = "{How to distinguish starbursts and quiescently star-forming galaxies: the 'bimodal' submillimetre galaxy population as a case study}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1203.1318},
 primaryClass = "astro-ph.CO",
 keywords = {radiative transfer, stars: formation, galaxies: high-redshift, galaxies: starburst, infrared: galaxies, submillimetre: galaxies},
     year = 2012,
    month = aug,
   volume = 424,
    pages = {951-970},
      doi = {10.1111/j.1365-2966.2012.21254.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.424..951H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2008Natur.454..492K,
   author = {{Kishimoto}, M. and {Antonucci}, R. and {Blaes}, O. and {Lawrence}, A. and 
	{Boisson}, C. and {Albrecht}, M. and {Leipski}, C.},
    title = "{The characteristic blue spectra of accretion disks in quasars as uncovered in the infrared}",
  journal = {\nat},
archivePrefix = "arXiv",
   eprint = {0807.3703},
     year = 2008,
    month = jul,
   volume = 454,
    pages = {492-494},
      doi = {10.1038/nature07114},
   adsurl = {http://adsabs.harvard.edu/abs/2008Natur.454..492K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2002ApJ...574..719M,
   author = {{Motta}, V. and {Mediavilla}, E. and {Mu{\~n}oz}, J.~A. and 
	{Falco}, E. and {Kochanek}, C.~S. and {Arribas}, S. and {Garc{\'{\i}}a-Lorenzo}, B. and 
	{Oscoz}, A. and {Serra-Ricart}, M.},
    title = "{Detection of the 2175 {\AA} Extinction Feature at z = 0.83}",
  journal = {\apj},
   eprint = {astro-ph/0204130},
 keywords = {ISM: Dust, Extinction, Cosmology: Gravitational Lensing, Galaxies: Quasars: Individual: Alphanumeric: SBS 0909+532},
     year = 2002,
    month = aug,
   volume = 574,
    pages = {719-725},
      doi = {10.1086/341118},
   adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...574..719M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012ApJ...748...40B,
   author = {{Boyer}, M.~L. and {Srinivasan}, S. and {Riebel}, D. and {McDonald}, I. and 
	{van Loon}, J.~T. and {Clayton}, G.~C. and {Gordon}, K.~D. and 
	{Meixner}, M. and {Sargent}, B.~A. and {Sloan}, G.~C.},
    title = "{The Dust Budget of the Small Magellanic Cloud: Are Asymptotic Giant Branch Stars the Primary Dust Source at Low Metallicity?}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1201.5384},
 primaryClass = "astro-ph.SR",
 keywords = {dust, extinction, Magellanic Clouds, stars: AGB and post-AGB, supernovae: general},
     year = 2012,
    month = mar,
   volume = 748,
      eid = {40},
    pages = {40},
      doi = {10.1088/0004-637X/748/1/40},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...748...40B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012MNRAS.419.2545R,
   author = {{Rowlands}, K. and {Dunne}, L. and {Maddox}, S. and {Bourne}, N. and 
	{Gomez}, H.~L. and {Kaviraj}, S. and {Bamford}, S.~P. and {Brough}, S. and 
	{Charlot}, S. and {da Cunha}, E. and {Driver}, S.~P. and {Eales}, S.~A. and 
	{Hopkins}, A.~M. and {Kelvin}, L. and {Nichol}, R.~C. and {Sansom}, A.~E. and 
	{Sharp}, R. and {Smith}, D.~J.~B. and {Temi}, P. and {van der Werf}, P. and 
	{Baes}, M. and {Cava}, A. and {Cooray}, A. and {Croom}, S.~M. and 
	{Dariush}, A. and {de Zotti}, G. and {Dye}, S. and {Fritz}, J. and 
	{Hopwood}, R. and {Ibar}, E. and {Ivison}, R.~J. and {Liske}, J. and 
	{Loveday}, J. and {Madore}, B. and {Norberg}, P. and {Popescu}, C.~C. and 
	{Rigby}, E.~E. and {Robotham}, A. and {Rodighiero}, G. and {Seibert}, M. and 
	{Tuffs}, R.~J.},
    title = "{Herschel-ATLAS/GAMA: dusty early-type galaxies and passive spirals}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1109.6274},
 keywords = {dust, extinction, galaxies: elliptical and lenticular, cD, galaxies: evolution, infrared: galaxies, submillimetre: galaxies},
     year = 2012,
    month = jan,
   volume = 419,
    pages = {2545-2578},
      doi = {10.1111/j.1365-2966.2011.19905.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.419.2545R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011ApJ...730...34S,
   author = {{Stoll}, R. and {Prieto}, J.~L. and {Stanek}, K.~Z. and {Pogge}, R.~W. and 
	{Szczygie{\l}}, D.~M. and {Pojma{\'n}ski}, G. and {Antognini}, J. and 
	{Yan}, H.},
    title = "{SN 2010jl in UGC 5189: Yet Another Luminous Type IIn Supernova in a Metal-poor Galaxy}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1012.3461},
 keywords = {galaxies: abundances, stars: massive, supernovae: general, supernovae: individual: SN 2010jl SN 2010gx},
     year = 2011,
    month = mar,
   volume = 730,
      eid = {34},
    pages = {34},
      doi = {10.1088/0004-637X/730/1/34},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...730...34S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2001MNRAS.328..223E,
   author = {{Edmunds}, M.~G.},
    title = "{An elementary model for the dust cycle in galaxies}",
  journal = {\mnras},
 keywords = {ISM: ABUNDANCES, DUST, EXTINCTION, GALAXIES: EVOLUTION, GALAXIES: ISM},
     year = 2001,
    month = nov,
   volume = 328,
    pages = {223-236},
      doi = {10.1046/j.1365-8711.2001.04859.x},
   adsurl = {http://adsabs.harvard.edu/abs/2001MNRAS.328..223E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1983ApJ...274..168D,
   author = {{Dwek}, E. and {A'Hearn}, M.~F. and {Becklin}, E.~E. and {Brown}, R.~H. and 
	{Capps}, R.~W. and {Dinerstein}, H.~L. and {Gatley}, I. and 
	{Morrison}, D. and {Telesco}, C.~M. and {Tokunaga}, A.~T. and 
	{Werner}, M.~W. and {Wynn-Williams}, C.~G.},
    title = "{The evolution of the infrared emission from the Type II supernova 1980k in NGC 6946 - The dust formation model}",
  journal = {\apj},
 keywords = {Astronomical Models, Cosmic Dust, Infrared Radiation, Spiral Galaxies, Stellar Evolution, Supernovae, Astronomical Photometry, Cosmology, Stellar Atmospheres, Thermal Emission},
     year = 1983,
    month = nov,
   volume = 274,
    pages = {168-174},
      doi = {10.1086/161434},
   adsurl = {http://adsabs.harvard.edu/abs/1983ApJ...274..168D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010Natur.464..380J,
   author = {{Jiang}, L. and {Fan}, X. and {Brandt}, W.~N. and {Carilli}, C.~L. and 
	{Egami}, E. and {Hines}, D.~C. and {Kurk}, J.~D. and {Richards}, G.~T. and 
	{Shen}, Y. and {Strauss}, M.~A. and {Vestergaard}, M. and {Walter}, F.
	},
    title = "{Dust-free quasars in the early Universe}",
  journal = {\nat},
archivePrefix = "arXiv",
   eprint = {1003.3432},
 primaryClass = "astro-ph.CO",
     year = 2010,
    month = mar,
   volume = 464,
    pages = {380-383},
      doi = {10.1038/nature08877},
   adsurl = {http://adsabs.harvard.edu/abs/2010Natur.464..380J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013AJ....146...62M,
   author = {{Meixner}, M. and {Panuzzo}, P. and {Roman-Duval}, J. and {Engelbracht}, C. and 
	{Babler}, B. and {Seale}, J. and {Hony}, S. and {Montiel}, E. and 
	{Sauvage}, M. and {Gordon}, K. and {Misselt}, K. and {Okumura}, K. and 
	{Chanial}, P. and {Beck}, T. and {Bernard}, J.-P. and {Bolatto}, A. and 
	{Bot}, C. and {Boyer}, M.~L. and {Carlson}, L.~R. and {Clayton}, G.~C. and 
	{Chen}, C.-H.~R. and {Cormier}, D. and {Fukui}, Y. and {Galametz}, M. and 
	{Galliano}, F. and {Hora}, J.~L. and {Hughes}, A. and {Indebetouw}, R. and 
	{Israel}, F.~P. and {Kawamura}, A. and {Kemper}, F. and {Kim}, S. and 
	{Kwon}, E. and {Lebouteiller}, V. and {Li}, A. and {Long}, K.~S. and 
	{Madden}, S.~C. and {Matsuura}, M. and {Muller}, E. and {Oliveira}, J.~M. and 
	{Onishi}, T. and {Otsuka}, M. and {Paradis}, D. and {Poglitsch}, A. and 
	{Reach}, W.~T. and {Robitaille}, T.~P. and {Rubio}, M. and {Sargent}, B. and 
	{Sewi{\l}o}, M. and {Skibba}, R. and {Smith}, L.~J. and {Srinivasan}, S. and 
	{Tielens}, A.~G.~G.~M. and {van Loon}, J.~T. and {Whitney}, B.
	},
    title = "{The HERSCHEL Inventory of The Agents of Galaxy Evolution in the Magellanic Clouds, a Herschel Open Time Key Program}",
  journal = {\aj},
 keywords = {catalogs, dust, extinction, infrared: galaxies, Magellanic Clouds, submillimeter: general, surveys },
     year = 2013,
    month = sep,
   volume = 146,
      eid = {62},
    pages = {62},
      doi = {10.1088/0004-6256/146/3/62},
   adsurl = {http://adsabs.harvard.edu/abs/2013AJ....146...62M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2008MNRAS.389..141M,
   author = {{Mattila}, S. and {Meikle}, W.~P.~S. and {Lundqvist}, P. and 
	{Pastorello}, A. and {Kotak}, R. and {Eldridge}, J. and {Smartt}, S. and 
	{Adamson}, A. and {Gerardy}, C.~L. and {Rizzi}, L. and {Stephens}, A.~W. and 
	{van Dyk}, S.~D.},
    title = "{Massive stars exploding in a He-rich circumstellar medium - III. SN 2006jc: infrared echoes from new and old dust in the progenitor CSM}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0803.2145},
 keywords = {circumstellar matter , supernovae: general , supernovae: individual: SN 2006jc , dust, extinction},
     year = 2008,
    month = sep,
   volume = 389,
    pages = {141-155},
      doi = {10.1111/j.1365-2966.2008.13516.x},
   adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.389..141M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015ApJ...800...50M,
   author = {{Matsuura}, M. and {Dwek}, E. and {Barlow}, M.~J. and {Babler}, B. and 
	{Baes}, M. and {Meixner}, M. and {Cernicharo}, J. and {Clayton}, G.~C. and 
	{Dunne}, L. and {Fransson}, C. and {Fritz}, J. and {Gear}, W. and 
	{Gomez}, H.~L. and {Groenewegen}, M.~A.~T. and {Indebetouw}, R. and 
	{Ivison}, R.~J. and {Jerkstrand}, A. and {Lebouteiller}, V. and 
	{Lim}, T.~L. and {Lundqvist}, P. and {Pearson}, C.~P. and {Roman-Duval}, J. and 
	{Royer}, P. and {Staveley-Smith}, L. and {Swinyard}, B.~M. and 
	{van Hoof}, P.~A.~M. and {van Loon}, J.~T. and {Verstappen}, J. and 
	{Wesson}, R. and {Zanardo}, G. and {Blommaert}, J.~A.~D.~L. and 
	{Decin}, L. and {Reach}, W.~T. and {Sonneborn}, G. and {Van de Steene}, G.~C. and 
	{Yates}, J.~A.},
    title = "{A Stubbornly Large Mass of Cold Dust in the Ejecta of Supernova 1987A}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1411.7381},
 primaryClass = "astro-ph.SR",
 keywords = {dust, extinction, infrared: ISM, infrared: stars, ISM: supernova remnants, submillimeter: ISM, submillimeter: stars, supernovae: individual: Supernova 1987A},
     year = 2015,
    month = feb,
   volume = 800,
      eid = {50},
    pages = {50},
      doi = {10.1088/0004-637X/800/1/50},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...800...50M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013EP&S...65..213A,
   author = {{Asano}, R.~S. and {Takeuchi}, T.~T. and {Hirashita}, H. and 
	{Inoue}, A.~K.},
    title = "{Dust formation history of galaxies: A critical role of metallicity for the dust mass growth by accreting materials in the interstellar medium}",
  journal = {Earth, Planets, and Space},
archivePrefix = "arXiv",
   eprint = {1206.0817},
 keywords = {Dust, extinction, galaxies: infrared, galaxies: evolution, galaxies: starburst, stars: formation},
     year = 2013,
    month = mar,
   volume = 65,
    pages = {213-222},
      doi = {10.5047/eps.2012.04.014},
   adsurl = {http://adsabs.harvard.edu/abs/2013EP%26S...65..213A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010MNRAS.406.2473P,
   author = {{Perley}, D.~A. and {Bloom}, J.~S. and {Klein}, C.~R. and {Covino}, S. and 
	{Minezaki}, T. and {Wo{\'z}niak}, P. and {Vestrand}, W.~T. and 
	{Williams}, G.~G. and {Milne}, P. and {Butler}, N.~R. and {Updike}, A.~C. and 
	{Kr{\"u}hler}, T. and {Afonso}, P. and {Antonelli}, A. and {Cowie}, L. and 
	{Ferrero}, P. and {Greiner}, J. and {Hartmann}, D.~H. and {Kakazu}, Y. and 
	{K{\"u}pc{\"u} Yolda{\c s}}, A. and {Morgan}, A.~N. and {Price}, P.~A. and 
	{Prochaska}, J.~X. and {Yoshii}, Y.},
    title = "{Evidence for supernova-synthesized dust from the rising afterglow of GRB 071025 at z{\tilde} 5}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0912.2999},
 primaryClass = "astro-ph.HE",
 keywords = {dust, extinction, gamma-ray burst: general, gamma-ray burst: individual: 071025},
     year = 2010,
    month = aug,
   volume = 406,
    pages = {2473-2487},
      doi = {10.1111/j.1365-2966.2010.16772.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.406.2473P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012ApJ...754L..14S,
   author = {{Salmi}, F. and {Daddi}, E. and {Elbaz}, D. and {Sargent}, M.~T. and 
	{Dickinson}, M. and {Renzini}, A. and {Bethermin}, M. and {Le Borgne}, D.
	},
    title = "{Dissecting the Stellar-mass-SFR Correlation in z = 1 Star-forming Disk Galaxies}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1206.1704},
 keywords = {galaxies: fundamental parameters, galaxies: high-redshift, galaxies: structure, Galaxy: evolution, Galaxy: formation},
     year = 2012,
    month = jul,
   volume = 754,
      eid = {L14},
    pages = {L14},
      doi = {10.1088/2041-8205/754/1/L14},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...754L..14S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010A&A...523A..20B,
   author = {{Bot}, C. and {Ysard}, N. and {Paradis}, D. and {Bernard}, J.~P. and 
	{Lagache}, G. and {Israel}, F.~P. and {Wall}, W.~F.},
    title = "{Submillimeter to centimeter excess emission from the Magellanic Clouds. II. On the nature of the excess}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1008.2875},
 keywords = {Magellanic Clouds, submillimeter: ISM, radio continuum: ISM, galaxies: ISM},
     year = 2010,
    month = nov,
   volume = 523,
      eid = {A20},
    pages = {A20},
      doi = {10.1051/0004-6361/201014986},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...523A..20B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009MNRAS.394.1307D,
   author = {{Dunne}, L. and {Maddox}, S.~J. and {Ivison}, R.~J. and {Rudnick}, L. and 
	{Delaney}, T.~A. and {Matthews}, B.~C. and {Crowe}, C.~M. and 
	{Gomez}, H.~L. and {Eales}, S.~A. and {Dye}, S.},
    title = "{Cassiopeia A: dust factory revealed via submillimetre polarimetry}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0809.0887},
 keywords = {supernovae: individual: Cassiopeia A , dust, extinction , supernova remnants , submillimetre},
     year = 2009,
    month = apr,
   volume = 394,
    pages = {1307-1316},
      doi = {10.1111/j.1365-2966.2009.14453.x},
   adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.394.1307D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010A&A...518L.154S,
   author = {{Santini}, P. and {Maiolino}, R. and {Magnelli}, B. and {Silva}, L. and 
	{Grazian}, A. and {Altieri}, B. and {Andreani}, P. and {Aussel}, H. and 
	{Berta}, S. and {Bongiovanni}, A. and {Brisbin}, D. and {Calura}, F. and 
	{Cava}, A. and {Cepa}, J. and {Cimatti}, A. and {Daddi}, E. and 
	{Dannerbauer}, H. and {Dominguez-Sanchez}, H. and {Elbaz}, D. and 
	{Fontana}, A. and {F{\"o}rster Schreiber}, N. and {Genzel}, R. and 
	{Granato}, G.~L. and {Gruppioni}, C. and {Lutz}, D. and {Magdis}, G. and 
	{Magliocchetti}, M. and {Matteucci}, F. and {Nordon}, R. and 
	{P{\'e}rez Garcia}, I. and {Poglitsch}, A. and {Popesso}, P. and 
	{Pozzi}, F. and {Riguccini}, L. and {Rodighiero}, G. and {Saintonge}, A. and 
	{Sanchez-Portal}, M. and {Shao}, L. and {Sturm}, E. and {Tacconi}, L. and 
	{Valtchanov}, I.},
    title = "{The dust content of high-z submillimeter galaxies revealed by Herschel}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1005.5678},
 keywords = {galaxies: evolution, galaxies: high-redshift, galaxies: ISM, infrared: galaxies, submillimeter: galaxies},
     year = 2010,
    month = jul,
   volume = 518,
      eid = {L154},
    pages = {L154},
      doi = {10.1051/0004-6361/201014748},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...518L.154S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2007ApJ...668..682D,
   author = {{Davis}, S.~W. and {Woo}, J.-H. and {Blaes}, O.~M.},
    title = "{The UV Continuum of Quasars: Models and SDSS Spectral Slopes}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0707.1456},
 keywords = {Accretion, Accretion Disks, Black Hole Physics, Galaxies: Active, Galaxies: Quasars: General},
     year = 2007,
    month = oct,
   volume = 668,
    pages = {682-698},
      doi = {10.1086/521393},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...668..682D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014Natur.511..326G,
   author = {{Gall}, C. and {Hjorth}, J. and {Watson}, D. and {Dwek}, E. and 
	{Maund}, J.~R. and {Fox}, O. and {Leloudas}, G. and {Malesani}, D. and 
	{Day-Jones}, A.~C.},
    title = "{Rapid formation of large dust grains in the luminous supernova 2010jl}",
  journal = {\nat},
archivePrefix = "arXiv",
   eprint = {1407.4447},
 primaryClass = "astro-ph.SR",
     year = 2014,
    month = jul,
   volume = 511,
    pages = {326-329},
      doi = {10.1038/nature13558},
   adsurl = {http://adsabs.harvard.edu/abs/2014Natur.511..326G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2008ApJ...684.1343N,
   author = {{Nozawa}, T. and {Kozasa}, T. and {Tominaga}, N. and {Sakon}, I. and 
	{Tanaka}, M. and {Suzuki}, T. and {Nomoto}, K. and {Maeda}, K. and 
	{Umeda}, H. and {Limongi}, M. and {Onaka}, T.},
    title = "{Early Formation of Dust in the Ejecta of Type Ib SN 2006jc and Temperature and Mass of the Dust}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0801.2015},
 keywords = {dust, extinction, supernovae: general, supernovae: individual: SN 2006jc},
     year = 2008,
    month = sep,
   volume = 684,
      eid = {1343-1350},
    pages = {1343-1350},
      doi = {10.1086/589961},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...684.1343N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011A&A...525A..61P,
   author = {{Pipino}, A. and {Fan}, X.~L. and {Matteucci}, F. and {Calura}, F. and 
	{Silva}, L. and {Granato}, G. and {Maiolino}, R.},
    title = "{The chemical evolution of elliptical galaxies with stellar and QSO dust production}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1008.3875},
 keywords = {dust, extinction, quasars: individual: SDSS J114816, galaxies: elliptical and lenticular, cD, ISM: abundances, galaxies: evolution},
     year = 2011,
    month = jan,
   volume = 525,
      eid = {A61},
    pages = {A61},
      doi = {10.1051/0004-6361/201014843},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...525A..61P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2006MNRAS.368.1169P,
   author = {{Pozzo}, M. and {Meikle}, W.~P.~S. and {Rayner}, J.~T. and {Joseph}, R.~D. and 
	{Filippenko}, A.~V. and {Foley}, R.~J. and {Li}, W. and {Mattila}, S. and 
	{Sollerman}, J.},
    title = "{Optical and infrared observations of the TypeIIP SN2002hh from days 3 to 397}",
  journal = {\mnras},
   eprint = {astro-ph/0602372},
 keywords = {circumstellar matter , supernovae: individual: SN2002hh , infrared: stars},
     year = 2006,
    month = may,
   volume = 368,
    pages = {1169-1195},
      doi = {10.1111/j.1365-2966.2006.10204.x},
   adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.368.1169P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2006ApJ...642...87P,
   author = {{Pereyra}, N.~A. and {Vanden Berk}, D.~E. and {Turnshek}, D.~A. and 
	{Hillier}, D.~J. and {Wilhite}, B.~C. and {Kron}, R.~G. and 
	{Schneider}, D.~P. and {Brinkmann}, J.},
    title = "{Characteristic QSO Accretion Disk Temperatures from Spectroscopic Continuum Variability}",
  journal = {\apj},
   eprint = {astro-ph/0506006},
 keywords = {Accretion, Accretion Disks, Galaxies: Quasars: General, Ultraviolet: General},
     year = 2006,
    month = may,
   volume = 642,
    pages = {87-95},
      doi = {10.1086/500919},
   adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...642...87P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1995ApJS...99..223P,
   author = {{Pun}, C.~S.~J. and {Kirshner}, R.~P. and {Sonneborn}, G. and 
	{Challis}, P. and {Nassiopoulos}, G. and {Arquilla}, R. and 
	{Crenshaw}, D.~M. and {Shrader}, C. and {Teays}, T. and {Cassatella}, A. and 
	{Gilmozzi}, R. and {Talavera}, A. and {Wamsteker}, W. and {Fransson}, C. and 
	{Panagia}, N.},
    title = "{Ultraviolet Observations of SN 1987A with the IUE Satellite}",
  journal = {\apjs},
 keywords = {STARS: INDIVIDUAL ALPHANUMERIC: SN 1987A, ULTRAVIOLET: STARS},
     year = 1995,
    month = jul,
   volume = 99,
    pages = {223},
      doi = {10.1086/192185},
   adsurl = {http://adsabs.harvard.edu/abs/1995ApJS...99..223P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2001MNRAS.324L..17P,
   author = {{Priddey}, R.~S. and {McMahon}, R.~G.},
    title = "{The far-infrared-submillimetre spectral energy distribution of high-redshift quasars}",
  journal = {\mnras},
   eprint = {astro-ph/0102116},
 keywords = {DUST, EXTINCTION, QUASARS: GENERAL, GALAXIES: STARBURST, INFRARED: ISM, SUBMILLIMETRE},
     year = 2001,
    month = jun,
   volume = 324,
    pages = {L17-L22},
      doi = {10.1046/j.1365-8711.2001.04548.x},
   adsurl = {http://adsabs.harvard.edu/abs/2001MNRAS.324L..17P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012MNRAS.421.3027B,
   author = {{Bourne}, N. and {Maddox}, S.~J. and {Dunne}, L. and {Auld}, R. and 
	{Baes}, M. and {Baldry}, I.~K. and {Bonfield}, D.~G. and {Cooray}, A. and 
	{Croom}, S.~M. and {Dariush}, A. and {de Zotti}, G. and {Driver}, S.~P. and 
	{Dye}, S. and {Eales}, S. and {Gomez}, H.~L. and {Gonz{\'a}lez-Nuevo}, J. and 
	{Hopkins}, A.~M. and {Ibar}, E. and {Jarvis}, M.~J. and {Lapi}, A. and 
	{Madore}, B. and {Micha{\l}owski}, M.~J. and {Pohlen}, M. and 
	{Popescu}, C.~C. and {Rigby}, E.~E. and {Seibert}, M. and {Smith}, D.~J.~B. and 
	{Tuffs}, R.~J. and {van der Werf}, P. and {Brough}, S. and {Buttiglione}, S. and 
	{Cava}, A. and {Clements}, D.~L. and {Conselice}, C.~J. and 
	{Fritz}, J. and {Hopwood}, R. and {Ivison}, R.~J. and {Jones}, D.~H. and 
	{Kelvin}, L.~S. and {Liske}, J. and {Loveday}, J. and {Norberg}, P. and 
	{Robotham}, A.~S.~G. and {Rodighiero}, G. and {Temi}, P.},
    title = "{Herschel-ATLAS/GAMA: a census of dust in optically selected galaxies from stacking at submillimetre wavelengths}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1201.1916},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: evolution, galaxies: ISM, galaxies: statistics, submillimetre: diffuse background, submillimetre: galaxies},
     year = 2012,
    month = apr,
   volume = 421,
    pages = {3027-3059},
      doi = {10.1111/j.1365-2966.2012.20528.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.421.3027B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010ApJ...715.1575S,
   author = {{Silvia}, D.~W. and {Smith}, B.~D. and {Shull}, J.~M.},
    title = "{Numerical Simulations of Supernova Dust Destruction. I. Cloud-crushing and Post-processed Grain Sputtering}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1001.4793},
 keywords = {dust, extinction, hydrodynamics, ISM: supernova remnants, shock waves},
     year = 2010,
    month = jun,
   volume = 715,
    pages = {1575-1590},
      doi = {10.1088/0004-637X/715/2/1575},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...715.1575S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011ApJ...741...37K,
   author = {{Kochanek}, C.~S.},
    title = "{Dusty Explosions from Dusty Progenitors: The Physics of SN 2008S and the 2008 NGC 300-OT}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1106.4722},
 primaryClass = "astro-ph.SR",
 keywords = {stars: evolution, supergiants, supernovae: general, supernovae: individual: SN 2008S 2008 NGC 300-OT},
     year = 2011,
    month = nov,
   volume = 741,
      eid = {37},
    pages = {37},
      doi = {10.1088/0004-637X/741/1/37},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...741...37K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009A&A...495...83M,
   author = {{Marziani}, P. and {Sulentic}, J.~W. and {Stirpe}, G.~M. and 
	{Zamfir}, S. and {Calvani}, M.},
    title = "{VLT/ISAAC spectra of the H{$\beta$} region in intermediate-redshift quasars. III. H{$\beta$} broad-line profile analysis and inferences about BLR structure}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0812.0251},
 keywords = {galaxies: quasars: general, galaxies: quasars: emission lines, black hole physics, line: profiles},
     year = 2009,
    month = feb,
   volume = 495,
    pages = {83-112},
      doi = {10.1051/0004-6361:200810764},
   adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...495...83M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009ApJ...691..650F,
   author = {{Fox}, O. and {Skrutskie}, M.~F. and {Chevalier}, R.~A. and 
	{Kanneganti}, S. and {Park}, C. and {Wilson}, J. and {Nelson}, M. and 
	{Amirhadji}, J. and {Crump}, D. and {Hoeft}, A. and {Provence}, S. and 
	{Sargeant}, B. and {Sop}, J. and {Tea}, M. and {Thomas}, S. and 
	{Woolard}, K.},
    title = "{Near-Infrared Photometry of the Type IIn SN 2005ip: The Case for Dust Condensation}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0807.3555},
 keywords = {circumstellar matter, supernovae: general, supernovae: individual: SN 2005ip, dust, extinction, infrared: stars},
     year = 2009,
    month = jan,
   volume = 691,
    pages = {650-660},
      doi = {10.1088/0004-637X/691/1/650},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...691..650F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011A&A...528A..14G,
   author = {{Gall}, C. and {Andersen}, A.~C. and {Hjorth}, J.},
    title = "{Genesis and evolution of dust in galaxies in the early Universe. II. Rapid dust evolution in quasars at z {\gsim} 6}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1101.1553},
 keywords = {galaxies: high-redshift, galaxies: starburst, galaxies: evolution, evolution, quasars: general, stars: massive},
     year = 2011,
    month = apr,
   volume = 528,
      eid = {A14},
    pages = {A14},
      doi = {10.1051/0004-6361/201015605},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...528A..14G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011ApJ...743...21S,
   author = {{Simcoe}, R.~A. and {Cooksey}, K.~L. and {Matejek}, M. and {Burgasser}, A.~J. and 
	{Bochanski}, J. and {Lovegrove}, E. and {Bernstein}, R.~A. and 
	{Pipher}, J.~L. and {Forrest}, W.~J. and {McMurtry}, C. and 
	{Fan}, X. and {O'Meara}, J.},
    title = "{Constraints on the Universal C IV Mass Density at z \~{} 6 from Early Infrared Spectra Obtained with the Magellan FIRE Spectrograph}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1104.4117},
 keywords = {galaxies: high-redshift, intergalactic medium, quasars: absorption lines},
     year = 2011,
    month = dec,
   volume = 743,
      eid = {21},
    pages = {21},
      doi = {10.1088/0004-637X/743/1/21},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...743...21S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013MNRAS.434..102S,
   author = {{Smith}, N.},
    title = "{The Crab nebula and the class of Type IIn-P supernovae caused by sub-energetic electron-capture explosions}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1304.0689},
 primaryClass = "astro-ph.HE",
 keywords = {circumstellar matter, stars: evolution, stars: mass-loss, supernovae: individual: SN 1994W, supernovae: individual: SN 2009kn, supernovae: individual: SN 2011ht},
     year = 2013,
    month = sep,
   volume = 434,
    pages = {102-113},
      doi = {10.1093/mnras/stt1004},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.434..102S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011A&A...528A..13G,
   author = {{Gall}, C. and {Andersen}, A.~C. and {Hjorth}, J.},
    title = "{Genesis and evolution of dust in galaxies in the early Universe. I. Modelling dust evolution in starburst galaxies}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1011.3157},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: high-redshift, galaxies: starburst, galaxies: evolution, evolution, quasars: general, stars: massive},
     year = 2011,
    month = apr,
   volume = 528,
      eid = {A13},
    pages = {A13},
      doi = {10.1051/0004-6361/201015286},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...528A..13G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2006ApJS..166..443E,
   author = {{El{\'{\i}}asd{\'o}ttir}, {\'A}. and {Hjorth}, J. and {Toft}, S. and 
	{Burud}, I. and {Paraficz}, D.},
    title = "{Extinction Curves of Lensing Galaxies out to z = 1}",
  journal = {\apjs},
   eprint = {astro-ph/0606649},
 keywords = {ISM: Dust, Extinction, Galaxies: ISM, Cosmology: Gravitational Lensing},
     year = 2006,
    month = oct,
   volume = 166,
    pages = {443-469},
      doi = {10.1086/507131},
   adsurl = {http://adsabs.harvard.edu/abs/2006ApJS..166..443E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013A&A...555A..99Z,
   author = {{Zhukovska}, S. and {Henning}, T.},
    title = "{Dust input from AGB stars in the Large Magellanic Cloud}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1305.3521},
 keywords = {stars: AGB and post-AGB, stars: mass-loss, dust, extinction, galaxies: evolution, Magellanic Clouds},
     year = 2013,
    month = jul,
   volume = 555,
      eid = {A99},
    pages = {A99},
      doi = {10.1051/0004-6361/201321368},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...555A..99Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2005MNRAS.357.1077H,
   author = {{Hirashita}, H. and {Nozawa}, T. and {Kozasa}, T. and {Ishii}, T.~T. and 
	{Takeuchi}, T.~T.},
    title = "{Extinction curves expected in young galaxies}",
  journal = {\mnras},
   eprint = {astro-ph/0501158},
 keywords = {supernovae: general, dust, extinction, galaxies: evolution, galaxies: high-redshift, galaxies: ISM, quasars: individual: SDSS J104845.05+463718.3},
     year = 2005,
    month = mar,
   volume = 357,
    pages = {1077-1087},
      doi = {10.1111/j.1365-2966.2005.08730.x},
   adsurl = {http://adsabs.harvard.edu/abs/2005MNRAS.357.1077H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{1991supe.conf...82L,
   author = {{Lucy}, L.~B. and {Danziger}, I.~J. and {Gouiffes}, C. and {Bouchet}, P.
	},
    title = "{Dust Condensation in the Ejecta of Supernova 1987A - Part Two}",
booktitle = {Supernovae},
     year = 1991,
   editor = {{Woosley}, S.~E.},
    pages = {82},
   adsurl = {http://adsabs.harvard.edu/abs/1991supe.conf...82L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2007AJ....134..294S,
   author = {{Shang}, Z. and {Wills}, B.~J. and {Wills}, D. and {Brotherton}, M.~S.
	},
    title = "{Spectral Properties from Ly{$\alpha$} to H{$\alpha$} for an Essentially Complete Sample of Quasars. I. Data}",
  journal = {\aj},
   eprint = {astro-ph/0703690},
 keywords = {galaxies: active, galaxies: nuclei, quasars: general, ultraviolet: general},
     year = 2007,
    month = jul,
   volume = 134,
    pages = {294-393},
      doi = {10.1086/518505},
   adsurl = {http://adsabs.harvard.edu/abs/2007AJ....134..294S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012ApJ...758..142K,
   author = {{Kochanek}, C.~S. and {Szczygie{\l}}, D.~M. and {Stanek}, K.~Z.
	},
    title = "{Unmasking the Supernova Impostors}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1202.0281},
 primaryClass = "astro-ph.SR",
 keywords = {stars: evolution, supergiants, supernovae: general, supernovae: individual: SN 1954J SN 1961V SN 1997bs SN 1999bw SN 2000ch SN 2001ac},
     year = 2012,
    month = oct,
   volume = 758,
      eid = {142},
    pages = {142},
      doi = {10.1088/0004-637X/758/2/142},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...758..142K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012ApJ...754..116M,
   author = {{M{\'e}nard}, B. and {Fukugita}, M.},
    title = "{Cosmic Dust in Mg II Absorbers}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1204.1978},
 keywords = {dust, extinction, galaxies: halos, quasars: absorption lines},
     year = 2012,
    month = aug,
   volume = 754,
      eid = {116},
    pages = {116},
      doi = {10.1088/0004-637X/754/2/116},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...754..116M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012MNRAS.423..451L,
   author = {{Lawrence}, A.},
    title = "{The UV peak in active galactic nuclei: a false continuum from blurred reflection?}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1110.0854},
 keywords = {accretion, accretion discs, galaxies: active, quasars: emission lines},
     year = 2012,
    month = jun,
   volume = 423,
    pages = {451-463},
      doi = {10.1111/j.1365-2966.2012.20889.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.423..451L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013MNRAS.435.2274W,
   author = {{Weidner}, C. and {Ferreras}, I. and {Vazdekis}, A. and {La Barbera}, F.
	},
    title = "{The (galaxy-wide) IMF in giant elliptical galaxies: from top to bottom}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1306.6332},
 keywords = {stars: luminosity function, mass function, galaxies: evolution, galaxies: star formation, galaxies: stellar content},
     year = 2013,
    month = nov,
   volume = 435,
    pages = {2274-2280},
      doi = {10.1093/mnras/stt1445},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.435.2274W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012ApJ...751...25M,
   author = {{Milisavljevic}, D. and {Fesen}, R.~A. and {Chevalier}, R.~A. and 
	{Kirshner}, R.~P. and {Challis}, P. and {Turatto}, M.},
    title = "{Late-time Optical Emission from Core-collapse Supernovae}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1203.0006},
 primaryClass = "astro-ph.HE",
 keywords = {ISM: individual objects: Cassiopeia A, ISM: supernova remnants, supernovae: individual: SN 1957D SN 1970G SN 1980K SN 1993J, supernovae: general},
     year = 2012,
    month = may,
   volume = 751,
      eid = {25},
    pages = {25},
      doi = {10.1088/0004-637X/751/1/25},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...751...25M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012AJ....143...17S,
   author = {{Smith}, N. and {Silverman}, J.~M. and {Filippenko}, A.~V. and 
	{Cooper}, M.~C. and {Matheson}, T. and {Bian}, F. and {Weiner}, B.~J. and 
	{Comerford}, J.~M.},
    title = "{Systematic Blueshift of Line Profiles in the Type IIn Supernova 2010jl: Evidence for Post-shock Dust Formation?}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1108.2869},
 primaryClass = "astro-ph.HE",
 keywords = {circumstellar matter, dust, extinction, stars: evolution, stars: mass-loss, stars: winds, outflows, supernovae: general},
     year = 2012,
    month = jan,
   volume = 143,
      eid = {17},
    pages = {17},
      doi = {10.1088/0004-6256/143/1/17},
   adsurl = {http://adsabs.harvard.edu/abs/2012AJ....143...17S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2008MNRAS.389..333Y,
   author = {{Yun}, M.~S. and {Aretxaga}, I. and {Ashby}, M.~L.~N. and {Austermann}, J. and 
	{Fazio}, G.~G. and {Giavalisco}, M. and {Huang}, J.-S. and {Hughes}, D.~H. and 
	{Kim}, S. and {Lowenthal}, J.~D. and {Perera}, T. and {Scott}, K. and 
	{Wilson}, G. and {Younger}, J.~D.},
    title = "{Spitzer IRAC infrared colours of submillimetre-bright galaxies}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0806.2158},
 keywords = {galaxies: active , galaxies: evolution , galaxies: high-redshift , galaxies: starburst , cosmology: observations , infrared: galaxies},
     year = 2008,
    month = sep,
   volume = 389,
    pages = {333-340},
      doi = {10.1111/j.1365-2966.2008.13565.x},
   adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.389..333Y},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014MNRAS.442.1440S,
   author = {{Schneider}, R. and {Valiante}, R. and {Ventura}, P. and {dell'Agli}, F. and 
	{Di Criscienzo}, M. and {Hirashita}, H. and {Kemper}, F.},
    title = "{Dust production rate of asymptotic giant branch stars in the Magellanic Clouds}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1404.7132},
 keywords = {stars: AGB and post-AGB, supernovae: general, dust, extinction, ISM: evolution, Magellanic Clouds},
     year = 2014,
    month = aug,
   volume = 442,
    pages = {1440-1450},
      doi = {10.1093/mnras/stu861},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.442.1440S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012ApJ...752...98C,
   author = {{Calzetti}, D. and {Liu}, G. and {Koda}, J.},
    title = "{Star Formation Laws: The Effects of Gas Cloud Sampling}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1204.5659},
 keywords = {galaxies: ISM, ISM: structure, stars: formation },
     year = 2012,
    month = jun,
   volume = 752,
      eid = {98},
    pages = {98},
      doi = {10.1088/0004-637X/752/2/98},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...752...98C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011MNRAS.416.1340H,
   author = {{Hirashita}, H. and {Kuo}, T.-M.},
    title = "{Effects of grain size distribution on the interstellar dust mass growth}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1105.4930},
 keywords = {dust, extinction, galaxies: dwarf, galaxies: evolution, galaxies: ISM, galaxies: spiral, ISM: clouds},
     year = 2011,
    month = sep,
   volume = 416,
    pages = {1340-1353},
      doi = {10.1111/j.1365-2966.2011.19131.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.416.1340H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009ApJ...700..579R,
   author = {{Rho}, J. and {Reach}, W.~T. and {Tappe}, A. and {Hwang}, U. and 
	{Slavin}, J.~D. and {Kozasa}, T. and {Dunne}, L.},
    title = "{Spitzer Observations of the Young Core-Collapse Supernova Remnant 1E0102-72.3: Infrared Ejecta Emission and Dust Formation}",
  journal = {\apj},
 keywords = {dust, extinction, infrared: general, supernova remnants, supernovae: general},
     year = 2009,
    month = jul,
   volume = 700,
    pages = {579-596},
      doi = {10.1088/0004-637X/700/1/579},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...700..579R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2004ApJ...614...69I,
   author = {{Iwamuro}, F. and {Kimura}, M. and {Eto}, S. and {Maihara}, T. and 
	{Motohara}, K. and {Yoshii}, Y. and {Doi}, M.},
    title = "{Fe II/Mg II Emission-Line Ratios of QSOs. II. z $\gt$ 6 Objects}",
  journal = {\apj},
   eprint = {astro-ph/0408517},
 keywords = {Galaxies: Active, Infrared: General, Galaxies: Quasars: Emission Lines, Galaxies: Quasars: General},
     year = 2004,
    month = oct,
   volume = 614,
    pages = {69-74},
      doi = {10.1086/423610},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...614...69I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015MNRAS.446.2089W,
   author = {{Wesson}, R. and {Barlow}, M.~J. and {Matsuura}, M. and {Ercolano}, B.
	},
    title = "{The timing and location of dust formation in the remnant of SN 1987A}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1410.7386},
 primaryClass = "astro-ph.SR",
 keywords = {supernovae: general, supernovae: individual: SN 1987A, ISM: supernova remnants, Magellanic Clouds},
     year = 2015,
    month = jan,
   volume = 446,
    pages = {2089-2101},
      doi = {10.1093/mnras/stu2250},
   adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.446.2089W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015MNRAS.451L..70M,
   author = {{Mancini}, M. and {Schneider}, R. and {Graziani}, L. and {Valiante}, R. and 
	{Dayal}, P. and {Maio}, U. and {Ciardi}, B. and {Hunt}, L.~K.
	},
    title = "{The dust mass in z $\gt$ 6 normal star-forming galaxies}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1505.01841},
 keywords = {dust, extinction, ISM: supernova remnants, galaxies: evolution, galaxies: high-redshift, galaxies: ISM, submillimetre: galaxies},
     year = 2015,
    month = jul,
   volume = 451,
    pages = {L70-L74},
      doi = {10.1093/mnrasl/slv070},
   adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.451L..70M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010A&A...515A..94Z,
   author = {{Zafar}, T. and {Watson}, D.~J. and {Malesani}, D. and {Vreeswijk}, P.~M. and 
	{Fynbo}, J.~P.~U. and {Hjorth}, J. and {Levan}, A.~J. and {Micha{\l}owski}, M.~J.
	},
    title = "{No evidence for dust extinction in GRB 050904 at z \~{} 6.3}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1002.4101},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: high-redshift, dust, extinction, gamma-ray burst: individual: GRB 050904},
     year = 2010,
    month = jun,
   volume = 515,
      eid = {A94},
    pages = {A94},
      doi = {10.1051/0004-6361/200913795},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...515A..94Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2006ApJ...652..157M,
   author = {{McGreer}, I.~D. and {Becker}, R.~H. and {Helfand}, D.~J. and 
	{White}, R.~L.},
    title = "{Discovery of a z = 6.1 Radio-Loud Quasar in the NOAO Deep Wide Field Survey}",
  journal = {\apj},
   eprint = {astro-ph/0607278},
 keywords = {Galaxies: High-Redshift, quasars: individual (FIRST J1427385+331241)},
     year = 2006,
    month = nov,
   volume = 652,
    pages = {157-162},
      doi = {10.1086/507767},
   adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...652..157M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014MNRAS.441.1040R,
   author = {{Rowlands}, K. and {Gomez}, H.~L. and {Dunne}, L. and {Arag{\'o}n-Salamanca}, A. and 
	{Dye}, S. and {Maddox}, S. and {da Cunha}, E. and {van der Werf}, P.
	},
    title = "{The dust budget crisis in high-redshift submillimetre galaxies}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1403.2995},
 keywords = {dust, extinction, ISM: evolution, galaxies: evolution, galaxies: high redshift, submillimetre: galaxies},
     year = 2014,
    month = jun,
   volume = 441,
    pages = {1040-1058},
      doi = {10.1093/mnras/stu605},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.441.1040R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010MNRAS.401L..48G,
   author = {{Gomez}, H.~L. and {Vlahakis}, C. and {Stretch}, C.~M. and {Dunne}, L. and 
	{Eales}, S.~A. and {Beelen}, A. and {Gomez}, E.~L. and {Edmunds}, M.~G.
	},
    title = "{Submillimetre variability of Eta Carinae: cool dust within the outer ejecta}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0911.0176},
 keywords = {stars: individual: {$\eta$} Carinae , stars: mass loss , submillimetre},
     year = 2010,
    month = jan,
   volume = 401,
    pages = {L48-L52},
      doi = {10.1111/j.1745-3933.2009.00784.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.401L..48G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015A&A...575A..95S,
   author = {{Sarangi}, A. and {Cherchneff}, I.},
    title = "{Condensation of dust in the ejecta of Type II-P supernovae}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1412.5522},
 primaryClass = "astro-ph.SR",
 keywords = {supernovae: general, astrochemistry, stars: massive, dust, extinction},
     year = 2015,
    month = mar,
   volume = 575,
      eid = {A95},
    pages = {A95},
      doi = {10.1051/0004-6361/201424969},
   adsurl = {http://adsabs.harvard.edu/abs/2015A%26A...575A..95S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1967AnAp...30.1039C,
   author = {{Cernuschi}, F. and {Marsicano}, F. and {Codina}, S.},
    title = "{Contribution to the theory on the formation of cosmic grains}",
  journal = {Annales d'Astrophysique},
     year = 1967,
    month = feb,
   volume = 30,
    pages = {1039},
   adsurl = {http://adsabs.harvard.edu/abs/1967AnAp...30.1039C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2017MNRAS.471.3152P,
   author = {{Popping}, G. and {Somerville}, R.~S. and {Galametz}, M.},
    title = "{The dust content of galaxies from z = 0 to z = 9}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1609.08622},
 keywords = {methods: numerical, dust, extinction, galaxies: evolution, galaxies: formation, galaxies: ISM},
     year = 2017,
    month = nov,
   volume = 471,
    pages = {3152-3185},
      doi = {10.1093/mnras/stx1545},
   adsurl = {http://adsabs.harvard.edu/abs/2017MNRAS.471.3152P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015A&A...577A..80M,
   author = {{Micha{\l}owski}, M.~J.},
    title = "{Dust production 680-850 million years after the Big Bang}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1503.08210},
 keywords = {stars: AGB and post-AGB, supernovae: general, dust: extinction, galaxies: high-redshift, galaxies: ISM, quasars: general},
     year = 2015,
    month = may,
   volume = 577,
      eid = {A80},
    pages = {A80},
      doi = {10.1051/0004-6361/201525644},
   adsurl = {http://adsabs.harvard.edu/abs/2015A%26A...577A..80M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012MNRAS.421.2187S,
   author = {{Sawicki}, M.},
    title = "{Stars, dust, and the growth of ultraviolet-selected sub-L* galaxies at redshift z{\tilde} 2}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1108.5186},
 keywords = {galaxies: evolution, galaxies: formation, galaxies: high-redshift, galaxies: star formation, galaxies: stellar content},
     year = 2012,
    month = apr,
   volume = 421,
    pages = {2187-2205},
      doi = {10.1111/j.1365-2966.2012.20452.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.421.2187S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016MNRAS.457.3775M,
   author = {{McKinnon}, R. and {Torrey}, P. and {Vogelsberger}, M.},
    title = "{Dust formation in Milky Way-like galaxies}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1505.04792},
 keywords = {dust, extinction, galaxies: evolution},
     year = 2016,
    month = apr,
   volume = 457,
    pages = {3775-3800},
      doi = {10.1093/mnras/stw253},
   adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.457.3775M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011ApJ...732..109M,
   author = {{Meikle}, W.~P.~S. and {Kotak}, R. and {Farrah}, D. and {Mattila}, S. and 
	{Van Dyk}, S.~D. and {Andersen}, A.~C. and {Fesen}, R. and {Filippenko}, A.~V. and 
	{Foley}, R.~J. and {Fransson}, C. and {Gerardy}, C.~L. and {H{\"o}flich}, P.~A. and 
	{Lundqvist}, P. and {Pozzo}, M. and {Sollerman}, J. and {Wheeler}, J.~C.
	},
    title = "{Dust and the Type II-plateau Supernova 2004dj}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1103.2885},
 primaryClass = "astro-ph.SR",
 keywords = {circumstellar matter, dust, extinction, supernovae: general, supernovae: individual: SN 2004dj},
     year = 2011,
    month = may,
   volume = 732,
      eid = {109},
    pages = {109},
      doi = {10.1088/0004-637X/732/2/109},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...732..109M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011A&A...527L...6P,
   author = {{Patat}, F. and {Taubenberger}, S. and {Benetti}, S. and {Pastorello}, A. and 
	{Harutyunyan}, A.},
    title = "{Asymmetries in the type IIn SN 2010jl}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1011.5926},
 keywords = {supernovae: general, supernovae: individual: SN 2010jl, dust, extinction, techniques: polarimetric},
     year = 2011,
    month = mar,
   volume = 527,
      eid = {L6},
    pages = {L6},
      doi = {10.1051/0004-6361/201016217},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...527L...6P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013MNRAS.429.2527M,
   author = {{Matsuura}, M. and {Woods}, P.~M. and {Owen}, P.~J.},
    title = "{The global gas and dust budget of the Small Magellanic Cloud}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1212.1468},
 keywords = {stars: AGB and post-AGB, stars: mass-loss, supernovae: general, dust, extinction, galaxies: evolution, galaxies: individual: the Magellanic Clouds},
     year = 2013,
    month = mar,
   volume = 429,
    pages = {2527-2536},
      doi = {10.1093/mnras/sts521},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.429.2527M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012ApJ...760...93H,
   author = {{Humphreys}, R.~M. and {Davidson}, K. and {Jones}, T.~J. and 
	{Pogge}, R.~W. and {Grammer}, S.~H. and {Prieto}, J.~L. and 
	{Pritchard}, T.~A.},
    title = "{The Unusual Temporal and Spectral Evolution of SN2011ht. II. Peculiar Type IIn or Impostor?}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1207.5755},
 primaryClass = "astro-ph.SR",
 keywords = {supernovae: individual: SN2011ht},
     year = 2012,
    month = nov,
   volume = 760,
      eid = {93},
    pages = {93},
      doi = {10.1088/0004-637X/760/1/93},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...760...93H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012MNRAS.422.1263H,
   author = {{Hirashita}, H.},
    title = "{Dust growth in the interstellar medium: how do accretion and coagulation interplay?}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1202.1345},
 keywords = {turbulence, ISM: clouds, dust, extinction, ISM: evolution, galaxies: evolution, galaxies: ISM},
     year = 2012,
    month = may,
   volume = 422,
    pages = {1263-1271},
      doi = {10.1111/j.1365-2966.2012.20702.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.422.1263H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012ApJ...748...12S,
   author = {{Silvia}, D.~W. and {Smith}, B.~D. and {Shull}, J.~M.},
    title = "{Numerical Simulations of Supernova Dust Destruction. II. Metal-enriched Ejecta Knots}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1111.0302},
 keywords = {dust, extinction, hydrodynamics, ISM: supernova remnants, shock waves},
     year = 2012,
    month = mar,
   volume = 748,
      eid = {12},
    pages = {12},
      doi = {10.1088/0004-637X/748/1/12},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...748...12S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2001ApJ...561L..23G,
   author = {{Goodrich}, R.~W. and {Campbell}, R. and {Chaffee}, F.~H. and 
	{Hill}, G.~M. and {Sprayberry}, D. and {Brandt}, W.~N. and {Schneider}, D.~P. and 
	{Kaspi}, S. and {Fan}, X. and {Gunn}, J.~E. and {Strauss}, M.~A.
	},
    title = "{J-Band Spectroscopy of the z = 5.74 Broad Absorption Line Quasar SDSSp J104433.04-012502.2}",
  journal = {\apjl},
 keywords = {Galaxies: Active, Galaxies: Nuclei, Galaxies: Quasars: Absorption Lines, Galaxies: Quasars: General, Galaxies: Quasars: Individual: Alphanumeric: SDSS 1044-0125},
     year = 2001,
    month = nov,
   volume = 561,
    pages = {L23-L25},
      doi = {10.1086/324466},
   adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...561L..23G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013ApJ...776..107S,
   author = {{Sarangi}, A. and {Cherchneff}, I.},
    title = "{The Chemically Controlled Synthesis of Dust in Type II-P Supernovae}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1309.5887},
 primaryClass = "astro-ph.SR",
 keywords = {astrochemistry, dust, extinction, ISM: supernova remnants, molecular processes, supernovae: general},
     year = 2013,
    month = oct,
   volume = 776,
      eid = {107},
    pages = {107},
      doi = {10.1088/0004-637X/776/2/107},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...776..107S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013ApJ...774....8T,
   author = {{Temim}, T. and {Dwek}, E.},
    title = "{The Importance of Physical Models for Deriving Dust Masses and Grain Size Distributions in Supernova Ejecta. I. Radiatively Heated Dust in the Crab Nebula}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1302.5452},
 keywords = {dust, extinction, infrared: ISM, ISM: individual objects: Crab Nebula, ISM: supernova remnants, pulsars: individual: PSR B0531+21 },
     year = 2013,
    month = sep,
   volume = 774,
      eid = {8},
    pages = {8},
      doi = {10.1088/0004-637X/774/1/8},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...774....8T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013ApJ...768..195W,
   author = {{Whalen}, D.~J. and {Even}, W. and {Lovekin}, C.~C. and {Fryer}, C.~L. and 
	{Stiavelli}, M. and {Roming}, P.~W.~A. and {Cooke}, J. and {Pritchard}, T.~A. and 
	{Holz}, D.~E. and {Knight}, C.},
    title = "{Illuminating the Primeval Universe with Type IIn Supernovae}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1302.0436},
 keywords = {early universe, galaxies: high-redshift, hydrodynamics, radiative transfer, stars: early-type, supernovae: general},
     year = 2013,
    month = may,
   volume = 768,
      eid = {195},
    pages = {195},
      doi = {10.1088/0004-637X/768/2/195},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...768..195W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011ApJ...743...73K,
   author = {{Kochanek}, C.~S.},
    title = "{The Astrophysical Implications of Dust Formation during the Eruptions of Hot, Massive Stars}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1109.2596},
 primaryClass = "astro-ph.SR",
 keywords = {dust, extinction, stars: evolution, stars: massive, stars: mass-loss, stars: winds, outflows, supernovae: general},
     year = 2011,
    month = dec,
   volume = 743,
      eid = {73},
    pages = {73},
      doi = {10.1088/0004-637X/743/1/73},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...743...73K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009MNRAS.395..342B,
   author = {{Bekki}, K. and {Stanimirovi{\'c}}, S.},
    title = "{The total mass and dark halo properties of the Small Magellanic Cloud}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0807.2102},
 keywords = {galaxies: dwarf , galaxies: kinematics and dynamics , galaxies: star clusters , galaxies: structure},
     year = 2009,
    month = may,
   volume = 395,
    pages = {342-350},
      doi = {10.1111/j.1365-2966.2009.14514.x},
   adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.395..342B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2004ApJ...614..796S,
   author = {{Slavin}, J.~D. and {Jones}, A.~P. and {Tielens}, A.~G.~G.~M.
	},
    title = "{Shock Processing of Large Grains in the Interstellar Medium}",
  journal = {\apj},
 keywords = {ISM: Cosmic Rays, ISM: Dust, Extinction, Shock Waves, ISM: Supernova Remnants},
     year = 2004,
    month = oct,
   volume = 614,
    pages = {796-806},
      doi = {10.1086/423834},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...614..796S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1998MNRAS.299L..29E,
   author = {{Edmunds}, M.~G. and {Eales}, S.~A.},
    title = "{Maximum dust masses in galaxies}",
  journal = {\mnras},
 keywords = {DUST, EXTINCTION, GALAXIES: EVOLUTION, GALAXIES: GENERAL, GALAXIES: ISM},
     year = 1998,
    month = sep,
   volume = 299,
    pages = {L29-L31},
      doi = {10.1046/j.1365-8711.1998.01971.x},
   adsurl = {http://adsabs.harvard.edu/abs/1998MNRAS.299L..29E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2008MNRAS.383..289P,
   author = {{Priddey}, R.~S. and {Ivison}, R.~J. and {Isaak}, K.~G.},
    title = "{Environments of z $\gt$ 5 quasars: searching for protoclusters at submillimetre wavelengths}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0709.0610},
 keywords = {galaxies: active , galaxies: high-redshift , cosmology: observations , submillimetre},
     year = 2008,
    month = jan,
   volume = 383,
    pages = {289-296},
      doi = {10.1111/j.1365-2966.2007.12536.x},
   adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.383..289P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2017ApJ...837L..21L,
   author = {{Laporte}, N. and {Ellis}, R.~S. and {Boone}, F. and {Bauer}, F.~E. and 
	{Qu{\'e}nard}, D. and {Roberts-Borsani}, G.~W. and {Pell{\'o}}, R. and 
	{P{\'e}rez-Fournon}, I. and {Streblyanska}, A.},
    title = "{Dust in the Reionization Era: ALMA Observations of a z = 8.38 Gravitationally Lensed Galaxy}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1703.02039},
 keywords = {early universe, galaxies: evolution, galaxies: formation, galaxies: high-redshift, galaxies: star formation, submillimeter: galaxies},
     year = 2017,
    month = mar,
   volume = 837,
      eid = {L21},
    pages = {L21},
      doi = {10.3847/2041-8213/aa62aa},
   adsurl = {http://adsabs.harvard.edu/abs/2017ApJ...837L..21L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011AJ....142...45A,
   author = {{Andrews}, J.~E. and {Clayton}, G.~C. and {Wesson}, R. and {Sugerman}, B.~E.~K. and 
	{Barlow}, M.~J. and {Clem}, J. and {Ercolano}, B. and {Fabbri}, J. and 
	{Gallagher}, J.~S. and {Landolt}, A. and {Meixner}, M. and {Otsuka}, M. and 
	{Riebel}, D. and {Welch}, D.~L.},
    title = "{Evidence for Pre-existing Dust in the Bright Type IIn SN 2010jl}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1106.0537},
 keywords = {circumstellar matter, dust, extinction, supernovae: general, supernovae: individual: SN 2010jl},
     year = 2011,
    month = aug,
   volume = 142,
      eid = {45},
    pages = {45},
      doi = {10.1088/0004-6256/142/2/45},
   adsurl = {http://adsabs.harvard.edu/abs/2011AJ....142...45A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011MNRAS.414..781M,
   author = {{Mattsson}, L.},
    title = "{Dust in the early Universe: evidence for non-stellar dust production or observational errors?}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1102.0570},
 keywords = {stars: AGB and post-AGB, supernovae: general, dust, extinction, galaxies: evolution, galaxies: high-redshift, quasars: general, quasars: individual: SDSS J1148+5251, galaxies: starburst},
     year = 2011,
    month = jun,
   volume = 414,
    pages = {781-791},
      doi = {10.1111/j.1365-2966.2011.18447.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.414..781M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014ApJ...790...40C,
   author = {{Cooray}, A. and {Calanog}, J. and {Wardlow}, J.~L. and {Bock}, J. and 
	{Bridge}, C. and {Burgarella}, D. and {Bussmann}, R.~S. and 
	{Casey}, C.~M. and {Clements}, D. and {Conley}, A. and {Farrah}, D. and 
	{Fu}, H. and {Gavazzi}, R. and {Ivison}, R.~J. and {La Porte}, N. and 
	{Lo Faro}, B. and {Ma}, B. and {Magdis}, G. and {Oliver}, S.~J. and 
	{Osage}, W.~A. and {P{\'e}rez-Fournon}, I. and {Riechers}, D. and 
	{Rigopoulou}, D. and {Scott}, D. and {Viero}, M. and {Watson}, D.
	},
    title = "{HerMES: The Rest-frame UV Emission and a Lensing Model for the z = 6.34 Luminous Dusty Starburst Galaxy HFLS3}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1404.1378},
 keywords = {galaxies: high-redshift, galaxies: starburst, gravitational lensing: strong, infrared: galaxies, submillimeter: galaxies},
     year = 2014,
    month = jul,
   volume = 790,
      eid = {40},
    pages = {40},
      doi = {10.1088/0004-637X/790/1/40},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...790...40C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012MNRAS.421.2917F,
   author = {{Foyle}, K. and {Wilson}, C.~D. and {Mentuch}, E. and {Bendo}, G. and 
	{Dariush}, A. and {Parkin}, T. and {Pohlen}, M. and {Sauvage}, M. and 
	{Smith}, M.~W.~L. and {Roussel}, H. and {Baes}, M. and {Boquien}, M. and 
	{Boselli}, A. and {Clements}, D.~L. and {Cooray}, A. and {Davies}, J.~I. and 
	{Eales}, S.~A. and {Madden}, S. and {Page}, M.~J. and {Spinoglio}, L.
	},
    title = "{The dust and gas properties of M83}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1201.2178},
 keywords = {galaxies: individual: M83, galaxies: ISM, galaxies: spiral, infrared: galaxies},
     year = 2012,
    month = apr,
   volume = 421,
    pages = {2917-2929},
      doi = {10.1111/j.1365-2966.2012.20520.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.421.2917F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2004ApJ...614..727M,
   author = {{Morse}, J.~A. and {Fesen}, R.~A. and {Chevalier}, R.~A. and 
	{Borkowski}, K.~J. and {Gerardy}, C.~L. and {Lawrence}, S.~S. and 
	{van den Bergh}, S.},
    title = "{Location of the Optical Reverse Shock in the Cassiopeia A Supernova Remnant}",
  journal = {\apj},
 keywords = {ISM: Individual: Name: Cassiopeia A, ISM: Kinematics and Dynamics, ISM: Supernova Remnants},
     year = 2004,
    month = oct,
   volume = 614,
    pages = {727-736},
      doi = {10.1086/423709},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...614..727M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015ApJ...803....7S,
   author = {{Slavin}, J.~D. and {Dwek}, E. and {Jones}, A.~P.},
    title = "{Destruction of Interstellar Dust in Evolving Supernova Remnant Shock Waves}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1502.00929},
 keywords = {dust, extinction, ISM: supernova remnants, ISM: abundances, shock waves},
     year = 2015,
    month = apr,
   volume = 803,
      eid = {7},
    pages = {7},
      doi = {10.1088/0004-637X/803/1/7},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...803....7S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012MNRAS.424.2659M,
   author = {{Mauerhan}, J. and {Smith}, N.},
    title = "{Supernova 1998S at 14 years postmortem: continuing circumstellar interaction and dust formation}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1204.1610},
 primaryClass = "astro-ph.SR",
 keywords = {supernovae: general, supernovae: individual: SN 1998S },
     year = 2012,
    month = aug,
   volume = 424,
    pages = {2659-2666},
      doi = {10.1111/j.1365-2966.2012.21325.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.424.2659M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012ApJ...750L...2C,
   author = {{Chandra}, P. and {Chevalier}, R.~A. and {Irwin}, C.~M. and 
	{Chugai}, N. and {Fransson}, C. and {Soderberg}, A.~M.},
    title = "{Strong Evolution of X-Ray Absorption in the Type IIn Supernova SN 2010jl}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1203.1614},
 primaryClass = "astro-ph.HE",
 keywords = {circumstellar matter, hydrodynamics, supernovae: general, supernovae: individual: SN 2010jl, X-rays: general},
     year = 2012,
    month = may,
   volume = 750,
      eid = {L2},
    pages = {L2},
      doi = {10.1088/2041-8205/750/1/L2},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...750L...2C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010ApJ...725..585A,
   author = {{Arendt}, R.~G. and {Dwek}, E. and {Blair}, W.~P. and {Ghavamian}, P. and 
	{Hwang}, U. and {Long}, K.~S. and {Petre}, R. and {Rho}, J. and 
	{Winkler}, P.~F.},
    title = "{Spitzer Observations of Dust Destruction in the Puppis A Supernova Remnant}",
  journal = {\apj},
 keywords = {dust, extinction, infrared: ISM, ISM: individual objects: Puppis A, ISM: supernova remnants},
     year = 2010,
    month = dec,
   volume = 725,
    pages = {585-597},
      doi = {10.1088/0004-637X/725/1/585},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...725..585A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015ApJ...801..141O,
   author = {{Owen}, P.~J. and {Barlow}, M.~J.},
    title = "{The Dust and Gas Content of the Crab Nebula}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1501.01510},
 keywords = {circumstellar matter, ISM: individual objects: Crab Nebula, ISM: supernova remnants},
     year = 2015,
    month = mar,
   volume = 801,
      eid = {141},
    pages = {141},
      doi = {10.1088/0004-637X/801/2/141},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...801..141O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014MNRAS.438.2765C,
   author = {{Calura}, F. and {Gilli}, R. and {Vignali}, C. and {Pozzi}, F. and 
	{Pipino}, A. and {Matteucci}, F.},
    title = "{The dust content of QSO hosts at high redshift}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1312.1087},
 keywords = {dust, extinction, galaxies: elliptical and lenticular, cD, galaxies: evolution, quasars: general, cosmology: observations},
     year = 2014,
    month = mar,
   volume = 438,
    pages = {2765-2783},
      doi = {10.1093/mnras/stt2329},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.438.2765C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012A&A...545L...7T,
   author = {{Taddia}, F. and {Stritzinger}, M.~D. and {Phillips}, M.~M. and 
	{Burns}, C.~R. and {Heinrich-Josties}, E. and {Morrell}, N. and 
	{Sollerman}, J. and {Valenti}, S. and {Anderson}, J.~P. and 
	{Boldt}, L. and {Campillay}, A. and {Castellon}, S. and {Contreras}, C. and 
	{Folatelli}, G. and {Freedman}, W.~L. and {Hamuy}, M. and {Krzeminski}, W. and 
	{Leloudas}, G. and {Maeda}, K. and {Persson}, S.~E. and {Roth}, M. and 
	{Suntzeff}, N.~B.},
    title = "{Supernova 2008J: early time observations of a heavily reddened SN 2002ic-like transient}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1208.2599},
 primaryClass = "astro-ph.HE",
 keywords = {supernovae: general, supernovae: individual: SN 2008J},
     year = 2012,
    month = sep,
   volume = 545,
      eid = {L7},
    pages = {L7},
      doi = {10.1051/0004-6361/201220105},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...545L...7T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009MNRAS.397.1621G,
   author = {{Gomez}, H.~L. and {Dunne}, L. and {Ivison}, R.~J. and {Reynoso}, E.~M. and 
	{Thompson}, M.~A. and {Sibthorpe}, B. and {Eales}, S.~A. and 
	{Delaney}, T.~M. and {Maddox}, S. and {Isaak}, K.},
    title = "{Accounting for the foreground contribution to the dust emission towards Kepler's supernova remnant}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0905.2564},
 keywords = {Supernovae: Kepler , ISM: submillimetre dust , radio lines: ISM , Galaxies: abundances , submillimetre},
     year = 2009,
    month = aug,
   volume = 397,
    pages = {1621-1632},
      doi = {10.1111/j.1365-2966.2009.15061.x},
   adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.397.1621G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2008MNRAS.384.1725H,
   author = {{Hirashita}, H. and {Nozawa}, T. and {Takeuchi}, T.~T. and {Kozasa}, T.
	},
    title = "{Extinction curves flattened by reverse shocks in supernovae}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0801.2649},
 keywords = {supernovae: general , dust, extinction , galaxies: evolution , galaxies: high-redshift , galaxies: ISM , quasars: individual: SDSS J104845.05+463718.3},
     year = 2008,
    month = mar,
   volume = 384,
    pages = {1725-1732},
      doi = {10.1111/j.1365-2966.2007.12834.x},
   adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.384.1725H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2001A&A...372L...5M,
   author = {{Maiolino}, R. and {Mannucci}, F. and {Baffa}, C. and {Gennari}, S. and 
	{Oliva}, E.},
    title = "{Discovery of strong CIV absorption in the highest redshift quasar}",
  journal = {\aap},
   eprint = {astro-ph/0104147},
 keywords = {INFRARED: GALAXIES, QUASARS: GENERAL, QUASARS: ABSORPTION LINES},
     year = 2001,
    month = jun,
   volume = 372,
    pages = {L5-L8},
      doi = {10.1051/0004-6361:20010523},
   adsurl = {http://adsabs.harvard.edu/abs/2001A%26A...372L...5M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013ApJ...763..110K,
   author = {{Kalirai}, J.~S. and {Anderson}, J. and {Dotter}, A. and {Richer}, H.~B. and 
	{Fahlman}, G.~G. and {Hansen}, B.~M.~S. and {Hurley}, J. and 
	{Reid}, I.~N. and {Rich}, R.~M. and {Shara}, M.~M.},
    title = "{Ultra-Deep Hubble Space Telescope Imaging of the Small Magellanic Cloud: The Initial Mass Function of Stars with M $\lt$\~{} 1 M $_{???}$}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1212.1159},
 keywords = {galaxies: photometry, galaxies: stellar content, Magellanic Clouds, methods: data analysis, methods: statistical, stars: luminosity function, mass function, techniques: photometric},
     year = 2013,
    month = feb,
   volume = 763,
      eid = {110},
    pages = {110},
      doi = {10.1088/0004-637X/763/2/110},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...763..110K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2001ASPC..238..321D,
   author = {{Demleitner}, M. and {Accomazzi}, A. and {Eichhorn}, G. and 
	{Grant}, C.~S. and {Kurtz}, M.~J. and {Murray}, S.~S.},
    title = "{ADS's Dexter Data Extraction Applet}",
booktitle = {Astronomical Data Analysis Software and Systems X},
     year = 2001,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 238,
   editor = {{Harnden}, Jr., F.~R. and {Primini}, F.~A. and {Payne}, H.~E.
	},
    pages = {321},
   adsurl = {http://adsabs.harvard.edu/abs/2001ASPC..238..321D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015ApJ...813...93S,
   author = {{Strolger}, L.-G. and {Dahlen}, T. and {Rodney}, S.~A. and {Graur}, O. and 
	{Riess}, A.~G. and {McCully}, C. and {Ravindranath}, S. and 
	{Mobasher}, B. and {Shahady}, A.~K.},
    title = "{The Rate of Core Collapse Supernovae to Redshift 2.5 from the CANDELS and CLASH Supernova Surveys}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1509.06574},
 keywords = {supernovae: general},
     year = 2015,
    month = nov,
   volume = 813,
      eid = {93},
    pages = {93},
      doi = {10.1088/0004-637X/813/2/93},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...813...93S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010CBET.2532....1N,
   author = {{Newton}, J. and {Puckett}, T.},
    title = "{Possible Supernova in UGC 5189A}",
  journal = {Central Bureau Electronic Telegrams},
     year = 2010,
    month = nov,
   volume = 2532,
   adsurl = {http://adsabs.harvard.edu/abs/2010CBET.2532....1N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2005ApJ...627L.113B,
   author = {{Barlow}, M.~J. and {Sugerman}, B.~E.~K. and {Fabbri}, J. and 
	{Meixner}, M. and {Fisher}, R.~S. and {Bowey}, J.~E. and {Panagia}, N. and 
	{Ercolano}, B. and {Clayton}, G.~C. and {Cohen}, M. and {Gledhill}, T.~M. and 
	{Gordon}, K. and {Tielens}, A.~G.~G.~M. and {Zijlstra}, A.~A.
	},
    title = "{Detection of a Massive Dust Shell around the Type II Supernova SN 2002hh}",
  journal = {\apjl},
   eprint = {astro-ph/0506542},
 keywords = {ISM: Dust, Extinction, Galaxies: Individual: NGC Number: NGC 6946, Stars: Supernovae: General, Stars: Supernovae: Individual: Alphanumeric: SN 2002hh},
     year = 2005,
    month = jul,
   volume = 627,
    pages = {L113-L116},
      doi = {10.1086/432440},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...627L.113B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2017MNRAS.465.3309D,
   author = {{De Looze}, I. and {Barlow}, M.~J. and {Swinyard}, B.~M. and 
	{Rho}, J. and {Gomez}, H.~L. and {Matsuura}, M. and {Wesson}, R.
	},
    title = "{The dust mass in Cassiopeia A from a spatially resolved Herschel analysis}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1611.00774},
 keywords = {supernovae: individual: Cassiopeia A, dust, extinction, ISM: supernova remnants, infrared: ISM},
     year = 2017,
    month = mar,
   volume = 465,
    pages = {3309-3342},
      doi = {10.1093/mnras/stw2837},
   adsurl = {http://adsabs.harvard.edu/abs/2017MNRAS.465.3309D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016A&A...596A..97D,
   author = {{De Cia}, A. and {Ledoux}, C. and {Mattsson}, L. and {Petitjean}, P. and 
	{Srianand}, R. and {Gavignaud}, I. and {Jenkins}, E.~B.},
    title = "{Dust-depletion sequences in damped Lyman-{$\alpha$} absorbers. A unified picture from low-metallicity systems to the Galaxy}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1608.08621},
 keywords = {ISM: abundances, dust, extinction, quasars: absorption lines},
     year = 2016,
    month = dec,
   volume = 596,
      eid = {A97},
    pages = {A97},
      doi = {10.1051/0004-6361/201527895},
   adsurl = {http://adsabs.harvard.edu/abs/2016A%26A...596A..97D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2000A&A...357..115T,
   author = {{Toft}, S. and {Hjorth}, J. and {Burud}, I.},
    title = "{The extinction curve of the lensing galaxy of B1152+199 at z=0.44}",
  journal = {\aap},
   eprint = {astro-ph/0003098},
 keywords = {GALAXIES: QUASARS: INDIVIDUAL: B1152+199, GALAXIES: ISM, ISM: DUST, EXTINCTION, ISM: EVOLUTION, COSMOLOGY: GRAVITATIONAL LENSING},
     year = 2000,
    month = may,
   volume = 357,
    pages = {115-119},
   adsurl = {http://adsabs.harvard.edu/abs/2000A%26A...357..115T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010A&A...518L.139O,
   author = {{Otsuka}, M. and {van Loon}, J.~T. and {Long}, K.~S. and {Meixner}, M. and 
	{Matsuura}, M. and {Reach}, W.~T. and {Roman-Duval}, J. and 
	{Gordon}, K. and {Sauvage}, M. and {Hony}, S. and {Misselt}, K. and 
	{Engelbracht}, C. and {Panuzzo}, P. and {Okumura}, K. and {Woods}, P.~M. and 
	{Kemper}, F. and {Sloan}, G.~C.},
    title = "{Dust in the bright supernova remnant N49 in the LMC}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1005.2787},
 keywords = {ISM: supernova remnants, dust, extinction, submillimeter: ISM, Magellanic Clouds},
     year = 2010,
    month = jul,
   volume = 518,
      eid = {L139},
    pages = {L139},
      doi = {10.1051/0004-6361/201014642},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...518L.139O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010ApJ...712.1092S,
   author = {{Sankrit}, R. and {Williams}, B.~J. and {Borkowski}, K.~J. and 
	{Gaetz}, T.~J. and {Raymond}, J.~C. and {Blair}, W.~P. and {Ghavamian}, P. and 
	{Long}, K.~S. and {Reynolds}, S.~P.},
    title = "{Dust Destruction in a Non-radiative Shock in the Cygnus Loop Supernova Remnant}",
  journal = {\apj},
 keywords = {dust, extinction, ISM: individual objects: Cygnus Loop, ISM: supernova remnants, shock waves},
     year = 2010,
    month = apr,
   volume = 712,
    pages = {1092-1099},
      doi = {10.1088/0004-637X/712/2/1092},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...712.1092S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1979Ap&SS..65..179C,
   author = {{Clayton}, D.~D.},
    title = "{Sudden grain nucleation and growth in supernova and nova ejecta}",
  journal = {\apss},
 keywords = {Condensates, Cosmic Dust, Interstellar Matter, Novae, Nucleation, Stellar Mass Ejection, Supernova Remnants, Abundance, Chemical Equilibrium, Ejecta, Gas Density, Thermodynamic Equilibrium},
     year = 1979,
    month = sep,
   volume = 65,
    pages = {179-189},
      doi = {10.1007/BF00643499},
   adsurl = {http://adsabs.harvard.edu/abs/1979Ap%26SS..65..179C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012ApJ...761...42S,
   author = {{Skibba}, R.~A. and {Engelbracht}, C.~W. and {Aniano}, G. and 
	{Babler}, B. and {Bernard}, J.-P. and {Bot}, C. and {Carlson}, L.~R. and 
	{Galametz}, M. and {Galliano}, F. and {Gordon}, K. and {Hony}, S. and 
	{Israel}, F. and {Lebouteiller}, V. and {Li}, A. and {Madden}, S. and 
	{Meixner}, M. and {Misselt}, K. and {Montiel}, E. and {Okumura}, K. and 
	{Panuzzo}, P. and {Paradis}, D. and {Roman-Duval}, J. and {Rubio}, M. and 
	{Sauvage}, M. and {Seale}, J. and {Srinivasan}, S. and {van Loon}, J.~T.
	},
    title = "{The Spatial Distribution of Dust and Stellar Emission of the Magellanic Clouds}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1210.7812},
 keywords = {dust, extinction, galaxies: evolution, galaxies: general, galaxies: ISM, infrared: galaxies, Magellanic Clouds},
     year = 2012,
    month = dec,
   volume = 761,
      eid = {42},
    pages = {42},
      doi = {10.1088/0004-637X/761/1/42},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...761...42S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012ApJ...753...33D,
   author = {{Dai}, Y.~S. and {Bergeron}, J. and {Elvis}, M. and {Omont}, A. and 
	{Huang}, J.-S. and {Bock}, J. and {Cooray}, A. and {Fazio}, G. and 
	{Hatziminaoglou}, E. and {Ibar}, E. and {Magdis}, G.~E. and 
	{Oliver}, S.~J. and {Page}, M.~J. and {Perez-Fournon}, I. and 
	{Rigopoulou}, D. and {Roseboom}, I.~G. and {Scott}, D. and {Symeonidis}, M. and 
	{Trichas}, M. and {Vieira}, J.~D. and {Willmer}, C.~N.~A. and 
	{Zemcov}, M.},
    title = "{A Population of Dust-rich Quasars at z \~{} 1.5}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1205.1808},
 keywords = {galaxies: active, galaxies: nuclei, galaxies: starburst, infrared: galaxies, quasars: general },
     year = 2012,
    month = jul,
   volume = 753,
      eid = {33},
    pages = {33},
      doi = {10.1088/0004-637X/753/1/33},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...753...33D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2017MNRAS.466..138K,
   author = {{Knudsen}, K.~K. and {Watson}, D. and {Frayer}, D. and {Christensen}, L. and 
	{Gallazzi}, A. and {Micha{\l}owski}, M.~J. and {Richard}, J. and 
	{Zavala}, J.},
    title = "{A merger in the dusty, z = 7.5 galaxy A1689-zD1?}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1603.03222},
 keywords = {galaxies: evolution, galaxies: formation, galaxies: high-redshift, galaxies: ISM, submillimetre: galaxies},
     year = 2017,
    month = apr,
   volume = 466,
    pages = {138-146},
      doi = {10.1093/mnras/stw3066},
   adsurl = {http://adsabs.harvard.edu/abs/2017MNRAS.466..138K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016MNRAS.463L.112F,
   author = {{Ferrara}, A. and {Viti}, S. and {Ceccarelli}, C.},
    title = "{The problematic growth of dust in high-redshift galaxies}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1606.07214},
 keywords = {dust, extinction, galaxies: high-redshift},
     year = 2016,
    month = nov,
   volume = 463,
    pages = {L112-L116},
      doi = {10.1093/mnrasl/slw165},
   adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.463L.112F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016ApJ...831..147Z,
   author = {{Zhukovska}, S. and {Dobbs}, C. and {Jenkins}, E.~B. and {Klessen}, R.~S.
	},
    title = "{Modeling Dust Evolution in Galaxies with a Multiphase, Inhomogeneous ISM}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1608.04781},
 keywords = {dust, extinction, Galaxy: evolution, ISM: abundances},
     year = 2016,
    month = nov,
   volume = 831,
      eid = {147},
    pages = {147},
      doi = {10.3847/0004-637X/831/2/147},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...831..147Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016A&A...587A.157B,
   author = {{Bocchio}, M. and {Marassi}, S. and {Schneider}, R. and {Bianchi}, S. and 
	{Limongi}, M. and {Chieffi}, A.},
    title = "{Dust grains from the heart of supernovae}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1601.06770},
 primaryClass = "astro-ph.HE",
 keywords = {supernovae: general, dust, extinction, local insterstellar matter, galaxies: high-redshift},
     year = 2016,
    month = mar,
   volume = 587,
      eid = {A157},
    pages = {A157},
      doi = {10.1051/0004-6361/201527432},
   adsurl = {http://adsabs.harvard.edu/abs/2016A%26A...587A.157B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2004ApJ...611L..13F,
   author = {{Farrah}, D. and {Priddey}, R. and {Wilman}, R. and {Haehnelt}, M. and 
	{McMahon}, R.},
    title = "{The X-Ray Spectrum of the z=6.30 QSO SDSS J1030+0524}",
  journal = {\apjl},
   eprint = {astro-ph/0406561},
 keywords = {Cosmology: Observations, Galaxies: Formation, Galaxies: High-Redshift, Galaxies: Quasars: Individual: Alphanumeric: SDSS J1030+0524, X-Rays: Galaxies},
     year = 2004,
    month = aug,
   volume = 611,
    pages = {L13-L16},
      doi = {10.1086/423669},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...611L..13F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014ApJ...786...55A,
   author = {{Arendt}, R.~G. and {Dwek}, E. and {Kober}, G. and {Rho}, J. and 
	{Hwang}, U.},
    title = "{Interstellar and Ejecta Dust in the Cas A Supernova Remnant}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1403.3008},
 keywords = {dust, extinction, infrared: ISM, ISM: individual objects: Cassiopeia A, ISM: supernova remnants},
     year = 2014,
    month = may,
   volume = 786,
      eid = {55},
    pages = {55},
      doi = {10.1088/0004-637X/786/1/55},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...786...55A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013ApJ...765L..43I,
   author = {{Ibeling}, D. and {Heger}, A.},
    title = "{The Metallicity Dependence of the Minimum Mass for Core-collapse Supernovae}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1301.5783},
 primaryClass = "astro-ph.SR",
 keywords = {stars: evolution, stars: formation, supernovae: general},
     year = 2013,
    month = mar,
   volume = 765,
      eid = {L43},
    pages = {L43},
      doi = {10.1088/2041-8205/765/2/L43},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...765L..43I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010CBET.2536....1B,
   author = {{Benetti}, S. and {Bufano}, F. and {Vinko}, J. and {Marion}, G.~H. and 
	{Pritchard}, T. and {Wheeler}, J.~C. and {Chatzopoulos}, E. and 
	{Shetrone}, M.},
    title = "{Supernova 2010jl in UGC 5189A}",
  journal = {Central Bureau Electronic Telegrams},
     year = 2010,
    month = nov,
   volume = 2536,
   adsurl = {http://adsabs.harvard.edu/abs/2010CBET.2536....1B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2007MNRAS.374..867P,
   author = {{Priddey}, R.~S. and {Gallagher}, S.~C. and {Isaak}, K.~G. and 
	{Sharp}, R.~G. and {McMahon}, R.~G. and {Butner}, H.~M.},
    title = "{A sensitive submillimetre survey of broad absorption-line quasars}",
  journal = {\mnras},
   eprint = {astro-ph/0610472},
 keywords = {galaxies: active, quasars: absorption lines, galaxies: starburst, submillimetre},
     year = 2007,
    month = jan,
   volume = 374,
    pages = {867-876},
      doi = {10.1111/j.1365-2966.2006.11200.x},
   adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.374..867P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015ApJ...799..158T,
   author = {{Temim}, T. and {Dwek}, E. and {Tchernyshyov}, K. and {Boyer}, M.~L. and 
	{Meixner}, M. and {Gall}, C. and {Roman-Duval}, J.},
    title = "{Dust Destruction Rates and Lifetimes in the Magellanic Clouds}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1411.4574},
 keywords = {dust, extinction, infrared: ISM, ISM: individual objects: MAGELLANIC CLOUDS, ISM: supernova remnants},
     year = 2015,
    month = feb,
   volume = 799,
      eid = {158},
    pages = {158},
      doi = {10.1088/0004-637X/799/2/158},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...799..158T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015ApJ...799...50L,
   author = {{Laki{\'c}evi{\'c}}, M. and {van Loon}, J.~T. and {Meixner}, M. and 
	{Gordon}, K. and {Bot}, C. and {Roman-Duval}, J. and {Babler}, B. and 
	{Bolatto}, A. and {Engelbracht}, C. and {Filipovi{\'c}}, M. and 
	{Hony}, S. and {Indebetouw}, R. and {Misselt}, K. and {Montiel}, E. and 
	{Okumura}, K. and {Panuzzo}, P. and {Patat}, F. and {Sauvage}, M. and 
	{Seale}, J. and {Sonneborn}, G. and {Temim}, T. and {Uro{\v s}evi{\'c}}, D. and 
	{Zanardo}, G.},
    title = "{The Influence of Supernova Remnants on the Interstellar Medium in the Large Magellanic Cloud Seen at 20-600 {$\mu$}m Wavelengths}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1410.5709},
 keywords = {dust, extinction, evolution, galaxies: ISM, ISM: clouds, ISM: supernova remnants, Magellanic Clouds, submillimeter: galaxies, submillimeter: ISM},
     year = 2015,
    month = jan,
   volume = 799,
      eid = {50},
    pages = {50},
      doi = {10.1088/0004-637X/799/1/50},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...799...50L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013ApJ...768...88F,
   author = {{Fransson}, C. and {Larsson}, J. and {Spyromilio}, J. and {Chevalier}, R. and 
	{Gr{\"o}ningsson}, P. and {Jerkstrand}, A. and {Leibundgut}, B. and 
	{McCray}, R. and {Challis}, P. and {Kirshner}, R.~P. and {Kjaer}, K. and 
	{Lundqvist}, P. and {Sollerman}, J.},
    title = "{Late Spectral Evolution of the Ejecta and Reverse Shock in SN 1987A}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1212.5052},
 primaryClass = "astro-ph.HE",
 keywords = {line: identification, line: profiles, supernovae: individual: 1987A, X-rays: general},
     year = 2013,
    month = may,
   volume = 768,
      eid = {88},
    pages = {88},
      doi = {10.1088/0004-637X/768/1/88},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...768...88F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012ApJ...751...42S,
   author = {{Seale}, J.~P. and {Looney}, L.~W. and {Wong}, T. and {Ott}, J. and 
	{Klein}, U. and {Pineda}, J.~L.},
    title = "{The Life and Death of Dense Molecular Clumps in the Large Magellanic Cloud}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1203.4505},
 keywords = {galaxies: individual: LMC, infrared: stars, instrumentation: spectrographs, Magellanic Clouds, stars: evolution, stars: formation},
     year = 2012,
    month = may,
   volume = 751,
      eid = {42},
    pages = {42},
      doi = {10.1088/0004-637X/751/1/42},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...751...42S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016MNRAS.456.1269B,
   author = {{Bevan}, A. and {Barlow}, M.~J.},
    title = "{Modelling supernova line profile asymmetries to determine ejecta dust masses: SN 1987A from days 714 to 3604}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1509.00858},
 primaryClass = "astro-ph.SR",
 keywords = {radiative transfer, supernovae: general, supernovae: individual: SN 1987A, ISM: supernova remnants},
     year = 2016,
    month = feb,
   volume = 456,
    pages = {1269-1293},
      doi = {10.1093/mnras/stv2651},
   adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.456.1269B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2008ApJ...682.1055N,
   author = {{Nath}, B.~B. and {Laskar}, T. and {Shull}, J.~M.},
    title = "{Dust Sputtering by Reverse Shocks in Supernova Remnants}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0804.3472},
 keywords = {dust, extinction, galaxies: high-redshift, supernova remnants },
     year = 2008,
    month = aug,
   volume = 682,
      eid = {1055-1064},
    pages = {1055-1064},
      doi = {10.1086/589224},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...682.1055N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015MNRAS.449.2588P,
   author = {{Petit}, A.~C. and {Krumholz}, M.~R. and {Goldbaum}, N.~J. and 
	{Forbes}, J.~C.},
    title = "{Mixing and transport of metals by gravitational instability-driven turbulence in galactic discs}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1411.7585},
 keywords = {conduction, turbulence, galaxies: evolution, galaxies: kinematics and dynamics},
     year = 2015,
    month = may,
   volume = 449,
    pages = {2588-2597},
      doi = {10.1093/mnras/stv493},
   adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.449.2588P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012ApJ...749L..25M,
   author = {{Mor}, R. and {Netzer}, H. and {Trakhtenbrot}, B. and {Shemmer}, O. and 
	{Lira}, P.},
    title = "{Extreme Star Formation in the Host Galaxies of the Fastest Growing Supermassive Black Holes at z = 4.8}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1203.1613},
 keywords = {galaxies: active, galaxies: star formation, quasars: general},
     year = 2012,
    month = apr,
   volume = 749,
      eid = {L25},
    pages = {L25},
      doi = {10.1088/2041-8205/749/2/L25},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...749L..25M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2002PASJ...54..975S,
   author = {{Shioya}, Y. and {Taniguchi}, Y. and {Murayama}, T. and {Ajiki}, M. and 
	{Nagao}, T. and {Fujita}, S.~S. and {Kakazu}, Y. and {Komiyama}, Y. and 
	{Okamura}, S. and {Oyabu}, S. and {Kawara}, K. and {Ohyama}, Y. and 
	{Kawabata}, K.~S. and {Ando}, H. and {Nishimura}, T. and {Hayashi}, M. and 
	{Ogasawara}, R. and {Ichikawa}, S.-I.},
    title = "{SDSSp J104433.04?012502.2 at z=5.74 is Gravitationally Magnified by an Intervening Galaxy}",
  journal = {\pasj},
   eprint = {astro-ph/0211388},
 keywords = {galaxies: high-redshift, galaxies: quasars: individual (SDSSp J104433.04012502.2), gravitational lensing},
     year = 2002,
    month = dec,
   volume = 54,
    pages = {975-979},
      doi = {10.1093/pasj/54.6.975},
   adsurl = {http://adsabs.harvard.edu/abs/2002PASJ...54..975S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014A&A...564A..25B,
   author = {{Biscaro}, C. and {Cherchneff}, I.},
    title = "{Molecules and dust in Cassiopeia A. I. Synthesis in the supernova phase and processing by the reverse shock in the clumpy remnant}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1401.5594},
 primaryClass = "astro-ph.SR",
 keywords = {astrochemistry, molecular processes, ISM: supernova remnants, circumstellar matter, supernovae: general, dust, extinction},
     year = 2014,
    month = apr,
   volume = 564,
      eid = {A25},
    pages = {A25},
      doi = {10.1051/0004-6361/201322932},
   adsurl = {http://adsabs.harvard.edu/abs/2014A%26A...564A..25B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012ApJ...750...77S,
   author = {{Szczygie{\l}}, D.~M. and {Prieto}, J.~L. and {Kochanek}, C.~S. and 
	{Stanek}, K.~Z. and {Thompson}, T.~A. and {Beacom}, J.~F. and 
	{Garnavich}, P.~M. and {Woodward}, C.~E.},
    title = "{Dust to Dust: Three Years in the Evolution of the Unusual SN 2008S}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1202.0279},
 primaryClass = "astro-ph.SR",
 keywords = {stars: evolution, supergiants, supernovae: individual: SN 2008S},
     year = 2012,
    month = may,
   volume = 750,
      eid = {77},
    pages = {77},
      doi = {10.1088/0004-637X/750/1/77},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...750...77S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011ApJ...743..186F,
   author = {{France}, K. and {McCray}, R. and {Penton}, S.~V. and {Kirshner}, R.~P. and 
	{Challis}, P. and {Laming}, J.~M. and {Bouchet}, P. and {Chevalier}, R. and 
	{Garnavich}, P.~M. and {Fransson}, C. and {Heng}, K. and {Larsson}, J. and 
	{Lawrence}, S. and {Lundqvist}, P. and {Panagia}, N. and {Pun}, C.~S.~J. and 
	{Smith}, N. and {Sollerman}, J. and {Sonneborn}, G. and {Sugerman}, B. and 
	{Wheeler}, J.~C.},
    title = "{HST-COS Observations of Hydrogen, Helium, Carbon, and Nitrogen Emission from the SN 1987A Reverse Shock}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1111.1735},
 primaryClass = "astro-ph.SR",
 keywords = {circumstellar matter, shock waves, supernovae: individual: SN 1987A},
     year = 2011,
    month = dec,
   volume = 743,
      eid = {186},
    pages = {186},
      doi = {10.1088/0004-637X/743/2/186},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...743..186F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016A&A...590A..65M,
   author = {{Micelotta}, E.~R. and {Dwek}, E. and {Slavin}, J.~D.},
    title = "{Dust destruction by the reverse shock in the Cassiopeia A supernova remnant}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1602.02754},
 keywords = {dust, extinction, ISM: supernova remnants, shock waves, supernovae: general, supernovae: individual: Cassiopeia A},
     year = 2016,
    month = may,
   volume = 590,
      eid = {A65},
    pages = {A65},
      doi = {10.1051/0004-6361/201527350},
   adsurl = {http://adsabs.harvard.edu/abs/2016A%26A...590A..65M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015Sci...348..413L,
   author = {{Lau}, R.~M. and {Herter}, T.~L. and {Morris}, M.~R. and {Li}, Z. and 
	{Adams}, J.~D.},
    title = "{Old supernova dust factory revealed at the Galactic center}",
  journal = {Science},
archivePrefix = "arXiv",
   eprint = {1503.07173},
 primaryClass = "astro-ph.SR",
     year = 2015,
    month = apr,
   volume = 348,
    pages = {413-418},
      doi = {10.1126/science.aaa2208},
   adsurl = {http://adsabs.harvard.edu/abs/2015Sci...348..413L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2017MNRAS.468.1505M,
   author = {{McKinnon}, R. and {Torrey}, P. and {Vogelsberger}, M. and {Hayward}, C.~C. and 
	{Marinacci}, F.},
    title = "{Simulating the dust content of galaxies: successes and failures}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1606.02714},
 keywords = {methods: numerical, dust, extinction, galaxies: evolution, galaxies: ISM},
     year = 2017,
    month = jun,
   volume = 468,
    pages = {1505-1521},
      doi = {10.1093/mnras/stx467},
   adsurl = {http://adsabs.harvard.edu/abs/2017MNRAS.468.1505M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016ApJ...825..136D,
   author = {{Dwek}, E.},
    title = "{Iron: A Key Element for Understanding the Origin and Evolution of Interstellar Dust}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1605.01957},
 keywords = {dust, extinction, Galaxy: abundances, ISM: abundances, nuclear reactions, nucleosynthesis, abundances, supernovae: general, solar neighborhood},
     year = 2016,
    month = jul,
   volume = 825,
      eid = {136},
    pages = {136},
      doi = {10.3847/0004-637X/825/2/136},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...825..136D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016A&A...589A.132B,
   author = {{Biscaro}, C. and {Cherchneff}, I.},
    title = "{Molecules and dust in Cassiopeia A. II. Dust sputtering and diagnosis of supernova dust survival in remnants}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1511.05487},
 primaryClass = "astro-ph.SR",
 keywords = {supernovae: general, supernovae: individual: Cassiopeia A, dust, extinction, circumstellar matter, ISM: supernova remnants},
     year = 2016,
    month = may,
   volume = 589,
      eid = {A132},
    pages = {A132},
      doi = {10.1051/0004-6361/201527769},
   adsurl = {http://adsabs.harvard.edu/abs/2016A%26A...589A.132B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013ApJ...777...73B,
   author = {{Boogert}, A.~C.~A. and {Chiar}, J.~E. and {Knez}, C. and {{\"O}berg}, K.~I. and 
	{Mundy}, L.~G. and {Pendleton}, Y.~J. and {Tielens}, A.~G.~G.~M. and 
	{van Dishoeck}, E.~F.},
    title = "{Infrared Spectroscopic Survey of the Quiescent Medium of Nearby Clouds. I. Ice Formation and Grain Growth in Lupus}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1309.2999},
 keywords = {infrared: ISM, infrared: stars, ISM: abundances, ISM: molecules, stars: formation},
     year = 2013,
    month = nov,
   volume = 777,
      eid = {73},
    pages = {73},
      doi = {10.1088/0004-637X/777/1/73},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...777...73B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2010ASPC..425..237C,
   author = {{Cherchneff}, I.},
    title = "{Dust Formation in Massive Stars and Their Explosive Ends}",
booktitle = {Hot and Cool: Bridging Gaps in Massive Star Evolution},
     year = 2010,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 425,
archivePrefix = "arXiv",
   eprint = {0909.0164},
 primaryClass = "astro-ph.SR",
   editor = {{Leitherer}, C. and {Bennett}, P.~D. and {Morris}, P.~W. and 
	{Van Loon}, J.~T.},
    month = jun,
    pages = {237},
   adsurl = {http://adsabs.harvard.edu/abs/2010ASPC..425..237C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2004MNRAS.351.1266W,
   author = {{Wyithe}, J.~S.~B.},
    title = "{The shallow slope of the z\~{} 6 quasar luminosity function: limits from the lack of multiple-image gravitational lenses}",
  journal = {\mnras},
   eprint = {astro-ph/0308290},
 keywords = {gravitational lensing, quasars: general},
     year = 2004,
    month = jul,
   volume = 351,
    pages = {1266-1276},
      doi = {10.1111/j.1365-2966.2004.07866.x},
   adsurl = {http://adsabs.harvard.edu/abs/2004MNRAS.351.1266W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2017MNRAS.465.4044B,
   author = {{Bevan}, A. and {Barlow}, M.~J. and {Milisavljevic}, D.},
    title = "{Dust masses for SN 1980K, SN1993J and Cassiopeia A from red-blue emission line asymmetries}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1611.05006},
 primaryClass = "astro-ph.SR",
 keywords = {radiative transfer, supernovae: general, supernovae: individual: SN 1980K, SN 1993J, Cas A, ISM: supernova remnants},
     year = 2017,
    month = mar,
   volume = 465,
    pages = {4044-4056},
      doi = {10.1093/mnras/stw2985},
   adsurl = {http://adsabs.harvard.edu/abs/2017MNRAS.465.4044B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016MNRAS.457.3241A,
   author = {{Andrews}, J.~E. and {Krafton}, K.~M. and {Clayton}, G.~C. and 
	{Montiel}, E. and {Wesson}, R. and {Sugerman}, B.~E.~K. and 
	{Barlow}, M.~J. and {Matsuura}, M. and {Drass}, H.},
    title = "{Early dust formation and a massive progenitor for SN 2011ja?}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1509.06379},
 primaryClass = "astro-ph.SR",
 keywords = {circumstellar matter, supernovae: general, supernovae: individual: SN 20011ja, stars: winds, outflows},
     year = 2016,
    month = apr,
   volume = 457,
    pages = {3241-3253},
      doi = {10.1093/mnras/stw164},
   adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.457.3241A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014ApJ...782L..23H,
   author = {{Hjorth}, J. and {Gall}, C. and {Micha{\l}owski}, M.~J.},
    title = "{Shaping the Dust Mass-Star-formation Rate Relation}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1401.5578},
 keywords = {dust, extinction, galaxies: evolution, galaxies: high-redshift, galaxies: ISM},
     year = 2014,
    month = feb,
   volume = 782,
      eid = {L23},
    pages = {L23},
      doi = {10.1088/2041-8205/782/2/L23},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...782L..23H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013A&A...558L...2W,
   author = {{Wallstr{\"o}m}, S.~H.~J. and {Biscaro}, C. and {Salgado}, F. and 
	{Black}, J.~H. and {Cherchneff}, I. and {Muller}, S. and {Bern{\'e}}, O. and 
	{Rho}, J. and {Tielens}, A.~G.~G.~M.},
    title = "{CO rotational line emission from a dense knot in Cassiopeia A. Evidence for active post-reverse-shock chemistry}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1309.4229},
 keywords = {ISM: supernova remnants, submillimeter: ISM, ISM: individual objects: Cassiopeia A},
     year = 2013,
    month = oct,
   volume = 558,
      eid = {L2},
    pages = {L2},
      doi = {10.1051/0004-6361/201322576},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...558L...2W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011MNRAS.418..820D,
   author = {{D{\'{\i}}az}, C.~G. and {Ryan-Weber}, E.~V. and {Cooke}, J. and 
	{Pettini}, M. and {Madau}, P.},
    title = "{A galaxy as the source of a C IV absorption system close to the epoch of reionization}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1104.4194},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: distances and redshifts, galaxies: high-redshift, intergalactic medium, early Universe},
     year = 2011,
    month = dec,
   volume = 418,
    pages = {820-827},
      doi = {10.1111/j.1365-2966.2011.19534.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.418..820D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011A&A...532A..45S,
   author = {{Stratta}, G. and {Gallerani}, S. and {Maiolino}, R.},
    title = "{Is GRB 050904 at z = 6.3 absorbed by dust?}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1106.4441},
 keywords = {dust, extinction, gamma-ray burst: individual: GRB 050904},
     year = 2011,
    month = aug,
   volume = 532,
      eid = {A45},
    pages = {A45},
      doi = {10.1051/0004-6361/201016414},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...532A..45S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015MNRAS.449.4079M,
   author = {{Mattsson}, L. and {Gomez}, H.~L. and {Andersen}, A.~C. and 
	{Matsuura}, M.},
    title = "{From flux to dust mass: Does the grain-temperature distribution matter for estimates of cold dust masses in supernova remnants?}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1504.02664},
 primaryClass = "astro-ph.SR",
 keywords = {Stars: AGB and post-AGB, supernovae: general, supernovae: individual: Crab nebula, dust, extinction},
     year = 2015,
    month = jun,
   volume = 449,
    pages = {4079-4090},
      doi = {10.1093/mnras/stv487},
   adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.449.4079M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010arXiv1007.0011P,
   author = {{Prieto}, J.~L. and {Szczygiel}, D.~M. and {Kochanek}, C.~S. and 
	{Stanek}, K.~Z. and {Thompson}, T.~A. and {Beacom}, J.~F. and 
	{Garnavich}, P.~M. and {Woodward}, C.~E.},
    title = "{The SN 2008S Progenitor Star: Gone or Again Self-Obscured?}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1007.0011},
 primaryClass = "astro-ph.SR",
 keywords = {Astrophysics - Solar and Stellar Astrophysics},
     year = 2010,
    month = jun,
   adsurl = {http://adsabs.harvard.edu/abs/2010arXiv1007.0011P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2017ApJ...836..129T,
   author = {{Temim}, T. and {Dwek}, E. and {Arendt}, R.~G. and {Borkowski}, K.~J. and 
	{Reynolds}, S.~P. and {Slane}, P. and {Gelfand}, J.~D. and {Raymond}, J.~C.
	},
    title = "{A Massive Shell of Supernova-formed Dust in SNR G54.1+0.3}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1701.01117},
 keywords = {dust, extinction, ISM: general, ISM: individual objects: SNR G54.1+0.3, ISM: supernova remnants, pulsars: individual: PSR J1930+1852},
     year = 2017,
    month = feb,
   volume = 836,
      eid = {129},
    pages = {129},
      doi = {10.3847/1538-4357/836/1/129},
   adsurl = {http://adsabs.harvard.edu/abs/2017ApJ...836..129T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011MNRAS.412.1070K,
   author = {{Kawara}, K. and {Hirashita}, H. and {Nozawa}, T. and {Kozasa}, T. and 
	{Oyabu}, S. and {Matsuoka}, Y. and {Shimizu}, T. and {Sameshima}, H. and 
	{Ienaka}, N.},
    title = "{Supernova dust for the extinction law in a young infrared galaxy at z{\tilde} 1}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1011.0511},
 keywords = {supernovae: general, dust, extinction, galaxies: evolution, galaxies: ISM, galaxies: starburst, infrared: galaxies},
     year = 2011,
    month = apr,
   volume = 412,
    pages = {1070-1080},
      doi = {10.1111/j.1365-2966.2010.17960.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.412.1070K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018NatAs...2...56Z,
   author = {{Zavala}, J.~A. and {Monta{\~n}a}, A. and {Hughes}, D.~H. and 
	{Yun}, M.~S. and {Ivison}, R.~J. and {Valiante}, E. and {Wilner}, D. and 
	{Spilker}, J. and {Aretxaga}, I. and {Eales}, S. and {Avila-Reese}, V. and 
	{Ch{\'a}vez}, M. and {Cooray}, A. and {Dannerbauer}, H. and 
	{Dunlop}, J.~S. and {Dunne}, L. and {G{\'o}mez-Ruiz}, A.~I. and 
	{Micha{\l}owski}, M.~J. and {Narayanan}, G. and {Nayyeri}, H. and 
	{Oteo}, I. and {Rosa Gonz{\'a}lez}, D. and {S{\'a}nchez-Arg{\"u}elles}, D. and 
	{Schloerb}, F.~P. and {Serjeant}, S. and {Smith}, M.~W.~L. and 
	{Terlevich}, E. and {Vega}, O. and {Villalba}, A. and {van der Werf}, P. and 
	{Wilson}, G.~W. and {Zeballos}, M.},
    title = "{A dusty star-forming galaxy at z = 6 revealed by strong gravitational lensing}",
  journal = {Nature Astronomy},
archivePrefix = "arXiv",
   eprint = {1707.09022},
     year = 2018,
    month = jan,
   volume = 2,
    pages = {56-62},
      doi = {10.1038/s41550-017-0297-8},
   adsurl = {http://adsabs.harvard.edu/abs/2018NatAs...2...56Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012A&A...543A..62J,
   author = {{Johansson}, D. and {Horellou}, C. and {Lopez-Cruz}, O. and 
	{Muller}, S. and {Birkinshaw}, M. and {Black}, J.~H. and {Bremer}, M.~N. and 
	{Wall}, W.~F. and {Bertoldi}, F. and {Castillo}, E. and {Ibarra-Medel}, H.~J.
	},
    title = "{Molecular gas and dust in the highly magnified z \~{} 2.8 galaxy behind the Bullet Cluster}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1208.6100},
 primaryClass = "astro-ph.CO",
 keywords = {submillimeter: galaxies, infrared: galaxies, cosmology: observations, gravitational lensing: strong},
     year = 2012,
    month = jul,
   volume = 543,
      eid = {A62},
    pages = {A62},
      doi = {10.1051/0004-6361/201117918},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...543A..62J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011ApJ...741...79O,
   author = {{O'Dowd}, M.~J. and {Schiminovich}, D. and {Johnson}, B.~D. and 
	{Treyer}, M.~A. and {Martin}, C.~D. and {Wyder}, T.~K. and {Charlot}, S. and 
	{Heckman}, T.~M. and {Martins}, L.~P. and {Seibert}, M. and 
	{van der Hulst}, J.~M.},
    title = "{SSGSS: The Spitzer-SDSS-GALEX Spectroscopic Survey}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1201.0107},
 keywords = {dust, extinction, galaxies: active, galaxies: ISM, galaxies: stellar content, infrared: galaxies},
     year = 2011,
    month = nov,
   volume = 741,
      eid = {79},
    pages = {79},
      doi = {10.1088/0004-637X/741/2/79},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...741...79O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011MNRAS.418..571F,
   author = {{Fallest}, D.~W. and {Nozawa}, T. and {Nomoto}, K. and {Umeda}, H. and 
	{Maeda}, K. and {Kozasa}, T. and {Lazzati}, D.},
    title = "{On the effects of microphysical grain properties on the yields of carbonaceous dust from Type II supernovae}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1105.4631},
 primaryClass = "astro-ph.SR",
 keywords = {supernovae: general, dust, extinction},
     year = 2011,
    month = nov,
   volume = 418,
    pages = {571-582},
      doi = {10.1111/j.1365-2966.2011.19506.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.418..571F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011ApJ...741L..20J,
   author = {{Jang}, M. and {Im}, M. and {Lee}, I. and {Urata}, Y. and {Huang}, K. and 
	{Hirashita}, H. and {Fan}, X. and {Jiang}, L.},
    title = "{Dust Properties in the Afterglow of GRB 071025 at z \~{} 5}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1110.3259},
 primaryClass = "astro-ph.CO",
 keywords = {dust, extinction, galaxies: high-redshift, galaxies: ISM, gamma-ray burst: general, gamma-ray burst: individual: GRB 071025},
     year = 2011,
    month = nov,
   volume = 741,
      eid = {L20},
    pages = {L20},
      doi = {10.1088/2041-8205/741/1/L20},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...741L..20J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2005MNRAS.363...57L,
   author = {{Lawrence}, A.},
    title = "{Blue, green and red bumps in active galactic nuclei}",
  journal = {\mnras},
   eprint = {astro-ph/0507100},
 keywords = {accretion, accretion discs, galaxies: active, quasars: general},
     year = 2005,
    month = oct,
   volume = 363,
    pages = {57-63},
      doi = {10.1111/j.1365-2966.2005.09392.x},
   adsurl = {http://adsabs.harvard.edu/abs/2005MNRAS.363...57L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016ApJ...826..150D,
   author = {{Dopita}, M.~A. and {Seitenzahl}, I.~R. and {Sutherland}, R.~S. and 
	{Vogt}, F.~P.~A. and {Winkler}, P.~F. and {Blair}, W.~P.},
    title = "{Forbidden Iron Lines and Dust Destruction in Supernova Remnant Shocks: The Case of N49 in the Large Magellanic Cloud}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1605.02385},
 keywords = {dust, extinction, ISM: individual objects: N49, ISM: supernova remnants, Magellanic Clouds, shock waves},
     year = 2016,
    month = aug,
   volume = 826,
      eid = {150},
    pages = {150},
      doi = {10.3847/0004-637X/826/2/150},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...826..150D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2012ASSL..384..145S,
   author = {{Smith}, N.},
    title = "{All Things Homunculus}",
booktitle = {Eta Carinae and the Supernova Impostors},
     year = 2012,
   series = {Astrophysics and Space Science Library},
   volume = 384,
   editor = {{Davidson}, K. and {Humphreys}, R.~M.},
    pages = {145},
      doi = {10.1007/978-1-4614-2275-4_7},
   adsurl = {http://adsabs.harvard.edu/abs/2012ASSL..384..145S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2011IAUS..280..228C,
   author = {{Cherchneff}, I. and {Sarangi}, A.},
    title = "{Molecules in Supernova Ejecta}",
 keywords = {supernovae: general, molecular processes, astrochemistry},
booktitle = {The Molecular Universe},
     year = 2011,
   series = {IAU Symposium},
   volume = 280,
archivePrefix = "arXiv",
   eprint = {1107.5668},
 primaryClass = "astro-ph.SR",
   editor = {{Cernicharo}, J. and {Bachiller}, R.},
    month = dec,
    pages = {228-236},
      doi = {10.1017/S1743921311025002},
   adsurl = {http://adsabs.harvard.edu/abs/2011IAUS..280..228C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011MNRAS.418..625S,
   author = {{Shimizu}, T. and {Kawara}, K. and {Sameshima}, H. and {Ienaka}, N. and 
	{Nozawa}, T. and {Kozasa}, T.},
    title = "{Extinction law in ultraluminous infrared galaxies at z{\tilde} 1}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1107.5381},
 keywords = {supernovae: general, dust, extinction, galaxies: evolution, galaxies: ISM, galaxies: starburst, infrared: galaxies},
     year = 2011,
    month = nov,
   volume = 418,
    pages = {625-637},
      doi = {10.1111/j.1365-2966.2011.19512.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.418..625S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010CBET.2539....1Y,
   author = {{Yamanaka}, M. and {Okushima}, T. and {Arai}, A. and {Sasada}, M. and 
	{Sato}, H.},
    title = "{Supernova 2010jl in UGC 5189A}",
  journal = {Central Bureau Electronic Telegrams},
     year = 2010,
    month = nov,
   volume = 2539,
   adsurl = {http://adsabs.harvard.edu/abs/2010CBET.2539....1Y},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1965AnAp...28..860C,
   author = {{Cernuschi}, F. and {Marsicano}, F.~R. and {Kimel}, I.},
    title = "{On polarisation of stellar light}",
  journal = {Annales d'Astrophysique},
     year = 1965,
    month = feb,
   volume = 28,
    pages = {860},
   adsurl = {http://adsabs.harvard.edu/abs/1965AnAp...28..860C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2017MNRAS.464..246B,
   author = {{Baba}, J. and {Morokuma-Matsui}, K. and {Saitoh}, T.~R.},
    title = "{Eventful evolution of giant molecular clouds in dynamically evolving spiral arms}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1609.00097},
 keywords = {methods: numerical, ISM: clouds, ISM: structure, galaxies: ISM, galaxies: kinematics and dynamics, galaxies: spiral},
     year = 2017,
    month = jan,
   volume = 464,
    pages = {246-263},
      doi = {10.1093/mnras/stw2378},
   adsurl = {http://adsabs.harvard.edu/abs/2017MNRAS.464..246B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{1987ESOC...26...79B,
   author = {{Bouchet}, P. and {Le Bertre}, T. and {Manfroid}, J. and {Stanga}, R. and 
	{Moneti}, A.},
    title = "{Infrared photometry of SN 1987A - The first four months}",
 keywords = {Infrared Photometry, Stellar Spectrophotometry, Supernova 1987a, Ejecta, Light Curve, Radii, Spectral Energy Distribution, Stellar Luminosity, Stellar Temperature},
booktitle = {European Southern Observatory Conference and Workshop Proceedings},
     year = 1987,
   series = {European Southern Observatory Conference and Workshop Proceedings},
   volume = 26,
   editor = {{Danziger}, I.~J.},
    pages = {79-85},
   adsurl = {http://adsabs.harvard.edu/abs/1987ESOC...26...79B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018MNRAS.473.4538G,
   author = {{Ginolfi}, M. and {Graziani}, L. and {Schneider}, R. and {Marassi}, S. and 
	{Valiante}, R. and {Dell'Agli}, F. and {Ventura}, P. and {Hunt}, L.~K.
	},
    title = "{Where does galactic dust come from?}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1707.05328},
 keywords = {stars: AGB and post-AGB, supernovae: general, dust, extinction, local interstellar matter, galaxies: evolution},
     year = 2018,
    month = feb,
   volume = 473,
    pages = {4538-4543},
      doi = {10.1093/mnras/stx2572},
   adsurl = {http://adsabs.harvard.edu/abs/2018MNRAS.473.4538G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018Natur.553...51M,
   author = {{Marrone}, D.~P. and {Spilker}, J.~S. and {Hayward}, C.~C. and 
	{Vieira}, J.~D. and {Aravena}, M. and {Ashby}, M.~L.~N. and 
	{Bayliss}, M.~B. and {B{\'e}thermin}, M. and {Brodwin}, M. and 
	{Bothwell}, M.~S. and {Carlstrom}, J.~E. and {Chapman}, S.~C. and 
	{Chen}, C.-C. and {Crawford}, T.~M. and {Cunningham}, D.~J.~M. and 
	{De Breuck}, C. and {Fassnacht}, C.~D. and {Gonzalez}, A.~H. and 
	{Greve}, T.~R. and {Hezaveh}, Y.~D. and {Lacaille}, K. and {Litke}, K.~C. and 
	{Lower}, S. and {Ma}, J. and {Malkan}, M. and {Miller}, T.~B. and 
	{Morningstar}, W.~R. and {Murphy}, E.~J. and {Narayanan}, D. and 
	{Phadke}, K.~A. and {Rotermund}, K.~M. and {Sreevani}, J. and 
	{Stalder}, B. and {Stark}, A.~A. and {Strandet}, M.~L. and {Tang}, M. and 
	{Wei{\ss}}, A.},
    title = "{Galaxy growth in a massive halo in the first billion years of cosmic history}",
  journal = {\nat},
archivePrefix = "arXiv",
   eprint = {1712.03020},
     year = 2018,
    month = jan,
   volume = 553,
    pages = {51-54},
      doi = {10.1038/nature24629},
   adsurl = {http://adsabs.harvard.edu/abs/2018Natur.553...51M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013EP&S...65..223K,
   author = {{Kemper}, F.},
    title = "{Stellar dust production and composition in the Magellanic Clouds}",
  journal = {Earth, Planets, and Space},
archivePrefix = "arXiv",
   eprint = {1212.3891},
 keywords = {Stars: AGB post-AGB stars, stars: mass loss, circumstellar matter, dust, Magellanic Clouds},
     year = 2013,
    month = mar,
   volume = 65,
    pages = {223-227},
      doi = {10.5047/eps.2012.04.013},
   adsurl = {http://adsabs.harvard.edu/abs/2013EP%26S...65..223K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011ApJ...742...80W,
   author = {{Winkler}, P.~F. and {Hamilton}, A.~J.~S. and {Long}, K.~S. and 
	{Fesen}, R.~A.},
    title = "{Time Evolution of the Reverse Shock in SN 1006}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1109.0204},
 primaryClass = "astro-ph.GA",
 keywords = {ISM: individual objects: SN 1006 SNR G327.6+14.6, ISM: supernova remnants, shock waves, supernovae: individual: SN 1006},
     year = 2011,
    month = dec,
   volume = 742,
      eid = {80},
    pages = {80},
      doi = {10.1088/0004-637X/742/2/80},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...742...80W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016ApJ...831..188G,
   author = {{Ghavamian}, P. and {Williams}, B.~J.},
    title = "{The Cold Dust Content of the Oxygen-rich Supernova Remnant G292.0+1.8}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1608.03373},
 primaryClass = "astro-ph.HE",
 keywords = {ISM: individual objects: G292.0+1.8, ISM: kinematics and dynamics, ISM: supernova remnants, plasmas, shock waves},
     year = 2016,
    month = nov,
   volume = 831,
      eid = {188},
    pages = {188},
      doi = {10.3847/0004-637X/831/2/188},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...831..188G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018MNRAS.475.2236K,
   author = {{Krumholz}, M.~R. and {Ting}, Y.-S.},
    title = "{Metallicity fluctuation statistics in the interstellar medium and young stars - I. Variance and correlation}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1708.06853},
 keywords = {diffusion, stars: abundances, ISM: abundances, Galaxy: abundances, galaxies: abundances, galaxies: ISM},
     year = 2018,
    month = apr,
   volume = 475,
    pages = {2236-2252},
      doi = {10.1093/mnras/stx3286},
   adsurl = {http://adsabs.harvard.edu/abs/2018MNRAS.475.2236K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018arXiv180204027A,
   author = {{Aoyama}, S. and {Hou}, K.-C. and {Hirashita}, H. and {Nagamine}, K. and 
	{Shimizu}, I.},
    title = "{Cosmological simulation with dust formation and destruction}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1802.04027},
 keywords = {Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
     year = 2018,
    month = feb,
   adsurl = {http://adsabs.harvard.edu/abs/2018arXiv180204027A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018arXiv180110166H,
   author = {{Hopkins}, P.~F. and {Squire}, J.},
    title = "{Ubiquitous Instabilities of Dust Moving in Magnetized Gas}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1801.10166},
 keywords = {Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Solar and Stellar Astrophysics, Physics - Fluid Dynamics, Physics - Plasma Physics},
     year = 2018,
    month = jan,
   adsurl = {http://adsabs.harvard.edu/abs/2018arXiv180110166H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2017arXiv170708230R,
   author = {{Rho}, J. and {Gomez}, H.~L. and {Boogert}, A. and {Smith}, M.~W.~L. and 
	{Lagage}, P.-O and {Dowell}, D. and {Clark}, C.~J.~R.},
    title = "{A Dust Twin of Cas A: Cool Dust and Pre-Solar Grain of Silica Revealed in the Supernova Remnant G54.1+0.3}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1707.08230},
 keywords = {Astrophysics - Astrophysics of Galaxies},
     year = 2017,
    month = jul,
   adsurl = {http://adsabs.harvard.edu/abs/2017arXiv170708230R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018MNRAS.476.1371C,
   author = {{Ceccarelli}, C. and {Viti}, S. and {Balucani}, N. and {Taquet}, V.
	},
    title = "{The evolution of grain mantles and silicate dust growth at high redshift}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1802.01142},
 keywords = {astrochemistry, dust, extinction, ISM: molecules, galaxies: high-redshift, galaxies: ISM},
     year = 2018,
    month = may,
   volume = 476,
    pages = {1371-1383},
      doi = {10.1093/mnras/sty313},
   adsurl = {http://adsabs.harvard.edu/abs/2018MNRAS.476.1371C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018arXiv180304286N,
   author = {{Nittler}, L.~R. and {Alexander}, C.~M.~O. and {Liu}, N. and 
	{Wang}, J.},
    title = "{Extremely $^{54}$Cr- and $^{50}$Ti-rich presolar oxide grains in a primitive meteorite: Formation in rare types of supernovae and implications for the astrophysical context of solar system birth}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1803.04286},
 primaryClass = "astro-ph.EP",
 keywords = {Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
     year = 2018,
    month = mar,
   adsurl = {http://adsabs.harvard.edu/abs/2018arXiv180304286N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018arXiv180301929Z,
   author = {{Zhukovska}, S. and {Henning}, T. and {Dobbs}, C.},
    title = "{Iron and silicate dust growth in the Galactic interstellar medium: clues from element depletions}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1803.01929},
 keywords = {Astrophysics - Astrophysics of Galaxies},
     year = 2018,
    month = mar,
   adsurl = {http://adsabs.harvard.edu/abs/2018arXiv180301929Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018arXiv180110382C,
   author = {{Ceverino}, D. and {Klessen}, R. and {Glover}, S.},
    title = "{FirstLight II: Star formation rates of primeval galaxies from z=5-15}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1801.10382},
 keywords = {Astrophysics - Astrophysics of Galaxies},
     year = 2018,
    month = jan,
   adsurl = {http://adsabs.harvard.edu/abs/2018arXiv180110382C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018arXiv180106859F,
   author = {{Fry}, B.~J. and {Fields}, B.~D. and {Ellis}, J.~R.},
    title = "{No Escape from the Supernova! Magnetic Imprisonment of Dusty Pinballs by a Supernova Remnant}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1801.06859},
 primaryClass = "astro-ph.HE",
 keywords = {Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
     year = 2018,
    month = jan,
   adsurl = {http://adsabs.harvard.edu/abs/2018arXiv180106859F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018arXiv180104217B,
   author = {{Bak Nielsen}, A.-S. and {Hjorth}, J. and {Gall}, C.},
    title = "{Early gray dust formation in the type IIn SN 2005ip}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1801.04217},
 primaryClass = "astro-ph.SR",
 keywords = {Astrophysics - Solar and Stellar Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
     year = 2018,
    month = jan,
   adsurl = {http://adsabs.harvard.edu/abs/2018arXiv180104217B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2017ApJ...843...95M,
   author = {{Mart{\'{\i}}nez-Gonz{\'a}lez}, S. and {W{\"u}nsch}, R. and 
	{Palou{\v s}}, J.},
    title = "{Can Dust Injected by SNe Explain the NIR-MIR Excess in Young Massive Stellar Clusters?}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1705.08899},
 keywords = {dust, extinction, galaxies: star clusters: general, galaxies: star clusters: individual: NGC 604, NGC 595, hydrodynamics, infrared: ISM},
     year = 2017,
    month = jul,
   volume = 843,
      eid = {95},
    pages = {95},
      doi = {10.3847/1538-4357/aa7510},
   adsurl = {http://adsabs.harvard.edu/abs/2017ApJ...843...95M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2010AIPC.1294..122C,
   author = {{Cherchneff}, I.},
    title = "{Molecules and Dust in the Early Universe: the Supernova Connection}",
 keywords = {Universe, supernovae, star formation, stellar clusters, Particle-theory and field-theory models of the early Universe, Supernovae, Star formation, Open clusters in external galaxies},
booktitle = {American Institute of Physics Conference Series},
     year = 2010,
   series = {American Institute of Physics Conference Series},
   volume = 1294,
   editor = {{Whalen}, D.~J. and {Bromm}, V. and {Yoshida}, N.},
    month = nov,
    pages = {122-127},
      doi = {10.1063/1.3518839},
   adsurl = {http://adsabs.harvard.edu/abs/2010AIPC.1294..122C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



==> OLD/yahapjbst <==
% yahapj.bst -- yet another ApJ bibtex style file
% Git SHA1 hash: $Id$
% Reference repository: https://github.com/pkgw/yahapj/
%
% The main features compared to other ApJ style files is that ArXiV
% and DOI links are added. ArXiV information is only shown for those
% entries that don't have more formal reference information. There are
% other improvements too.
%
% Because this style file embeds links, your LaTeX file must use the
% hyperref package. For non-butt-ugly links, try:
%
% \usepackage[breaklinks,colorlinks,urlcolor=blue,citecolor=blue,linkcolor=blue]{hyperref}
%
% Copyright notice: This work is dedicated to the public domain. You
% have unlimited permission to copy, distribute, and modify it.
%
% For more information about this file and its provenance, consult
% README.md in the Git repository from which it was obtained. You can
% track these down using the SHA1 hash listed at the top of this file.
% (Googling for the hash value should hopefully be sufficient.)

ENTRY
  { address
    archive
    archivePrefix
    author
    booktitle
    chapter
    doi
    edition
    editor
    eprint
    howpublished
    institution
    isbn
    journal
    key
    month
    note
    number
    organization
    pages
    primaryClass
    publisher
    school
    series
    title
    type
    url
    volume
    year
  }
  {}
  { label extra.label sort.label short.list }

INTEGERS { output.state before.all mid.sentence after.sentence after.block work.strlen }

FUNCTION {init.state.consts}
{ #0 'before.all :=
  #1 'mid.sentence :=
  #2 'after.sentence :=
  #3 'after.block :=
}

STRINGS { s t }

FUNCTION {output.nonnull}
{ 's :=
  output.state mid.sentence =
    { ", " * write$ }
    { output.state after.block =
        { add.period$ write$
          newline$
          "\newblock " write$
        }
        { output.state before.all =
            'write$
            { add.period$ " " * write$ }
          if$
        }
      if$
      mid.sentence 'output.state :=
    }
  if$
  s
}

FUNCTION {output}
{ duplicate$ empty$
    'pop$
    'output.nonnull
  if$
}

FUNCTION {output.check}
{ 't :=
  duplicate$ empty$
    { pop$ "empty " t * " in " * cite$ * warning$ }
    'output.nonnull
  if$
}

FUNCTION {fin.entry}
{ duplicate$ empty$
    'pop$
    'write$
  if$
  newline$
}

FUNCTION {new.block}
{ output.state before.all =
    'skip$
    { after.block 'output.state := }
  if$
}

FUNCTION {new.sentence}
{ output.state after.block =
    'skip$
    { output.state before.all =
        'skip$
        { after.sentence 'output.state := }
      if$
    }
  if$
}

FUNCTION {add.blank}
{  " " * before.all 'output.state :=
}

FUNCTION {not}
{   { #0 }
    { #1 }
  if$
}

FUNCTION {and}
{   'skip$
    { pop$ #0 }
  if$
}

FUNCTION {or}
{   { pop$ #1 }
    'skip$
  if$
}

FUNCTION {new.block.checkb}
{ empty$
  swap$ empty$
  and
    'skip$
    'new.block
  if$
}

FUNCTION {field.or.null}
{ duplicate$ empty$
    { pop$ "" }
    'skip$
  if$
}

FUNCTION {capitalize}
{ "u" change.case$ "t" change.case$ }

FUNCTION {space.word}
{ " " swap$ * " " * }

% Here's how BibTeX does internationalization:

FUNCTION {bbl.and}
{ "and"}

FUNCTION {bbl.editors}
{ "eds." }

FUNCTION {bbl.editor}
{ "ed." }

FUNCTION {bbl.edby}
{ "edited by" }

FUNCTION {bbl.edition}
{ "edn." }

FUNCTION {bbl.volume}
{ "Vol." }

FUNCTION {bbl.of}
{ "of" }

FUNCTION {bbl.number}
{ "no." }

FUNCTION {bbl.nr}
{ "no." }

FUNCTION {bbl.in}
{ "in" }

FUNCTION {bbl.pages}
{ "" }

FUNCTION {bbl.page}
{ "" }

FUNCTION {bbl.chapter}
{ "Ch." }

FUNCTION {bbl.techrep}
{ "Tech. Rep." }

FUNCTION {bbl.mthesis}
{ "Master's thesis" }

FUNCTION {bbl.phdthesis}
{ "PhD thesis" }

FUNCTION {bbl.first}
{ "1st" }

FUNCTION {bbl.second}
{ "2nd" }

FUNCTION {bbl.third}
{ "3rd" }

FUNCTION {bbl.fourth}
{ "4th" }

FUNCTION {bbl.fifth}
{ "5th" }

FUNCTION {bbl.st}
{ "st" }

FUNCTION {bbl.nd}
{ "nd" }

FUNCTION {bbl.rd}
{ "rd" }

FUNCTION {bbl.th}
{ "th" }

MACRO {jan} {"Jan."}

MACRO {feb} {"Feb."}

MACRO {mar} {"Mar."}

MACRO {apr} {"Apr."}

MACRO {may} {"May"}

MACRO {jun} {"Jun."}

MACRO {jul} {"Jul."}

MACRO {aug} {"Aug."}

MACRO {sep} {"Sep."}

MACRO {oct} {"Oct."}

MACRO {nov} {"Nov."}

MACRO {dec} {"Dec."}

FUNCTION {eng.ord}
{ duplicate$ "1" swap$ *
  #-2 #1 substring$ "1" =
     { bbl.th * }
     { duplicate$ #-1 #1 substring$
       duplicate$ "1" =
         { pop$ bbl.st * }
         { duplicate$ "2" =
             { pop$ bbl.nd * }
             { "3" =
                 { bbl.rd * }
                 { bbl.th * }
               if$
             }
           if$
          }
       if$
     }
   if$
}

INTEGERS { nameptr namesleft numnames numtrunc }

FUNCTION {format.names}
{ 's :=
  #0 'numtrunc :=
  #1 'nameptr :=
  s num.names$ 'numnames :=
  numnames 'namesleft :=
  numnames #5 >
    { #3 'numtrunc := }
    {}
  if$
  { namesleft #0 > }
  { s nameptr
    "{vv~}{ll}{, jj}{, f.}" format.name$
    't :=
    nameptr #1 >
      {
        nameptr #1 - numtrunc =
          {
            #1 'namesleft :=
            "others" 't :=
          }
          {}
        if$

        namesleft #1 >
          { ", " * t * }
          {
            numnames #1 >
              { "," * }
              'skip$
            if$
            s nameptr "{ll}" format.name$ duplicate$ "others" =
              { 't := }
              { pop$ }
            if$
            t "others" =
              {
                " {et~al.}" *
              }
              { " \& " * t * }
            if$
          }
        if$
      }
      't
    if$
    nameptr #1 + 'nameptr :=
    namesleft #1 - 'namesleft :=
  }
  while$
}

FUNCTION {format.names.ed}
{ 's :=
  #1 'nameptr :=
  s num.names$ 'numnames :=
  numnames 'namesleft :=
    { namesleft #0 > }
    { s nameptr
      "{f.~}{vv~}{ll}{, jj}"
      format.name$
      't :=
      nameptr #1 >
        {
          namesleft #1 >
            { ", " * t * }
            {
              numnames #2 >
                { "," * }
                'skip$
              if$
              s nameptr "{ll}" format.name$ duplicate$ "others" =
                { 't := }
                { pop$ }
              if$
              t "others" =
                {
                  " {et~al.}" *
                }
                { " \& " * t * }
              if$
            }
          if$
        }
        't
      if$
      nameptr #1 + 'nameptr :=
      namesleft #1 - 'namesleft :=
    }
  while$
}

FUNCTION {format.key}
{ empty$
    { key field.or.null }
    { "" }
  if$
}

FUNCTION {format.authors}
{ author empty$
    { "" }
    { author format.names }
  if$
}

FUNCTION {format.editors}
{ editor empty$
    { "" }
    { editor format.names
      editor num.names$ #1 >
        { ", " * bbl.editors * }
        { ", " * bbl.editor * }
      if$
    }
  if$
}

FUNCTION {format.in.editors}
{ editor empty$
    { "" }
    { editor format.names.ed
    }
  if$
}

FUNCTION {format.note}
{ note empty$
    { "" }
    { note #1 #1 substring$
      duplicate$ "{" =
        'skip$
        { output.state mid.sentence =
          { "l" }
          { "u" }
        if$
        change.case$
        }
      if$
      note #2 global.max$ substring$ *
    }
  if$
}

FUNCTION {format.title}
{ title empty$
    { "" }
    { title
    }
  if$
}

FUNCTION {format.full.names}
{'s :=
  #1 'nameptr :=
  s num.names$ 'numnames :=
  numnames 'namesleft :=
    { namesleft #0 > }
    { s nameptr
      "{vv~}{ll}" format.name$
      't :=
      nameptr #1 >
        {
          namesleft #1 >
            { ", " * t * }
            {
              numnames #2 >
                { "," * }
                'skip$
              if$
              s nameptr "{ll}" format.name$ duplicate$ "others" =
                { 't := }
                { pop$ }
              if$
              t "others" =
                {
                  " {et~al.}" *
                }
                { " \& " * t * }
              if$
            }
          if$
        }
        't
      if$
      nameptr #1 + 'nameptr :=
      namesleft #1 - 'namesleft :=
    }
  while$
}

FUNCTION {author.editor.key.full}
{ author empty$
    { editor empty$
        { key empty$
            { cite$ #1 #3 substring$ }
            'key
          if$
        }
        { editor format.full.names }
      if$
    }
    { author format.full.names }
  if$
}

FUNCTION {author.key.full}
{ author empty$
    { key empty$
         { cite$ #1 #3 substring$ }
          'key
      if$
    }
    { author format.full.names }
  if$
}

FUNCTION {editor.key.full}
{ editor empty$
    { key empty$
         { cite$ #1 #3 substring$ }
          'key
      if$
    }
    { editor format.full.names }
  if$
}

FUNCTION {make.full.names}
{ type$ "book" =
  type$ "inbook" =
  or
    'author.editor.key.full
    { type$ "proceedings" =
        'editor.key.full
        'author.key.full
      if$
    }
  if$
}

FUNCTION {output.bibitem}
{ newline$
  "\bibitem[{" write$
  label write$
  ")" make.full.names duplicate$ short.list =
     { pop$ }
     { * }
   if$
  "}]{" * write$
  cite$ write$
  "}" write$
  newline$
  ""
  before.all 'output.state :=
}

FUNCTION {format.archive}
{ archivePrefix empty$
    { "" }
    { archivePrefix ":" *}
  if$
}

FUNCTION {format.primaryClass}
{ primaryClass empty$
    { "" }
    { " [" primaryClass * "]" *}
  if$
}

FUNCTION {format.eprint}
% Only print eprint info if no page info and no booktitle info --
% what we're really going for is print the eprint info only if there's
% no "official" reference info to work with.
{ eprint empty$
  pages empty$ not
  booktitle empty$ not or or
    { "" }
     { archive empty$
          {"\href{http://arxiv.org/abs/" eprint * "}" *
             "{{\sffamily " * format.archive * eprint *
              format.primaryClass * "}}" *}
          {"\href{" archive *  "/" * eprint * "}" *
             "{{\sffamily " * format.archive * eprint *
              format.primaryClass * "}}" *}
       if$
     }
  if$
}


FUNCTION {n.dashify}
{
  't :=
  ""
    { t empty$ not }
    { t #1 #1 substring$ "-" =
        { t #1 #2 substring$ "--" = not
            { "--" *
              t #2 global.max$ substring$ 't :=
            }
            {   { t #1 #1 substring$ "-" = }
                { "-" *
                  t #2 global.max$ substring$ 't :=
                }
              while$
            }
          if$
        }
        { t #1 #1 substring$ *
          t #2 global.max$ substring$ 't :=
        }
      if$
    }
  while$
}

FUNCTION {word.in}
{ bbl.in
  " " * }

FUNCTION {format.date}
{ year duplicate$ empty$
    { "empty year in " cite$ * "; set to ????" * warning$
       pop$ "????" }
    'skip$
  if$
  extra.label *
  before.all 'output.state :=
  after.sentence 'output.state :=
}

FUNCTION {format.btitle}
{ title
}

FUNCTION {tie.or.space.connect}
{ duplicate$ text.length$ #3 <
    { "~" }
    { " " }
  if$
  swap$ * *
}

FUNCTION {either.or.check}
{ empty$
    'pop$
    { "can't use both " swap$ * " fields in " * cite$ * warning$ }
  if$
}

FUNCTION {format.bvolume}
{ volume empty$
    { "" }
    { bbl.volume volume tie.or.space.connect
      series empty$
        'skip$
        { bbl.of space.word * series * }
      if$
      "volume and number" number either.or.check
    }
  if$
}

FUNCTION {format.number.series}
{ volume empty$
    { number empty$
        { series field.or.null }
        { output.state mid.sentence =
            { bbl.number }
            { bbl.number capitalize }
          if$
          number tie.or.space.connect
          series empty$
            { "there's a number but no series in " cite$ * warning$ }
            { bbl.in space.word * series * }
          if$
        }
      if$
    }
    { "" }
  if$
}

FUNCTION {is.num}
{ chr.to.int$
  duplicate$ "0" chr.to.int$ < not
  swap$ "9" chr.to.int$ > not and
}

FUNCTION {extract.num}
{ duplicate$ 't :=
  "" 's :=
  { t empty$ not }
  { t #1 #1 substring$
    t #2 global.max$ substring$ 't :=
    duplicate$ is.num
      { s swap$ * 's := }
      { pop$ "" 't := }
    if$
  }
  while$
  s empty$
    'skip$
    { pop$ s }
  if$
}

FUNCTION {convert.edition}
{ edition extract.num "l" change.case$ 's :=
  s "first" = s "1" = or
    { bbl.first 't := }
    { s "second" = s "2" = or
        { bbl.second 't := }
        { s "third" = s "3" = or
            { bbl.third 't := }
            { s "fourth" = s "4" = or
                { bbl.fourth 't := }
                { s "fifth" = s "5" = or
                    { bbl.fifth 't := }
                    { s #1 #1 substring$ is.num
                        { s eng.ord 't := }
                        { edition 't := }
                      if$
                    }
                  if$
                }
              if$
            }
          if$
        }
      if$
    }
  if$
  t
}

FUNCTION {format.edition}
{ edition empty$
    { "" }
    { output.state mid.sentence =
        { convert.edition "l" change.case$ " " * bbl.edition * }
        { convert.edition "t" change.case$ " " * bbl.edition * }
      if$
    }
  if$
}

INTEGERS { multiresult }

FUNCTION {multi.page.check}
{ 't :=
  #0 'multiresult :=
    { multiresult not
      t empty$ not
      and
    }
    { t #1 #1 substring$
      duplicate$ "-" =
      swap$ duplicate$ "," =
      swap$ "+" =
      or or
        { #1 'multiresult := }
        { t #2 global.max$ substring$ 't := }
      if$
    }
  while$
  multiresult
}

FUNCTION {string.length}
{ % Copied from "Taming the BeaST", by Nicolas Markey, Fig 4
  #1 'work.strlen :=
  { duplicate$ duplicate$ #1 work.strlen substring$ = not }
    { work.strlen #1 + 'work.strlen := }
  while$
  pop$ work.strlen
}

FUNCTION {first.page}
{ 't :=
  ""
    {  t empty$ not t #1 #1 substring$ "-" = not and }
    { t #1 #1 substring$ *
      t #2 global.max$ substring$ 't :=
    }
  while$
  % remove possible trailing plus sign
  duplicate$ duplicate$ string.length #1 substring$ "+" =
    { duplicate$ string.length #1 - #1 swap$ substring$ }
    { }
  if$
}

FUNCTION {format.pages}
{ pages empty$
    { "" }
    { pages first.page }
  if$
}

FUNCTION {format.journal.pages}
{ pages empty$
    'skip$
    { duplicate$ empty$
        { pop$ format.pages }
        {
          ", " *
          pages first.page *
        }
      if$
    }
  if$
}

FUNCTION {format.vol.num.pages}
{ volume field.or.null
}

FUNCTION {format.chapter.pages}
{ chapter empty$
    { "" }
    { type empty$
        { bbl.chapter }
        { type "l" change.case$ }
      if$
      chapter tie.or.space.connect
    }
  if$
}

FUNCTION {format.in.ed.booktitle}
{ booktitle empty$
    { "" }
    { editor empty$
        { word.in booktitle * }
        { word.in booktitle *
          ", " *
          editor num.names$ #1 >
            { bbl.editors }
            { bbl.editor }
          if$
          * " " *
          format.in.editors *
        }
      if$
    }
  if$
}

FUNCTION {format.thesis.type}
{ type empty$
    'skip$
    { pop$
      type "t" change.case$
    }
  if$
}

FUNCTION {format.tr.number}
{ type empty$
    { bbl.techrep }
    'type
  if$
  number empty$
    { "t" change.case$ }
    { number tie.or.space.connect }
  if$
}

FUNCTION {format.article.crossref}
{
  word.in
  " \cite{" * crossref * "}" *
}

FUNCTION {format.book.crossref}
{ volume empty$
    { "empty volume in " cite$ * "'s crossref of " * crossref * warning$
      word.in
    }
    { bbl.volume volume tie.or.space.connect
      bbl.of space.word *
    }
  if$
  " \cite{" * crossref * "}" *
}

FUNCTION {format.incoll.inproc.crossref}
{
  word.in
  " \cite{" * crossref * "}" *
}

FUNCTION {format.publisher}
{ publisher empty$
    { "empty publisher in " cite$ * warning$ }
    'skip$
  if$
  ""
  address empty$ publisher empty$ and
    'skip$
    {
      add.blank "(" *
      address empty$
        'skip$
        { address * }
      if$
      publisher empty$
        'skip$
        { address empty$
            'skip$
            { ": " * }
          if$
          publisher *
        }
      if$
      ")" *
    }
  if$
  output
}

STRINGS {oldname}

FUNCTION {name.or.dash}
{ 's :=
   oldname empty$
     { s 'oldname := s }
     { s oldname =
         { "---" }
         { s 'oldname := s }
       if$
     }
   if$
}

FUNCTION {format.edn.btitle} % Title should be on stack.
{ duplicate$ empty$ edition empty$ or
    'skip$
    { ", " * format.edition * }
  if$
}

FUNCTION {format.ed.booktitle} % The title should be on the stack.
{ duplicate$ empty$
  { "no book title in " cite$ * warning$ "" pop$ }
  { editor empty$
    author empty$ or  % Empty author means editor already given.
      'format.edn.btitle
      { format.edn.btitle ", " * bbl.editor * " " * format.in.editors * }
      if$
  }
  if$
}

FUNCTION {format.full.book.spec} % The title should be on the stack.
{ series empty$
    { format.ed.booktitle
      volume empty$
	{ number empty$
	    'skip$
	    { " there's a number but no series in " cite$ * warning$
	      " No." number tie.or.space.connect * }
	    if$
	}
	{ ", Vol." volume tie.or.space.connect *
	  number empty$
	    'skip$
	    {"Both volume and number fields in " * cite$ * warning$ }
	    if$
	}
	if$
    }
    { volume empty$
	{ format.ed.booktitle ", " * series *
	  number empty$
	    'skip$
	    { " No." number tie.or.space.connect * }
	    if$
	}
	{ series ", Vol." volume tie.or.space.connect *
          ", " * swap$ format.ed.booktitle *
	  number empty$
	    'skip$
	    {"Both volume and number fields in " * cite$ * warning$ }
	    if$
	}
        if$
    }
    if$
}

FUNCTION {maybe.doi.link.prepend}
{ % Expects some citation text to be on the stack
 doi empty$
  { url empty$
     { }
     { "\href{" url * "}{" * swap$ * }
    if$
  }
  { "\href{http://dx.doi.org/" doi * "}{" * swap$ * }
 if$
}

FUNCTION {maybe.doi.link.end}
{ % Expects some citation text to be on the stack
 doi empty$ url empty$ and
  { }
  { "}" * }
 if$
}

FUNCTION {format.journal}
{
  journal empty$
    { "" } % warning will be issued by output.check
    { "\JournalTitle{" journal * "}" * }
  if$
}

FUNCTION {article}
{ output.bibitem
  format.authors "author" output.check
  author format.key output
  name.or.dash
  format.date "year" output.check
  crossref missing$
    { format.journal "journal" output.check
      maybe.doi.link.prepend
      format.vol.num.pages output
    }
    { format.article.crossref
      maybe.doi.link.prepend
      output.nonnull
      format.pages output
    }
  if$
  format.journal.pages
  maybe.doi.link.end
  format.eprint output
  format.note output
  fin.entry
}

FUNCTION {book}
{ output.bibitem
  author empty$
    { format.editors "author and editor" output.check
      editor format.key output
      name.or.dash
    }
    { format.authors output.nonnull
      name.or.dash
      crossref missing$
        { "author and editor" editor either.or.check }
        'skip$
      if$
    }
  if$
  format.date "year" output.check
  title format.full.book.spec output
  format.publisher
  format.pages output
  format.eprint output
  format.note output
  fin.entry
}

FUNCTION {booklet}
{ output.bibitem
  format.authors output
  author format.key output
  name.or.dash
  format.date "year" output.check
  format.title "title" output.check
  howpublished output
  address output
  format.eprint output
  format.note output
  fin.entry
}

FUNCTION {inbook}
{ output.bibitem
  author empty$
    { format.editors "author and editor" output.check
      editor format.key output
      name.or.dash
    }
    { format.authors output.nonnull
      name.or.dash
      crossref missing$
        { "author and editor" editor either.or.check }
        'skip$
      if$
    }
  if$
  format.date "year" output.check
  title format.full.book.spec output
  format.publisher
  format.pages "pages" output.check
  format.eprint output
  format.note output
  fin.entry
}

FUNCTION {incollection}
{ output.bibitem
  format.authors "author" output.check
  author format.key output
  name.or.dash
  format.date "year" output.check
  bbl.in " " * booktitle format.full.book.spec *
  maybe.doi.link.prepend maybe.doi.link.end output
  format.publisher
  format.pages "pages" output.check
  format.eprint output
  format.note output
  fin.entry
}

FUNCTION {inproceedings}
{ output.bibitem
  format.authors "author" output.check
  author format.key output            % added
  format.date "year" output.check
  bbl.in " " * booktitle format.full.book.spec *
  maybe.doi.link.prepend maybe.doi.link.end output
  publisher empty$
    { organization output
      address output
    }
    { organization output
      format.publisher
    }
  if$
  format.pages output
  format.eprint output
  format.note output
  fin.entry
}

FUNCTION {conference} { inproceedings }

FUNCTION {manual}
{ output.bibitem
  format.authors output
  author format.key output
  name.or.dash
  format.date "year" output.check
  format.btitle "title" output.check
  format.edition output
  organization output
  address output
  format.eprint output
  format.note output
  fin.entry
}

FUNCTION {mastersthesis}
{ output.bibitem
  format.authors "author" output.check
  author format.key output
  name.or.dash
  format.date "year" output.check
  bbl.mthesis format.thesis.type output.nonnull
  school "school" output.check
  address output
  format.eprint output
  format.note output
  fin.entry
}

FUNCTION {misc}
{ output.bibitem
  format.authors output
  author format.key output
  name.or.dash
  format.date "year" output.check
  format.title output
  howpublished output
  format.eprint output
  format.note output
  fin.entry
}

FUNCTION {phdthesis}
{ output.bibitem
  format.authors "author" output.check
  author format.key output
  name.or.dash
  format.date "year" output.check
  bbl.phdthesis format.thesis.type output.nonnull
  school "school" output.check
  address output
  format.eprint output
  format.note output
  fin.entry
}

FUNCTION {proceedings}
{ output.bibitem
  editor empty$
    { organization output
      organization format.key output }
    { format.editors output }
  if$
  name.or.dash
  format.date "year" output.check
  title format.full.book.spec output
  publisher empty$ not      % No need for warning if no pub.
    { format.publisher }
    { editor empty$         % For empty editor, organization was already given.
        'skip$
        { organization output }
      if$
      address output
    }
  if$
  format.pages output
  format.eprint output
  format.note output
  fin.entry
}

FUNCTION {techreport}
{ output.bibitem
  format.authors "author" output.check
  author format.key output
  name.or.dash
  format.date "year" output.check
  format.title "title" output.check
  format.tr.number output.nonnull
  institution "institution" output.check
  address output
  format.eprint output
  format.note output
  fin.entry
}

FUNCTION {unpublished}
{ output.bibitem
  format.authors "author" output.check
  author format.key output
  name.or.dash
  format.date "year" output.check
  format.eprint output
  format.note "note" output.check
  fin.entry
}

FUNCTION {default.type} { misc }

READ

FUNCTION {sortify}
{ purify$
  "l" change.case$
}

INTEGERS { len }

FUNCTION {chop.word}
{ 's :=
  'len :=
  s #1 len substring$ =
    { s len #1 + global.max$ substring$ }
    's
  if$
}

FUNCTION {format.lab.names}
{ 's :=
  s #1 "{vv~}{ll}" format.name$
  s num.names$ duplicate$
  #2 >
    { pop$
      " {et~al.}" *
    }
    { #2 <
        'skip$
        { s #2 "{ff }{vv }{ll}{ jj}" format.name$ "others" =
            {
              " {et~al.}" *
            }
            { " \& " * s #2 "{vv~}{ll}" format.name$
              * }
          if$
        }
      if$
    }
  if$
}

FUNCTION {author.key.label}
{ author empty$
    { key empty$
        { cite$ #1 #3 substring$ }
        'key
      if$
    }
    { author format.lab.names }
  if$
}

FUNCTION {author.editor.key.label}
{ author empty$
    { editor empty$
        { key empty$
            { cite$ #1 #3 substring$ }
            'key
          if$
        }
        { editor format.lab.names }
      if$
    }
    { author format.lab.names }
  if$
}

FUNCTION {editor.key.label}
{ editor empty$
    { key empty$
        { cite$ #1 #3 substring$ }
        'key
      if$
    }
    { editor format.lab.names }
  if$
}

FUNCTION {calc.short.authors}
{ type$ "book" =
  type$ "inbook" =
  or
    'author.editor.key.label
    { type$ "proceedings" =
        'editor.key.label
        'author.key.label
      if$
    }
  if$
  'short.list :=
}

FUNCTION {calc.label}
{ calc.short.authors
  short.list
  "("
  *
  year duplicate$ empty$
     { pop$ "????" }
     'skip$
  if$
  *
  'label :=
}

FUNCTION {sort.format.names}
{ 's :=
  #1 'nameptr :=
  ""
  s num.names$ 'numnames :=
  numnames #8 >
    { s nameptr
      "{vv{ } }{ll{ }}{  f{ }}{  jj{ }}"
      format.name$ 't :=
      t sortify *
      "   "  *
      "zzzzz" *
    }
    { numnames 'namesleft :=
      { namesleft #0 > }
      { s nameptr
        "{vv{ } }{ll{ }}{  f{ }}{  jj{ }}"
        format.name$ 't :=
        nameptr #1 >
          {
            "   "  *
            namesleft #1 = t "others" = and
              { "zzzzz" * }
              { t sortify * }
            if$
          }
          { t sortify * }
        if$
        nameptr #1 + 'nameptr :=
        namesleft #1 - 'namesleft :=
      }
    while$
    }
  if$
}

FUNCTION {sort.format.title}
{ 't :=
  "A " #2
    "An " #3
      "The " #4 t chop.word
    chop.word
  chop.word
  sortify
  #1 global.max$ substring$
}

FUNCTION {author.sort}
{ author empty$
    { key empty$
        { "to sort, need author or key in " cite$ * warning$
          ""
        }
        { key sortify }
      if$
    }
    { author sort.format.names }
  if$
}

FUNCTION {author.editor.sort}
{ author empty$
    { editor empty$
        { key empty$
            { "to sort, need author, editor, or key in " cite$ * warning$
              ""
            }
            { key sortify }
          if$
        }
        { editor sort.format.names }
      if$
    }
    { author sort.format.names }
  if$
}

FUNCTION {editor.sort}
{ editor empty$
    { key empty$
        { "to sort, need editor or key in " cite$ * warning$
          ""
        }
        { key sortify }
      if$
    }
    { editor sort.format.names }
  if$
}

FUNCTION {presort}
{ calc.label
  label sortify
  "    "
  *
  type$ "book" =
  type$ "inbook" =
  or
    'author.editor.sort
    { type$ "proceedings" =
        'editor.sort
        'author.sort
      if$
    }
  if$
  #1 entry.max$ substring$
  'sort.label :=
  sort.label
  *
  "    "
  *
  title field.or.null
  sort.format.title
  *
  #1 entry.max$ substring$
  'sort.key$ :=
}

ITERATE {presort}

SORT

STRINGS { last.label next.extra }

INTEGERS { last.extra.num number.label }

FUNCTION {initialize.extra.label.stuff}
{ #0 int.to.chr$ 'last.label :=
  "" 'next.extra :=
  #0 'last.extra.num :=
  #0 'number.label :=
}

FUNCTION {forward.pass}
{ last.label label =
    { last.extra.num #1 + 'last.extra.num :=
      last.extra.num int.to.chr$ 'extra.label :=
    }
    { "a" chr.to.int$ 'last.extra.num :=
      "" 'extra.label :=
      label 'last.label :=
    }
  if$
  number.label #1 + 'number.label :=
}

FUNCTION {reverse.pass}
{ next.extra "b" =
    { "a" 'extra.label := }
    'skip$
  if$
  extra.label 'next.extra :=
  extra.label
  duplicate$ empty$
    'skip$
    { "{\natexlab{" swap$ * "}}" * }
  if$
  'extra.label :=
  label extra.label * 'label :=
}

EXECUTE {initialize.extra.label.stuff}

ITERATE {forward.pass}

REVERSE {reverse.pass}

FUNCTION {bib.sort.order}
{ sort.label
  "    "
  *
  year field.or.null sortify
  *
  "    "
  *
  title field.or.null
  sort.format.title
  *
  #1 entry.max$ substring$
  'sort.key$ :=
}

ITERATE {bib.sort.order}

SORT

FUNCTION {begin.bib}
{ preamble$ empty$
    'skip$
    { preamble$ write$ newline$ }
  if$
  "\begin{thebibliography}{}"
  write$ newline$
  "\providecommand\natexlab[1]{#1}"
  write$ newline$
  "\providecommand\JournalTitle[1]{#1}"
  write$ newline$
}

EXECUTE {begin.bib}

EXECUTE {init.state.consts}

ITERATE {call.type$}

FUNCTION {end.bib}
{ newline$
  "\end{thebibliography}" write$ newline$
}

EXECUTE {end.bib}


==> Tables/Table_1.tex <==
\begin{table*}
\caption{Recent automated approaches on photo-z estimation.}
\label{table:MLs}      
\centering          
\begin{tabular}{p{2cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{2.2cm}|p{2.2cm}|p{3.5cm}} 
% {c c c c c l l l l }
\hline\hline       
                      % To combine 4 columns into a single one 
  & Method & Input data & Objects & $z_{s}$ range & Depth & Survey 
  \\
\hline
    \citet{Schmidt2020} & kNN & $ugrizy$ to grey scale 48x48 images & Galaxies & $0 < z \leq 2$ & $i < 25.3$ & mock galaxy for LSST from DESC
    \\
    \hline
      \citet{Pasquet2019}
    & ANN & $ugriz$ 64x64 images +E(B-V) & Galaxies & $z<0.4$ & petrosian mag $r \leq 17.8$ & SDSS-DR12  \\
    \hline
     \cite{2019MNRAS.482.3116A} 
    & METAPHOr, ANN, template fitting & $ugri$ GAaP & Galaxies & $z_{s} \leq 1$ &  $r \leq 21$ & SDSS-DR9 + KiDS ESO-DR3 + GAMA-DR2 +2dFGRS
    \\
    \hline
     \cite{Shuntov2020} 
    & ANN & $ugriz$ 64x64 images & Galaxies & $z_{s} \leq 0.4$ &  $r_{Petro} \leq 17.8$ & SDSS/BOSS-DR12 +GAMA-DR3
    \\
    \hline
    \cite{2018AJ....155....1G} & kNN & UV 
    + $ugrizy$ 
    + $YJHK$  & Galaxies &  $0.3 < z_{s} < 3.0$ & $i < 25$ & mock galaxy catalogs for Euclid, WFIRST, and/or CASTOR
    \\
    \hline
    \cite{2020MNRAS.493L..70C} & kNN & UV + $ugriz$ + w1w2w3w4 & QSOs  & --- & $14.7<r<22.6$ & SDSS-DR12 +2MASS +WISE 
    \\
    \hline
    \cite{2020arXiv200301511N} & kNN & $grizy$ & Galaxies & $z_{s}>0.01$  & $18.5<i<25$ &SDSS/BOSS-DR14 +DEEP2/3DR4 +VANDELSDR2 +COSMOS +C3R2 +COSMOS2015
    \\
    \hline
    \cite{2013MNRAS.432.1483C} & tree based & $ugriz$ + $BRI$ & Galaxies &  $0.02 \leq z_{s} \leq 0.3$ & $B_{AB}<$24.1 & SDSS/MGS-DR7 +DEEP2-DR4
    \\
    \hline
    \cite{2010ApJ...715..823G} & tree based & $ugriz$ & Galaxies & $z_{s} \leq 0.55$ &$r_{Petro} < 17.77$ & SDSS-DR6 +2dF-SDSS LRG +2SLAQ + DEEP2
    \\
    \hline
    \cite{2016MNRAS.455.2387A} & Gaussian process & $griz$ +$RIZ$ +$YJH$ & Galaxies & $0 \leq z_{s} \leq 2 $ & $RIZ< 25 $ & SDSS/BOSS
    \\
    \hline
    \cite{2019ascl.soft10014S} & ensemble of ANNs, trees and kNN & $ugriz$ & Galaxies &$z_{s}<0.8$ & $i_{AB}\lesssim 22.5$ & SDSS/BOSS-DR10
    \\
\end{tabular}
\end{table*}

\begin{table*}
\caption{Comparison on photometric redshift estimation. Values are given here whenever they are provided in the main text of the references.}
\label{table:comparison}      
\centering          
\begin{tabular}{p{3cm}|p{3cm}|p{2cm}|p{2cm}|p{3cm}} 
% \hline\hline       
                      % To combine 4 columns into a single one 
 & $\sigma_{mad}$ &Bias & rms & fraction of outliers
  \\
  \hline\hline
  \citet{Schmidt2020} (trainZ), ANNz2, BPZ, Delight, EAZY, FlexZBoost, GPz, Lephare, METAPhoR, CMNN, SkyNet, TPZ
  & &
  -0.2086, 0.00063, -0.00175, -0.00185, -0.00218, -0.00027, -0.00000, -0.00161, 0.00000, -0.00132, -0.00167, 0.00309 &
  0.1808, 0.0270, 0.0215, 0.0212, 0.0225, 0.0154, 0.0197, 0.0236, 0.0264, 0.0184, 0.0219, 0.0161 &
  0\%, 4.4\%, 3.5\%, 3.8\%, 3.4\%, 2\%, 5.2\%, 5.8\%, 3.7\% , 3.5\%, 3.6\%, 3.3\%
    \\
    \hline
      \citet{Pasquet2019} & 0.00912 &0.0001& & 0.31\%
      \\
    \hline
   \cite{2019MNRAS.482.3116A} METAPHOR, ANNz2, BPZ &
    & -0.004,−0.008,-0.020 & 0.065, 0.078, 0.048 & 0.98\% , 1.60\% 1.13\%
    \\
    \hline
     \cite{Shuntov2020} &
    0.0066 & & & 0.31\%
    \\
    \hline
    \cite{2018AJ....155....1G} & $\sigma =0.0165\pm 0.0001 $ & $−0.0001\pm 0.0$ & & 4\%
    \\
    \hline
    \cite{2020MNRAS.493L..70C} & $ \mathrm{rms}(z_{p} - z_{s}) = 0.36$  &&& 
    \\
    \hline
    \cite{2020arXiv200301511N} 
    $0.00< z_{p}<0.20$,
$0.20< z_{p}< 0.40$, $0.40 < z_{p}< 0.60$& & wide:-0.008,-0.009,-0.011, deep/ UltraDeep: -0.005, -0.011, 0.004 & & (biweight) wide: 0.131\%, 0.144\% , 0.159\%, deep/ UltraDeep: 0.198\% , 0.163\%, 0.180\% 
    \\
    \hline
    \cite{2013MNRAS.432.1483C}
    regression mode, classification mode& & -0.00008, 0.00218 & 0.0225, 0.0246& 0\% , 0\%
    \\
    \hline
    \cite{2010ApJ...715..823G} & for $(z_{p} − z_{s} )/\sigma _{68\%}$ $\mu =−0.006$ and $\sigma= 0.985$ with Gaussian fitting && & 1.9\% for $(z_{p} - z_{s})> 3\sigma z_{p}$
    \\
    \hline
    \cite{2016MNRAS.455.2387A} GP-GL, GP-VL, GP-VC & &
    0.0946, 0.828, 0.0294
    & 0.1420, 0.1251, 0.0435 &
    5.3\% , 5.5\% , 4.7\%
    \\
    \hline
%    \cite{2019ascl.soft10014S} & && &    \\
  
\end{tabular}
\end{table*}
